Higher-Order Transformer Derivative Estimates for Explicit Pathwise Learning Guarantees

An inherent challenge in computing fully-explicit generalization bounds for transformers involves obtaining covering number estimates for the given transformer class $T$. Crude estimates rely on a uniform upper bound on the local-Lipschitz constants of transformers in $T$, and finer estimates require an analysis of their higher-order partial derivatives. Unfortunately, these precise higher-order derivative estimates for (realistic) transformer models are not currently available in the literature as they are combinatorially delicate due to the intricate compositional structure of transformer blocks. This paper fills this gap by precisely estimating all the higher-order derivatives of all orders for the transformer model. We consider realistic transformers with multiple (non-linearized) attention heads per block and layer normalization. We obtain fully-explicit estimates of all constants in terms of the number of attention heads, the depth and width of each transformer block, and the number of normalization layers. Further, we explicitly analyze the impact of various standard activation function choices (e.g. SWISH and GeLU). As an application, we obtain explicit pathwise generalization bounds for transformers on a single trajectory of an exponentially-ergodic Markov process valid at a fixed future time horizon. We conclude that real-world transformers can learn from $N$ (non-i.i.d.) samples of a single Markov process's trajectory at a rate of ${O}(\operatorname{polylog}(N)/\sqrt{N})$.

==> Bookkeeping/Commenting.tex <==
% %%% Editing
% \usepackage{soul}

% \usepackage[colorinlistoftodos]{todonotes}
% \WarningFilter{todonotes}{The length marginparwidth}
% \newcommand{\ML}[1]{\textcolor{red}{[\textbf{ML}: #1]}}
% \newcommand{\RS}[1]{{\color{purple} [\textbf{RS}: {#1}] }}

% %%%% COMMENTING (Temporary)

% \NewDocumentCommand{\AK}{mo}{
%     \IfValueF{#2}{
%     %%%%% NO Margin Note
%                         {{\scriptsize
%                             \textcolor{violet}{ 
%                             \textbf{A:}
%                             \textit{{#1}}
%                             }
%                         }}
%         }
%     %%%% Margin Note
%     \IfValueT{#2}{
%                         \marginnote{{\scriptsize
%                             \textcolor{violet}{ 
%                             \textbf{A:}
%                             \textit{{#1}}
%                             }
%                         }}
%         }
%                     }
                    
% \NewDocumentCommand{\Yan}{mo}{
%     \IfValueF{#2}{
%     %%%%% NO Margin Note
%                         {{\scriptsize
%                             \textcolor{cyan}{ 
%                             \textbf{Y:}
%                             \textit{{#1}}
%                             }
%                         }}
%         }
%     %%%% Margin Note
%     \IfValueT{#2}{
%                         \marginnote{{\scriptsize
%                             \textcolor{cyan}{ 
%                             \textbf{Y:}
%                             \textit{{#1}}
%                             }
%                         }}
%         }
%                     } 

                    

% \definecolor{darkgreen}{rgb}{0.0, 0.2, 0.13}


% %%%% COMMENTING
% \NewDocumentCommand{\del}{m}{
%     {\color{gray}{ \tiny {#1} }}
% }

% \definecolor{cobaltt}{rgb}{0.0, 0.28, 0.67}
% \definecolor{deepcerise}{rgb}{0.85, 0.2, 0.53}
% \NewDocumentCommand{\add}{m}{{\color{violet}{{#1}}}}
% \newcommand{\change}[1]{{\color{ForestGreen}{#1}}} %  deepcerise

==> Bookkeeping/Extras/Unbounded_Case.tex <==
% \newpage
% \section{Supplementary Examples - Unbounded Domains}
% \label{s:Proofs_Supporting}

% Some readers may be curious on how to extend our theory to the case of unbounded Euclidean domains.  This can be done by smoothly ``clipping'' functions, analogously to the technique in~\cite{cohen2023neural}.
% % \begin{example}[Polynomials]
% % \label{ex:log_growth}
% % If $g:\mathbb{R}^d\to\mathbb{R}$ is a polynomial of degree $\Delta$, then $C\eqdef \|g\|_{C^s}=\|g\|_{C^{\Delta}}$ for all $s\ge \Delta$.   Thus, $g\in C^{\infty}_{poly:C,r}(\mathbb{R}^d,\mathbb{R})$ for all $r\ge 0$.
% % \end{example}

% We briefly mention that this can even be applied to the sum-of-squared errors (SSE) loss function while preserving its convexity and unique minimum at the origin.  This is shown in the following example.
% % Many smooth and convex loss functions, with a minimum at $0$, can be modified to exhibit roughly the same shape and minimum on an arbitrarily large region of $\mathbb{R}^D\times \mathbb{R}^D$.  As the next example shows, all that one must do is ``truncate'' by multiplication with a Gaussian.
% \begin{example}[Smoothly Clipped SSE Loss (Non-Polynomial)]
% \label{eq:smooth_loss}
% The SSE loss function $\ell_{0}(y,\hat{y})\eqdef \|y-\hat{y}\|^2$ is smooth, convex and is minimized by $y=\hat{y}$; however, all of its derivatives become unbounded when it is considered on the domain $\mathbb{R}^{2d}$.  
% % \hfill\\
% This can easily be corrected by considering the following ``smoothly clipped SSE loss'' as a surrogate for $\ell_0$, which is effectively indistinguishable from $\ell_{0}$ on the large interval about $0$.  More specifically, fix a ``temperature parameter'' $\lambda>0$ and define $\ell_{\lambda}:\mathbb{R}^{d}\times \mathbb{R}^d\to [0,\infty)$ by
% \[
%         \ell_{\lambda}(y,\hat{y})
%     \eqdef 
%         \|y-\hat{y}\|^2 \, e^{-\lambda \, \|y-\hat{y}\|^2}
% .
% \]
% Like $\ell_{0}$, when $\lambda>0$, the loss function $\ell_{\lambda}$ also has a minimum at $0$ and is convex the open interval
% $
% (\mathcal{O}(-1/\lambda),\mathcal{O}(1/\lambda))
% $% (-c/\lambda,c/\lambda)$
% ,  where $\mathcal{O}$ hides a positive absolute constant. %c\eqdef (5-17^{1/2})^{1/2}/2>0$
% Importantly, unlike $\ell_0$, when $\lambda>0$ then $\ell_{\lambda}$ satisfies Assumption~\ref{eq:smooth_loss} (see Proposition~\ref{prop:ExpFlattenedSSE_ExampleDetails} in Appendix~\ref{s:Proofs_Supporting}).
% \hfill\\
% Finally, observe that $\ell_{\lambda} $ converges to $ \ell_0$ pointwise as $\lambda \downarrow 0$.
% \end{example}

% \begin{proposition}[{Details on the loss function from Example~\ref{eq:smooth_loss}}]
% \label{prop:ExpFlattenedSSE_ExampleDetails}
% Let $\lambda>0$, $D\in \mathbb{N}_+$, and define $\ell:\mathbb{R}^{2D}\ni (y,\hat{y})\eqdef \|y-\hat{y}\|^2 \, e^{-\lambda \, \|y-\hat{y}\|^2}\in [0,\infty)$.  Then, for each $s\in \mathbb{N}$, we have
% \[
%     \|\ell\|_{C^s} = 
%     \begin{cases} 
% O(1) , \quad & \mbox{if} \quad 2 \lambda \geq e^{-1} , \\ 
% O [ (2\lambda e)^{-s/2} ] ,  \quad & \mbox{if} \quad 0 < 2\lambda < e^{-1} .  
%     \end{cases} 
% \]
% \end{proposition}







% \begin{proof}[{Proof of Proposition~\ref{prop:ExpFlattenedSSE_ExampleDetails}}]

% %Denote $z=y-\hat{y} \in \mathbb{R}^d$ with $z_i = y_i - \hat{y}_i$, $i=1$, ..., $d$. 
% %Define $l(z):=l(y,\hat{y})$.
% Denote $z=(y, \hat{y})=(y_1, \cdots, y_D, \hat{y}_1, \cdots, \hat{y}_D)\in \mathbb{R}^{2D}$. 
%  By induction we can show  
% \begin{align} 
%   \frac{\partial^k l(z)}{\partial z_{\alpha_1} \cdots \partial z_{\alpha_k}} 
%    =  \big( c_k   
%    + (-2\lambda)^k  \| z\|^2 
%     \big) e^{-\lambda \| z \|^2}  z_{\alpha_1} \cdots z_{\alpha_k} ,  
%     \label{ell-partial-k}
% \end{align} 
% where the coefficients $c_k$ are recursively determined by 
% \begin{align} 
% & c_1 = 2, \quad c_k = (-2\lambda) c_{k-1} + 2 (-2\lambda)^{k-1} ,  \quad k\geq 2 , \notag 
% \end{align} 
% and admit the following closed-form expression
% \begin{align} 
%  & c_k = 2 (-2\lambda)^{k-1} + 2(-2\lambda) \frac{1 - (-2\lambda)^{k-1}}{1-(-2\lambda)} , \, k\geq 2  \notag \\ 
%  & \quad = (-2\lambda)^{k-1} \frac{2(1+3\lambda)}{1 + 2\lambda} + \frac{ -4\lambda }{1 + 2\lambda} 
%  , \, k\geq 2 . \notag 
% \end{align}  
% The above expression implies $|c_k|\leq 3 (2\lambda)^{k-1} + 2$. 
% From~\eqref{ell-partial-k}, we have 
% \begin{align} 
%   \Big| \frac{\partial^k l(z)}{\partial z_{\alpha_1} \cdots \partial z_{\alpha_k}} \Big|  
%    = & \Big| \big( c_k   
%    + (- 2\lambda)^k   \| z\|^2 
%     \big) e^{-\lambda \| z \|^2}  z_{\alpha_1} \cdots z_{\alpha_k} \Big| \notag \\ 
%    \leq & 
%    \big[ | c_k |   
%    + ( 2 \lambda)^k   \| z\|^2 
%     \big] e^{-\lambda \| z \|^2} \| z \|^k \notag \\ 
%     \leq & 
%     \big[ 2 + 3 ( 2\lambda )^{k-1}  
%    + ( 2 \lambda)^k   \| z\|^2 
%     \big] e^{-\lambda \| z \|^2} \| z \|^k , 
% \label{|ell-partial-k|}
%    % \leq & 
%     %\big[ 2 + 3 ( 2\lambda )^{k-1}  
%    %+ ( 2 \lambda)^k   \| z\|^2 
%     %\big] e^{-\lambda \| z \|^2} \| z \|^k k^{-k/2} , 
% \end{align} 
% %where the last inequality is due to that under the constraint $\|z\|=r\geq 0$, we have $\max_{z\in \mathbb{R}^d} |z_{\alpha_1} \cdots z_{\alpha_k}|=r^k k^{-k/2}$.  
% For each $k$ fixed, the maximum of the right side of the last equality of \eqref{|ell-partial-k|} is 


% \bigskip 
% \begin{comment} 
% Since 
% \begin{align} 
%  & \Big| \big( c_k   
%    + (-2\lambda)^k  \| z\|^2 
%     \big) e^{-\lambda \| z \|^2}  z_{\alpha_1} \cdots z_{\alpha_k} \Big|    \notag \\ 
% \leq & 
%  \big( | c_k |   
%    + |(-2\lambda)^k|   \| z\|^2 
%     \big) e^{-\lambda \| z \|^2}  |z_{\alpha_1} \cdots z_{\alpha_k}| \notag  \\ 
% \leq & 
%  \big( | c_k |   
%    + |(-2\lambda)^k|   \| z\|^2 
%     \big) e^{-\lambda \| z \|^2}  \| z\|^k k^{-k/2} , \notag 
% \end{align} 
% it follows that for each $k=1$, ..., $s-1$ and each $\alpha\in \{1, ..., d\}^k$ fixed, 
% \begin{align} 
%  \Big\| \frac{\partial^k l(z)}{\partial z_{\alpha_1} \cdots \partial z_{\alpha_k}} \Big\|_\infty  
%    = & \Big\| \big( c_k   
%    + (-\lambda)^k 2^k  \| z\|^2 
%     \big) e^{-\lambda \| z \|^2}  z_{\alpha_1} \cdots z_{\alpha_k} \Big\|_\infty   \notag \\ 
%  \leq &   \max_{r\geq 0} \big[ \big( | c_k |   
%    + |(-\lambda)^k| 2^k  r^2 
%     \big) e^{-\lambda r^2} r^k k^{-k/2} \big]   , \notag 
% \end{align}  
% By the first order condition, the maximum is attained at $r=k^{1/2} (2\lambda)^{-1/2}$. We substitute 
% $r=k^{1/2} (2\lambda)^{-1/2}$ into the right side of the above inequality to obtain 
% \begin{align} 
%  \Big\| \frac{\partial^k l(z)}{\partial z_{\alpha_1} \cdots \partial z_{\alpha_k}} \Big\|_\infty  
%  \leq &   \max_{r\geq 0} \big[ \big( | c_k |   
%    + |(-\lambda)^k| 2^k  r^2 
%     \big) e^{-\lambda r^2} r^k k^{-k/2} \big]    \notag  \\ 
%     = &  \big( |c_k| + (2\lambda)^{k-1} k  \big) e^{- k/2}  (2\lambda)^{-k/2} \notag \\ 
%     \leq & \Big[ (2\lambda)^{k-1} 3 + 2 
%     + (2\lambda)^{k-1} k  \Big] e^{- k/2}  (2\lambda)^{-k/2} \notag 
% \end{align}  
% \end{comment}


% \begin{comment} 
% The maxium of the right side of the last equality is attained at $k=$. 


% By the Rademacher-Stephanov theorem \citep[Theorems 3.1.6 and 3.1.9]{Federer_GeometricMeasureTheoryBook_1969} and \eqref{ell-partial-k}, we have that
% \begin{align} 
%  \operatorname{Lip} \Big( \frac{\partial^{s-1} l(z)}{\partial z_{\alpha_1} \cdots \partial z_{\alpha_{s-1}}} \Big)  
%    =& \max_{z\in \mathbb{R}^{2D}}  \Big| \nabla_z \Big( \frac{\partial^{s-1} l(z)}{\partial z_{\alpha_1} \cdots \partial z_{\alpha_{s-1}}} 
%     \Big) \Big|    \notag 
% \end{align} 

% \begin{align} 
% \nabla_z \Big[ \frac{\partial^{s-1} l(z)}{\partial z_{\alpha_1} \cdots \partial z_{\alpha_{s-1}}} \Big] 
% = & (-2\lambda)^{s-1} 2z e^{-\lambda\|z\|^2} z_1\cdots z_{s-1}  
% \\
%  &+ (c_{s-1} + (-2\lambda)^{s-1} \|z\|^2 ) (-2\lambda) z e^{-\lambda\|z\|^2} z_1 \cdots z_{s-1} \notag \\ 
%  \notag
%  & + (c_{s-1} + (-2\lambda)^{s-1} \|z\|^2 ) e^{-\lambda\|z\|^2} \big( \sum_{j=1}^{s-1} e_{\alpha_j} \prod_{l=1\neq j}^{s-1} z_{\alpha_l} \big) 
% \notag 
% \end{align} 
% \end{comment} 

    
% \end{proof}


==> Bookkeeping/Historical_Versions/2024_04_25.tex <==
% \documentclass{article}


% % if you need to pass options to natbib, use, e.g.:
% %     \PassOptionsToPackage{numbers, compress}{natbib}
% % before loading neurips_2024


% % ready for submission
% % \usepackage{neurips_2024}


% % to compile a preprint version, e.g., for submission to arXiv, add add the
% % [preprint] option:
% \usepackage[preprint]{neurips_2024}


% % to compile a camera-ready version, add the [final] option, e.g.:
% %     \usepackage[final]{neurips_2024}


% % to avoid loading the natbib package, add option nonatbib:
% %    \usepackage[nonatbib]{neurips_2024}


% \usepackage[utf8]{inputenc} % allow utf-8 input
% \usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage{hyperref}       % hyperlinks
% \usepackage{url}            % simple URL typesetting
% \usepackage{booktabs}       % professional-quality tables
% \usepackage{amsfonts}       % blackboard math symbols
% \usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{microtype}      % microtypography
% \usepackage{xcolor}         % colors


% % \documentclass[aap]{imsart}
% % Theorems with 
% % \theoremstyle{plain}
% % \documentclass[twoside,11pt]{article}

% % \usepackage{blindtext}

% % Any additional packages needed should be included after jmlr2e.
% % Note that jmlr2e.sty includes epsfig, amssymb, natbib and graphicx,
% % and defines many common macros, such as 'proof' and 'example'.
% %
% % It also sets the bibliographystyle to plainnat; for more information on
% % natbib citation styles, see the natbib documentation, a copy of which
% % is archived at http://www.jmlr.org/format/natbib.pdf

% % Available options for package jmlr2e are:
% %
% %   - abbrvbib : use abbrvnat for the bibliography style
% %   - nohyperref : do not load the hyperref package
% %   - preprint : remove JMLR specific information from the template,
% %         useful for example for posting to preprint servers.
% %
% % Example of using the package with custom options:
% %
% % \usepackage[abbrvbib, preprint]{jmlr2e}
% % \usepackage[abbrvbib, preprint]{jmlr2e}

% % \documentclass[aap]{imsart}

% %% Packages
% % \RequirePackage{amsmath,amsfonts,amssymb}
% % \usepackage{amsthm}
% % \RequirePackage[numbers,sort&compress]{natbib}
% %\RequirePackage[authoryear]{natbib}%% uncomment this for author-year citations
% % \RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
% % \RequirePackage{graphicx}

% % \startlocaldefs

% %% 
% %% Copyright 2007-2020 Elsevier Ltd
% %% 
% %% This file is part of the 'Elsarticle Bundle'.
% % \documentclass[preprint,12pt,authoryear]{elsarticle}
% % \usepackage{amssymb}
% % \journal{Stochastic Processes and Their Applications}

% % % SCIMODS_Wrapped_2022
% % \documentclass[11pt]{article}


% \usepackage[utf8]{inputenc}
% % \usepackage[10pt]{extsizes} % <- Override Spring Size


% \input{math_commands}
% \usepackage{natbib}
% \usepackage{lipsum}

% % Springer
% % \raggedbottom
% % \newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
% % \setlength\heavyrulewidth{0.3ex}
% % \usepackage{lscape}


% % \ShortHeadings{Reality Only Happens Once}{Horvath, Kratsios, Limmer, Saqur, and Yang}

% \input{Bookkeeping/Commenting}

% %\author{%
% %  David S.~Hippocampus\thanks{Use footnote for providing further information
% %    about author (webpage, alternative address)---\emph{not} for acknowledging
% %    funding agencies.} \\
% %  Department of Computer Science\\
% %  Cranberry-Lemon University\\
% %  Pittsburgh, PA 15213 \\
% %  \texttt{hippo@cs.cranberry-lemon.edu} \\
%   % examples of more authors
%   % \And
%   % Coauthor \\
%   % Affiliation \\
%   % Address \\
%   % \texttt{email} \\
%   % \AND
%   % Coauthor \\
%   % Affiliation \\
%   % Address \\
%   % \texttt{email} \\
%   % \And
%   % Coauthor \\
%   % Affiliation \\
%   % Address \\
%   % \texttt{email} \\
%   % \And
%   % Coauthor \\
%   % Affiliation \\
%   % Address \\
%   % \texttt{email} \\
% %}

% \begin{document}
% % AAP
% % \begin{frontmatter}
% \title{Reality Only Happens Once: \\ 
% One-Path %Pathwise
% Generalization Bounds for Transformers}
% % Automatic Deep Kalman Filters


% \author{
% Yannick Limmer  \\
% Department of Mathematics \\
% Oxford-Man Institute \\
% University of Oxford\\
% \texttt{limmery@maths.ox.ac.uk} \\
% \And 
% Anastasis Kratsios  \\
% Department of Mathematics \\
% McMaster University \\
% Vector Institute \\
% \texttt{kratsioa@mcmaster.ca} \\
% \And    
% Xuwei Yang \\
% Department of Mathematics  \\
% McMaster University \\
% \texttt{yangx212@mcmaster.ca} \\
% \And
% Raeid Saqur \\
% Department of Computer Science \\
% University of Toronto \\
% Vector Institute \\
% \texttt{raeidsaqur@cs.toronto.edu} \\
% \And
% Blanka Horvath  \\
% Department of Mathematics \\
% Oxford-Man Institute \\
% University of Oxford\\
% \texttt{horvath@maths.ox.ac.uk} \\
% } 
% \maketitle

% \AK{
% To Dos:
% \begin{enumerate}
%     \item Make sure 1-Lip target function in assumption of main theorem.
% \end{enumerate}
% }

% \begin{abstract}
% One of the inherent challenges in deploying transformers on time series is that \emph{reality only happens once}; namely, one typically only has access to a single trajectory of the data-generating process comprised of non-i.i.d.\ observations.  
% We thus derive non-asymptotic bounds on the future-time $t$ generalization of a transformer network trained on $N\le t$ observations from a single path from an unknown function of a Markov process whose kernel satisfies a log-Sobolev inequality.  
% % 
% Our bound, converges at the optimal rate of $\mathcal{O}(1/\sqrt{N})$, and consists of three components: 1) the first quantifies the gap between the stationary distribution of the data-generating Markov process and its distribution at time $t$, which converges to $0$.  2) The next term encodes the complexity of the transformer model and, given enough time, eventually converges to $0$ at the rate $\mathcal{O}(1/N^{s})$ for any $s>0$. 3) The third term encodes the validity 
% that the bound holds with probability at least $1-\delta$, converges at a rate of $\mathcal{O}(\sqrt{\log(1/\delta)}/\sqrt{N})$.
% Our bounds depend explicitly on the activation function, a number of self-attention heads, depth, width, and parameter bounds defining the transformer; we consider the $\operatorname{Swish}$, $\operatorname{GeLU}$, and $\tanh$ activation functions.
% %%% A bit long
% % Traditionally,  modelling assumptions of financial models typically (tacitly) assume the availability of multiple identically distributed samples (or i.i.d.\ trajectories from the time series generating mechanism) in order to fit the models to data or to derive convergence rates and error bounds for them.
% %  The latter may or may not be a restrictive assumption depending on observed market reality, but the more changes in regimes occur in the market during the observation period, the more important it becomes to be able to let go of the i.i.d assumption of the observed samples. 
% % This challenge is particularly prevalent when training, or fine-tuning pre-trained transformers, while only having access to samples of a single trajectory of the time series. Such \textit{one-shot} learning constraint is currently a limiting bottleneck for research contributions in this area. 
% % In this paper we tackle this challenge by deriving bounds on the future-time generalization of a transformer trained on samples from a single time series history.  Though our primary interest is motivated by financial time series, the applicability of our results go beyond financial applications, they include any modelling setup where future predictions are to be inferred from an observation of a single realisation of a (non-stationary) path.
% % In our solution, we represent the time series (as an unknown transformation) 
% % as a transformation of a Markov process, where 
% % both the Markov Process and the transformation are assumed to be unknown. The only a-priori assumption we make on the Markov kernel is that it is exponentially contracting (i.e. it has a spectral gap).  
% % \textbf{XXX rate-to-constant trade-off}
% % Consequentially, our generalization bounds are asymptotically dimension-free and, given enough time, any rate $O(N^{-s/d})$ can be realized.  
% % Our generalization bound quantitatively depends on the number of attention heads, depth, width of the transformer network, and the activation functions: we consider their the Swish, GeLU, or $\tanh$.
% \end{abstract}

% %%%%%%%%%%%%%%%%%%%%% Section 1 %%%%%%%%%%%%%%%%%%%%%
% \section{Introduction}
% \label{s:Intro}

% Transformer networks are rapidly taking center stage in deep learning due to the undeniable success of GPT-type models in natural language processing (NLP); e.g.~\cite{achiam2023gpt}, and their success in computer vision; e.g.~\cite{dosovitskiy2020image}.  Nevertheless, our understanding of why and how transformers one sequential learning tasks, e.g.\ in NLP tasks or in time series analysis tasks \citep{zhou2021informer}, is only still developing.  This is especially the case for statistical guarantees for transformer models that do not assume that the data is i.i.d.\ but rather has a rich temporal structure; as is the case in most time series prediction problems in
% physic~\cite{PualBaschnagelStochasticPhys_book_2013}, medical~\cite{beck1983markov}, reinforcement learning \cite{SuttonBardo_RLBook_2018}, optimal control~\cite{Nizar_ControlBook_2013}, and in finance~\cite{FollmerSchiedStochFinanceBoko_2011}.



% In this paper, we study the ability of transformers to generalize beyond the data on which they were trained.  Many pre-trained/trained transformers typically \textit{fine-tuned} using observations along a single trajectory of a time series, whose sequential realizations (path) are not i.i.d.\ but for which there is a more general temporal relationship.  We, therefore, consider the \textit{realizable} learning problem where the user is supplied with $N$ paired samples $(X_1,Y_1),\dots,(X_N,Y_N)$, where each input $Y_n=f^{\star}(X_n)$ for a smooth (unknown) \textit{target function} $f^{\star}:\mathbb{R}^{d\times M}\to \mathbb{R}^D$ to be learned, depending on a history length $M$, and where the inputs are generated by a time-homogeneous Markov process $X_{\cdot}\eqdef (X_n)_{n=1}^{\infty}$.

% The performance of any transformer model transformer model $\mathcal{T}:\mathbb{R}^{d\times M}\to \mathbb{R}^D$ is quantified via a smooth loss function $\ell:\mathbb{R}^D\times \mathbb{R}^D\to \mathbb{R}$.  The generalization of such a $\mathcal{T}$ is measured by the gap between its \textit{empirical risk} $\mathcal{R}^{(N)}$, computed from the single-path training data, and its \textit{(true) $t$-future risk} $\mathcal{R}_t$ at a (possibly infinite) future time $N\le t\le \infty$ ($t\in \mathbb{N}_+$) 
% % (defined in Section~\ref{s:Prelim}). 
% % Our main result is illustrated in Figure~\ref{fig:phase_diagram__theoremsummary}.
% % \begin{figure}[H]
% %     \centering
% %     \input{figs/bm.tex}
% %     % \includegraphics[height=2in]{figs/genbounds.pdf}
% %     \caption{Phase diagram: Generalization bounds for transformers trained on a single path.}
% %     \label{fig:phase_diagram__theoremsummary}
% % \end{figure}
% % 
% % We consider an \textit{realizable} PAC setting problem, determined by a smooth $1$-Lipschitz \textit{target function} $f^{\star}:\mathbb{R}^d\to \mathbb{R}^D$ which we would like to learn using a sequence of random observations $\big((X_t,Y_t)\big)_{t\in \mathbb{N}}$ as our training data.  That is, for each $t\in\mathbb{N}_+$
% % \[
% %     Y_t \eqdef f^{\star}(X_t) 
% %     %+ \varepsilon_t.
% % \]
% defined by
% % We aim to learn $f$ from a \textit{single path}.  The ability of a model to reliably recover the function $f:\mathbb{R}^d\to\mathbb{R}^D$ at time $t$, given the input $X_t$, is quantified by the \textit{$t$-future risk}
% \[
%     \mathcal{R}_t(f)
%     \eqdef 
%     \mathbb{E}\big[
%         % \|f(X_t)-f^{\star}(X_t)\|
%         \ell(\mathcal{T}(X_t),f^{\star}(X_t))
%     \big]
% \]
% where $\mathcal{R}_{t}$ (resp.\ $\mathcal{R}_{\infty}$) is computed with respect to the distribution of $X_t$ (resp.\ \textit{stationary distribution} of $X_{\cdot}$).
% The time-$t$ excess-risk $\mathcal{R}_t$, which is generally unobservable, is estimated by a single-path estimator known as the empirical risk computed using all the noisy samples to observed thus far
% \[
%     \mathcal{R}^{(N)}(f)
%     \eqdef 
%     \frac1{N}\,\sum_{n=1}^N\,
%             % \|f(X_n)-Y_n\|
%             \ell(\mathcal{T}(X_n),f^{\star}(X_n))
%     .
% \]
% Our objective is to obtain a statistical learning guarantee bounding the gap between the empirical risk and the $t$-future risk of transformer models trained on a single path.


% Informally, our main results yield a sequence of \textit{progressively accelerating generalization bounds}, on the \textit{future time} $t\ge N$ predictive power of a transformer model trained from $N$ samples of an unknown function of an unknown Markov process $X_{\cdot}$, with no spectral gap.  
% Let $\transformer_{L,W,H}^{D,d,M}$ be the class of transformed with $H$ attention heads, hidden MLP layers $L$, and MLP width $W$; then for respective input and output dimensions $d$ and $D$, and history length $M$.  Then, the following holds
% \[
%         \sup_{\mathcal{T} \in \transformer_{L,W,H}^{D,d,M}}
%         \,
%             \big|
%                 \mathcal{R}_t(\mathcal{T})-\mathcal{R}^{(N)}(\mathcal{T})
%             \big|
%     \lesssim
%         \underbrace{
%             \kappa^t
%         }_{\term{time}}
%         +
%         \underbrace{
%             \sum_{s=1}^{\infty}\,
%                 I_{N\in [
%                 \tau_s,\tau_{s+1}
%                 )}
%                 \,
%                 C_s\,\operatorname{rate}_s(N,t)
%         }_{\term{complexity}
%             \text{ (Exponential decay in $N$)}
%         }
%         +
%         \underbrace{
%             \frac{c\sqrt{\log(1/\delta)}}{\sqrt{N}}
%         }_{\term{hprob}}
% \]
% with probability at least $1-\delta$.  

% \paragraph{Non-Stationarity Term:} \Cref{time} quantifies the rate at which the data-generating process $X_{\cdot}$ becomes stationary and it only depends on the time $t$ and a constant $0<\kappa<1$ depending only on $X_{\cdot}$; we follow the notational convention that $\kappa^{\infty}\eqdef \lim\limits_{t\to \infty}\,\kappa^t = 0$.

% \vspace{-1em}
% \paragraph{Complexity Term:} \Cref{complexity} encodes the complexity of the transformer network in terms of the number of self-attention heads, depth, width, and the activation function considered.  Each constant $C_1\le \dots \le C_s\le \dots$ collects the higher-order sensitivities (derivatives of order up to $s\in \mathbb{N}_+$) of the transformer model.  Each $0=\tau_0\le \tau_1\le\dots \tau_s\le $ indicates the times at which there is a phase-transition in the convergence rate of the generalization bound accelerates.  Once $t\ge \tau_s$ then the convergence rate of~\Cref{complexity} accelerates by an exponential factor of $1$.
% % to $0$ at a rate of $\tilde{\mathcal{O}}(1/N^{(s+1)/d \vee 2})$ and no longer $\tilde{\mathcal{O}}(1/N^{(s+1)/d \vee 2 })$
% % , and $0<\kappa<1$ and $c>0$ are constants with $\kappa$ depending only on the law of the data-generating process $X_{\cdot}$.
% Explicitly, $\tau_1\eqdef 0$ and subsequence $\tau_s$ is defined recursively by
% \[
%     \tau_s
% \eqdef 
%     \inf\big\{ t\ge \tau_{s-1}
%         :\,
%         C_s\operatorname{rate}_s(N) \le C_{s-1}\operatorname{rate}_{s-1}(N)
%     \big\}
% \]
% and the convergence rate function is given explicitly by
% \[
%         \operatorname{rate}_s(N,t)
%     \eqdef 
%         % % \left(
%         %     %% Time-Shift Term
%         %         % I_{t<\infty}\,
%         %         \kappa^t\,
%         %     +
%         %         %%% Concentration Term
%         %         \frac{
%         %             \sqrt{2\ln(1/\delta)}
%         %         }{
%         %             N^{1/2}
%         %         }
%         %         %%% Mean Term
%         %         +\,
%                 %%% NEW: Generate Rate
%                 \begin{cases}
%                    \frac{
%                        \log(
%                             c\, N
%                         )^{d/(2s) + 1}
%                    }{
%                         c\, N^{1/2}
%                    } 
%                     & \mbox{ if } 1=d<2s\\
%                    %%%%
%                    \frac{
%                        \log(
%                             c\, N
%                         )
%                    }{
%                         c\, N^{1/2}
%                    } 
%                     & \mbox{ if } d=2s\\
%                 %%%%
%                    \frac{
%                        \log(
%                             c\, N
%                         )^{d-2s+s/d}
%                    }{
%                        c_2\,  N^{s/d}
%                    } 
%                     & \mbox{ if } d=2s\\
%                 \end{cases}
%     % \right)
% \]
% where $c\eqdef 1-\kappa$ and $0< \kappa< 1$ depend only the data-generating Markov process.

% \paragraph{Probabilistic Validity Term:} \Cref{hprob} captures the cost of the bound being valid with probability at least $1-\delta$.  From classical learning theory, we know that this term cannot be improved. It is responsible for the overall convergence rate of our generalization bound being ``stuck'' at the optimal (Monte-Carlo) rate of $\mathcal{O}(1/\sqrt{N})$; since the other two terms converge exponentially to $0$.


% A secondary contribution of our paper is the computation of the higher-order derivatives of the transformer model, i.e.\ the constants $C_s$, in terms of the number of attention heads, depth and width of the transformed model, and weight restriction, as we the activation functions used.  We consider the usual $\operatorname{Swish}$ of \cite{ramachandran2017searching}, the $\operatorname{GeLU}$ of \cite{hendrycks2016gaussian}, and the $\tanh$ activation functions (all of which are smooth).  

% \subsection{Related Work}
% \label{s:PrelatedWork}

% The mathematical foundations of transformer networks have recently come into focus in the deep learning theory community.  Most of the available statistical guarantees for transformers either concern: in-context learning for linear transformers \cite{zhang2024trained,garg2022can}, transformers \cite{von2023transformers,akyrek2023what} trained with gradient descent, or instance-dependant bounds \cite{trauger2023sequence} for general transformers.  
% % Unfortunately, these results assume that the transformers are trained on i.i.d.\ data. Thus, these results do not apply to the aforementioned time series prediction problems where data is not i.i.d.\ but is generated by a Markov process.  
% These results, however, do not apply in time series analysis contexts where each training sample is not independent of the others but is rather generated by some recursive stochastic process, e.g.\ a Markov process.

% Analytic counterparts to the statistical guarantees for transformers have also emerged.  These include universal approximation theorems for transformer networks \cite{yun2019transformers,yun2020n,fang2023attention} and contained universal approximation results for networks leveraging generalized attention mechanisms \cite{kratsios2022universal}, and the identification of function classes which can be efficiently approximated by transformers special classes \cite{likhosherstov2021expressive,frieder2024mathematical}.  Transformers have also been shown to be Turing complete  \cite{bhattamishra2020computational}. 

% Generalization bounds for multilayer perceptions (MLPs) have been actively studied for years.  For classification problems, these generalization bounds often rely on bounding the VC-dimension of classes of MLPs, depending on their depth, width, norm bounds on their parameters and activation functions \cite{bartlett1998almost,MR3960917}, or similar quantities.  In regression problems, one instead controls the Rademacher complexity of similar classes of MLPs \cite{bartlett2017spectrally,neyshabur2018the,pmlr-v97-yin19b}, due to the results such as \cite{koltchinskii2001rademacher,bartlett2002rademacher}, or turns to instance-dependant bounds which control the path-norm of the MLP \cite{neyshabur2015norm, golowich2020size,galanti2024norm} and local variants of these quantities; e.g.~\cite{Bartlett_LocalRadComplex_AnnStat_2005} or~\cite{hou2023instance}.  
% % These path norms are effectively the upper bounds of the Lipschitz constant of the instantiated model.  
% Our generalization bounds also partially borrow ideas from both of these directions. However, we use high-order sensitivities (partial derivatives) of our transformer networks to obtain tighter bounds for large enough $N$.  
% This does not yield a faster rate, since the $\mathcal{O}(1/\sqrt{N})$ rate is optimal and cannot generally be removed from~\Cref{hprob}, but it allows us to control better one of the two terms which do not arise from contraction of measure but rather quantify the complexity of the transformer hypothesis class.  Thus, a key part of our \textit{technical contributions} is the computation of these higher-order derivatives ($C^s$-norms) both of the transformer and the MLP models using smooth activation functions.  

% Most of the above statistical learning results operate under the assumption that one has access to $N$ i.i.d.\ samples from the data, which is typically not the case in most time series analysis problems.  Though there are results for non i.i.d.\ data using martingale arguments, e.g.~\cite{pmlr-v32-kontorovicha14}, that literature is less developed that the standard i.i.d.\ setting.  Our results thus also add to the later literature.  


% Our main result operates under the assumption that the stationary distribution of the Markov chain and its kernels all satisfy a log-Sobolev inequality (LSI).  Since their introduction, LSIs have been heavily studied \cite{GrossLogSobolev,LedouxNourdinPEccati_SteinGAFA_OTIneq_2015,Zimmerman_JFALogSobolev,InglisPapageourgio_JFAGibbsLogSobolev_PTRF_2019,ChenChewiNilesWeed_MixtureDimFreLogSob_JFA_2021} and have found numerous applications in differential privacy \cite{minami2016differential,ye2022differentially}, optimization \cite{LeCunetal_JStatMech_EntropSGD_2019}, random matrix theory \cite{Winger_AnnMath_1955_I,Winger_AnnMath_1955_II}, optimal transport \cite{DoleraMaini_AHPCStat_LipContinuityProbOT}, since they typically imply~\cite{Gozlan_LSI_II_AHPC_DFRatesSnowflake,Gozlan_LSI_IC_VPDE__DFConcentration} and effectively characterizes \cite{Gozlan_LSI_III_AnnProb_2009} dimension-free rate for concentration of measure.

% We require that the data-generating Markov process has an exponentially contracting Markov kernel \cite{Kloeckner_2020CounterCurse_ESAIM}.  For Markov chains, i.e.\ finite-state space Markov processes, this means that that the generator ($Q$-matrix) of the Markov chain has a \textit{spectral gap}.  These spectral gaps are actively studied in the Markov chain literature \cite{mufa1996estimation,kontoyiannis2012geometric,atchade2021approximate,MR3383563,kloeckner2019effective} since these have a finite mixing time, meaning that they distribution of such Markov chains approaches their stationary limit after a large finite time has elapsed; i.e.\ they have well-behaved (approximate) mixing times~\cite{montenegro2006mathematical,hsu2015mixing,BZ_Mixing}.

% \section{Preliminaries}
% \label{s:Prelim}
% We now record the notation used in our paper.  We then record the definition of the transformer model and probabilistic notions such as log-Sobolev inequalities.
% \subsection{Notation}
% \label{s:Prelim__ss:Notation}
% % \begin{notation}[Functions and Operators]
% % For convenience, we fix the following notation.
% % \begin{itemize}[nosep]
% %     \item \emph{Set of Functions}. We use $[X,Y]$ to denote a set of maps from a set $X$ to a set $Y$.
% %     \item \emph{Simplex}. For $N \in \N$ we write $\Delta_N\eqdef \{u\in [0,1]^N:\,\sum_{i=1}^N\,u_i=1\}$.
% %     \item \emph{Realized Path up to time $t$} is denoted by $x_{\le t}\eqdef (x_s)_{s\in \mathbb{Z},\,s\le t}$.
% %     \item \emph{Temporal Re-centering Operator}. Set $\tau_t:\,{\mathbb{R}^{d}}^{\mathbb{Z}}\to {\mathbb{R}^{d}}^{\mathbb{N}}$, for all $x_{\cdot}\in {\mathbb{R}^{d}}^{\mathbb{Z}}$ and $s\in \mathbb{Z}$ with $\tau_t(x_{\cdot})_s\eqdef x_{s-t}$.
% %     \item \emph{Extension Operator}. Define $E_M:{\mathbb{R}^{d}}^{\mathbb{M}}\to{\mathbb{R}^{d}}^{\mathbb{Z}}$, for all $x_{\cdot}\in {\mathbb{R}^{d}}^{M}$ and $s\in \mathbb{N}$ via $E_M(x_{\cdot})_s\eqdef x_{s}I_{M\le s\le 0}$.
% %     \item \emph{Restriction Operator}. Fix $R_M:{\mathbb{R}^{d}}^{\mathbb{Z}}\to {\mathbb{R}^{d}}^{\mathbb{M}}$, for all $x_{\cdot}\in {\mathbb{R}^{d}}^{\mathbb{Z}}$ and $s\in \mathbb{N}$ by $R_M(x_{\cdot})\eqdef (x_s)_{-M<s\le 0}$.
% % \end{itemize}
% % \end{notation}
% Much of our analysis is concerned with describing the \textit{regularity} of functions.  Here, regularity is quantified by the maximum magnitude of the partial derivatives of a function transformer model.  The definition of the related norms build on the following multi-index notation.
% \begin{notation}[Multi-index Notation]\label{not:Multivariate}
% We will fix the following multivariate notation.
% \begin{itemize}[nosep]
%     \item Multi-indices $\alpha \eqdef (\alpha_1, \ldots, \alpha_k) \in \N^k, k \in \N$ are denoted by Greek letters.
%     \item The sum of entries is given by $\vert \alpha \vert \eqdef \sum_{i=1}^k \alpha_k$.
%     \item Its faculty is defined by $\alpha!  \eqdef \prod_{i=1}^k \alpha_k!$,
%     \item We denote the derivative w.r.t. $\alpha$ by $D^\alpha \eqdef \partial^{\vert \alpha \vert} / \partial x_1^{\alpha_1} \cdots \partial x_k^{\alpha_k}$ if $\vert \alpha \vert > 0$ else $D^\alpha$ is the identity operator.
%     \item For a vector $x \in \R^k$, we write $x^\alpha \eqdef \prod_{i=1}^k x_k^{\alpha_k}$.
%     \item We define the relation $\alpha \prec \beta$ for $\beta \in \N^k$ if one of the three following holds 
%     \begin{enumerate}[label=(\roman*), nosep]
%         \item $\vert \alpha \vert < \vert \beta \vert$;
%         \item $\vert \alpha \vert = \vert \beta \vert$, and $\alpha_1 < \beta_1$; or 
%         \item $\vert \alpha \vert = \vert \beta \vert$, and $\alpha_i = \beta_i$ for $i \in \myset{1}{j-1}$ and $\alpha_j < \beta_j$ for $j \in \myset{2}{k}$.
%     \end{enumerate}
%     \item Unit vectors $e_i \in \{0,1\}^k$ are defined by $(e_i)_j = 0$ for $i \neq j$ and  $(e_i)_i = 1$.
% \end{itemize}
% \end{notation}
% For any $s>0$, the norm $\|\cdot\|_{C^s}$ of a smooth function $f:\R^d\to \R$ is defined by
% \[
%     \|f\|_{C^s}
% \eqdef 
%         \max_{k=1,\dots,s-1}\,
%         \max_{\alpha\in \{1,\dots,d\}^d}
%         \,
%             \Big\|
%                 \frac{\partial^k f}{
%                     \partial x_{\alpha_1}\dots\partial x_{\alpha_k}
%                 }
%             \Big\|_{\infty}
%     +
%         \max_{\alpha \in \{1,\dots,d\}^{s-1}}\,
%             \operatorname{Lip}\big(
%                 \frac{\partial^{s-1}f}{\partial x_{\alpha_1}\dots\partial x_{\alpha_{s-1}}}
%             \big)
% \]
% We will use the following notation to tabulate the sizes of a $C^s$-norm.
% \begin{notation}[Derivatives]\label{not:DerivativeBounds} Let $k \in \N$, $K \in \R^k$ be a set, $f: K \to \R^m$ a function and $\alpha\in\Order^k_n$ an ordered multi-index. Then,
% \begin{itemize}[nosep]
%     \item the uniform bound of $\alpha$-like derivatives on $K$ is given by 
%     \begin{align*}
%         C^f_K(\alpha) \eqdef \max_{i \in \myset{1}{m}} \max_{\gamma \sim \alpha} \Vert D^\gamma f_i \Vert_K,
%     \end{align*}
%     \item we write $\Vert K \Vert \eqdef \sup_{x \in K} \Vert x \Vert$, and 
%     \item for a matrix $A \in \R^{n\times m}$ we write $C^A \eqdef \max_{i \in \myset{1}{n}, j \in \myset{1}{m}} \vert A_{i,j}\vert$.
% \end{itemize}
% \end{notation}
% We use the following notation to streamline the analytic challenges the tacking of $C^s$-norms.
% \begin{notation}[Order operator for multi-indeces]\label{not:Order}
% Define the order operator $\order$ for multi-indeces by
% \begin{align*}
%     \order: \N^k \longrightarrow \N^k, \quad \alpha_1, \ldots, \alpha_k \longmapsto \alpha_{\tau_\alpha(1)}, \ldots, \alpha_{\tau_\alpha(k)},
% \end{align*}
% where $\tau_\alpha: \myset{1}{k} \to \myset{1}{k}$ s.t. $\alpha_{\tau_\alpha(1)} \geq  \ldots \geq  \alpha_{\tau_\alpha(k)}$.  We write $\alpha \eqorder \beta$ if $\order(\alpha) = \order(\beta)$ for $\alpha, \beta \in \N^k$. Further, denote by $\Order^k_{n}$ the set $\{\order(\alpha) :  \alpha \in \N^k, \vert \alpha \vert = n \}$ and write $\Order^k_{\leq n} \eqdef \{\order(\alpha) :  \alpha \in \N^k, \vert \alpha \vert \leq n \}$. Eventually, define $N(\alpha) \eqdef \# \vert \{ \alpha' \in \N^k : \order(\alpha') = \alpha \} \vert$. 
% \end{notation}
% We often segment, truncate, or manipulate time series using the following indexing operations.
% \begin{notation}[Time Series Notation]
% The following notation is when indexing paths of any time series.
% \begin{itemize}[nosep]
%     \item \emph{Realized Path up to time $t$} is denoted by $x_{\le t}\eqdef (x_s)_{s\in \mathbb{Z},\,s\le t}$.
%     \item \emph{Segment of a Path} Given a sequence $x\in \mathbb{R}^{\mathbb{Z}}$ and integers $s\le t$, we denote $x_{[s:t]}\eqdef (x_i)_{i=s}^t$.
%     % \item \emph{Temporal Re-centering Operator}. Set $\tau_t:\,{\mathbb{R}^{d}}^{\mathbb{Z}}\to {\mathbb{R}^{d}}^{\mathbb{N}}$, for all $x_{\cdot}\in {\mathbb{R}^{d}}^{\mathbb{Z}}$ and $s\in \mathbb{Z}$ with $\tau_t(x_{\cdot})_s\eqdef x_{s-t}$.
%     % \item \emph{Extension Operator}. Define $E_M:{\mathbb{R}^{d}}^{\mathbb{M}}\to{\mathbb{R}^{d}}^{\mathbb{Z}}$, for all $x_{\cdot}\in {\mathbb{R}^{d}}^{M}$ and $s\in \mathbb{N}$ via $E_M(x_{\cdot})_s\eqdef x_{s}I_{M\le s\le 0}$.
%     % \item \emph{Restriction Operator}. Fix $R_M:{\mathbb{R}^{d}}^{\mathbb{Z}}\to {\mathbb{R}^{d}}^{\mathbb{M}}$, for all $x_{\cdot}\in {\mathbb{R}^{d}}^{\mathbb{Z}}$ and $s\in \mathbb{N}$ by $R_M(x_{\cdot})\eqdef (x_s)_{-M<s\le 0}$.
% \end{itemize}
% \end{notation}
% Lastly, we recorded some additional notations that were required throughout our manuscript.
% \begin{notation}[Miscellaneous]
% The following notation is when indexing paths of any time series.
% \begin{itemize}[nosep]
%     \item \emph{$N$-Simplex}. For $N \in \N$ we write $\Delta_N\eqdef \{u\in [0,1]^N:\,\sum_{i=1}^N\,u_i=1\}$.
%     \item \emph{Infinite powers}: For $c\in (0,1)$, we define $c^{\infty}\eqdef \lim\limits_{t\to \infty}\, c^t = 0$.
% \end{itemize}
% \end{notation}


% \subsection{The Transformer Model}
% \label{s:Prelim_ss:Transformer}

% In this paper, we will consider sequential deep learning models defined by multi-head attention transformer models.  We will now formulate these models.

% For any $F\in \mathbb{N}_+$, we will consider a weighted (parametric) variant of the \textit{layer normalization} function of \cite{ba2016layer}, which allows for a variable level of regularization.  Our weighted \textit{layer normalization} is defined by $\operatorname{LayerNorm}:\mathbb{R}^F\to \mathbb{R}^F$ defined for any $u\in \mathbb{R}^F$ by 
% \[
%     \layernorm(u;\gamma,\beta,w)\eqdef  
%     % \begin{cases}
%         \gamma\, 
%         \frac{(u-\mu_u^w)}{1 + \softplus(\sigma_u^w)} + \beta 
%         % & \mbox{ if } u\neq 0\\
%     %     0 & \mbox{ if } u=0
%     % \end{cases}
% \]
% where $\mu_u^w\eqdef \sum_{i=1}^F\, \frac{w}{F} u_i$ and $(\sigma_u^w)^2 \eqdef \sum_{i=1}^F\, \frac{w}{F}\,\|u_i-\mu_u\|^2$, $\softplus \eqdef \ln (1 + \exp(\cdot))$, parameters $\beta\in \mathbb{R}^F$ and $\gamma \in \mathbb{R}$, and the normalization strength parameter $w\in [0,1]$ with $w=1$ being the default choice.   Here, we prohibit the layer norm from magnifying the size of its outputs when the layer-wise weighted variance $\sigma_u^w$ is small; note, this formulation avoids division by $0$ when the entries of $u$ are identical.

% We will also make use of the reshape operators which are standard in most deep learning software, which for any $F_1,F_2\in \mathbb{N}_+$ are given by $\reshape_{F_1\times F_2}$ map any vector $u\in \mathbb{R}^{F_1F_2}$ to the $F_1\times F_2$ matrix
% \[
%     \reshape_{F_1\times F_2}(x)_{i,j}\eqdef x_{(i-1)F_2 +j}
%     .
% \]
% We denote the inverse of the map $\reshape_{F_1\times F_2}$ by $\vectorize_{F_1,F_2}:\mathbb{R}^{F_1\times F_2}\to\mathbb{R}^{F_1F_2}$.

% Eventually, let us recall the definition of the $\softmax$ operator.
% For $F \in \N$, we define
% \begin{align*}%\label{id:Softmax}
%     \softmax:
%             \R^F 
%         \to     
%             \R^F,
%     \quad 
%             x 
%         \mapsto 
%             \left(
%                     {\exp(x_i)}
%                 /
%                     {\textstyle\sum_{j = 0}^{F-1} \exp(x_j)}
%             \right)_{i=0}^{F-1}.
% \end{align*}
% Our transformer block extends the definition in \cite{vaswani2017attention}, allowing the intermediate feedforward neural network to pass information across all time steps instead of operating on each time step individually.
% We also allow the transformer block to extend or contract the length of the generated sequence.  

% \begin{definition}[Multi-Head Self-Attention]\label{defn:MultiHead}
% Fix $\idim \in \N$. For $x \in  \R^{(1+M) \times \idim}$, $Q, K \in \R^{\kdim \times \idim}$, and $V \in \R^{\vdim \times \idim}$, where have key-dimension $\kdim \in \N$ and value-dimension $\vdim \in \N$; we define
% \begin{align*}%\label{id:Attention}
%         \attention(
%             x; Q, K, V 
%         )
%     \eqdef    
%         \bigg(
%             \sum_{j=0}^M
%                 \softmax\left(
%                     \Big(
%                         \frac{\langle
%                             Qx_m, Kx_i
%                         \rangle}{\sqrt{d_k}
%                         }
%                     \Big)_{i = 0}^{M}
%                 \right)_j
%                 Vx_j
%         \bigg)_{m=0}^M
%     \in \R^{(M + 1) \times \vdim}.
% \end{align*}
% For $H \in \N$, set $Q \eqdef (Q^{(h)})_{h=1}^H, K \eqdef (K^{(h)})_{h=1}^H \subseteq \R^{\kdim \times \idim}$, $V \eqdef (V^{(h)})_{h=1}^H \subseteq \R^{\vdim \times \idim}$, and $W \eqdef (W^{(h)})_{h=1}^H \subseteq \R^{\idim \times \vdim}$. For $x \in  \R^{(1+M) \times \idim}$, we define
% \begin{align*}%\label{id:MultiHead}
%         \multihead(x; Q, K, V, W) 
%     \eqdef 
%         \bigg(
%             \sum_{h = 1}^H
%                 W^{(h)} \attention(
%                     x; Q^{(h)}, K^{(h)}, V^{(h)}
%                 )_m 
%         \bigg)_{m = 0}^M \in \R^{(M+1) \times \idim}.
% \end{align*}
% \end{definition}
% \begin{definition}[Transformer Block]
% \label{defn:TransformerBlock}
% Fix a non-affine activation function $\sigma\in C^{\infty}(\R)$.  
% Fix a dimensional multi-index $d=(\idim, \kdim, \vdim, \ldim, \odim) \in \N^{5}$, a sequence length $M \in \N_+$, and a number of self-attention heads $H\in \mathbb{N}_+$.  
% A transformer block is a permutation equivariant map $\tblock:\mathbb{R}^{(1+M)\times \idim}\to \mathbb{R}^{(1+M)\times \odim}$ represented for each $x\in \mathbb{R}^{(1+M)\times \idim}$
% \begin{align}\label{eq:TB}
% \begin{aligned}
%         \tblock (x) 
%     & \eqdef  
%         \Big(
%         \layernorm\big(
%         B^{(1)} x'_m + B^{(2)} \big(\sigma\bullet (A\, x'_m + a)\big) ;\, \gamma_2,\beta_2,w_2
%         \big)
%         \Big)_{m=0}^M
%     \\
%         x'
%     & \eqdef 
%         \Big(
%     \layernorm\big(
%         x_m + \multihead(x; Q, K, V, W)_m;\,\gamma_1, \beta_1,w_1
%         \big)
%         \Big)_{m=0}^M
%     % \\
%     %     x_0 
%     % & \eqdef 
%     %     \reshape_{(1+M_0)\times d_0}(x)
% \end{aligned}
% \end{align}
% for $\gamma_1,\gamma_2\in \mathbb{R}$, 
% $w_1,w_2\in [0,1]$, 
% $\beta_1\in \mathbb{R}^{\idim}$, 
% $\beta_2\in \mathbb{R}^{\odim}$, 
% $A\in \mathbb{R}^{\ldim \times \idim}$, $a\in \mathbb{R}^{\ldim}$, 
% $B^{(1)} \in \mathbb{R}^{\odim \times \idim}$, $B^{(2)} \in \mathbb{R}^{\odim \times \ldim}$, and $Q, K, V, W$ as in \Cref{defn:MultiHead}.

% We denote a class of transformer blocks with representation~\eqref{eq:TB} by $\tblockclass_{d,M,H,C}$, where the constants $\smash{C \eqdef (C^{\gamma_1}, C^{\gamma_2}, C^{\beta_1}, C^{\beta_2}, C^a, C^A, C^{B^{(1)}}, C^{B^{(2)}}, C^{Q}, C^{K}, C^{V}, C^{W})}$ bound the respective parameters. 
    
% \begin{comment}
% The restriction for $C>0$ such that
% $
% \vert \gamma_1 \vert, 
% \vert \gamma_2 \vert, 
% \vert \beta_1 \vert,
% \vert \beta_2 \vert,
% \vert a \vert,
% \Vert A \Vert,
% \Vert B^{(1)} \Vert, 
% \Vert B^{(2)} \Vert, 
% \Vert Q^{(h)} \Vert,
% \Vert K^{(h)} \Vert,
% \Vert V^{(h)} \Vert, 
% \Vert W^{(h)} \Vert < C 
% $ 
% for all $h \in \myset{1}{H}$, is denoted by $\tblock^C_{d,M,H}$.
% \end{comment}
% \end{definition}

% \begin{definition}[Transformer]
% \label{defn:Transformer}
% Fix depth $L\in \mathbb{N}_+$, memory $M\in \mathbb{N}$, width $W\in \mathbb{N}_+$, number of heads $H\in \mathbb{N}_+$, and input-output dimensions $D,d\in\mathbb{N}_+$.  
% A transformer (network) is a map $\transformer: \mathbb{R}^{(1+M)\times D}\to \mathbb{R}^d$ with representation
% \begin{equation}
% \label{eq:Transformer_Nets}
%         \transformer(x)
%     =
%         A \big(
%             \vectorize_{1 + M, \odim^{L}}
%             \circ 
%             \tblock_L
%             \circ 
%             \dots 
%             \circ 
%             \tblock_1
%             (x)
%         \big)
%     +
%         b
% \end{equation}
% where multi-indices 
% $d^{l}=(\idim^{l},\kdim^{l},\vdim^{l},\ldim^{l},\odim^{l})$ 
% are such that 
% $\idim^1=D$, 
% $\idim^{l+1}=\odim^l$ 
% for each $l=1, \dots,L-1$, 
% and where 
% $H \eqdef (H^l)_{l=1}^L$ are the number of self-attention heads,
% $C' \eqdef (C^l)_{l=1}^L$ the parameter bounds,
% and for $l=1,\dots,L$ 
% we have $\tblock_l \in \tblock_{d^{l},M,H^{l},C^l}$
% .
% Furthermore, $A \in \mathbb{R}^{d \times (1+M)\odim^{L}}$ and $b\in \mathbb{R}^d$.

% The set of transformer networks with representation~\eqref{eq:Transformer_Nets} and parameters bound by $C$ is denoted by $\transformerclass_{L,H,C}^{D,d,M}$, where $C \eqdef (*C', C^A, C^b)$. If the specification is clear, we write $\transformerclass_{L,H,C}^{D,d,M} \equiv \transformerclass$ for short.
% \begin{comment}
% The restriction for $C > 0$ $\tblock_l \in \tblock^C_{d^{l},M^{l},H^{l}}$ for all $l \in \myset{0}{L-1}$, together with $\vert b \vert, \Vert A \Vert < \infty$ is denoted by $\transformer_{L,W,H}^{D,d,M; C}$.
% \end{comment}
% \end{definition} 


% \subsection{Log-Sobolev Inequalities and Moment Conditions}
% \label{s:Prelim__ss:LSI_MomentConditions}

% Fix dimensions $d,D\in \mathbb{N}_+$ and let $P$ be a Markov kernel on a non-empty Borel $\mathcal{X}\subseteq \mathbb{R}^d$ with initial distribution $X_0\sim \mu_0\in \mathcal{P}(\mathbb{R}^d)$, and with associated Markov process $X_{\cdot}\eqdef (X_t)_{t\in \mathbb{N}_0}$ given by $X_t\sim \mu_t\eqdef P^t \mu_0$.  
% % We consider a sequence of independent, not necessarily identically distributed, random variables $\varepsilon_{\cdot}\eqdef (\varepsilon_t)_{t \in \mathbb{N}}$ taking values in $\mathbb{R}^d$ and independent of $X_{\cdot}$ with a uniformly bounded first moment
% % \begin{equation}
% % \label{eq:UBFM}
% %     \Delta_{\text{noise}}\eqdef \sup_{t\in \mathbb{N}_+}\, \mathbb{E}[|\varepsilon_t|] < \infty
% % .
% % \end{equation}

% The \textit{entropy functional} $\mathcal{H}_{\mu}$ associated to any Borel probability measure $\mu$ on $\mathbb{R}^d$ acts on smooth functions $g:\mathbb{R}^d\to \mathbb{R}$ by
% \[
%     \mathbb{H}_{\mu}(g) \eqdef \mathbb{E}_{X\sim \mu}
%         \Big[
%             g(X)
%             \log\Big(
%                 \frac{g(X)}{\mathbb{E}_{Z\sim \mu}[g(Z)]}
%             \Big)
%         \Big]
% .
% \]
% The entropy functional can be used to express the log-Sobolev inequalities.  
% \begin{definition}[Log-Sobolev Inequality]
% \label{defn:LSI}
% A probability measure $\mu$ on $\mathbb{R}^d$ is said to satisfy a log-Sobolev with constant $C>0$ ($\operatorname{LSI}_C$) if for every smooth function $g:\mathbb{R}^d\to\mathbb{R}$
% \[
%     \mathbb{H}_{\mu}(g^2)
%     \le 
%     C 
%     \mathbb{E}_{X\sim \mu}[\|\nabla g(X)\|^2]
% \]
% \end{definition}
% We require that the Markov process is time-homogeneous to admit a satisfactory measure.  
% Further, we require that its Markov kernel and that stationary measure all satisfy $\operatorname{LSI}_C$.
% \begin{assumption}[Satisfactions of the Log-Sobolev Inequality]
% \label{ass:MC}
% There exists a $C>0$ such that $\bar{\mu}$, $\mu_0$, and $P(x,\cdot)$ all satisfy $\operatorname{LSI}_C$, for each $x\in \mathcal{X}$.
% \end{assumption}
% \begin{assumption}[Exponential Moments]
% \label{ass:Exp_Moment}
% There exist $\lambda,\tilde{C}>0$ and $\gamma\in (0,1)$ such that: for each $x\in \mathcal{X}$ we have $\mathbb{E}_{X\sim P(x,\cdot)}[e^{\lambda|X|}]\le \gamma\, e^{\lambda|x|}+\tilde{C}$.
% \end{assumption}

% \begin{comment}


% \AK{$s>(1+M)\,d/2$}

% \begin{lemma}
%     Fix $D, d, M, L, W, H \in \N$ and $C_1 > 0$. Then, there exists for any compact set $K \subseteq \R^{(1+M) \times d}$ a constant $C_2 > 0$ such that for all $\transformer \in \transformer_{L,W,H}^{D,d,M; C_1}$ holds that $\Vert \transformer \Vert_{C^\infty(K)} < C_2$.
% \end{lemma}
% \begin{proof}
%     Fix $C_1> 0$ and a compact set $K \subseteq \R^{(1+M) \times d}$. Let $\mathcal{P}$ denote the space of permissible parameters of $\transformer_{L,W,H}^{D,d,M; C}$, equipped with the canonic topology and the insertion map $\iota: \mathcal{P} \to \transformer_{L,W,H}^{D,d,M; C}$. Clearly, the space $\mathcal{P}$ is compact due to the bound $C_1$.

%     An analogue argument to the one in \Cref{lem:TransformerIsSmooth} shows that the map 
%     \begin{align*}
%         \tau: \mathcal{P} \times K \longrightarrow \R^d, \quad p, x \longmapsto \iota(p)(x)
%     \end{align*}
%     is smooth, and proves, since $\mathcal{P} \times K$ compact, that there is a constant $C_2 > 0$ with $\Vert \transformer \Vert_{C^\infty(K)} < C_2$ for all $\transformer \in \iota[\mathcal{P}] = \transformer_{L,W,H}^{D,d,M; C_1}$.
% \end{proof}
% \end{comment}

% \begin{comment}
% \textcolor{gray}{
% \begin{definition}[Transformer Block]
% %\label{defn:TransformerBlock}
% Fix a non-affine activation function $\sigma\in C^{\infty}$.  
% Fix a dimensional multi-index $d=(d_0,d_1,d_2,d_3,d_4)$, a memory multi-index $M=(M_0,M_1)$, and a number of self-attention heads $H\in \mathbb{N}_+$.  
% A transformer block is a map $\mathcal{T}:\mathbb{R}^{(1+M)\times d_{0}}\to \mathbb{R}^{(1+M_0)\times d_{4}}$ admitting the following representation: for each $x\in \mathbb{R}^{(1+M_1)\times d_{in}}$
% \begin{equation}
% %\label{eq:TB}
% \begin{aligned}
%     \mathcal{T}(x) = &  \operatorname{reshape}_{(1+M_1)\times d_4} \circ \operatorname{LayerNorm}(x_2 ;\, \gamma_2,\beta_2,w_2)\\
%     x_2 = & B(x_1,\sigma\bullet (A\, x_1 + a)) \byyan{\quad \textit{Concatenation?}}\\
%     x_1 = & \operatorname{LayerNorm}(x + x_0 ;\,\gamma_1, \beta_1,w_1)
% \end{aligned}
% \end{equation}
%  for some $\beta_1\in \mathbb{R}^{(1+M_0)\,d_2}$, 
% $w_1,w_2\in [0,1]$, $\beta_2\in \mathbb{R}^{(1+M_1)\,d_4}$, $\gamma_1,\gamma_2\in \mathbb{R}$, 
% $A\in \mathbb{R}^{d_3\times (1+M_0)\,d_2}$, $a\in \mathbb{R}^{d_3}$, $B\in \mathbb{R}^{(1+M_1)d_4\times ((1+M_0)d_2+ d_3)}$
% , for each attention head $h=1,\dots,H$ with weights $W^{(h)} \in \mathbb{R}^{d_2\times d_1}$\yannick{This needs to map to $d_0$.} and values $V^{(h)}\in \mathbb{R}^{d_1\times d_0}$ \yannick{The value dimension doesnt need to coincide with the key/query dimension.} matrices and the vector $u\in \mathbb{R}^F$ \yannick{we don't need $u$, right?} is given by the \textbf{multi-head self-attention}
% \[
% \begin{aligned}
%         x_0 
% =  &
%         \Biggl(
%             \sum_{h=1}^H\, W^{(h)} \sum_{j=0}^{M_0}\, \alpha_{m,j}^{(h)}(x)\, V^{(h)} \,x_j
%         \Biggr)_{m=0}^{M_0}
%     %%%
%     \in \mathbb{R}^{(1+M_0)\,d_2}
% \\
%     \alpha^{(h)}(x)
% = & 
%     \Biggl(
%         \frac{
%             e^{
%                 \langle 
%                         Q^{(h)} x_m
%                     ,
%                         K^{(h)} x_j
%                 \rangle
%             }
%         }{
%             \sum_{j=0}^{M_0}\, e^{
%                 \langle 
%                         Q^{(h)} x_m
%                     ,
%                         K^{(h)} x_j
%                 \rangle
%             }
%         }
%     \Biggr)_{m,j=0}^{M_0}
% \end{aligned}
% \]
% with \textit{queries} and \textit{keys} matrices in each attention head $Q^{(h)},K^{(h)}\in \mathbb{R}^{d_1\times d_0}$.  
% \hfill\\
% \noindent We denote the transformer blocks with representation~\eqref{eq:TB} by $\mathcal{TB}_{d,M,H}$.
% \end{definition}
% }

% \textcolor{gray}{
% \begin{definition}[Transformer]
% %\label{defn:Transformer}
% Fix depth $L\in \mathbb{N}_+$, memory $M\in \mathbb{N}$, width $W\in \mathbb{N}_+$, number of heads $H\in \mathbb{N}_+$ parameters, and $D,d\in\mathbb{N}_+$.  
% A transformer (network) is defined as a map $\transformer: \mathbb{R}^{(1+M)\times D}\to \mathbb{R}^d$ with representation\footnote{%
% By a minor abuse of notation, we identified $\mathbb{R}^{1\times d}$ with $\mathbb{R}^d$ in the final layer of~\eqref{eq:Transformer_Nets}. \yannick{Again, not necessary with $A$.}}
% \begin{equation}
% % \label{eq:Transformer_Nets}
%         \transformer(x)
%     =
%         A
%             \big(\mathcal{T}_L\circ \dots \circ \mathcal{T}_1\circ \operatorname{vec}_{(1+M_0^{(0)}),d_1^{(0)}}(x)\big)
%         +
%         b
% \end{equation}
% \yannick{the vec is not needed for the input, but the output}where $A\in \mathbb{R}^{d\times (1+M)d}$ \yannick{This matrix should collect terms, right?}, $b\in \mathbb{R}^d$, and for $l=1,\dots,L$ each $\mathcal{T}_l \in \mathcal{TB}_{d^{(l)},M^{(l)},H^{(l)}}$ where the multi-indices 
% $d^{(l)}=(d^{(l)}_0,d^{(l)}_1,d^{(l)}_2,d^{(l)}_4)$, $M^{(l)}=(M^{(l)}_0,M^{(l)}_1)$, satisfying: $d_0^1=D$, 
% % $d_4^L=D$, 
% $M_0^1=M$, and $M_1^L=0$ \yannick{I dont think we need that, we have the $A$ to collect}, for each $l=1,\dots,L-1$ we have $d_0^{l+1}=d_4^l$ and $M_1^{(l+1)}=M_0^l$, and where $H^{(l)}\le H$ for $l=1,\dots,L$.  
% % \hfill\\
% The set of transformer networks with representation~\eqref{eq:Transformer_Nets} is denoted by $\mathcal{T}_{L,W,H}^{D,d:M}$.
% \end{definition} 
% }


% \begin{lemma}
% \label{lem:regularity_1}
% \AK{
% If $\sigma\in C^{\infty}(\mathbb{R})$ and the matrices in each block have bounded real eigenvalues, can @Yannick and @Xuwei please bound the $C^k$ norm constant over this class (Assuming bounded weights and biases in each transformer block).
% }    
% \end{lemma}
% \end{comment}



% \begin{comment}
% \subsection{Risk Bounds}
% \label{s:Risk_Bounds}

% Suppose that $Z_{\cdot}\eqdef (Z_t)_{t\ge 0}$ is a stochastic process with values on $\mathbb{R}^{D\times d}$ defined on a complete filtered probability space $(\Omega,\mathcal{F},\mathbb{F}\eqdef(\mathcal{F}_t)_{t\ge 0},\mathbb{P})$ with right-continuous filtration and suppose that $X_{\cdot}$ has the strong Markov property with a time-homogeneous Markov kernel.  
% Suppose also that $X_{\cdot}$ has exponentially contracting Markov kernel, in the sense of \cite{JFA}, meaning that: there exists some $0\le \tilde{\kappa}<1$ such that for all $x_1,x_2\in \mathbb{R}^D$ and all $t,s\ge 0$, we have
% \begin{equation}
% \label{eq:exp_contracting_kernel}
%         \mathcal{W}_1\Big(
%             \operatorname{Law}(X_t|X_0=x_1)
%             ,
%             \operatorname{Law}(X_s|X_0=x_2),
%         \Big)
%     \lesssim
%         D \, \kappa^{|t-s|}\, \|x_1-x_2\|
% ,
% \end{equation}
% where $\lesssim$ hides a constant $D\ge 1$ independent of $t,s,x_1,$ and $x_2$.

% Let $\tau_{\cdot}\eqdef (\tau_n)_{n\in \mathbb{N}}$ be a sequence of $\mathbb{P}$-a.s.\ increasing $\mathbb{F}$-stopping times with $\tau_0=0$ $\mathbb{P}$-a.s. and, each of which has well-defined Laplace transform $\psi_n$ (moment generating function) satisfying the following growth condition: there exists some $0<\tilde{\kappa}<1$ such that for all $n\in \mathbb{N}$
% \begin{equation}
% \label{sub_Laplacian_condition}
%     \psi_n(\kappa) \le \tilde{\kappa}^{-n}
%     \,\,\mbox{ and }\,\,
%     \psi_n(\kappa) \le \tilde{\kappa}^n
%     .
% \end{equation}
% \begin{example}[Deterministic Times]
% \label{ex:deterministic_times}
% Let $(t_n)_{n\in \mathbb{N}}$ be an sequence in $[0,\infty)$ with $t_0=0$.  Then, the degenerate stopping times $\tau_n=t_n$ $\mathbb{P}$-a.s. satisfy condition~\eqref{sub_Laplacian_condition}.
% \AK{Check}
% \end{example}
% % \begin{example}
% %%% Ill fix this up later.
% % \label{ex:PoissonTimesWithVaryingIntensity}
% % Set $\kappa=\tilde{\kappa}$.  
% % For each $n\in \mathbb{N}_+$, let $\tau_n=\sum_{i=1}^n \, P_i$ where each $P_i$ is a Poisson random variable with intensity 
% % \[
% % \lambda_i
% % \le 
% % \min\biggl\{
% % \frac{\kappa\log(1/\kappa^i)}{1-\kappa}
% % ,
% % \frac{\kappa\log(\kappa^i)}{\kappa-1}
% % \biggr\}.
% % \]
% % If $\tau_0\eqdef 0$ then condition~\eqref{sub_Laplacian_condition} holds.
% % \AK{Check}
% % \end{example}

% Let us interpret the process $Z_{\cdot}$ as supervised pairs $(X_{t},Y_{t})\eqdef Z_t$ for all $t\ge 0$, where $X_t$ is a $\mathbb{R}^D$-valued process and $Y_t$ is an $\mathbb{R}^d$-valued process.  Let $\mu$ denote the stationary measure of the process $Z_{\cdot}$, which we use to quantify the asymptotic risk of our model \AK{explain and define obv}.  
% For any given $N\in \mathbb{N}_+$ we consider the empirical (random) measure
% \[
% \mathbb{P}^N\eqdef \frac1{N}\,\sum_{n=1}^N\, \delta_{Z_{\tau_n}}
% \]
% which we use to quantify the empirical risk.

% \AK{Using the previous results I will get risk bounds; single path!}

% \newpage~\newpage


% %%%%%%%%%%%%%%%%%%%%% Section 2 %%%%%%%%%%%%%%%%%%%%%
% \section{Setting}
% Fix $d,D,T,K\in \mathbb{N}_+$, an unknown map $f^{\star}\in [(\mathbb{R}^d)^{\mathbb{Z}},{\mathbb{R}^{F\times D}}^{\mathbb{Z}}]$, and a ``progressively observed'' path $x_{\cdot}^{\star}\eqdef (x_t)_{t\in \mathbb{Z}} \in(\mathbb{R}^d)^{\mathbb{Z}}$.  Set $y_{\cdot}\eqdef (y_t)_{t\in \mathbb{Z}}\in \mathbb{R}^{D}$ where: for each $t\in \mathbb{Z}$ we set
% \[
% y_t\eqdef f^{\star}(\tau_t(x_{\le t}^{\star}))
% \]
% We are given a family of \textit{pre-trained} transformer networks $f^1,\dots,f^K\in [\mathbb{R}^{d\times M}:\mathbb{R}^{F\times D}]$, as in Definition~\ref{defn:Transformer}, where $\mathbb{R}^{d\times M}$ is indexed by $\{-M+1,\dots,0\}$ with the index $0$ representing the present time, $-M+1$ representing $M-1$ steps in the past, and $M$ capturing the memory of the model $f^k$.

% For each $k=1,\dots,K$, the map $f^k$ generates a causal deep learning model $\bar{f}^k$ with memory $M$ by sequentially applying the map $f^k$ to the progressively observed times series $x_{\cdot}$.  This is formalized a map $\bar{f}^k:(\mathbb{R}^{d})^{\mathbb{Z}} \to (\mathbb{R}^{F\times D})^{\mathbb{Z}}$ given for each $x_{\cdot}\in {\mathbb{R}^{d}}^{\mathbb{Z}}$ and $t\in \mathbb{Z}$
% \[
%     \bar{f}^k(x_{\cdot})_t\eqdef f^k\circ R_M\circ \tau_t(x_{\cdot})
% \]



% \subsection{Problem}
% % 
% \end{comment}


% \section{Setting and Main Result}
% \label{s:Main_Result}

% We consider smooth loss and target functions functions that are concentrated on a compact region, along with their derivatives. The growth rate of the $C^s$ norm of the loss function and its derivatives quantifies the degree of concentration.  
% One easily verifies that any function in the Schwartz class satisfies this former of the following conditions, similar conditions are considered in the random feature model literature; see e.g.~\cite{XXX}, or polynomials.
% \begin{definition}[Smoothness Growth Rate]
% \label{ass:Loss}
% Let $d,D\in \mathbb{R}$.  A smooth function $g:\mathbb{R}^d\to \mathbb{R}$ is said to belong to the class $C^{\infty}_{poly:C,r}(\mathbb{R}^d,\mathbb{R}^D)$ (resp.\ $C^{\infty}_{exp:C,r}(\mathbb{R}^d,\mathbb{R}^D)$) if there exist $C,r\ge 0$ such that:
% \begin{enumerate}
%     % \item[(i)] \textbf{Logarithmic Decay:} $\|\ell\|_{C^s} \le C_{\ell}\, \log(1+s)^{-r_{\ell}}$
%     \item[(i)] \textbf{Polynomial Growth -  $C^{\infty}_{poly:C,r}(\mathbb{R}^d,\mathbb{R}^D)$:} $\|g\|_{C^s} \le C\, s^{r}$,
%     \item[(ii)] \textbf{Exponential Growth -  $C^{\infty}_{exp:C,r}(\mathbb{R}^d,\mathbb{R}^D)$:} $\|g\|_{C^s} \le C\, e^{s\,r}$,
% \end{enumerate}
% \end{definition}
% \begin{example}
% \label{ex:log_growth}
% If $g:\mathbb{R}^d\to\mathbb{R}$ is a polynomial of degree $\Delta$, then $C\eqdef \|g\|_{C^s}=\|g\|_{C^{\Delta}}$ for all $s\ge \Delta$.   Thus, $g\in C^{\infty}_{poly:C,r}(\mathbb{R}^d,\mathbb{R})$ for all $r\ge 0$.
% \end{example}
% Many smooth and convex loss functions, with a minimum at $0$, can be modified to exhibit roughly the same shape and minimum on an arbitrarily large region of $\mathbb{R}^D\times \mathbb{R}^D$.  As the next example shows, all that one must do is ``truncate'' by multiplication with a Gaussian.
% \begin{example}[Modified SSE]
% \label{eq:smooth_loss}
% The loss function $\ell(y,\hat{y})\eqdef \|y-\hat{y}\|^2 \, e^{-\lambda \, \|y-\hat{y}\|^2}$ for a given (large) temperature parameter $\lambda>0$ is a surrogate for the sum-of-squared-errors ($\|y-\hat{y}\|^2$) loss function with the additional property that its $C^s$ norms are bounded.  
% % \hfill\\
% This is because the function $t\mapsto t^2\,e^{-\lambda\,t^2}$ is a smooth surrogate for $t^2$ with rapidly decaying $C^s$ norms, in that it also has a minimum at $0$, and is concave in the following (large) interval about the origin
% \[
% (-c/\lambda,c/\lambda)
% \]
% where $c\eqdef (5-17^{1/2})^{1/2}/2>0$.  
% As shown in Proposition~\ref{prop:ExpFlattenedSSE_ExampleDetails}, $\ell$ satisfies Assumption~\ref{eq:smooth_loss}, it has minimum at $0$, and is convex on $[-c/\lambda,c/\lambda]$.  
% \AK{Check 1-lip, or rescale. using Xuwei's stuff}
% \end{example}
% We will consider an analogous quantification of the regularity of the target function $f^{\star}$.  


% \AK{Convert $\|\cdot\|$ to $\ell$}


% We consider an \textit{realizable} PAC learning problem, determined by a smooth $1$-Lipschitz \textit{target function} $f^{\star}:\mathbb{R}^d\to \mathbb{R}^D$ which we would like to learn using a sequence of random observations $\big((X_t,Y_t)\big)_{t\in \mathbb{N}}$ as our training data.  That is, for each $t\in\mathbb{N}_+$
% \[
%     Y_t \eqdef f^{\star}(X_t) 
%     %+ \varepsilon_t.
% \]
% We aim to learn $f$ from a \textit{single path}.  The ability of a model to reliably recover the function $f:\mathbb{R}^d\to\mathbb{R}^D$ at time $t$, given the input $X_t$, is quantified by the \textit{$t$-future risk}
% \[
%     \mathcal{R}_t(f)
%     \eqdef 
%     \mathbb{E}\big[
%         % \|f(X_t)-f^{\star}(X_t)\|
%         \ell(f(X_t),f^{\star}(X_t))
%     \big]
% .
% \]
% The time-$t$ excess-risk $\mathcal{R}_t$, which is generally unobservable, is estimated by a single-path estimator known as the empirical risk computed using all the noisy samples to observed thus far
% \[
%     \mathcal{R}^{(N)}(f)
%     \eqdef 
%     \frac1{N}\,\sum_{n=1}^N\,
%             % \|f(X_n)-Y_n\|
%             \ell(f(X_t),f^{\star}(X_t))
%     .
% \]
% Our objective is to obtain a statistical learning guarantee on the quality of our estimate of the target function given by the \textit{time $t\ge N$ generalization}
% \[
%     \big|\mathcal{R}_t(f)-\mathcal{R}^{(N)}(f)\big|
%     .
% \]


% \AK{
% \begin{itemize}
%     \item Must check rates: need to be (1+M)D and not d
%     \item Check if we want $\|f^{\star}\|_{C^s}\le ...$ 
% \end{itemize}
% }
% \begin{theorem}[Single Path Adaptive Generalization Bounds for Transformer]
% \label{thrm:main}
% Under Assumptions~\ref{ass:MC} and~\ref{ass:Exp_Moment}, let $f^{\star}:\mathbb{R}^{{(1+M)\times D} }\to \mathbb{R}^{{d}}$ be a smooth $1$-Lipschitz map \byyan{and fix a class of transformer models $\transformerclass$ with the same (co-)domain.  }
% There exists some $\kappa\in(0,1)$ depending only on the Markov chain $X_{\cdot}$ and some $t_0\in \mathbb{N}_0$ such that for each $t_0\le N \le t \le \infty$, each ``rate-to-constant-tradeoff parameter'' $s\in \mathbb{N}_+$, and every ``confidence level'' $\delta \in (0,1]$ the following
% \[
% \resizebox{1\linewidth}{!}{$%% BEGIN RESIZE BOX$}
%         \frac{
%         \sup_{\mathcal{T}\in \transformerclass}
%         \,
%             \big|
%                 \mathcal{R}_{\max\{t,N\}}(\mathcal{T})-\mathcal{R}^{(N)}(\mathcal{T})
%             \big|
%         }{
%             \byyan{
%                 C^{\transformerclass}_{K_{0}}(s)
%             }
%         }
%     \lesssim
%             %% Time-Shift Term
%                 % I_{t<\infty}\,
%                 \kappa^t\,
%             +
%                 %%% Concentration Term
%                 \frac{
%                     \sqrt{2\ln(1/\delta)}
%                 }{
%                     N^{1/2}
%                 }
%                 %%% Mean Term
%                 +\,
%                 %%% NEW: Generate Rate
%                 \begin{cases}
%                    \frac{
%                        \log\big(
%                             c\, N
%                         \big)^{d/(2s) + 1}
%                    }{
%                         c\, N^{1/2}
%                    } 
%                     & \mbox{ if } 
%                     {(1+M)D}
%                     <2s\\
%                    %%%%
%                    \frac{
%                        \log\big(
%                             c\, N
%                         \big)
%                    }{
%                         c\, N^{1/2}
%                    } 
%                     & \mbox{ if } 
%                     {(1+M)D}
%                     =2s\\
%                 %%%%
%                    \frac{
%                        \log\big(
%                             c\, N
%                         \big)^{d-2s+s/d}
%                    }{
%                        c_2\,  N^{s/d}
%                    } 
%                     & \mbox{ if } 
%                     {(1+M)D}
%                     =2s\\
%                 \end{cases}
% $}
% \]
% holds with probability at least $1-\delta$; where $c\eqdef 1-\kappa$ and $c_2\eqdef c^{s/d}$ and we use the notation $\kappa^{\infty}\eqdef 0$.  
% \hfill\\
% Moreover for $s \in \N_+$, we define the $s$-regularity bound
% \begin{align*}
%         C^{\transformerclass}_{K_{0}}(s) 
%         \eqdef 
%         \textstyle
%         \sup_{\transformer \in \transformerclass}
%         \max_{i \in \myset{1}{d}}
%         \max_{\substack{\alpha \in \N^{\byyan{(1+M)\times} D} , \byyan{\vert \alpha \vert \leq s}}} \Vert D^\alpha \transformer_i \Vert_K,
% \end{align*}
% of which an explicit bound is given in \Cref{prop:transformerSobolevBound}, which depends only on $K_0$ and the class of transformers $\transformerclass$ used.
% \end{theorem}

% \subsection{Overview of Proof}
% % \paragraph{Step 1 - Computing The Regularity of the Transformer Model}
% The first step in deriving our generalization bounds is to quantify the regularity of the transformer model, as a function of its depth, number of attention heads, and norm of its weight matrices.  

% Here, by \textit{regularity}, we mean the number and size of the continuous partial derivatives admitted by the transformer. To quantify the size of the partial derivatives of the transformer we first remark that it is \textit{smooth}; that is, it admits continuous partial derivatives of all orders.
% \begin{lemma}\label{lem:TransformerIsSmooth}
%     Fix $D, d, M, L, H, C$, as in \Cref{defn:Transformer}, then every transformer $\transformer \in \transformerclass_{L,H,C}^{D,d,M}$ is smooth.% $C^\infty(\R^{(1+M)\times d})$.
% \end{lemma}

% Now that we have computed the regularity of the transformer model, as quantified by its $\|\cdot\|_{C^s}$ norms, we can then instead uniformly bound the generalization capacity of the slightly larger but more tractable hypothesis classes $C^s_R(\mathbb{R}^d)$; where $f\in C^s_R(\R^d)$ if $\|f\|_{C^s}\le R$.  
% That is, we bound the right-hand side of
% \begin{equation}
% \label{eq:risk_bound__decomposition}
%        \sup_{g\in \transformer_{L,W,H}^{D,d,M}}\,
%         \,
%         \big|
%             \mathcal{R}_t(g)-\mathcal{R}^{(N)}(g)
%         \big|
%     \le 
%         \inf_{s\in \N}
%         \,
%             % \underbrace{
%                 \sup_{g\in \mathcal{C}^s_R(\mathbb{R}^d)}
%                 \,
%                 \big|
%                     \mathcal{R}_t(g)-\mathcal{R}^{(N)}(g)
%                 \big|
%             % }_{\mbox{Term to Bound}}
% \end{equation}
% where, critically, $R_{L,W,H}^{s:D,d,M}$ is the maximum of the $\|\cdot\|_{C^s}$-norm on the class $\transformer_{L,W,H}^{D,d,M}$.  We compute this quantity now, for each $s\in \N$. \yannick{I think we have to go over this paragraph above with the new notation.}
% \begin{proposition}[$C^s$-Norm Bound of Transformers]
% \label{prop:transformerSobolevBound}
%     Fix $n \in \N_+$. In the notation of \Cref{defn:Transformer} and the multivariate notation established in \Cref{not:Multivariate,not:Order,not:DerivativeBounds} let $\transformer \in \transformerclass_{L,H,C}^{D,d,M}$, then
%     it holds for $\alpha \in \N^{(1+M) \times D}$, $\vert \alpha \vert \eqdef n$, that 
%     \begin{align}\label{id:TransformerSobolevBound1}
%         C^{\transformer}_{K_{0}}(\alpha)
%         &\leq
%         \odim^L(1+M)\alpha!
%         \cdot
%         C^A 
%         \cdot
%         C^L(\alpha),
%     \end{align}
%     where $C^{1}(\alpha) \eqdef C^{\tblock_1}_{K_{0}}(\alpha)$ and for $l \in \myset{2}{L}$, 
%     \begin{align}\label{id:TransformerSobolevBound2}
%         C^{l}(\alpha) \eqdef 
%         &\leq
%         \alpha! \sum_{\beta \in \Order^{\Tilde{d}_l}_{\leq n}}  N(\beta)C^{\tblock_l}_{K_{l-1}}(\beta)
%         \sum_{\eta, \zeta \in \calP'(\order(\alpha),\beta)} 
%         \prod_{j=1}^{n} \frac{
%             C^l(\order(\zeta^{(j)}))^{\vert \eta^{(j)} \vert}
%         }{
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         }.
%     \end{align}
%     For this, $K_0 \subset \R^{(1+M) \times D}$ is a compact set, $K_l \eqdef \tblock_l[K_{l-1}]$,  $\Tilde{d}_{l} \eqdef (1+M_{l})\idim^{l}$, and a bound for $C^{\tblock_l}_{K_{l-1}}(\beta)$ is given by \Cref{thm:TransformerBlockSobolevBound}, only depending on the transformer block class $\tblockclass_{d^l, M^l, H^l, C^l}$.
% \end{proposition}
% % \paragraph{Step 2 - Generalization Bounds for $(s,R)$-Smooth Functions}
% % For any $s,R>0$, we use $\mathcal{C}^s_R(\mathbb{R}^d)$ to denote the closed ball of a given radius $R>0$ about the zero function in $C^s(\mathbb{R}^d)$.  
% Now that we have bounded the supremum term in~\eqref{eq:risk_bound__decomposition}, for any given number of partial derivatives $s\in \N$, it remains to translate this into a bound.  We can do this by relating it to the so-called \textit{smooth Wasserstein distance} $d_s$ between the distribution of the Markov chain at time $\mu_t$ and its empirical distribution $\mu^{(N)}\eqdef \frac1{N}\sum_{n=1}^N\, \delta_{X_n}$ obtained by collecting samples up to time $N$.  The \textit{smooth Wasserstein distance} $d_s$, studied by \cite{Kloeckner_2020CounterCurse_ESAIM,Riekert_ConcentrationOfMeasure2022,hou2022instance}, is the maximum mean discrepancy (MMD)-type distance quantifying the distance between any two Borel probability measures $\mu,\nu$ on $\R^d$ as the maximal distance which they can produced when tested on any function in $C^s_1(\R^d)$; that is
% \[
%     d_s(\mu,\nu) 
%     \eqdef 
%         \sup_{g\in \mathcal{C}^s_1(\mathbb{R}^d)}\, 
%         % \mu[g]-\nu[g]
%         \mathbb{E}_{X\sim \mu}[g(X)]
%         -
%         \mathbb{E}_{Y\sim \nu}[g(Y)]
% .
% \]
% \begin{remark}
% When $s=1$, $d_s$ is simply the $1$-Wasserstein distance used in adversarial learning \citep{arjovsky2017wasserstein}.  This can be seen from the Kantorovich-Rubinstein duality, see \citep[Theorem 5.10 and Equation (5.11)]{VillaniBook_2009}, as well as the characterization of $1$-Lipschitz functions as Lebesgue almost-everywhere once continuously differentiable functions by the Rademacher-Stephanov Theorem, see \citep[Theorems 3.1.6-3.1.9]{Federer_GeometricMeasureTheoryBook_1969}.  
% \end{remark}

% The $d_s$ distance between the process distribution at time $t$ $\mu_t$ and the running empirical distribution $\mu^{(N)}$ can be difficult to relate in general.  The idea is instead to ``fast forward time'' and bound the $d_s$-distance between $\mu^{(N)}$ and the \textit{stationary distribution} $\mu_{\infty}$ of the data-generating Markov chain $X_{\cdot}$.  Then, we can ``rewind time'' and bound the $d_s$-distance between the stationary distribution $\mu_{\infty}$ and the distribution $\mu_t$ of the Markov process up to time $t$.  This can be done since the Markov process has a finite mixing time, which we show in the course of the proof of the next result.  The combined estimates on the $d_s$-distances $d(\mu^{(N)},\mu_{\infty})$ and $d(\mu_{\infty},\mu_t)$ together with some concentration of measure arguments yield the following result which bounds each of the supremal terms on the right-hand side of~\eqref{eq:risk_bound__decomposition}.


% \begin{proposition}[Excess Risk-Bound]
% \label{prop:Concentation}
% Under Assumptions~\ref{ass:MC} and~\ref{ass:Exp_Moment}, let $f^{\star}:\mathbb{R}^d\to \mathbb{R}$, $\ell:\mathbb{R}^{2D}\to \mathbb{R}$, and $R,r>0$ be a such that the composite map $\mathbb{R}^d\ni x\mapsto \ell(f^{\star}(x),f(x))$ belongs to $\mathcal{C}_{R}^s(\mathbb{R}^d)$ for all $f\in C^2_r(\mathbb{R}^d)$.
% % \hfill\\
% Then, there exists some $\kappa\in(0,1)$ depending only on the Markov chain $X_{\cdot}$ and some $t_0\in \mathbb{N}_0$ such that for each $t_0\le N < t \le \infty$, each ``rate-to-constant-tradeoff parameter'' $s\in \mathbb{N}_+$, and every ``confidence level'' $\delta \in (0,1]$ the following
% \[
%         \sup_{g\in \mathcal{C}^s_R(\mathbb{R}^d)}
%         \,
%         \frac{
%             \big|
%                 \mathcal{R}_{\max\{t,N\}}(g)-\mathcal{R}^{(N)}(g)
%             \big|
%         }{R}
%     \lesssim
%             %% Time-Shift Term
%                 % I_{t<\infty}\,
%                 \kappa^t\,
%             +
%                 %%% Concentration Term
%                 \frac{
%                     \sqrt{2\ln(1/\delta)}
%                 }{
%                     N^{1/2}
%                 }
%                 %%% Mean Term
%                 +\,
%                 %%% NEW: Generate Rate
%                 \begin{cases}
%                    \frac{
%                        \log\big(
%                             c\, N
%                         \big)^{d/(2s) + 1}
%                    }{
%                         c\, N^{1/2}
%                    } 
%                     & \mbox{ if } 1=d<2s\\
%                    %%%%
%                    \frac{
%                        \log\big(
%                             c\, N
%                         \big)
%                    }{
%                         c\, N^{1/2}
%                    } 
%                     & \mbox{ if } d=2s\\
%                 %%%%
%                    \frac{
%                        \log\big(
%                             c\, N
%                         \big)^{d-2s+s/d}
%                    }{
%                        c_2\,  N^{s/d}
%                    } 
%                     & \mbox{ if } d=2s\\
%                 \end{cases}
% \]
% holds with probability at least $1-\delta$; where $0<\kappa <1$, and we use the notation $\kappa^{\infty}\eqdef 0$.
% \end{proposition}

% In order to obtain the proof of Theorem~\ref{thrm:main}, using these results, it remains to uniformly bound the $C^s$-norm of the composite function $\ell(f^{\star},\mathcal{T})$ over all our set of transformers considered in Proposition~\ref{prop:transformerSobolevBound}.  
% This can be computed via the following lemma.

% \begin{lemma}[$C^s$-Norm of loss of between two functions]
% \label{lem:control_loss__SSE}
% \AK{Put HERE When Xuwei is done!}
% \end{lemma}


% \AK{Perhaps we make some plots here}

% \AK{Contrast to Rademacher bounds (in the i.i.d.\ case)}


% \section*{Summary}




% \newpage
% \appendix


% \section{Proof Details}

% The next lemma will help us relate the $C^s$-regularity of a model, a target function, and a loss function to their composition and product.  
% We use it to relate the $C^s$-regularity of a transformed model $\mathcal{T}:\mathbb{R}^d\to \mathbb{R}^D$, the target function $f^{\star}:\mathbb{R}^d\to \mathbb{R}^D$, and the loss function $\ell:\mathbb{R}^{2D}\to \mathbb{R}$ to their composition
% \begin{equation}
% \label{eq:composite_to_concentrate}
% \begin{aligned}
% \ell_{\mathcal{T}}:  \mathbb{R}^{d}& \to \mathbb{R} \\
% x & \mapsto \ell\big(\mathcal{T}(x),f^{\star}(x)\big)
% .
% \end{aligned}
% \end{equation}
% One we computed have the $C^s$-regularity of $\ell_{\mathcal{T}}$, we can apply a concentration of measure-type argument based on an optimal transport-type duality, as in~\cite{amit2022integral,hou2023instance,benitez2023out,kratsios2024tighter}, to obtain our generalization bounds.  A key technical point where our analysis largely deviates from the mentioned derivations, is that we are not relying on any i.i.d.\ assumptions.


% \begin{lemma}[$C^s$-Norm of loss of between two functions]
% \label{lem:control_loss__SSE}
% Let $d,D,s\in \mathbb{N}_+$, $f_1,f_2:\mathbb{R}^d\to \mathbb{R}^D$ be of class $C^{s}$ and $\ell:\mathbb{R}^{2D}\to\mathbb{R}$ be smooth.  If there are constants $C_1,C_2, \widetilde{C}_1,\dots,\widetilde{C}_s\geq 0$ such that:
% $\|f_i\|_{C^s} \le C_i$ for $i=1,2$ and for $j=1,\dots,s$ we have
% $\|\ell\|_{C^j} \le \widetilde{C}_j$ then 
% \begin{align} 
%     \|\ell(f_1,f_2)\|_{C^s} 
%     \le & 
%     \max_{k=1, \cdots, s-1} \max_{\alpha \in \{1, \cdots, d\}^k}
%     \sum_{1 \leq |\beta| \leq k}  \widetilde{C}_{|\beta|}  
%         \sum_{\eta, \zeta \in \calP(\alpha,\beta)} \alpha! 
%         \prod_{j=1}^{k} \frac{
%           (C_1 C_2 )^{|\eta^{(j)}|}  
%         }{
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         }  \notag \\ 
%        & + \max_{\alpha \in \{1, \cdots, d\}^{s-1} }  \sum_{1 \leq |\beta| \leq s-1} \widetilde{C}_{|\beta|+1}   
%         \sum_{\eta, \zeta \in \calP(\alpha,\beta)} \alpha! 
%         \prod_{j=1}^{s-1} \frac{
%            (C_1 C_2)^{|\eta(j)|}  
%         }{
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         } \notag 
% \end{align} 
% \end{lemma}

% \begin{proof} [{Proof of Lemma~\ref{lem:control_loss__SSE}}]
% We first derive the general bound; which we then specialize to the case where the growth rate of $\ell$ is known. 
% We first observe that
% \begin{align} 
% \label{eq:definition_Cs__norm}
%  \big\| \ell( f_1, f_2 ) \big\|_{C^s} 
%   = 
%   % &
%     \underbrace{
%         \max_{k=1, \cdots, s-1} \max_{\alpha \in \{1, \cdots, d\}^k} \| D^\alpha \ell(f_1(x), f_2(x)) \|_\infty 
%     }_{\term{t:A}}
%   % \\
%   + 
%   % &
%   \underbrace{
%     \max_{\alpha \in \{1, \cdots, d\}^{s-1} } \operatorname{Lip}\big(  D^\alpha \ell(f_1(x), f_2(x))  \big) 
%     }_{\term{t:B}}
% .
%   % \notag 
% \end{align} 
% \paragraph{{General Case - Term~\Cref{t:A}}:}
% By Theorem~\ref{thm:FaaDiBruno}, we can represent the derivatives of $\ell(f_1(x), f_2(x))$ through the multivariate Fa\`a di Bruno formula. For each $k=1$, ..., $s-1$ fixed, and for each $\alpha\in \{1, \cdots, d\}^k$, we have 
% \begin{align} 
%  D^\alpha \ell(f_1(x), f_2(x)) 
%         =
%         \sum_{1 \leq |\beta| \leq k} (D^\beta \ell)(f_1(x), f_2(x))
%         \sum_{\eta, \zeta \in \calP(\alpha,\beta)} \alpha! 
%         \prod_{j=1}^{k} \frac{
%             [D^{\zeta^{(j)}} (f_1(x), f_2(x))]^{\eta^{(j)}}
%         }{
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         } .  \notag 
% \end{align} 
% It follows from the triangle inequality and the positive homogeneity of the $\|\cdot \|_\infty$ norm that  
% \begin{align} 
%  & \Big\| (D^\alpha \ell)(f_1(x), f_2(x)) \Big\|_\infty \notag \\ 
% \leq  & \sum_{1 \leq |\beta| \leq k}  \big\| (D^\beta \ell)(f_1(x), f_2(x)) \big\|_\infty 
%         \sum_{\eta, \zeta \in \calP(\alpha,\beta)} \alpha! 
%         \prod_{j=1}^{k} \frac{
%            \big\|  [D^{\zeta^{(j)}} (f_1(x), f_2(x))]^{\eta^{(j)}} \big\|_\infty 
%         }{
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         } 
% \notag \\ 
% \leq & 
% \sum_{1 \leq |\beta| \leq k}  \widetilde{C}_{|\beta|}  
%         \sum_{\eta, \zeta \in \calP(\alpha,\beta)} a! 
%         \prod_{j=1}^{k} \frac{
%           (C_1 C_2 )^{|\eta^{(j)}|}  
%         }{
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         } \notag \\ 
%          \leq & 
% \sum_{1 \leq |\beta| \leq k}  \widetilde{C}_{|\beta|}  
%         \sum_{\eta, \zeta \in \calP(\alpha,\beta)} \alpha !
%         \frac{
%           (C_1 C_2 )^{ \sum_{j=1}^k |\eta^{(j)}|}  
%         }{ \prod_{j=1}^k
%            \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         } 
%         \notag \\ 
%  = & 
% \sum_{1 \leq |\beta| \leq k}  \widetilde{C}_{|\beta|}  (C_1 C_2 )^{  |\beta|}  
%      \Big[   \sum_{\eta, \zeta \in \calP(\alpha,\beta)} \alpha !
%         \prod_{j=1}^k
%         \frac{
%           1
%         }{
%            \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         }  \Big] 
% \label{eq:bound_t:A}
% \end{align} 

% Consider the special case 
% \begin{align} 
%  & g^{(i)}(x_1, \cdots, x_d) = \exp\big( \sum_{j=1}^d x_j \big) : \mathbb{R}^d \to \mathbb{R}, \quad 
%  i = 1, ..., 2D , \notag  \\ 
%  &  \ell( g^{(1)}, \cdots , g^{(2D)} ) = \exp\big( \sum_{i=1}^{2D} g^{(i)} \big) : 
% \mathbb{R}^{2D} \to \mathbb{R} . \notag 
% \end{align} 

% \begin{align} 
% & \frac{\partial }{\partial g^{(i)}} \ell(g^{(1)}, \cdots , g^{(2D)}) = \ell(g^{(1)}, \cdots , g^{(2D)}) , \quad 
%   \frac{\partial g^{(i)}(x_1, \cdots, x_d)}{\partial x_j} = g^{(i)}(x_1, \cdots, x_d) 
%  \notag 
% \end{align} 

%  \begin{align} 
% & \frac{\partial }{\partial x^j }  \ell(g^{(1)}(x_1, \cdots, x_d), \cdots , g^{(2D)}(x_1, \cdots, x_d))   \notag \\ 
%  =& \sum_{i=1}^{2D} \frac{\partial }{\partial g^{(i)}}   \ell(g^{(1)}(x_1, \cdots, x_d), \cdots , g^{(2D)}(x_1, \cdots, x_d)) 
%  \frac{\partial g^{(i)}(x_1, \cdots, x_d)}{\partial x_j}    \notag \\ 
%   =& \sum_{i=1}^{2D}    \ell(g^{(1)}(x_1, \cdots, x_d), \cdots , g^{(2D)}(x_1, \cdots, x_d)) 
%   g^{(i)}(x_1, \cdots, x_d) \notag   \\ 
% = & \sum_{i=1}^{2D} \frac{\partial }{\partial g^{(i)}}   \ell(g^{(1)}(x), \cdots , g^{(2D)}(x)) 
%  \frac{\partial g^{(i)}(x)}{\partial x_j}    \notag \\ 
%   =&  \ell(g^{(1)}(x), \cdots , g^{(2D)}(x))  \sum_{i=1}^{2D}   
%   g^{(i)}(x) \notag 
% \end{align} 


% By the multivariate Fa\`a di Bruno formula. For each $k=1$, ..., $s-1$ fixed, and for each $\alpha\in \{1, \cdots, d\}^k$, we have 
% \begin{align} 
% & D^\alpha \ell(g^{(1)}(x), \cdots, g^{(2D)}(x)) \notag \\ 
% = &
%         \sum_{1 \leq |\beta| \leq k} (D^\beta \ell)(g^{(1)}(x), \cdots, g^{(2D)}(x))
%         \sum_{\eta, \zeta \in \calP(\alpha,\beta)} \alpha! 
%         \prod_{j=1}^{k} \frac{
%             [D^{\zeta^{(j)}} (g^{(1)}(x), \cdots, g^{(2D)}(x))]^{\eta^{(j)}}
%         }{
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         } .  \notag 
% \end{align} 





% Taking $x_1 = \cdots = x_d = 0$, we have 


% \paragraph{{General Case - Term~\Cref{t:B}}:}
% For each $\alpha\in \{1, \cdots, d\}^{s-1}$, by the multivariate Fa\`a di Bruno formula, we have    
% \begin{align}
%         D^\alpha \ell(f_1(x), f_2(x)) 
%         =
%         \sum_{1 \leq |\beta| \leq s-1} (D^\beta \ell)(f_1(x), f_2(x)) 
%         \sum_{\eta, \zeta \in \calP(\alpha,\beta)} \alpha! 
%         \prod_{j=1}^{s-1} \frac{
%             [D^{\zeta^{(j)}}(f_1(x), f_2(x))]^{\eta^{(j)}}
%         }{
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         }. 
%         \notag 
%     \end{align} 
% The Lipschitz constants of the derivatives satisfy 
% \begin{align}
%     &  \operatorname{Lip} \big(  D^\alpha \ell(f_1(x), f_2(x)) \big)  \notag \\ 
%     = & 
%         \sum_{1 \leq |\beta| \leq s-1} \operatorname{Lip} \big( (D^\beta \ell)(f_1(x), f_2(x)) \big)   
%         \sum_{\eta, \zeta \in \calP(\alpha,\beta)} \alpha! 
%         \prod_{j=1}^{s-1} \frac{
%            \operatorname{Lip}\big( [D^{\zeta^{(j)}}(f_1(x), f_2(x))]^{\eta^{(j)}} \big) 
%         }{
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         } 
%         \notag \\ 
%     \leq  & 
%         \sum_{1 \leq |\beta| \leq s-1} \widetilde{C}_{|\beta|+1}   
%         \sum_{\eta, \zeta \in \calP(\alpha,\beta)} \alpha ! 
%         \prod_{j=1}^{s-1} \frac{
%            (C_1 C_2)^{|\eta(j)|}  
%         }{
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         }.
% \label{eq:bound_t:B}
%     \end{align} 
% %    \begin{align} 
% %   \operatorname{Lip} \big( [D^{\zeta^{(j)}}(f_1(x), f_2(x))]^{\eta^{(j)}} \big)  
% % = & \operatorname{Lip} \big( [D^{\zeta^{(j)}}f_1(x), \,  D^{\zeta^{(j)}} f_2(x)]^{\eta^{(j)}} \big)  
% %    \notag \\ 
% %    = & (C_1 C_2)^{|\eta(j)|} \notag 
% %    \end{align} 

% %By the Rademacher-Stephanov theorem \citep[Theorems 3.1.6 and 3.1.9]{Federer_GeometricMeasureTheoryBook_1969}, 
% %\begin{align} 
% % \operatorname{Lip} \big( D^\alpha \ell(f_1(x), f_2(x)) \big)  
% % = & \max_{x\in \mathbb{R}^d} \Big| \nabla_x \Big(  D^\alpha \ell(f_1(x), f_2(x)) \Big) \Big| \notag \\ 
% % = & \max_{x\in \mathbb{R}^d} \Big| \big( D_{x_1}  D^\alpha \ell(f_1(x), f_2(x)) , \cdots, D_{x_d}  D^\alpha 
% % \ell(f_1(x), f_2(x)) \big) \Big|  
% % \notag 
% %\end{align} 

% \paragraph{Completing the General Case:}
% Combining our estimates for terms~\Cref{t:A} and~\Cref{t:B} respectively obtained in~\eqref{eq:bound_t:A} and~\eqref{eq:bound_t:B},
% we obtain an upper-bound for~\eqref{eq:definition_Cs__norm} via
% \begin{align} 
% \nonumber
%  \big\| \ell( f_1, f_2 ) \big\|_{C^s} 
%   \le &
%     \sum_{1 \leq |\beta| \leq k}  
%     %%%
%     \widetilde{C}_{|\beta|}  
%     \,
%     %%%
%         \sum_{\eta, \zeta \in \calP(\alpha,\beta)} 
%         \alpha! 
%         \,
%         \prod_{j=1}^{k} \frac{
%           (C_1 C_2 )^{|\eta^{(j)}|}  
%         }{
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         } 
% \\
%  + &
%     \sum_{1 \leq |\beta| \leq s-1} 
%     %%
%     \widetilde{C}_{|\beta|+1}   
%     \,
%     %%%
%         \sum_{\eta, \zeta \in \calP(\alpha,\beta)} 
%         \alpha! 
%         \,
%         \prod_{j=1}^{s-1} \frac{
%            (C_1 C_2)^{|\eta(j)|}  
%         }{
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         }.
% \label{eq:called_bound}
% \end{align} 

% \paragraph{Special Cases of Interest:}
% In particular, if $\ell$ belongs either to $C^{\infty}_{poly:C,r}(\mathbb{R}^d,\mathbb{R}^D)$ or to $C^{\infty}_{exp:C,r}(\mathbb{R}^d,\mathbb{R}^D)$, , as in Definition~\eqref{ass:Loss}, then: there exists constants $C_{\ell},r_{\ell}>0$ s.t.\ for each $j=1,\dots,s$ we have
% \begin{enumerate}
%     \item[(i)] \textbf{Polynomial Growth -  $C^{\infty}_{poly:C,r}(\mathbb{R}^d,\mathbb{R}^D)$ Case:} 
%     \[
%             \|\ell\|_{C^j}
%         \le
%             C\, j^{r}
%         \eqdef 
%             \tilde{C}_j
%     ,
%     \]
%     \item[(ii)] \textbf{Exponential Growth -  $C^{\infty}_{exp:C,r}(\mathbb{R}^d,\mathbb{R}^D)$ Case:} 
%     \[
%             \|\ell\|_{C^j} 
%         \le 
%             C\,e^{j\,r}
%         \eqdef 
%             \tilde{C}_j
%     .
%     \]
% \end{enumerate}
% Consequentially, in cases (i) and (ii), the bound in~\eqref{eq:called_bound} respectively becomes
% \begin{enumerate}
%     \item[(i)] \textbf{Polynomial Growth -  $C^{\infty}_{poly:C,r}(\mathbb{R}^d,\mathbb{R}^D)$ Case:} 
% \begin{align}
%  \big\| \ell( f_1, f_2 ) \big\|_{C^s} 
%   \le &
%     \sum_{1 \leq |\beta| \leq k}  
%     %%%
%     % \widetilde{C}_{|\beta|}  
%     C\, |\beta|^{r}
%     \,
%     %%%
%         \sum_{\eta, \zeta \in \calP(\alpha,\beta)} 
%         \alpha! 
%         \,
%         \prod_{j=1}^{k} \frac{
%           (C_1 C_2 )^{|\eta^{(j)}|}  
%         }{
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         } 
% \\
%  + &
%     \sum_{1 \leq |\beta| \leq s-1} 
%     %%
%     % \widetilde{C}_{|\beta|+1} 
%     C\, {(|\beta|+1)}^{r}
%     \,
%     %%%
%         \sum_{\eta, \zeta \in \calP(\alpha,\beta)} 
%         \alpha! 
%         \,
%         \prod_{j=1}^{s-1} \frac{
%            (C_1 C_2)^{|\eta(j)|}  
%         }{
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         }.
% \label{eq:called_bound__polynomial_case}
% \end{align}
%     \item[(ii)] \textbf{Exponential Growth -  $C^{\infty}_{exp:C,r}(\mathbb{R}^d,\mathbb{R}^D)$ Case:} 
% \begin{align}
%  \big\| \ell( f_1, f_2 ) \big\|_{C^s} 
%   \le &
%     \sum_{1 \leq |\beta| \leq k}  
%     %%%
%     % \widetilde{C}_{|\beta|}  
%     C\, e^{r\,|\beta|}
%     \,
%     %%%
%         \sum_{\eta, \zeta \in \calP(\alpha,\beta)} 
%         \alpha! 
%         \,
%         \prod_{j=1}^{k} \frac{
%           (C_1 C_2 )^{|\eta^{(j)}|}  
%         }{
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         } 
% \\
%  + &
%     \sum_{1 \leq |\beta| \leq s-1} 
%     %%
%     % \widetilde{C}_{|\beta|+1} 
%     C\, e^{r\,(|\beta|+1)}
%     \,
%     %%%
%         \sum_{\eta, \zeta \in \calP(\alpha,\beta)} 
%         \alpha! 
%         \,
%         \prod_{j=1}^{s-1} \frac{
%            (C_1 C_2)^{|\eta(j)|}  
%         }{
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         }.
% \label{eq:called_bound__exponential_case}
% \end{align}
% \end{enumerate}




% \end{proof} 





% \begin{remark}
% \label{rem:concentration}
% Next, we refine the strategy used in~\cite{hou2023instance} to convert our uniform risk-bound to a concentration of measure problem. Once done, the remainder of the proof will be to obtain bounds on the rate at which this measure concentrates.
% \end{remark}
% \begin{proof}[{Proof of Proposition~\ref{prop:Concentation}}]
% % \hfill\\
% % \noindent\textbf{Computing the $C^s$-norms of $\ell(f,\hat{f})$}
% % \AK{Need Xuwei's Lemma here}
% By hypothesis, $\tilde{f}\in C^s_r(\mathbb{R}^d)$ the induced map
% \begin{equation}
% \label{eq:composite_to_concentrate}
% \begin{aligned}
% f:  \mathbb{R}^{d}& \to \mathbb{R} \\
% x & \mapsto f(x)\eqdef \ell\big(f^{\star}(x),\tilde{f}(x)\big)
% \end{aligned}
% \end{equation}
% belongs to $C_R^s(\mathbb{R}^d)$.

% % \hfill\\
% \noindent\textbf{Conversion to a Concentration of Measure Problem}
% \hfill\\


% Denote the empirical (random) measure associated with the samples $\{(X_n,Y_n)\}_{n=1}^N$ by $\mu^{(N)}\eqdef \frac1{N}\sum_{n=1}^N\, \delta_{(X_n,Y_n)}$.
% Note that the generalization bound is $0$ for any constant function; therefore, we consider the bound over $C_R^s(\mathbb{R}^d)\setminus \operatorname{Lip}_0$ where $\operatorname{Lip}_0$ denotes the set of constant functions from $\mathbb{R}^d$ to $\mathbb{R}$.  Note the bijection between $C_R^s(\mathbb{R}^d)\setminus \operatorname{Lip}_0$ and $C_1^s(\mathbb{R}^d)\setminus \operatorname{Lip}_0$ given by $f\mapsto \frac1{\max\{1,\|f\|_{C^s(\mathbb{R}^d)}\}} f$.  Therefore, we compute
% \allowdisplaybreaks
% \begin{align}
% \nonumber
%         \sup_{g\in \mathcal{C}^s_R(\mathbb{R}^d)}
%         \,
%         \big|
%             \mathcal{R}_{\max\{t,N\}}(g)-\mathcal{R}^{(N)}(g)
%         \big|
%     \le &
%         R\,
%         \sup_{g\in \mathcal{C}^s_1(\mathbb{R}^d)}
%         \,
%         \big|
%             \mathcal{R}_{\max\{t,N\}}(g)-\mathcal{R}^{(N)}(g)
%         \big|
%     \\
% \nonumber
%     \le &
%         R\, d_{C^s}(\mu_{\max\{t,N\}},\mu^{(N)})
%     \\
%     \label{eq:TB_Bounded}
%     \le &
%         R\, \Big(
%             \underbrace{
%                 d_{C^s}(\mu_{\max\{t,N\}},\bar{\mu})
%             }_{\term{term_II}}
%     % \\
%     % &
%         +
%             \underbrace{
%                 d_{C^s}(\bar{\mu},\mu^{(N)})
%             }_{\term{term_I}}
%     \Big)
% .
% \end{align}
% Next, we bound terms $\text{(I)}$ and $\text{(II)}$.  

% \paragraph{Bounding Term~\eqref{term_II}}
% Under the uniform log-Sobolev Assumption~\ref{ass:MC},~\cite[Theorem 1.3]{BobkovGotze_1999_JFA} can be applied to $\bar{\mu}$ and $P(x,\cdot)$ for each $x\in \mathcal{X}$, implying that the transport inequalities hold: for each $\nu\in\mathcal{P}(\mathcal{X})$ and each $\tilde{\mu}\in \{\bar{\mu},\mu_0\}\cup \{P(x,\cdot)\}_{x\in \mathcal{X}}$
% \begin{equation}
% \label{eq:term_II__transport_inequalities}
%     \mathcal{W}_1(\tilde{\mu},\nu)^2
% \le 
%     2C^2\, \operatorname{KL}(\nu|\tilde{\mu})
% \end{equation}
% where we recall the definition of the Kullback–Leibler divergence $\operatorname{KL}(\nu|\mu)\eqdef \mathbb{E}_{X\sim \nu}[\log(\frac{d\nu}{d\mu}(X))]$.  Thus,~\eqref{eq:term_II__transport_inequalities} implies that the following exponential contractility property of the Markov kernel: there exists some $\kappa \in (0,1)$ such that for each $x,\tilde{x}\in \mathcal{X}$ and every $t\in \mathbb{N}_+$
% \begin{equation}
% \label{eq:exp_contract}
%     \mathcal{W}_1\big(P^t(x,\cdot),P^t(\tilde{x},\cdot)\big)
%     \le 
%     \kappa^t\, \|x-\tilde{x}\|
%     .
% \end{equation}
% Furthermore,~\eqref{eq:exp_contract} implies that 
% the conditions for~\citep[Theorem 1.5]{Riekert_ConcentrationOfMeasure2022} are met; whence, for every $\varepsilon\ge 0$ and each $N\in \mathbb{N}$ the following holds with probability at-least $
% 1-\exp\big(\frac{-N\,\varepsilon^2(1-\kappa)^2}{2C^2}\big)
% $
% \begin{equation}
% \label{eq:term_II__concentration}
%         d_s(\bar{\mu},\mu^{(N)})
%     \le 
%         \mathbb{E}\big[d_s(\bar{\mu},\mu^{(N)})\big]
%         +
%         \varepsilon
% .
% \end{equation}
% Upon setting $\varepsilon \eqdef 
% \frac{C\sqrt{2\ln(1/\delta)}}{\sqrt{N\,(1-\kappa^2)}}$,~\eqref{eq:term_II__concentration} implies that: for every $N\in \mathbb{N}$ and each $\delta \in (0,1]$ the following holds with probability at-least $1-\delta$
% \begin{equation}
% \label{eq:term_II__concentration___mod}
%         d_s(\bar{\mu},\mu^{(N)})
%     \le 
%         \underbrace{
%             \mathbb{E}\big[d_s(\bar{\mu},\mu^{(N)})\big]
%         }_{\term{term_III}}
%         +
%         \frac{C\sqrt{2\ln(1/\delta)}}{\sqrt{N\,(1-\kappa^2)}}
% .
% \end{equation}
% It remains to bound the expectation term~\eqref{term_III} in~\eqref{eq:term_II__concentration___mod} to bound term~\eqref{term_II}.

% Under the exponential moment assumption~\ref{ass:Exp_Moment}, we have that
% \begin{equation}
% \label{eq:exp_moment_repackaged}
% \mathbb{E}_{X\sim P(x,\cdot)}[e^{\beta|X|}-1]\le \gamma\, (e^{\beta|x|}-1) + (C-1+\gamma)
% .
% \end{equation}
% Therefore \citep[Proposition 1.3]{Riekert_ConcentrationOfMeasure2022}, implies that $\sup_{t\in \mathbb{N}_0}\, \mathbb{E}[e^{\beta|X_t|}-1]<\infty$.  Whence, \citep[Assumption 2]{Riekert_ConcentrationOfMeasure2022} holds with Young function $\Phi(x)=\frac1{\max\{1,\sup_{t\in \mathbb{N}_+\}}\mathbb{E}[e^{\beta|X_t}-1]}\,(e^{\beta|X_t|}-1)$; namely, $\sup_{t\in \mathbb{N}_0}\, \mathbb{E}[\Phi(|X_t|)]\le 1$.  Consequentially,~\citep[Theorem 1.1]{Riekert_ConcentrationOfMeasure2022} applies from which we conclude that there is some $t_0\in \mathbb{N}_+$ such that for all $N\ge t_0$
% \begin{equation}
% \label{eq:Bound_on_Expectation}
%     \eqref{term_III}
%     =
%     \mathbb{E}\big[d_s(\bar{\mu},\mu^{(N)})\big]
%     \lesssim
%     \,
%     \log\big(
%         (1-\kappa)\, N
%     \big)^{s}
%     \,
%     %%% NEW: Generate Rate
%         \begin{cases}
%            \frac{
%                \log\big(
%                     (1-\kappa)\, N
%                 \big)^{d/(2s) + 1}
%            }{
%                 (1-\kappa)^{1/2}\, N^{1/2}
%            } 
%             & \mbox{ if } 1=d<2s\\
%            %%%%
%            \frac{
%                \log\big(
%                     (1-\kappa)\, N
%                 \big)
%            }{
%                 (1-\kappa)^{1/2}\,N^{1/2}
%            } 
%             & \mbox{ if } d=2s\\
%         %%%%
%            \frac{
%                \log\big(
%                     (1-\kappa)\, N
%                 \big)^{d-2s+s/d}
%            }{
%                 (1-\kappa)^{s/d}\, N^{s/d}
%            } 
%             & \mbox{ if } d=2s\\
%         \end{cases}
% .
% \end{equation}


% Combining the order estimate of~\eqref{term_III} in~\eqref{eq:Bound_on_Expectation} with the estimate in~\eqref{eq:term_II__concentration___mod} implies that: for every $N\ge t_0$ and each $\delta \in (0,1]$ we have
% \begin{equation}
% \label{eq:term_II__concentration___done}
%         d_s(\bar{\mu},\mu^{(N)})
%     \lesssim
%         \,
%         %%% Concentration Term
%         \frac{
%             \sqrt{2\ln(1/\delta)}
%         }{
%             N^{1/2}
%         }
%         %%% Mean Term
%         +\,
%         %%% NEW: Generate Rate
%             \begin{cases}
%                \frac{
%                    \log\big(
%                         c\, N
%                     \big)^{d/(2s) + 1}
%                }{
%                     c\, N^{1/2}
%                } 
%                 & \mbox{ if } 1=d<2s\\
%                %%%%
%                \frac{
%                    \log\big(
%                         c\, N
%                     \big)
%                }{
%                     c\, N^{1/2}
%                } 
%                 & \mbox{ if } d=2s\\
%             %%%%
%                \frac{
%                    \log\big(
%                         c\, N
%                     \big)^{d-2s+s/d}
%                }{
%                    c_2\,  N^{s/d}
%                } 
%                 & \mbox{ if } d=2s\\
%             \end{cases}
% \end{equation}
% where $c\eqdef (1-\kappa), c_2\eqdef c^{s/d}\in (0,1)$.

% \paragraph{Bounding Term~\eqref{term_I}}
% We compute 
% \allowdisplaybreaks
% \begin{align}
% \nonumber
%     \eqref{term_I} = 
%         d_{C^s}(\mu_{\max\{t,N\}},\bar{\mu})
%     \eqdef &
%         \sup_{g\in \mathcal{C}^s_1(\mathbb{R}^d)}\, \mu_{\max\{t,N\}}[g]-\bar{\mu}[g]
% \\
%     \le & 
%     \label{eq:inclusion_CsLip}
%         \sup_{g\in \operatorname{Lip}_1(\mathbb{R}^d)}\, \mu_{\max\{t,N\}}[g]-\bar{\mu}[g]
% \\
%     = & 
%     \label{eq:KRDuality}
%         \mathcal{W}_1(\mu_{\max\{t,N\}},\bar{\mu})
% \\
%     = & 
%     % \label{eq:stationarity}
%         \mathcal{W}_1(P^t\mu_0,\bar{\mu})
% \\
%     = & 
%     \label{eq:stationarity}
%         \mathcal{W}_1(P^t\mu_0,P^t\bar{\mu})
% \\
%     \le & 
%     \label{eq:exp_contract2}
%         \kappa^t\, 
%         \mathcal{W}_1(\mu_0,\bar{\mu})
%     \eqdef 
%         \kappa^t\,C
% \end{align}
% where~\eqref{eq:inclusion_CsLip} held by definition of the MMD $d_{C^s}$ and by the inclusion of $\mathcal{C}_1^s(\mathbb{R}^d)\subset \operatorname{Lip}_1(\mathbb{R}^d)$,~\eqref{eq:KRDuality} held by Kantorovich duality (see \citep[Theorem 5.10]{VillaniBook_2009}),~\eqref{eq:stationarity} held since $\bar{\mu}$ is the stationary probability measure for the Markov chain $X_{\cdot}$, it is invariant to the action of the Markov kernel, and~\eqref{eq:exp_contract2} followed from \citep[Corollary 21]{olivera2019density} since we deduced the exponential contractility property~\eqref{eq:exp_contract} of the Markov kernel.  Note that $C\eqdef \mathcal{W}_1(\mu_0,\bar{\mu})$ is a constant depending only on the initial and stationary distributions of the Markov chain.

% \paragraph{Conclusion}
% Incorporating the estimates for~\eqref{term_I} and~\eqref{term_II} into the right-hand side of~\eqref{eq:TB_Bounded} implies that: for every $t,N\ge t_0$, $s\in \mathbb{N}_+$, and each $\delta\in (0,1]$ the following holds
% \[
%         \sup_{g\in \mathcal{C}^s_R(\mathbb{R}^d)}
%         \,
%         \frac{
%             \big|
%                 \mathcal{R}_{\max\{t,N\}}(g)-\mathcal{R}^{(N)}(g)
%             \big|
%         }{R}
%     \lesssim
%             %% Time-Shift Term
%                 I_{t<\infty}\,\kappa^t\,
%             +
%                 %%% Concentration Term
%                 \frac{
%                     \sqrt{2\ln(1/\delta)}
%                 }{
%                     N^{1/2}
%                 }
%                 %%% Mean Term
%                 +\,
%                 %%% NEW: Generate Rate
%                 \begin{cases}
%                    \frac{
%                        \log\big(
%                             c\, N
%                         \big)^{d/(2s) + 1}
%                    }{
%                         c\, N^{1/2}
%                    } 
%                     & \mbox{ if } 1=d<2s\\
%                    %%%%
%                    \frac{
%                        \log\big(
%                             c\, N
%                         \big)
%                    }{
%                         c\, N^{1/2}
%                    } 
%                     & \mbox{ if } d=2s\\
%                 %%%%
%                    \frac{
%                        \log\big(
%                             c\, N
%                         \big)^{d-2s+s/d}
%                    }{
%                        c_2\,  N^{s/d}
%                    } 
%                     & \mbox{ if } d=2s\\
%                 \end{cases}
% \]
% with probability at-least $1-\delta$; where $c\eqdef (1-\kappa)$ and $\kappa\in (0,1)$; where $I_{t<\infty}k^{\infty}\eqdef 0$ if $t=\infty$.
% \end{proof}



% \section{Bounding higher-order multivariate derivatives of composite functions}

% In this section, we will derive a bound for the Sobolev norm of multivariate composite functions.

% \subsection{Multivariate Fa\`a di Bruno formula revisited}
% We begin by establishing notation and stating the multivariate Fa\`a di Bruno formula from \cite{ConstantineSavits96}.

% \begin{theorem}[Multivariate Fa\`a di Bruno Formula, \cite{ConstantineSavits96}]\label{thm:FaaDiBruno}
%     Let $n, m, k \in \N$, $\alpha \in \N^k$ with $\vert \alpha \vert = n$, and define 
%     \begin{align*}
%         h(x_1, \ldots, x_k) \eqdef f^{(1)}(g^{(1)}(x_1, \ldots, x_k), \ldots, g^{(m)}(x_1, \ldots, x_k)).
%     \end{align*}
%     Then, using the multivariate notation from \Cref{not:Multivariate},
%     \begin{align*}
%         D^\alpha h(x) 
%         =
%         \sum_{1 \leq |\beta| \leq n} (D^\beta f)(g(x))
%         \sum_{\eta, \zeta \in \calP(\alpha,\beta)} \alpha! 
%         \prod_{j=1}^{n} \frac{
%             [D^{\zeta^{(j)}} g(x)]^{\eta^{(j)}}
%         }{
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         }.
%     \end{align*}
%     where 
%     \begin{multline*}
%         \calP(\alpha, \beta) = \Big\{ \eta \eqdef (\eta^{(1)}, \ldots, \eta^{(n)}) \in (\N^m)^n, \zeta\eqdef (\zeta^{(1)}, \ldots, \zeta^{(n)}) \in (\N^k)^n : \\
%          \exists j \leq m: \eta^{(i)} = 0, \zeta^{(i)} = 0 \text{ for } i < j, |\eta^{(i)}| > 0 \text{ for } i \geq j, \\
%          \textstyle 0 \prec \zeta^{(j)} \prec \ldots \prec \zeta^{(n)}, \sum_{i=1}^{n} \eta^{(i)} = \beta \text{ and } \sum_{i=1}^{n} |\eta^{(i)}|\zeta^{(i)} = \alpha \Big\} .
%     \end{multline*}
% \end{theorem}
% \begin{proof}
%     See \cite{ConstantineSavits96}.
% \end{proof}

% \begin{comment}
% \subsection{Bounds in Derivative-Depth}
% The goal of this section is to bound the derivative of composite functions by grouping over the multi-indices sum, i.e. all derivatives $D^\alpha$ with $\vert \alpha \vert = n$ are bounded uniformly.

% \begin{theorem}\label{thm:GeneralDerivativeBound}
%     In the notation of \Cref{thm:FaaDiBruno}, we have for a compact set $K \subseteq \R^k$
%     \begin{align*}
%         C^h_K(n)
%         &\leq
%         n!
%         \sum_{n' = 1}^n  \binom{n' + m - 1}{m - 1}  C^f_{g[K]}(n') 
%         \sum_{\eta, \zeta \in \calP^{d, k}_{n, n'}}
%         \prod_{j=1}^{n} 
%         \frac{1}{\eta^{(j)}!}
%         \left(\frac{
%             C^g_K(\vert \zeta^{(j)}\vert)
%         }{
%             \zeta^{(j)}!
%         }\right)^{|\eta^{(j)}|}.
%     \end{align*}
%     where 
%     \begin{itemize}[nosep]
%         \item $C^h_K(n) \eqdef \max_{\vert \alpha \vert = n}\Vert D^\alpha h\Vert_K$,
%         \item $C^f_{g[K]}(n') \eqdef \max_{\vert \alpha \vert = n'}\Vert D^\alpha f\Vert_{g[K]}$, 
%         \item $C^g_K(n') \eqdef \max_{\vert \alpha \vert = n'}\Vert D^\alpha g\Vert_K$,
%     \end{itemize}
%     and 
%     \begin{align*}
%     \calP^{d, k}_{n, n'} \eqdef \Big\{ &\eta \eqdef (\eta^{(1)}, \ldots, \eta^{(n)}) \in (\N^m)^n, \zeta\eqdef (\zeta^{(1)}, \ldots, \zeta^{(n)}) \in (\N^k)^n : \\
%     & \exists j \leq m: \eta^{(i)} = 0, \zeta^{(i)} = 0 \text{ for } i < j, |\eta^{(i)}| > 0 \text{ for } i \geq j, \\
%     & \textstyle 0 \prec \zeta^{(j)} \prec \ldots \prec \zeta^{(n)}, \big\vert \sum_{i=1}^{n} \eta^{(i)} \vert = n' \text{ and }  \vert \sum_{i=1}^{n} |\eta^{(i)}|\zeta^{(i)} \big\vert = n \Big\} .
% \end{align*}
% \end{theorem}

% \begin{proof}
% We have    
% \begin{align*}
%     \Vert D^\alpha h \Vert_K
%     &\leq
%     \sum_{1 \leq |\beta| \leq n} \Vert D^\beta f\Vert_{g[K]}
%     \sum_{\eta, \zeta \in \calP(\alpha,\beta)} \alpha! 
%     \prod_{j=1}^{n} \frac{
%         \prod_{i=1}^{m}
%         \Vert (D^{\zeta^{(j)}} g)_i \Vert_K^{\eta^{(j)}_i}
%     }{
%         \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%     } \\
%     &\leq
%     \sum_{1 \leq |\beta| \leq n} \Vert D^\beta f\Vert_{g[K]}
%     \sum_{\eta, \zeta \in \calP(\alpha,\beta)} \alpha! 
%     \prod_{j=1}^{n} 
%     \frac{1}{\eta^{(j)}!}
%     \left(\frac{
%         C^g_K(\vert \zeta^{(j)}\vert)
%     }{
%         \zeta^{(j)}!
%     }\right)^{|\eta^{(j)}|}.
% \end{align*}
% Defining 
% \begin{align*}
%     \calP_n(\beta) \eqdef \Big\{ &\eta \eqdef (\eta^{(1)}, \ldots, \eta^{(n)}) \in (\N^m)^n, \zeta\eqdef (\zeta^{(1)}, \ldots, \zeta^{(n)}) \in (\N^k)^n : \\
%     & \exists j \leq m: \eta^{(i)} = 0, \zeta^{(i)} = 0 \text{ for } i < j, |\eta^{(i)}| > 0 \text{ for } i \geq j, \\
%     & \textstyle 0 \prec \zeta^{(1)} \prec \ldots \prec \zeta^{(n)}, \sum_{i=1}^{n} \eta^{(i)} = \beta \text{ and }  \big\vert \sum_{i=1}^{n} |\eta^{(i)}|\zeta^{(i)} \big\vert = n \Big\} .
% \end{align*}
% results in 
% \begin{align*}
%     C^h_K(n)
%     &\leq
%     n!
%     \sum_{1 \leq |\beta| \leq n} \Vert D^\beta f\Vert_{g[K]}
%     \sum_{\eta, \zeta \in \calP_n(\beta)}
%     \prod_{j=1}^{n} 
%     \frac{1}{\eta^{(j)}!}
%     \left(\frac{
%         C^g_K(\vert \zeta^{(j)}\vert)
%     }{
%         \zeta^{(j)}!
%     }\right)^{|\eta^{(j)}|} \\
%     &\leq
%     n!
%     \sum_{1 \leq |\beta| \leq n}  C^f_{g[K]}(\vert \beta \vert)   
%     \sum_{\eta, \zeta \in \calP^{d, k}_{n, |\beta|}}
%     \prod_{j=1}^{n} 
%     \frac{1}{\eta^{(j)}!}
%     \left(\frac{
%         C^g_K(\vert \zeta^{(j)}\vert)
%     }{
%         \zeta^{(j)}!
%     }\right)^{|\eta^{(j)}|} \\
%     & =
%     n!
%     \sum_{n' = 1}^n  \binom{n' + m - 1}{m - 1}  C^f_{g[K]}(n') 
%     \sum_{\eta, \zeta \in \calP^{d, k}_{n, n'}}
%     \prod_{j=1}^{n} 
%     \frac{1}{\eta^{(j)}!}
%     \left(\frac{
%         C^g_K(\vert \zeta^{(j)}\vert)
%     }{
%         \zeta^{(j)}!
%     }\right)^{|\eta^{(j)}|}.
% \end{align*}
% \end{proof}

% \end{comment}
% \begin{comment}
% \begin{corollary}\label{cor:GeneralDerivativeBound2}
%     In the notation of \Cref{thm:GeneralDerivativeBound}, it holds that 
%     \begin{align*}
%         C^h_K(n)
%         \leq
%         \sum_{n' = 1}^n  
%         B(n, n')
%         C^f_{g[K]}(n') 
%         \prod_{l=1}^n \big(1 + C^g_K(l)\big)^{n'} ,
%     \end{align*}
% \end{corollary}
% \begin{proof}
%     Since  $\sum_{i=1}^{s} \vert \eta^{(i)} \vert = n'$, we have
%     \begin{align*}
%         C^h_K(n)
%         &\leq
%         n!
%         \sum_{n' = 1}^n  \binom{n' + m - 1}{m - 1}  C^f_{g[K]}(n') 
%         \sum_{\eta, \zeta \in \calP^{d, k}_{n, n'}}
%         \prod_{j=1}^{n} 
%         \frac{1}{\eta^{(j)}!}
%         \left(\frac{
%             C^g_K(\vert \zeta^{(j)}\vert)
%         }{
%             \zeta^{(j)}!
%         }\right)^{|\eta^{(j)}|} 
%     \\
%         &\leq
%         n!
%         \sum_{n' = 1}^n  \binom{n' + m - 1}{m - 1}  C^f_{g[K]}(n') 
%         \sum_{\eta, \zeta \in \calP^{d, k}_{n, n'}}
%         \prod_{j=1}^{n} 
%         \frac{\big(1 + C^g_K(\vert \zeta^{(j)}\vert)\big)^{|\eta^{(j)}|} }{\eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}}
%     \\
%         &\leq
%         n!
%         \sum_{n' = 1}^n  \binom{n' + m - 1}{m - 1}  C^f_{g[K]}(n') 
%         \sum_{\eta, \zeta \in \calP^{d, k}_{n, n'}}
%         \prod_{j=1}^{n} 
%         \frac{
%         \big(1 + C^g_K(j)\big)^{n'} 
%         }{
%         \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         }
%     \\
%         &=
%         \sum_{n' = 1}^n  \binom{n' + m - 1}{m - 1}  C^f_{g[K]}(n') 
%         \prod_{l=1}^n \big(1 + C^g_K(l)\big)^{n'} 
%         \sum_{\eta, \zeta \in \calP^{d, k}_{n, n'}}
%         \prod_{j=1}^{n} 
%         \frac{
%         n!
%         }{
%         \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         }
%     \end{align*}.
% \end{proof}
% \end{comment}
% \begin{comment}
% \begin{corollary}
%     In the notation of \Cref{cor:GeneralDerivativeBound2}, if there exists an $\Tilde{n} \leq n$ such that $C_K^g(\Tilde{n}) = 0$ it holds that 
%     \begin{align*}
%         C^h_K(n)
%         \leq
%         \sum_{n' = 1}^n  
%         B'(n, n')
%         C^f_{g[K]}(n') 
%         \prod_{l=1}^{\Tilde{n} - 1} \big(1 + C^g_K(l)\big)^{n'}.
%     \end{align*}
%     where 
%     \begin{align*}
%         B'(n, n')
%         \eqdef 
%         \binom{n' + m - 1}{m - 1}
%         \sum_{\eta, \zeta \in \calP^{d, k}_{n, n'}}
%         \prod_{j=1}^{n} 
%         \frac{
%         n! \mathbbm{1}_{\{\zeta^{(j)}<\Tilde{n}\}}
%         }{
%         \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         }.
%     \end{align*}
% \end{corollary}
% \begin{proof}
%     Analogue to \Cref{cor:GeneralDerivativeBound2}.
% \end{proof}
% \end{comment}
% \begin{comment}

% \begin{corollary}[Max derivative]
%     In the notation of \Cref{cor:GeneralDerivativeBound2}, 
%     \begin{align*}
%         C^h_K(n)
%         &\leq
%         \sum_{n' = 1}^n C^f_{g[K]}(n') 
%         (C^g_K)^{n'}
%         B(n, n')
%     \end{align*}
%     where $C^g_K \eqdef \max_{k \in \myset{1}{n}} C^g_K(k)$ and 
%     \begin{align*}
%         B(n, n')
%         \eqdef 
%         \binom{n' + m - 1}{m - 1}
%         \sum_{\eta, \zeta \in \calP^{d, k}_{n, n'}}
%         \prod_{j=1}^{n} 
%         \frac{
%         n!
%         }{
%         \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         }.
%     \end{align*}
% \end{corollary}
% \begin{proof}
%     Follows directly from $\sum_{i=1}^{n}\eta^{(i)} = n'$.
% \end{proof}

% \yannick{I believe this is tighter than \Cref{cor:GeneralDerivativeBound2} and more useful.}

% \end{comment}

% \subsection{Bounds in Derivative Type}


% The goal of this section is to bound the derivative of composite functions by grouping with respect to $\eqorder$, defined in \Cref{not:Order}.
% \begin{theorem}\label{thm:DerivativeBoundByType}
% In the notation of \Cref{thm:FaaDiBruno}, we have for a compact set $K \subseteq \R^k$ and an ordered multi-index $\alpha \in \Order^k_{n}$
% \begin{align*}
% C^h_K(\alpha)
%     &\leq
%     \alpha! \sum_{\beta \in \Order^m_{\leq n}}  N(\beta) C^f_{g[K]}(\beta)
%     \sum_{\eta, \zeta \in \calP'(\alpha,\beta)} 
%     \prod_{j=1}^{n} \frac{
%         C^g_K(\order(\zeta^{(j)}))^{\vert \eta^{(j)} \vert}
%     }{
%         \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%     },
% \end{align*}
% where $C^h_K(\cdot)$, $C^f_{g[K]}(\cdot)$, $C^g_K(\cdot)$ are defined as in \Cref{not:DerivativeBounds}; and 
% \begin{multline*}
%     \calP'(\alpha, \beta) = \Big\{ \eta \eqdef (\eta^{(1)}, \ldots, \eta^{(n)}) \in (\N^m)^n, \zeta\eqdef (\zeta^{(1)}, \ldots, \zeta^{(n)}) \in (\N^k)^n : \\
%     \exists j \leq m: \eta^{(i)} = 0, \zeta^{(i)} = 0 \text{ for } i < j, |\eta^{(i)}| > 0 \text{ for } i \geq j, \\
%     \textstyle 0 < \zeta^{(j)} \vartriangleleft \ldots \vartriangleleft \zeta^{(n)}, \sum_{i=1}^{n} \eta^{(i)} = \beta \text{ and } \sum_{i=1}^{n} |\eta^{(i)}|\zeta^{(i)} = \alpha \Big\} ,
% \end{multline*}
% where $\alpha \vartriangleleft \beta$ for $\alpha, \beta \in \N^k$ if $\vert \alpha \vert \leq \vert \beta \vert$ and  $\alpha \neq \beta$.
% \end{theorem}
% \begin{proof}
% We have for $\alpha \in \Order^k_{n}$
% \begin{align*}
%     C^h_K(\alpha)
%     &\leq
%     \max_{\gamma \eqorder \alpha}
%     \sum_{1 \leq |\beta| \leq n} \Vert D^\beta f\Vert_{g[K]}
%     \sum_{\eta, \zeta \in \calP(\gamma,\beta)} \alpha! 
%     \prod_{j=1}^{n} \frac{
%         \prod_{i=1}^{m}
%         \Vert (D^{\zeta^{(j)}} g)_i \Vert_K^{\eta^{(j)}_i}
%     }{
%         \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%     } \\
%     &\leq
%     \sum_{1 \leq |\beta| \leq n} C^f_{g[K]}(\order (\beta))
%     \max_{\gamma \eqorder \alpha}
%     \sum_{\eta, \zeta \in \calP(\gamma,\beta)} \alpha! 
%     \prod_{j=1}^{n} \frac{
%         C^g_K(\order(\zeta^{(j)}))^{\vert \eta^{(j)} \vert}
%     }{
%         \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%     }.
% \end{align*}
% Then 
% \begin{align*}
%     \mySet{\eta, (\order(\zeta^{(1)}), ..., \order(\zeta^{(n)}))}{ (\eta, \zeta) \in \calP'(\alpha, \beta)}
% \end{align*}
% is invariant in $\alpha$ with respect to $\eqorder$ and thus
% \begin{align*}
%     C^h_K(\alpha)
%     &\leq
%     \sum_{1 \leq |\beta| \leq n} C^f_{g[K]}(\order (\beta))
%     \sum_{\eta, \zeta \in \calP'(\alpha,\beta)} \alpha! 
%     \prod_{j=1}^{n} \frac{
%         C^g_K(\order(\zeta^{(j)}))^{\vert \eta^{(j)} \vert}
%     }{
%         \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%     }.
% \end{align*}
% Further, notice that
% \begin{align*}
%     \mySet{((\vert \eta^{(1)}\vert, \eta^{(1)}!), \ldots, (\vert \eta^{(n)}\vert, \eta^{(n)}!)), \zeta}{ (\eta, \zeta) \in \calP'(\alpha, \beta)}
% \end{align*}
% is invariant in $\beta$ with respect to $\eqorder$ and the assertion follows.
% \end{proof}

% \begin{corollary}\label{cor:DerivativeBoundAffine}
%     In the notation of \Cref{thm:DerivativeBoundByType}, if $f$ is affine-linear, 
%     \begin{align*}
%         C^h_K(\alpha)
%         &\leq
%         m \alpha! C^f_{g[K]}(e_1)
%         C^g_K(\alpha),
%     \end{align*}
%     where $C^f_{g[K]}(e_1)$ is the maximum weight of the matrix representing $f$. 
% \end{corollary}
% \begin{proof}
%     \Cref{thm:DerivativeBoundByType} yields
%     \begin{align*}
%         C^h_K(\alpha)
%         &\leq
%         m \alpha! C^f_{g[K]}(e_1)
%         \sum_{\eta, \zeta \in \calP'(\alpha,\beta)} 
%         \prod_{j=1}^{n} \frac{
%             C^g_K(\order(\zeta^{(j)}))^{\vert \eta^{(j)} \vert}
%         }{
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         },
%     \end{align*}
%     and since $\calP'(\alpha, e_1) = \{(0, ..., 0, e_1), (0, ..., 0, \alpha) \}$ the result follows.
% \end{proof}

% \begin{comment}
% \subsection{Special Cases}

% \begin{corollary}[Affine linear transformations]
% In the notation of \Cref{thm:GeneralDerivativeBound}, if $f$ is affine-linear, 
%     \begin{align*}
%         C^h_K(n)
%         &\leq
%         C^f_{g[K]}(1) 
%         C^g_K(n)
%         \sum_{\vert \alpha \vert = n}
%         \frac{
%         m \cdot n! 
%         }{
%             \alpha !
%         }.
%     \end{align*}
% \end{corollary}
% \begin{proof}
%     \Cref{thm:GeneralDerivativeBound} yields
%     \begin{align*}
%         C^h_K(n)
%         &\leq
%         n!
%         \sum_{n' = 1}^n  \binom{n' + m - 1}{m - 1}  C^f_{g[K]}(n') 
%         \sum_{\eta, \zeta \in \calP^{d, k}_{n, n'}}
%         \prod_{j=1}^{n} 
%         \frac{1}{\eta^{(j)}!}
%         \left(\frac{
%             C^g_K(\vert \zeta^{(j)}\vert)
%         }{
%             \zeta^{(j)}!
%         }\right)^{|\eta^{(j)}|}.
%     \end{align*}
%     Since $C^f_{g[K]}(n') = 0$  for $n'>1$, 
%     \begin{align*}
%         C^h_K(n)
%         &\leq
%         m \cdot n! \cdot
%           C^f_{g[K]}(1) 
%         \sum_{\eta, \zeta \in \calP^{d, k}_{n, 1}}
%         \prod_{j=1}^{n} 
%         \frac{1}{\eta^{(j)}!}
%         \left(\frac{
%             C^g_K(\vert \zeta^{(j)}\vert)
%         }{
%             \zeta^{(j)}!
%         }\right)^{|\eta^{(j)}|}.
%     \end{align*}
%     The definition of $\calP^{d, k}_{n, 1}$ forces $\zeta^{(j)}, \eta^{(j)} = 0$ for $j < n$, $|\eta^{(n)}| = \eta^{(n)}! = 1$, as well as $\vert \zeta^{(n)}\vert = n$, which yields
%     \begin{align*}
%         C^h_K(n)
%         &\leq
%         m \cdot n! \cdot
%           C^f_{g[K]}(1) 
%         \sum_{\eta, \zeta \in \calP^{d, k}_{n, 1}}
%         \left(\frac{
%             C^g_K(n)
%         }{
%             \zeta^{(n)}!
%         }\right)\\
%         &\leq
%         C^f_{g[K]}(1) 
%         C^g_K(n)
%         \sum_{\vert \alpha \vert = n}
%         \frac{
%         m \cdot n! 
%         }{
%             \alpha !
%         }.
%     \end{align*}
% \end{proof}
% \end{comment}

% \begin{comment}
% \subsection{Combinatorics}

% Recall 
%     \begin{align*}
%         B(n, n')
%         \eqdef 
%         \binom{n' + m - 1}{m - 1}
%         \sum_{\eta, \zeta \in \calP^{d, k}_{n, n'}}
%         \prod_{i=1}^{n} 
%         \frac{
%         n!
%         }{
%         \eta^{(i)}!(\zeta^{(i)}!)^{|\eta^{(i)}|}
%         }.
%     \end{align*}
% where
%     \begin{align*}
%     \calP^{d, k}_{n, n'} 
%     = \Big\{ &\eta \eqdef (\eta^{(1)}, \ldots, \eta^{(n)}) \in (\N^m)^n, \zeta\eqdef (\zeta^{(1)}, \ldots, \zeta^{(n)}) \in (\N^k)^n : \\
%     & \exists j \leq m: \eta^{(i)} = 0, \zeta^{(i)} = 0 \text{ for } i < j, |\eta^{(i)}| > 0 \text{ for } i \geq j, \\
%     & \textstyle 0 \prec \zeta^{(j)} \prec \ldots \prec \zeta^{(n)},  \sum_{i=1}^{n} \vert \eta^{(i)} \vert = n' \text{ and }  \vert \sum_{i=1}^{n} |\eta^{(i)}|\zeta^{(i)} \big\vert = n \Big\} .
%     \end{align*}
% This yields
% \begin{align*}
%     B(n, n') = 
%         \binom{n' + m - 1}{m - 1}
%         \sum_{j=1}^n
%         \sum_{\eta \in E^{d, k}_{n, n', j}}
%         \sum_{\zeta \in Z^{d, k}_{n, n', j}(\eta) }
%         \prod_{i=1}^{n} 
%         \frac{
%         n!
%         }{
%         \eta^{(i)}!(\zeta^{(i)}!)^{|\eta^{(i)}|}
%             },
% \end{align*}
% where 
% \begin{align*}
%     E^{d, k}_{n, n', j} 
%     = \Big\{ &\eta \eqdef (\eta^{(1)}, \ldots, \eta^{(n)}) \in (\N^m)^n: \\
%     & \eta^{(i)} = 0 \text{ for } i < j, |\eta^{(i)}| > 0 \text{ for } i \geq j, 
%     \textstyle  \sum_{i=1}^{n} \vert \eta^{(i)} \vert = n' \Big\} ,
%     \\
%     Z^{d, k}_{n, n', j}(\eta) 
%     = \Big\{ &\eta \eqdef (
%     \zeta\eqdef (\zeta^{(1)}, \ldots, \zeta^{(n)}) \in (\N^k)^n : \\
%     & \zeta^{(i)} = 0 \text{ for } i < j, 
%     \textstyle 0 \prec \zeta^{(j)} \prec \ldots \prec \zeta^{(n)}, \text{ and }  \sum_{i=1}^{n} |\eta^{(i)}|\vert \zeta^{(i)} \vert = n \Big\} .
% \end{align*}
% With writing $\eta! \eqdef \prod_{i=1}^n \eta^{(i)}!$, we arrive at 
% \begin{align*}
%      B(n, n') &= 
%         \binom{n' + m - 1}{m - 1}
%         \sum_{j=1}^n
%         \sum_{\eta \in E^{d, k}_{n, n', j}}
%         \frac{1}{\eta!}
%         \sum_{\zeta \in Z^{d, k}_{n, n', j}(\eta) }
%         \prod_{i=1}^{n} 
%         \frac{
%         n!
%         }{
%         (\zeta^{(i)}!)^{|\eta^{(i)}|}
%         }. \\
%         &= 
%         \binom{n' + m - 1}{m - 1}
%         \sum_{j=1}^n
%         \sum_{\substack{\gamma \in \N^n , \vert \gamma \vert = n'}}
%         D(\gamma)
%         \sum_{\zeta \in Z^{d, k}_{n, n', j}(\gamma) }
%         \prod_{i=1}^{n} 
%         \frac{
%         n!
%         }{
%         (\zeta^{(i)}!)^{\gamma_i}
%         },
% \end{align*}
% where 
% \begin{align*}
%     D(\gamma) \eqdef  \sum_{{\eta \in E^{d, k}_{n, n', j} , \vert \eta^{(i)}\vert = \gamma_i }}
%         \frac{1}{\eta!}.
% \end{align*}
    
% \end{comment}

% \section{Bounding Higher-Order Multivariate Derivatives of Transformer Building Blocks}
% \subsection{Softmax}

% \begin{lemma}[Representation of higher-order $\softmax$ derivatives]\label{lem:SoftmaxDerivativeRepresentation}
% For $F \in \N$ and
% \begin{align*}%\label{id:Softmax}
%     \smax:
%             \R^F 
%         \to     
%             \R^F,
%     \quad 
%             x 
%         \mapsto 
%             \left(
%                     {\exp(x_i)}
%                 /
%                     {\textstyle\sum_{j = 0}^{F-1} \exp(x_j)}
%             \right)_{i=1}^{F}.
% \end{align*}
% there exists for any multi-index $\alpha \in \N^F$ and $m \in \myset{1}{F}$ indicators $(a_{i, j}^k)_{i, j \in I(\alpha)}^{k \in \myset{1}{\vert \alpha \vert!}} \subseteq \{0, 1\}$ such that 
% \begin{align}
%     \smax^{(\alpha)} (x_m) = \sum_{k = 1}^{\vert \alpha \vert!} \smax(x_{m}) \prod_{i,j \in I(\alpha)} (a^k_{i,j}  - \smax(x_{j})), \label{id:SoftmaxDerivativeShape}
% \end{align}
% where $I(\alpha)\eqdef \{(i, j): i = 1, \ldots, F, j = 1, \ldots, \alpha_i\}$.
% \end{lemma}
% \begin{proof}
%     For $\vert \alpha \vert = 0$, we have $n \in \myset{1}{F}$ s.t. $\alpha_n = 1$, therfore 
%     \begin{align*}
%         \smax^{(\alpha)} (x_m) = \frac{\partial \smax}{\partial x_{n}} (x_{m}) = \smax(x_{m})\left( \delta_{m n} - \smax(x_{n})\right),
%     \end{align*}
%     which is of the form \eqref{id:SoftmaxDerivativeShape}. Now, let $\alpha \in \N^F$ arbitrary, therefore, by defining $\alpha' \in \N^F$ by $\alpha'_i \eqdef \alpha_i$ for $i \neq n$ and $\alpha'_n \eqdef \alpha_n - 1$ (w.l.o.g. $\alpha_n > 0$). We have 
%     \begin{align*}
%         \smax^{(\alpha)} (x_m) 
%         & = \frac{\partial \smax^{(\alpha')}}{\partial x_{n}} (x_{m}) \\
%         & = \frac{\partial}{\partial x_{n}} \sum_{k = 1}^{\vert \alpha' \vert!} \smax(x_{m}) \prod_{i,j \in I(\alpha')}(a^{\prime k}_{i,j}  - \smax(x_{j})).
%     \end{align*}
%     Since for any $k$
%     \begin{align*}
%         & \frac{\partial}{\partial x_{n}} \smax(x_{m}) \prod_{i,j \in I(\alpha')}(a^{\prime k}_{i,j}  - \smax(x_{j})) \\
%         & = \smax(x_{m})\left( \delta_{m n} - \smax(x_{n})\right)  \prod_{i,j \in I(\alpha')} (a^{\prime k}_{i,j}  - \smax(x_{j})) \\ 
%         & \quad +  \smax(x_{m}) \sum_{i',j' \in I(\alpha')}  
%          - \smax(x_{j'})\left(\delta_{j',n} - \smax(x_{n})\right) 
%         \prod_{\substack{i,j \in I(\alpha) \\ (i,j) \neq (i',j')}}(a^{\prime k}_{i,j}  - \smax(x_{j})),
%     \end{align*}
%     we can define $(a_{i, j}^k)_{i, j \in I(\alpha)}^{k \in \myset{1}{\vert \alpha' \vert + 1}} \subseteq \{0, 1\}$ such that
%     \begin{align*}
%         \frac{\partial}{\partial x_{n}} \smax(x_{m}) \prod_{i,j \in I(\alpha')}(a^{\prime k}_{i,j}  - \smax(x_{j}))
%         = \sum_{k=1}^{\vert \alpha \vert}\smax(x_{m}) \prod_{i,j \in I(\alpha)} (a^{k}_{i,j}  - \smax(x_{j})). 
%     \end{align*}
%     Since $\vert \alpha \vert ! = \vert \alpha \vert \cdot \vert \alpha' \vert !$, this concludes the proof.
% \end{proof} 

% \begin{proof} 

% \begin{align} 
%   \softmax^{(\alpha)}(x_0, x_1, ..., x_{F-1})  = 
%   \Big( \Big( \frac{e^{x_0}}{\sum_{j=0}^{F-1} e^{x_j} } \Big)^{(\alpha)} , \, 
%     \Big( \frac{e^{x_1}}{\sum_{j=0}^{F-1} e^{x_j} } \Big)^{(\alpha)} , \, \cdots, \, 
%      \Big( \frac{e^{x_{F-1}}}{\sum_{j=0}^{F-1} e^{x_j} } \Big)^{(\alpha)} \Big) \notag 
% \end{align} 

% The $i$-th component of the softmax function can be represented as 
% \begin{align} 
% &  \frac{e^{x_i}}{\sum_{j=0}^{F-1} e^{x_j} } = f_i( g(x_0, x_1, ..., x_{F-1})    ) 
%   \notag \\ 
%   & g(x_0, x_1, ..., x_{F-1}) = \big( g_0, g_1, ..., g_{F-1} \big)
%   = \big( e^{x_0}, e^{x_1}, \, ..., \, e^{x_{F-1}} \big) \notag \\ 
%   & f_i (g_0, g_1, ..., g_{F-1}) = \frac{g_i}{ \sum_{j=0}^{F-1} g_j } . \notag 
% \end{align} 
% For simplicity of notation, we denote $x=(x_0, x_1, ..., x_{F-1}) \in \mathbb{R}^F$. 
% By Theorem~\ref{thm:FaaDiBruno}, we have 
% \begin{align} 
%  D^\alpha f_i(g(x)) 
%  = \sum_{1 \leq |\beta| \leq n} (D^\beta f_i)(g(x)) 
%  \sum_{\eta, \zeta \in \calP(\alpha,\beta)} \alpha! 
%         \prod_{j=1}^{n} \frac{
%             [D^{\zeta^{(j)}} g(x)]^{\eta^{(j)}}
%         }{
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         }. 
%         \notag 
% \end{align} 

% \begin{align} 
%  D^{\zeta^{(j)}} g(x) = \big( D^{\zeta^{(j)}} g_0(x), D^{\zeta^{(j)}} g_1(x), \, ..., \, 
%   D^{\zeta^{(j)}} g_{F-1}(x) \big)  \notag 
% \end{align} 

% We can show by induction that for $i\neq j_1$, ..., $j_n$
% \begin{align} 
%  \frac{\partial^{\alpha_1+\cdots + \alpha_n} f_i}{\partial g_{j_1}^{\alpha_1} \cdots \partial g_{j_n}^{\alpha_n}} 
%   = (-1)^{\alpha_1+\cdots + \alpha_n} (\alpha_1+\cdots + \alpha_n)! \frac{g_i}{ ( \sum_{j=0}^{F-1} g_j )^{\alpha_1+\cdots + \alpha_n+1} }   \notag 
% \end{align} 


% \end{proof} 


% \begin{lemma}[Bound on higher-order $\softmax$ derivatives]
%     With \Cref{not:DerivativeBounds}, it holds for any set $K \in \R^k, k\in \N$ and any $\alpha \in \Order^k_{< \infty}$ that
%     \begin{align*}
%         C^{\smax}(\alpha) \leq \vert \alpha \vert!.
%     \end{align*}
% \end{lemma}
% \begin{proof}
%     This is a direct consequence of the representation in \Cref{lem:SoftmaxDerivativeRepresentation} together with $\Vert \smax \Vert = 1$.
% \end{proof}


% \subsection{Multi-Head Self-Attention}
% \yannick{This needs an update with the index notation $\idim, \kdim, \vdim, \odim$.}
% \begin{lemma}[Dot product]\label{lem:Dotp}
%     In the notation of \Cref{defn:MultiHead} and for $m \in \myset{1}{M}$
%     \begin{align*}
%         \dotp_m(\,\cdot\,; Q, K): 
%                 \R^{(M+1)d_0} 
%             \longrightarrow 
%                 \R^{M}
%             , \quad
%                 x
%             \longmapsto
%                 \langle
%                     Qx_m, Kx_j
%                 \rangle_{j = 0}^{M} 
%     \end{align*}
%     we have using \Cref{not:DerivativeBounds}
%     \begin{enumerate}
%     \item $ C^{\dotp_m}_K(e_1) \leq  2 d_0 d_1 \Vert K \Vert C^{Q}C^{K}$, where $C^Q \eqdef \max_{i, i' \in \myset{1}{d_1}\times \myset{1}{d_0}} \vert Q_{i, i'}\vert$, $C^K$ analogously, and $\Vert K \Vert \eqdef \max_{x \in K} \Vert x \Vert$. Additionally,
%     \item  $ C^{\dotp_m}_K( \alpha ) \leq  2 d_1  C^{Q}C^{K}$, for $\vert \alpha \vert = 2$, and 
%     \item $C^{\dotp_m}_K(\alpha) = 0$ for $\vert \alpha \vert > 2$.
%     \end{enumerate}
%     Since all bounds are not dependent on $m$ we write $C^{\dotp}$ short for $C^{\dotp_m}$.
% \end{lemma}
% \begin{proof}%
%     \begin{enumerate}[wide]%
%     \item  Let $l = (l_1, l_2) \in \myset{1}{(M+1)} \times \myset{1}{d_0}$. 
%     Assume $l_1 = m$. If $j \neq m$, then
%         \begin{align*}
%                 D^{e_l}\dotp_m(x; Q, K)_j 
%             =   
%                 D^{e_l}
%                 \sum_{i=1}^{d_1}
%                  (Kx_j)_i
%                 \sum_{i'=1}^{d_0}
%                     Q_{i, i'}(x_m)_{i'}
%             =   
%                 \sum_{i=1}^{d_1}
%                 \bigg(\sum_{i'=1}^{d_0}
%                     K_{i, i'}(x_j)_{i'}
%                     \bigg)
%                 Q_{i, l_2},
%         \end{align*}
%     implying
%     \begin{align}\label{id:DotPSimple}
%             \Vert D^{e_l}\dotp_m(x; Q, K) \Vert 
%         \leq 
%             \Vert K \Vert
%             \sum_{i=1}^{d_1}
%             Q_{i, l_2}
%             \sum_{i'=1}^{d_0}
%                 K_{i, i'}
%         \leq 
%             d_0 d_1
%             \Vert K \Vert
%             C^{Q}C^{K}
%         .
%     \end{align}
%     If $j = m$, 
%         \begin{align*}
%                 D^{e_l}\dotp_m(x; Q, K)_j 
%             &=   
%                 D^{e_l}
%                 \sum_{i=1}^{d_1}
%                 \bigg(\sum_{i'=1}^{d_0}
%                     K_{i, i'}(x_m)_{i'}
%                     \bigg)
%                 \bigg(\sum_{i'=1}^{d_0}
%                     Q_{i, i'}(x_m)_{i'}
%                     \bigg) \\ 
%             &=   
%                 \sum_{i=1}^{d_1}
%                     \bigg(
%                     K_{i, l_2}
%                 \sum_{i'=1}^{d_0}
%                     Q_{i, i'}(x_m)_{i'}
%                 +
%                     Q_{i, l_2}
%                 \sum_{i'=1}^{d_0}
%                     K_{i, i'}(x_m)_{i'}
%                     \bigg)
%         \end{align*}
%    therefore implying     
%     \begin{align*}
%             \Vert D^{e_l}\dotp_m(x; Q, K) \Vert 
%         \leq 
%             2 d_0 d_1
%             \Vert K \Vert
%             C^{Q}C^{K}
%         .
%     \end{align*}
%     If $l_1 \neq m$ then for $j \neq l_1$, $D^{e_l}\dotp_m(x; Q, K)_j = 0$, for $j = l_1$
%     \begin{align*}
%                 D^{e_l}\dotp_m(x; Q, K)_j 
%             =   
%                 D^{e_l}
%                 \sum_{i=1}^{d_1}
%                 (Qx_m)_i
%                 \sum_{i'=1}^{d_0}
%                 K_{i, i'}(x_j)_{i'}
%             =   
%                 \sum_{i=1}^{d_1}
%                 \bigg(\sum_{i'=1}^{d_0}
%                     Q_{i, i'}(x_m)_{i'}
%                     \bigg)
%                 K_{i, l_2},
%         \end{align*}
%         and we obtain \eqref{id:DotPSimple} analogously.
%     \item If $l_1 = m$ and $j \neq m$
%     \begin{align*}
%         D^{e_l}\bigg(
%             (x_m)_{l_2}
%                 \sum_{i=1}^{d_1}
%                 \bigg(\sum_{i'=1}^{d_0}
%                     k_{i, i'}(x_j)_{i'}
%                     \bigg)
%                 q_{i, l_2}
%             \bigg) = 0,
%     \end{align*}
%     implying $\Vert D^{2e_l}\dotp_m(x; Q, K) \Vert \leq 0$, what analogously holds for $l_1 \neq m$. However, for $l_1 = m$ and  $j = m$
%     \begin{align*}
%         D^{e_l}\bigg(
%                 \sum_{i=1}^{d_1}
%                     K_{i, l_2}
%                 \sum_{i'=1}^{d_0}
%                     Q_{i, i'}(x_m)_{i'}
%                 +
%                     Q_{i, l_2}
%                 \sum_{i'=1}^{d_0}
%                     K_{i, i'}(x_m)_{i'} \bigg)
%          = 
%                 \sum_{i=1}^{d_1}
%                     K_{i, l_2}
%                     Q_{i, l_2}
%                 +
%                     Q_{i, l_2}
%                     K_{i, l_2}
%     \end{align*}
%     we have
%     \begin{align*}
%             \Vert D^{2e_l}\dotp_m(x; Q, K) \Vert 
%         \leq 
%             2 
%             d_1 
%             C^{Q}C^{K}
%         .
%     \end{align*}
%     \item  Let $l' = (l'_1, l'_2) \in \myset{1}{(M+1)} \times \myset{1}{d_0}$. Assume $l_1 = m$, $j \neq m$. If $l'_1 \neq j$, $D^{e_l + e_{l'}}\dotp_m(x; Q, K)_j = 0$. For $l'_1 = j$ follows $D^{e_l + e_{l'}}\dotp_m(x; Q, K)_j =  \sum_{i = 1}^{d_1} K_{i, l'_2}Q_{i, l_2}$. If $l_1 = m$, $j \neq m$, we have  $D^{e_l + e_{l'}}\dotp_m(x; Q, K)_j = 0$ in the case that $l'_1 \neq m$, and for $l'_1 \neq m$ we obtain
%     \begin{align*}
%         D^{e_l + e_{l'}}\dotp_m(x; Q, K)_j = 
%                 \sum_{i=1}^{d_1}
%                     K_{i, l_2}
%                     Q_{i, l'_2}
%                 +
%                     Q_{i, l_2}
%                     K_{i, l'_2}.
%     \end{align*}
%     This means, we can use the bound 
%     \begin{align*}
%             \Vert D^{e_l + e_{l'}}\dotp_m(x; Q, K) \Vert 
%         \leq 
%             2 
%             d_1 
%             C^{Q}C^{K}
%         .
%     \end{align*}
% \end{enumerate}
% \end{proof}
% \begin{lemma}[Self-Attention]\label{lem:Attention}
%     Using the notation of  \Cref{not:DerivativeBounds}, \Cref{defn:MultiHead} and \Cref{lem:Dotp}, it holds that
%    \begin{align*}%\label{id:Attention}
%     C_K^{
%         \attention
%     }(\alpha)
%     \leq    
%     d_0
%     (M + 1)
%     C^V
%     \left(
%         \Vert K \Vert
%         C_K^{
%             \smax \circ \dotp
%         }(\alpha)
%     +
%         \sum_{l=1}^{(M+1)d_0}
%         \alpha_l
%         C_K^{
%             \smax \circ \dotp
%         }(\alpha - e_l)
%     \right)
% \end{align*} 
% where 
% \begin{align}
% C^{\smax \circ \dotp}_K(\alpha)
%     &\leq
%     \alpha! \sum_{\beta \in \Order^{M+1}_{\leq n}}  N(\beta) C^{\smax}_{\dotp[K]}(\beta)
%     \sum_{\eta, \zeta \in \calP'(\alpha,\beta)} 
%     \prod_{j=1}^{n} \frac{
%         C^{\dotp}_K(\order(\zeta^{(j)}))^{\vert \eta^{(j)} \vert}
%     }{
%         \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%     }. \label{id:SmaxDpCompositeBound}
% \end{align}
% \end{lemma}
% \begin{proof}
%     Fix $\alpha \in \N^k$, and note that
%     \begin{align*}
%         \Vert
%             D^{\alpha}
%             \attention(
%                 x; Q, K, V 
%             ) 
%         \Vert
%         \leq
%         \max_{m\in \myset{0}{M}}
%         \max_{i\in \myset{0}{d_2}}
%         \Vert
%             D^{\alpha}
%             \attention(
%                 x; Q, K, V 
%             )_{m,i}
%         \Vert
%     \end{align*}
%     and
%     \begin{align*}
%          \Vert
%         D^{\alpha}
%         \attention(&
%             x; Q, K, V 
%         )_{m,i}
%         \Vert \\
%         &\leq
%         \sum_{j=0}^M
%         \sum_{i'=0}^{d_0}
%         \Vert
%             D^{\alpha}
%             \smax \circ \dotp(x; Q, K)_j
%             V_{i, i'}(x_j)_{i'}
%         \Vert \\
%         &\leq
%         d_0(M + 1)
%         \max_{j\in \myset{0}{M}}
%         \max_{i'\in \myset{0}{d_0}}
%         \Vert
%             D^{\alpha}
%             \smax \circ \dotp(x; Q, K)_j
%             V_{i, i'}(x_j)_{i'}
%         \Vert.
%     \end{align*}
%     Due to the extended Leibnitz rule \cite{Hardy06}, we have
%     \begin{multline*}
%         \Vert
%             D^{\alpha}
%             \smax \circ \dotp(x; Q, K)_j
%             V_{i, i'}(x_j)_{i'}
%         \Vert
%         \\ \leq
%         \Vert
%             D^{\alpha}
%             \smax \circ \dotp(x; Q, K)_j
%             V_{i, i'}(x_j)_{i'}
%         \Vert
%         +
%         \sum_{l=1}^{(M+1)d_0}
%         V_{i, i'}
%         \alpha_l
%         \Vert
%             D^{\alpha - e_l}
%             \smax \circ \dotp(x; Q, K)_j
%         \Vert.
%     \end{multline*}
%     \Cref{id:SmaxDpCompositeBound} follows direclty from \Cref{thm:DerivativeBoundByType}.
% \end{proof}

% \begin{corollary}[Multi-head Self-Attention]\label{cor:MultiHead}
%     In the notation of \Cref{defn:MultiHead}, \Cref{thm:DerivativeBoundByType} and \Cref{lem:Dotp} it holds that 
%     \begin{align*}
%         C^{\multihead}_K(\alpha)
%         &\leq
%         \alpha! 
%         d_2 
%         C^{W}
%         C^{\attention}_K(\alpha)
%     \end{align*}
%     where 
%     \begin{align*}
%         C^{\attention}_K \eqdef  \max_{h \in \myset{1}{H}}C^{\attention(\, \cdot\,; Q^{(h)}, K^{(h)}, V^{(h)})}_K , \quad C^{W} \eqdef \max_{h \in \myset{1}{H}} W^{(h)}.
%     \end{align*}
% \end{corollary}
% \begin{proof}
%     Follows directly from \Cref{cor:DerivativeBoundAffine} and \Cref{lem:Attention}.
% \end{proof}

% \subsection{Activation Functions}
% \begin{lemma}[Derivatives of $\softplus$]
%     For 
%     \begin{align*}
%         \softplus: \R \to \R, \quad x \mapsto \ln (1 + \exp(\cdot))
%     \end{align*}
%     it holds 
%     \begin{align*}
%         \softplus^{(1)}(x) = \sigmoid(x) \eqdef 1 / (1 + \exp(-x))
%     \end{align*}
%     and for $n \in \N$
%     \begin{align*}
%         \softplus^{(n + 1)}(x) = \sigmoid^{(n)}(x) = \sum_{k=0}^n(-1)^{n+k}k!S_{n,k}\sigmoid(x)(1-\sigmoid(x))^k,
%     \end{align*}
%     where $S_{n,k}$ are the Stirling numbers of the second kind, $S_{n,k} \eqdef \frac{1}{k!} \sum_{j=0}^{k} (-1)^{k-j} \binom{k}{j} j^n$.
% \end{lemma}
% \begin{proof}
% We start with Fa\`a di Bruno's formula,
% \begin{align*}
%     \frac{d^n}{dt^n}\sigmoid(x)=\frac{d^n}{dx^n}\frac{1}{f(x)}=\sum_{k=0}^n(-1)^kk!f^{-(k+1)}(x)B_{n,k}(f(x)),
% \end{align*}
% where \(f(x) \eqdef 1 + \exp(-x)\) and \(B_{n,k}(f(x))\) denotes the Bell polynomials evaluated on $f(x)$. Next, we know the \(k\)-th derivative of \(f(x)\) is given by
% \begin{align*}
%    \frac{d^k}{dt^k}f(x)=(1-k)_k+ke^{-x}.
% \end{align*}
% Now, using the definition of the Bell polynomials \(B_{n,k}(f(t))\), we have
% \begin{align*}
%     B_{n,k}(f(x))=(-1)^nS_{n,k}e^{-kx},
% \end{align*}
% where \(S_{n,k}\) represents the Stirling numbers of the second kind. Substituting the expression for \(B_{n,k}(f(x))\) into the derivative of \(\sigmoid(x)\), we obtain
% \begin{align*}
%     \frac{d^n}{dx^n}\sigmoid(x)=\sum_{k=0}^n(-1)^{n+k}k!S_{n,k}\sigmoid(x)(1-\sigmoid(x))^k.
% \end{align*}
% \end{proof}

% \begin{lemma}[Derivatives of $\operatorname{GELU}$]
% %https://arxiv.org/abs/2305.12073 

% For 
%     \begin{align*}
%         \operatorname{GELU}: \R \to \R, \quad x \mapsto x \Phi(x) , 
%     \end{align*}
% it holds 
% \begin{align}
%        & \operatorname{GELU}'(x) = \Phi(x) + x\phi(x), \notag \\ 
%         & \operatorname{GELU}^{(n)}(x) = n \varphi^{(n-2)}(x) + x \phi^{(n-1)}(x), \quad n\geq 2 ,  
%         \label{GELUn}
%     \end{align}
% with $\phi(x)=\frac{1}{\sqrt{2\pi}}e^{-x^2/2}$, $\Phi(x)=\int_{-\infty}^x \phi(u) du$. 
% The $n$-th derivative of $\phi(x)$ is given by 
% \begin{align} 
%  \frac{d^n}{d x^n} \phi(x) = \frac{1}{\sqrt{2\pi}} e^{-x^2/2} \Big[ \sum_{k=0}^n \binom{n}{k} B_{(2n+k)\frac{1-(-1)^k}{2}} 2^{k/2} 
%   \frac{\Gamma(\frac{k+1}{2})}{\Gamma(\frac{1}{2})} x^{n-k} \Big] , \notag  
% \end{align} 
% with  
% \begin{align} 
%  B_{(2n+k)\frac{1-(-1)^k}{2}} 
%  = 
%  \begin{cases} 
%  1 , \quad & \mbox{$k$ even},  \\ 
%  0, \quad & \mbox{$k$ odd} . 
%  \end{cases} \notag 
% \end{align} 
% \end{lemma}

% \begin{proof} 
% By induction we can show that \eqref{GELUn} holds. 
% And the representation of the $n$-th derivative of $\phi(x)$ follows from~\cite{Oliveira2012RepresentationOT}. 
% \end{proof} 


% \begin{lemma}[Derivatives of $\tanh$]
% %https://math.stackexchange.com/questions/2625632/nth-derivative-of-tanh 

% For $\tanh: \mathbb{R} \mapsto \mathbb{R}$, the $n$-th derivatives have the representation  
% \begin{align} 
% & \frac{d^n}{d x^n} \tanh{x} = C_n(\tanh{x}) ,\notag \\ 
% & C_n(z) = (-2)^n (z+1) \sum_{k=0}^n \frac{k!}{2^k} \binom{n}{k} (z-1)^k , \quad n\geq 1 . \notag 
% \end{align} 
% \end{lemma}

% \begin{proof} 
% See~\cite{Boyadzhiev2007}. 
% \end{proof} 




% \begin{lemma}[Derivatives of $\operatorname{SWISH}$]
% For 
%     \begin{align*}
%         \operatorname{SWISH}: \R \to \R, \quad x \mapsto \frac{x}{1+e^{-x}} 
%     \end{align*}
%     it holds for $n\geq 1$ 
%     \begin{align} 
%     \frac{d^n}{d x^n} \operatorname{SWISH}(x) 
%     = n \sum_{k=1}^{n} (-1)^{k-1} (k-1)! S_{n, k} \sigmoid^k(x) 
%     + x \sum_{k=1}^{n+1} (-1)^{k-1} (k-1)! S_{n+1, k} \sigmoid^k(x) , \notag  
%     \end{align} 
% where $S_{n,k}$ are Stirling numbers of the second kind, i.e., 
% \begin{align} 
%  S_{n,k} = \frac{1}{k!} \sum_{j=0}^k (-1)^j \binom{k}{j} (k-j)^n . \notag
% \end{align} 
% \end{lemma}

% \begin{proof} 
% By induction, we can show that 
% \begin{align} 
% \frac{d^n}{d x^n} \operatorname{SWISH}(x) = n \sigmoid^{(n-1)}(x) + x \sigmoid^{(n)}(x) , \quad n \geq 1 . \notag 
% \end{align}  
% By~\cite[Theorem 2]{MINAI1993845}, the derivatives of the sigmod function can be represented as  
% \begin{align}
% \sigmoid^{(n)}(x) = \sum_{k=1}^{n+1} (-1)^{k-1} (k-1)! S_{n+1, k} \sigmoid^k(x) , \ n\geq 1 . \notag 
% \end{align} 
% Combining the above two equations, we obtain the general form of the $n$-th derivative of the SWISH function.  
% \end{proof} 




% \subsection{Layer Norm}
% \begin{lemma}[Derivative Bounds of the Layer Norm]\label{lem:LayerNorm}
%     Fix $k \in \N$, $\beta\in \mathbb{R}^F$, $\gamma \in \mathbb{R}$, and $w\in [0,1]$. For the layer norm, given by 
%     \begin{gather*}
%         \layernorm: \R^k \rightarrow \R^k,\quad  x \mapsto  
%         \gamma\, 
%         f(x)
%         g\circ\Sigma(x) + \beta; 
%     \\
%         f: \R^k \rightarrow \R^k,\quad  x \mapsto  x-M(x);
%     \qquad
%         g: \R \rightarrow \R, \quad  u \mapsto  \frac{1}{\sqrt{1 + u}};
%     \\
%         M: \R^k \rightarrow \R, \quad  x \mapsto  \frac{w}{k} \sum_{i=1}^k\,  x_i;
%     \qquad
%         \Sigma: \R^k \rightarrow \R, \quad  x \mapsto  \frac{w}{k}\, \sum_{i=1}^k\,  (x_i-M(x))^2;
%     \end{gather*}
%     holds for a compact symmetric set $K$ (using \Cref{not:DerivativeBounds})
%     \begin{align*}
%         C^{\layernorm}_K(\alpha) \leq  
%         \alpha!
%         \sum_{\substack{\alpha' \leq \alpha\\ \vert \alpha \vert = n-1}} 
%             \sum_{m = 1}^{n=1} \frac{(2m+1)!! }{2^{2m}}
%             \sum_{\eta, \zeta \in \calP'(\alpha', m)} 
%             \prod_{j=1}^{n} \frac{
%                 C^\Sigma_K(\order(\zeta^{(j)}))^{\vert \eta^{(j)} \vert}
%             }{
%                 \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%             },
%     \end{align*}
%     where $C^\Sigma_K(\alpha) = 2w \Vert K \Vert$ for $\vert \alpha \vert = 1$, $C^\Sigma_K(\alpha) = 2w$ for $\vert \alpha \vert = 2$, and $C^\Sigma_K(\alpha) = 0$ otherwise.
% \end{lemma}
% \begin{proof}
% Note that 
% \begin{align*} %https://math.stackexchange.com/questions/2011926/proving-nth-derivative-of-sqrtx-by-induction
%     g^{(n)}(x) = (-1)^n \frac{(2n+1)!}{n!2^{2n}} (1+x)^{-\frac{1}{2}-n},
% \end{align*}
% implying $C^g_K(n) \leq (2n+1)!! 2^{-2n}$, $!!$ denoting the double factorial. We have further $C^{f}_K(\alpha) \leq \mathbbm{1}_{\vert \alpha \vert = 1}$ and a direct computation yields
% \begin{align*}
%     C^\Sigma_K(\alpha) \leq \begin{cases}
%         2w\Vert K \Vert 
%         &
%         \text{ for } \vert \alpha \vert = 1
%         \\
%         2w
%         &
%         \text{ for } \vert \alpha \vert = 2
%         \\
%         0
%         &
%         \text{ else. } 
%     \end{cases}
% \end{align*}
% By \Cref{thm:DerivativeBoundByType}, 
% \begin{align*}
%     C^{g\circ \Sigma}_K(\alpha)
%     &\leq
%     \alpha! \sum_{m = 1}^n C^g_{\Sigma[K]}(m)
%     \sum_{\eta, \zeta \in \calP'(\alpha, m)} 
%     \prod_{j=1}^{n} \frac{
%         C^\Sigma_K(\order(\zeta^{(j)}))^{\vert \eta^{(j)} \vert}
%     }{
%         \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%     }.
% \end{align*}
% Accoding to the general multivariate Leibnitz rule, it holds that 
% \begin{align*}
% D^{\alpha}(f \cdot (g \circ \Sigma)) 
% = \sum_{\beta \leq \alpha}  \frac{\alpha!}{\beta!(\alpha - \beta)!} D^{\beta}f \cdot D^{\alpha - \beta}(g\circ \Sigma) %\prod_{i=1}^k{\alpha_i \choose \beta_i}.
% \end{align*}
% which implies
% \begin{align*}
%         C^{\layernorm}_K (\alpha)
%     \leq  
%         \sum_{\beta \leq \alpha, \vert \beta \vert = 1}  \frac{\alpha!}{(\alpha - \beta)!} 
%             C^{g\circ \Sigma}_K(\alpha - \beta) %\prod_{i=1}^k{\alpha_i \choose \beta_i}.
% \end{align*}
% \yannick{The case $\beta = 0$ is missing.}
% \end{proof}

% \subsection{Feedforward Neural Network}
% \begin{definition}[Single-Layer Feedforward Neural Network]\label{defn:ff}
% Fix a non-affine activation function $\sigma\in C^{\infty}(\R)$ and dimensions $\idim, \ldim, \odim \in \N$.
% A feedforward neural network is a map $\neuraln:\mathbb{R}^{\idim}\to \mathbb{R}^{\odim}$ represented for each $x\in \mathbb{R}^{\idim}$ by
% \begin{align}\label{eq:FF}
%         \neuraln (x) 
%     & \eqdef  
%         B^{(1)} x + B^{(2)} \big(\sigma\bullet (A\, x + a)\big)
% \end{align}
% for
% $A\in \mathbb{R}^{\ldim \times \idim}$, $a\in \mathbb{R}^{\ldim}$, 
% $B^{(1)} \in \mathbb{R}^{\odim \times \idim}$, and $B^{(2)} \in \mathbb{R}^{\odim \times \ldim}$.
% \end{definition}
% \begin{lemma}[Derivative Bounds of Neural Networks]\label{lem:FeedForward}
%     In the notation of \Cref{not:DerivativeBounds}, \Cref{lem:Dotp}, and \Cref{defn:ff}, it holds that
%     \begin{align*}
%         C^{\neuraln}_K(\alpha)
%         &\leq
%             C^{B^{(1)}}\mathbbm{1}_{\vert \alpha \vert = 1}
%         +
%             \ldim (\alpha!)^2 C^{B^{(2)}}
%             \sum_{m=1}^n  C^\sigma_{{h}[K]}(m)
%         \cdot
%         (C^{A})^m
%         \sum_{\eta, \zeta \in \calP'(\alpha,m)} 
%         \prod_{j=1}^{n} \frac{
%             \mathbbm{1}_{\vert \zeta^{(j)} \vert \leq 1}
%         }{
%             \eta^{(j)}!
%         },
%     \end{align*}
%     where $h[K]$ is defined as the image of $h(x) \eqdef Ax + a$ on $K$. 
% \end{lemma}
% \begin{proof}
%     Write $\neuraln(x) =  B^{(1)} x + B^{(2)}((g_i(x))_{i=1}^{\ldim})$, where for $i \in \myset{1}{\ldim}$
%     \begin{align*}
%         g_i(x) \eqdef \sigma((Ax + a)_i).
%     \end{align*}
%     If we define $h_i(x) \eqdef h(x)_i$, we follow with \Cref{thm:DerivativeBoundByType}
%     \begin{align*}
%     C^{g_i}_K(\alpha)
%         &\leq
%         \alpha! \sum_{m=1}^n  C^\sigma_{{h}[K]}(m)
%         \cdot
%         (C^{A})^m
%         \sum_{\eta, \zeta \in \calP'(\alpha,m)} 
%         \prod_{j=1}^{n} \frac{
%             \mathbbm{1}_{\vert \zeta^{(j)} \vert \leq 1}
%         }{
%             \eta^{(j)}!
%         }
%         \eqdef
%     C^{g}_K(\alpha)
%         ,
%     \end{align*}
%     and due to the component wise application of the activation function it holds that \begin{align*}
%         \Vert D^\alpha \max_{i \in \myset{1}{\ldim}} g_i(x) \Vert_K = \max_{i \in \myset{1}{\ldim}} C^{g_i}_K(\alpha) \leq C^{g}_K(\alpha).
%     \end{align*}
%     Using \Cref{cor:DerivativeBoundAffine}, we obtain
%     \begin{align*}
%         C^{\neuraln}_K(\alpha)
%         &\leq
%             C^{B^{(1)}}\mathbbm{1}_{\vert \alpha \vert = 1}
%         +
%             \ldim \alpha! C^{B^{(2)}}
%             C^g_K(\alpha).
%     \end{align*}
% \end{proof}

% \subsection{Transfomers}

% \begin{proof}[{Proposition~\ref{prop:transformerSobolevBound}}]
%     The bounds \eqref{id:TransformerSobolevBound1} are a direct consequence of \Cref{thm:DerivativeBoundByType} and \eqref{id:TransformerSobolevBound2} follows directly from \Cref{cor:DerivativeBoundAffine}.
% \end{proof}

% \begin{theorem}\label{thm:TransformerBlockSobolevBound} 
%     Let $K$ be a compact set, $\tblock$ a transformer block as in \Cref{defn:TransformerBlock}, and $\alpha \in \Order^{(1 + M)\idim}_n, n \in \N$. Then,
%     \begin{align*}
%         C^{\tblock}_K(\alpha) &\leq
%         \alpha! \sum_{\beta \in \Order^{\odim}_{\leq n}}  N(\beta) C^{\layernorm}_{K\tagA}(\beta)
%         \sum_{\eta, \zeta \in \calP'(\alpha,\beta)} 
%         \prod_{j=1}^{n} \frac{
%             C\tagA_K(\order(\zeta^{(j)}))^{\vert \eta^{(j)} \vert}
%         }{
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         }, 
%     \end{align*}
%     where for all $\gamma \in \Order^{(1 + M)\idim}_{\leq n}$:
%     \begin{align*}
%         C\tagA_K(\gamma) & \eqdef 
%         \gamma! \sum_{\beta \in \Order^{\idim}_{\leq n}}  N(\beta) C^{\neuraln}_{K\tagB}(\beta)
%         \sum_{\eta, \zeta \in \calP'(\gamma,\beta)} 
%         \prod_{j=1}^{n} \frac{
%             C\tagB_K(\order(\zeta^{(j)}))^{\vert \eta^{(j)} \vert}
%         }{
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         },
%     \\
%         C\tagB_K(\gamma) & \eqdef
%         \gamma! \sum_{\beta \in \Order^{\idim}_{\leq n}}  N(\beta) C^{\layernorm}_{K\tagC}(\beta)
%         \sum_{\eta, \zeta \in \calP'(\gamma,\beta)} 
%         \prod_{j=1}^{n} \frac{
%             C\tagC_K(\order(\zeta^{(j)}))^{\vert \eta^{(j)} \vert}
%         }{
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         },
%     \\
%         C\tagC_K(\gamma) & \eqdef \mathbbm{1}_{\vert \gamma \vert = 1} + C^{\multihead}_K(\gamma).
%     \end{align*}
%     In the above, $K\tagC = \bigcup_{m = 0}^M\multihead_m[K]$, $K\tagB = \layernorm[K\tagC]$, and $K\tagA = \neuraln[K\tagB]$.
    
%     For respective multi-indices, a bound for $C^{\layernorm}_{K\tagA}, C^{\layernorm}_{K\tagC}$ is given by \Cref{lem:LayerNorm}, $C^{\neuraln}_{K\tagB}$ is bounded in \Cref{lem:FeedForward}, and a bound for $C^{\multihead}_{K}$ is given in \Cref{cor:MultiHead}.
% \end{theorem}
% \begin{proof}
%     This is a direct consequence of \Cref{thm:DerivativeBoundByType}.
% \end{proof}


% \begin{comment}
% \newpage
% \section{Old: Bounding Higher Derivative Norms in Transformer Models}
% \subsection{Results based on the chain rule}

% Recall the chain rule
% \begin{align*}
% \frac{df_n \circ f_{n-1} \circ ... \circ f_1}{dx} = \frac{df_n}{df_{n-1}} \cdot \frac{df_{n-1}}{df_{n-2}} \cdot \ldots \cdot \frac{df_2}{df_1} \cdot \frac{df_1}{dx}.
% \end{align*}
% Here, the functions \( f_1, f_2, \ldots, f_n \) represent the compositions of transformations in the transformer class, and \( x \) is the input variable. Each \( {df_i}/{df_{i-1}} \) denotes the derivative of the \( i \)th transformation with respect to the \( (i-1) \)th transformation. This equation enables us to compute the derivative of the composite transformation with respect to the input variable.

% If we are interested in higher order derivatives, we can make use of Faa di Bruno's formula, which for \( f \circ g(x) \) and \( n \in \mathbb{N} \) is given by
% \begin{align*}
% \frac{d^n}{dx^n} f(g(x)) = \sum \frac{n!}{\prod_{k=1}^{n} m_k! (k!)^{m_k}} \cdot f^{(m_1 + m_2 + \cdots + m_n)}(g(x)) \cdot \prod_{k=1}^{n} g^{(k)}(x)^{m^k},
% \end{align*}
% where the sum is taken over all \(n\)-tuples of non-negative integers \((m_1, m_2, \ldots, m_n)\) satisfying the constraint \(1\cdot m_1 + 2\cdot m_2 + \cdots + n\cdot m_n = n\). Let's simplify notation by 
% \begin{align*}
%     \mathcal{M}^n &\eqdef \mySet{m := (m_1, m_2, \ldots, m_n) \in \N^n}{1\cdot m_1 + 2\cdot m_2 + \cdots + n\cdot m_n = n}, \\
%     \vert m \vert &\eqdef \sum_{k=1}^n m_k, \quad \forall m \in \mathcal{M}^n, \\
%     \alpha(m) &\eqdef \frac{n!}{\prod_{k=1}^{n} m_k! (k!)^{m_k}}, \quad \forall m \in \mathcal{M}^n,
% \end{align*}
% and we arrive at 
% \begin{align*}
%     \frac{d^n}{dx^n} f(g(x)) = \sum_{m \in \mathcal{M}^n} \alpha(m) \cdot f^{(\vert m \vert)}(g(x)) \cdot \prod_{k=1}^{n} g^{(k)}(x)^{m^k}.
% \end{align*}
% Since for all $m \in \mathcal{M}^n$
% \begin{align*}
%     \Big\Vert \prod_{k=1}^{n} g^{(k)}(x)^{m^k} \Big \Vert_\infty 
%     =
%     \prod_{k=1}^{n} \big\Vert g^{(k)}(x)^{m^k} \big\Vert_\infty 
%     \leq 
%     \prod_{k=1}^{n} \left( 1 + \Vert g^{(k)}(x)\Vert_\infty^{n}  \right),
% \end{align*}
% we have 
% \begin{align*}
%     \Big\Vert \frac{d^n}{dx^n} f(g(x)) \Big\Vert_\infty 
%     & \leq 
%     M(n)
%     \prod_{k=1}^{n} \left( 1 + \Vert g^{(k)}(x)\Vert_\infty^{n}  \right)
%     \sum_{k = 1}^N \Vert f^{(k)}(g(x)) \Vert_\infty, \\
%     & \leq 
%     M(n)
%     \prod_{k=1}^{n} \left( 1 + \Vert g^{(k)}(x)\Vert_\infty^{n}  \right)
%     \sum_{k = 1}^N \Vert f^{(k)}(x) \Vert_\infty,
% \end{align*}
% where $M(n) := \max_{k=1}^n \sum_{m \in \mathcal{M}, \vert m \vert = k} \alpha(m)$.

% \begin{proof}[{Lemma~\ref{lem:TransformerIsSmooth}}]
%     The smoothness of $\attention$ follows directly from the smoothness of $\softmax$, which immediately implies smoothness of $\multihead$ since the operators used for its definition are smooth. Furthermore, the $\layernorm$ is smooth due to its smooth and lower-bounded denominator and the activation function $\sigma$ is smooth by definition, therefore we conclude that $\tblock \in \tblock_{d',M',H'}$ is smooth for every $d', M', H' \in \N$ and we obtain smoothness of $\transformer \in \transformer_{L,W,H}^{D,d,M}$ as a consequence.
% \end{proof}


% \subsection{Explicit derivatives}

% \begin{lemma}[Derivatives of $\softmax$]
% For 
% \begin{align*}%\label{id:Softmax}
%     \softmax:
%             \R^F 
%         \to     
%             \R^F,
%     \quad 
%             x 
%         \mapsto 
%             \left(
%                     {\exp(x_i)}
%                 /
%                     {\textstyle\sum_{j = 0}^{F-1} \exp(x_j)}
%             \right)_{i=0}^{F-1}.
% \end{align*}
% it holds for a multi-index $m := (m_1, \ldots, m_k) \in \myset{0}{F-1}^k, k \in \N$ that 
% \begin{align*}
%     \softmax^{(m)} (x) = \sum \softmax(x_{m_0}) \prod_{i=1}^k (...  - \softmax(x_{m_i}))
% \end{align*}
% \end{lemma}
% \begin{proof}
%     For $m_0, m_1 \in \myset{0}{F-1}$ we have
%     \begin{align*}
%         \frac{\partial \softmax}{\partial x_{m_1}} (x_{m_0}) = \softmax(x_{m_0})\left( \delta_{m_0m_1} - \softmax(x_{m_1})\right)
%     \end{align*}
%     For $m_2 \in \myset{0}{F-1}$ we have
%     \begin{align*}
%         \frac{\partial \softmax}{\partial x_{m_1}x_{m_2}} (x_{m_0}) &=
%         \softmax(x_{m_0})
%         \left( \delta_{m_0m_2} - \softmax(x_{m_2})\right)
%         \left( \delta_{m_0m_1} - \softmax(x_{m_1})\right) \\
%         &-
%         \softmax(x_{m_0})
%         \softmax(x_{m_1})
%         \left( \delta_{m_1m_2} - \softmax(x_{m_2})\right)
%     \end{align*}
%     For $m_3 \in \myset{0}{F-1}$ we have
%     \begin{align*}
%         &\frac{\partial \softmax}{\partial x_{m_1}x_{m_2}x_{m_3}} (x_{m_0}) \\
%         =
%         &+
%         \softmax(x_{m_0})
%         \left( \delta_{m_0m_1} - \softmax(x_{m_1})\right) 
%         \left( \delta_{m_0m_2} - \softmax(x_{m_2})\right)
%         \left( \delta_{m_0m_3} - \softmax(x_{m_3})\right) \\
%         &-
%         \softmax(x_{m_0})
%         \left( \delta_{m_0m_1} - \softmax(x_{m_1})\right) 
%         \softmax(x_{m_2})
%         \left( \delta_{m_2m_3} - \softmax(x_{m_3})\right) \\
%         &-
%         \softmax(x_{m_0})
%         \softmax(x_{m_1})
%         \left( \delta_{m_0m_2} - \softmax(x_{m_2})\right)
%         \left( \delta_{m_1m_3} - \softmax(x_{m_3})\right) \\
%         &-
%         \softmax(x_{m_0})
%         \softmax(x_{m_1})
%         \left( \delta_{m_1m_2} - \softmax(x_{m_2})\right) 
%         \left( \delta_{m_0m_3} - \softmax(x_{m_3})\right) \\
%         &-
%         \softmax(x_{m_0})
%         \softmax(x_{m_1})
%         \left( \delta_{m_1m_2} - \softmax(x_{m_2})\right) 
%         \left( \delta_{m_1m_3} - \softmax(x_{m_3})\right) \\
%         &+
%         \softmax(x_{m_0})
%         \softmax(x_{m_1})
%         \softmax(x_{m_2})
%         \left( \delta_{m_2m_3} - \softmax(x_{m_3})\right) \\
%         %
%         %
%         %
%     \end{align*}
% \end{proof}
% \begin{lemma}[Derivatives of $\softplus$]
%     For 
%     \begin{align*}
%         \softplus: \R \to \R, \quad x \mapsto \ln (1 + \exp(\cdot))
%     \end{align*}
%     it holds 
%     \begin{align*}
%         \softplus^{(1)}(x) = \sigmoid(x) \eqdef 1 / (1 + \exp(-x))
%     \end{align*}
%     and for $n \in \N$
%     \begin{align*}
%         \softplus^{(n + 1)}(x) = \sigmoid^{(n)}(x) = \sum_{k=0}^n(-1)^{n+k}k!S_{n,k}\sigmoid(x)(1-\sigmoid(x))^k,
%     \end{align*}
%     where $S_{n,k}$ are the Stirling numbers of the second kind, $S_{n,k} \eqdef \frac{1}{k!} \sum_{j=0}^{k} (-1)^{k-j} \binom{k}{j} j^n$.
% \end{lemma}
% \begin{proof}
% We start with Fa\`a di Bruno's formula,
% \begin{align*}
%     \frac{d^n}{dt^n}\sigmoid(x)=\frac{d^n}{dx^n}\frac{1}{f(x)}=\sum_{k=0}^n(-1)^kk!f^{-(k+1)}(x)B_{n,k}(f(x)),
% \end{align*}
% where \(f(x) \eqdef 1 + \exp(-x)\) and \(B_{n,k}(f(x))\) denotes the Bell polynomials evaluated on $f(x)$. Next, we know the \(k\)-th derivative of \(f(x)\) is given by
% \begin{align*}
%    \frac{d^k}{dt^k}f(x)=(1-k)_k+ke^{-x}.
% \end{align*}
% Now, using the definition of the Bell polynomials \(B_{n,k}(f(t))\), we have
% \begin{align*}
%     B_{n,k}(f(x))=(-1)^nS_{n,k}e^{-kx},
% \end{align*}
% where \(S_{n,k}\) represents the Stirling numbers of the second kind. Substituting the expression for \(B_{n,k}(f(x))\) into the derivative of \(\sigmoid(x)\), we obtain
% \begin{align*}
%     \frac{d^n}{dx^n}\sigmoid(x)=\sum_{k=0}^n(-1)^{n+k}k!S_{n,k}\sigmoid(x)(1-\sigmoid(x))^k.
% \end{align*}
% \end{proof}

% \begin{lemma}[Derivatives of $\layernorm$]
% For 
% \[
%     \layernorm(x;\gamma,\beta,w)\eqdef  
%         \gamma\, 
%         \frac{(x-\mu_x^w)}{1 + \softplus(\sigma_x^w)} + \beta 
% \]
% it holds for a multi-index $m := (m_1, \ldots, m_k) \in \myset{0}{F-1}^k, k \in \N$ that 
% \begin{align*}
%     \layernorm^{(m)}(x;\gamma,\beta,w) = ...
% \end{align*}
% \end{lemma}
% \begin{proof}
%     Define 
%     \begin{align*}
%     \begin{cases}
%         f(x) := \gamma (x - \mu_x^w) \\ 
%         g(x) := {1}/({1 + \softplus(\sigma_x^w)}),
%     \end{cases}
%     \end{align*}
%     then we see
%     \begin{align*}
%         \layernorm^{(m)}(x;\gamma,\beta,w) = f(x)g^{(m)} + \sum_{i=1}^k\frac{\partial f}{\partial x_{m_i}}(x)\frac{\partial g}{\partial x_{m_1} \cdots x_{m_{i-1}} x_{m_{i+1}}x_{m_k}}(x).
%     \end{align*}
%     Note that we can write $g = h \circ \softplus \circ \sigma^w$ for 
%     \begin{align*}
%         h(x) := \frac{1}{1+x}.
%     \end{align*}
%     \yannick{There exists a special formula for one dimensional compositions, see \cite{ConstantineSavits96}.}
% \end{proof}



% \newpage
% \end{comment}

% % \section{Shirayev-Wonham Filtering}
% % \paragraph{From \cite[Chapter 9]{LipShiryaev_I_2001}.}
% % Consider a complete probability space $(\Omega, \mathcal{F}, P)$ equipped with a nondecreasing sequence of right-continuous sub-$\sigma$-algebras $\mathcal{F}_t, 0 \leq t \leq T$. Let $\theta = (\theta_t, \mathcal{F}_t)$, $0 \leq t \leq T$, denote a real right-continuous Markov process taking values in the countable set $E = \{\alpha, \beta, \gamma, \ldots\}$. Additionally, let $W = (W_t, \mathcal{F}_t)$, $0 \leq t \leq T$, be a standard Wiener process independent of $\theta$, and let $\xi_0$ be a $\mathcal{F}_0$-measurable random variable independent of $\theta$. We assume the existence of nonanticipative functionals $A_t(\epsilon, x)$ and $B_t(x)$ that define
% % \begin{align}
% %     d\xi_t = A_t(\theta_t, \xi) dt + B_t(\xi)dW_t
% % \end{align}
% % and satisfy the following conditions.
% % \begin{gather}
% %     A^2_t(\epsilon_t, x) \leq L_1 \int_0^t (1 + x_s^2)dK(s) + L_2(1 + \epsilon^2_t + x^2_t), 
% %     \label{id:LS1}
% % \\
% %     0 < C \leq B^2_t(x) \leq L_1 \int_0^t (1 + x_s^2)dK(s) + L_2(1 + x^2_t),  
% %     \label{id:LS2}
% % \\
% %     |A_t(\epsilon_t, x) - A_t(\epsilon_t, y)|^2 + |B_t(x) - B_t(y)|^2
% %     \leq L_1 \int_0^t (x_s - y_s)^2 dK(s) + L_2(x_t - y_t)^2, 
% %     \label{id:LS3}
% % \end{gather}
% % where $C, L_1, L_2$ are certain constants, $K(s)$ is a non-decreasing right continuous function, $0 \leq K(s) \leq 1, x \in C_T, y \in C_T, \epsilon_t \in E, 0 \leq t \leq T$.

% % Along with \Cref{id:LS1,id:LS2,id:LS3} it will also be assumed that
% % \begin{align}
% %     M\xi^2_0 < \infty,
% %     \label{id:LS4}
% % \end{align}
% % and
% % \begin{align}
% %     M \int_0^T \theta^2_t dt < \infty. 
% %     \label{id:LS5}
% % \end{align}

% % Define 
% % \begin{align*}
% %     p_\beta(t) &\eqdef P(\theta_t = \beta), \\
% %     p_{\beta\alpha}(t, s) &\eqdef P(\theta_t = \beta|\theta_s = \alpha), \quad 0 \leq s < t \leq T, \quad \beta, \alpha \in E,
% % \end{align*}
% % and assume there exist a function $\lambda_{\alpha\beta}(t), 0 \leq t \leq T, \alpha, \beta \in E$, that is 
% % \begin{gather}
% %     \text{continuous over \(t\),  (uniformly over \(\alpha, \beta\))}
% %     \label{id:LS6}
% %     \\
% %     |\lambda_{\alpha\beta}(t)| \leq K 
% %     \label{id:LS7}
% %     \\
% %     |p_{\beta\alpha}(t + \Delta, t) - \delta(\beta, \alpha) - \lambda_{\alpha\beta}(t) \cdot \Delta| \leq o(\Delta),
% %     \label{id:LS8}
% % \end{gather}
% % where \(\delta(\beta, \alpha)\) is a Kronecker's symbol and the value \(o(\Delta)/\Delta \rightarrow 0 \) as \(\Delta \rightarrow 0\) (uniformly over \(\alpha, \beta\)).  

% % \begin{theorem}
% % Let the \Cref{id:LS1,id:LS2,id:LS3,id:LS4,id:LS5,id:LS6,id:LS7,id:LS8} be fulfilled. Then the a posteriori probability $\pi_\beta(t)$, $\beta \in \mathcal{E}$, satisfies a system of equations
% % \begin{align*}
% % \pi_\beta(t) = p_\beta(0) + \int_0^t \mathcal{L}^*\pi_\beta(u)du + \int_0^t \pi_\beta(u)\frac{A_u(\beta, \xi) - \bar{A}_u(\xi)}{B_u(\xi)} d\bar{W}_u,
% % \end{align*}
% % where
% % \begin{align*}
% % \mathcal{L}^*\pi_\beta(u) &= \sum_{\gamma \in \mathcal{E}} \lambda_{\gamma\beta}(u)\pi_\gamma(u), \\
% % \bar{A}_u(\xi) &= \sum_{\gamma \in \mathcal{E}} A_u(\gamma, \xi)\pi_\gamma(u),
% % \end{align*}
% % and $ \bar{W} = (\bar{W}_t, \mathcal{F}_t) $ is a Wiener process with
% % \begin{align*}
% %     \bar{W}_t = \int_0^t \frac{d\xi_u - \bar{A}_u(\xi)du}{B_u(\xi)}.
% % \end{align*}
% % \end{theorem}

% % \newpage

% \begin{comment}
% \section{Old and Future Ideas}
% \subsection{Embedding Uncertainty Into the Transformer Model}

% \AK{History instead of memory, to align with RL community.}

% \yannick{Do we need it with the new approach?}

% Fix a regularization parameter $\varepsilon>0$.  
% For $d\in \mathbb{N}_+$ any measures $\mu,\nu \in \mathcal{P}(\mathbb{R}^d)$ with density with respect to the Lebesgue measure on $\mathbb{R}^d$ and with exponential moments, we define their \textit{entropy-regularized $2$-Wasserstein distance}, denoted by $\operatorname{OT}^{\varepsilon}$, by
% \[
%     \operatorname{OT}^{\varepsilon}(\mu,\nu)
%     \eqdef
%     \min_{\pi\in \operatorname{Cpl}(\mu,\nu)}
%     \,
%     \mathbb{E}_{(X_1,X_2)\sim \pi}\biggl[
%         \|X_1-X_2\|^2
%         -
%         \varepsilon\,
%         \mathbb{E}_{Z\sim \mu}\Big[
%             \log\Big(\frac{p_{\nu}}{p_{\mu}}(Z)\Big)
%         \Big]
%     \biggr]
% \]
% where $p_{\nu}$ and $p_{\mu}$ are the respective Radon-Nikodym derivatives of $\nu$ and $\mu$ with respect to the Lebesgue measure on $\mathbb{R}^d$.


% Fix memory hyperparameters hyperparameter $\alpha>0$ and $M\in \mathbb{N}_+$.  
% %
% Unlike classical time series models, the sequential deep learning models $\hat{f}^1,\dots,\hat{f}^k$ do not capture uncertainty.  Here, instead of postulating a single distribution/measure on the space of inputs and output as in \cite{xxx}, a family of probability measures as in robust finance \cite{xxx} or PAC learning theory \cite{xxx}, or even considering extremal worst-case results over all possible paths as in \cite{xxx}, we instead progressively infer randomness.  That is, we construct a sequence/discrete-flow of probability measures capturing the error distribution of each sequential deep learning model.
% %
% Each model $\mathcal{T}\in \mathcal{T}_{L,W,H}^{D,d:M}$ is lifted to a measure-valued model taking values in the space $\mathcal{N}_d$ of Gaussian measures on $\mathbb{R}^d$.  We can do this by leveraging the sequential structure of the learning problem.  

% Specifically, consider a map 
% \begin{equation}
% \label{eq:uncertain_transformer}
% \begin{aligned}
%     \boldsymbol{\mathcal{T}}:\mathbb{R}^{2(1+M)\,d}\times \mathbb{R}^{2(1+M)\,D} & \to \mathcal{N}_d
%     \\
%     y_{[-2M-2:-1]}\times x_{[-2M:0]} & \mapsto \mathcal{N}_d\big(\mathcal{T}(x_{[-M:0]}),\Sigma(y_{[-M-1:-1]},x_{[-M:0]}|\mathcal{T})\big)
% \end{aligned}
% \end{equation}
% where we have indexed vectors in $\mathbb{R}^{(1+M)\,d}$ by one shifted time-step in the past, to emphasize that they correspond to \textit{historically} observed targets, and where for each $j,k=1,\dots,D$, the $j,k^{th}$ entry of the \textit{uncertainty} matrix $\Sigma_{j,k}\eqdef \Sigma(y_{[-M-1:-1]},x_{[-M:0]}|\mathcal{T})_{j,k}$ is given by
% \begin{equation*}
% \begin{aligned}
%     \Sigma_{j,k}
%         % \Sigma(y_{[-M-1:-1]},x_{[-M:0]}|\mathcal{T})|\mathcal{T}))_{j,k}
%     &
%     \eqdef 
%         \frac1{
%             1
%             -
%             \sum_{s=t-M}^t\,
%                 e^{-\alpha 2\,(t-s)}
%         }
%     \,
%         \sum_{s=-M}^0
%             e^{-\alpha(t-s)}
%             \,
%             \big(
%                 (E_s)_j
%                 -(\bar{E}_s)_j
%             \big)
%             \big(
%                 (E_s)_k
%                 -(\bar{E}_s)_k
%             \big)
%     \\
%     E_s & \eqdef 
%         \|\mathcal{T}(x_{[-M-s-1:-s-1]}) - y_{-s}\|^2
% \end{aligned}
% \end{equation*}
% where, $s=-M,\dots,0$, and $j,k=1,\dots,D$.

% \begin{lemma}
% \label{lem:regularity_2}
% Fix regularization hyperparameters $\varepsilon,\lambda>0$ and a map $\boldsymbol{\mathcal{T}}$ as in~\eqref{eq:uncertain_transformer} as consider the associated \textit{loss} $\ell(\cdot|\mathcal{T}):\boldsymbol{\mathcal{T}}:\mathbb{R}^{(3+2M)\,d}\times \mathbb{R}^{2(1+M)\,D} \to \mathcal{R}$ mapping each $y_{[-2M-2:0]}\times x_{[-2M:0]} \in \mathbb{R}^{(3+2M)\,d}\times \mathbb{R}^{2(1+M)\,D}$ by
% \begin{equation}
% \begin{aligned}
%     % \ell(\cdot|\mathcal{T}):\boldsymbol{\mathcal{T}}:\mathbb{R}^{(3+2M)\,d}\times \mathbb{R}^{2(1+M)\,D} & \to \mathcal{R}
%     % \\
%     % y_{[-2M-2:-1]}\times x_{[-2M:0]} & \mapsto 
%     \operatorname{OT}^{\varepsilon}
%         \Big(
%                 \mathcal{N}_d(y_0,\lambda\,I_d)
%             \,
%             ,
%             \,
%                 \mathcal{N}_d\big(\mathcal{T}(x_{[-M:0]}),\Sigma(y_{[-M-1:-1]},x_{[-M:0]}|\mathcal{T})\big)
%         \Big).
% \end{aligned}
% \end{equation}
% \AK{@Yannick and @Xuwei we want the smoothness of this map, ie its $C^k$ norms; using the previous first lemma.
% }    
% \end{lemma}
% \begin{proof}[{Proof of Lemma~\ref{lem:regularity_2}}]
% Fix $y_{[-2M-2:0]}\times x_{[-2M:0]} \in \mathbb{R}^{(3+2M)\,d}\times \mathbb{R}^{2(1+M)\,D}$.  We compute
% \allowdisplaybreaks
% \begin{align}
% \nonumber
%     &
%         \operatorname{OT}^{\varepsilon}
%         \Big(
%                 \mathcal{N}_d(y_0,\lambda\,I_d)
%             \,
%             ,
%             \,
%                 \mathcal{N}_d\big(\mathcal{T}(x_{[-M:0]}),\Sigma(y_{[-M-1:-1]},x_{[-M:0]}|\mathcal{T})\big)
%         \Big)
%     \\
%     \label{eq:simplification_OT__Centering}
%     = & 
%         \|y_0-\mathcal{T}(x_{[-M:0]})\|^2
%     \\
%     \nonumber
%     & +
%         \operatorname{OT}^{\varepsilon}
%             \Big(
%                     \mathcal{N}_d(0,\lambda\,I_d)
%                 \,
%                 ,
%                 \,
%                     \mathcal{N}_d\big(0,\Sigma(y_{[-M-1:-1]},x_{[-M:0]}|\mathcal{T})\big)
%             \Big)
%     \\
%     \label{eq:simplification_OTCentered}
%     = & 
%         \|y_0-\mathcal{T}(x_{[-M:0]})\|^2
%     \\
%     \nonumber
%     & +
%         % I used this naming
%         % K_0 \eqdef \lambda\,I_d
%         % K_1 \eqdef \Sigma(y_{[-M-1:-1]},x_{[-M:0]}|\mathcal{T})
%     \operatorname{tr}(\lambda\,I_d) 
%     +
%     \operatorname{tr}\big(
%         \Sigma(y_{[-M-1:-1]},x_{[-M:0]}|\mathcal{T})
%     \big)
%     \\
%     \nonumber
%     &
%     - 
%     \frac{\varepsilon}{2}\,
%         \big(
%             % Constant Factor Bit
%             d\log(2) - 2d
%         \big)
%     \\
%     \nonumber
%         % Important Bit
%     &
%         -
%         \frac{\varepsilon}{2}\,
%             \operatorname{tr}\Big(
%                 \big(
%                         I_d + \frac{4^2}{\varepsilon^2}\,(\lambda\,I_d)(\Sigma(y_{[-M-1:-1]},x_{[-M:0]}|\mathcal{T}))
%                 \big)^{1/2}
%             \Big)
%     \\
%     \nonumber
%     &
%             -\frac{\varepsilon}{2}\,
%                 \log\Big(
%                     \big(
%                             I_d + \frac{4^2}{\varepsilon^2}\,(\lambda\,I_d)(\Sigma(y_{[-M-1:-1]},x_{[-M:0]}|\mathcal{T}))
%                     \big)^{1/2}
%                 \Big)
%         \Big)
% %%%%%
% %%%%%
% %%%%%
% %%%% Simple simplifications
% %%%%%
% %%%%%
% %%%%%
%     \\
%     \nonumber
%     = & 
%         \|y_0-\mathcal{T}(x_{[-M:0]})\|^2
%     \\
%     \nonumber
%     & +
%         % I used this naming
%         % K_0 \eqdef \lambda\,I_d
%         % K_1 \eqdef \Sigma(y_{[-M-1:-1]},x_{[-M:0]}|\mathcal{T})
%     d\lambda
%     +
%     \operatorname{tr}\big(
%         \Sigma(y_{[-M-1:-1]},x_{[-M:0]}|\mathcal{T})
%     \big)
%     \\
%     \nonumber
%     &
%     - 
%     \frac{\varepsilon\,d(\log(2) - 2)}{2}\,
%     \\
%     \nonumber
%         % Important Bit
%     &
%         -
%         \frac{\varepsilon}{2}\,
%             \operatorname{tr}\Big(
%                 \big(
%                         I_d + \frac{4^2}{\varepsilon^2}\,(\lambda\,I_d)(\Sigma(y_{[-M-1:-1]},x_{[-M:0]}|\mathcal{T}))
%                 \big)^{1/2}
%             \Big)
%     \\
%     \nonumber
%     &
%             -\frac{\varepsilon}{2}\,
%                 \log\Big(
%                     \big(
%                             I_d + \frac{4^2}{\varepsilon^2}\,(\lambda\,I_d)(\Sigma(y_{[-M-1:-1]},x_{[-M:0]}|\mathcal{T}))
%                     \big)^{1/2}
%                 \Big)
%         \Big)
% %%%%%
% %%%%%
% %%%%%
% %%%% Simple simplifications II (Just baby factoring)
% %%%%%
% %%%%%
% %%%%%
%     \\
%     \nonumber
%     = & 
%         \|y_0-\mathcal{T}(x_{[-M:0]})\|^2
%     +
%     d
%     \big(
%     \lambda +1 - \log(2)/2
%     \big)
%     +
%     \operatorname{tr}\big(
%         \Sigma(y_{[-M-1:-1]},x_{[-M:0]}|\mathcal{T})
%     \big)
%     \\
%     \nonumber
%         % Important Bit
%     &
%         -
%         \underbrace{
%             \frac{\varepsilon}{2}\,
%             \operatorname{tr}\Big(
%                 \big(
%                         I_d + \frac{4^2}{\varepsilon^2}\,(\lambda\,I_d)(\Sigma(y_{[-M-1:-1]},x_{[-M:0]}|\mathcal{T}))
%                 \big)^{1/2}
%             \Big)
%         }_{\text{(I)}}
%     \\
%     \nonumber
%     &
%         -
%         \underbrace{
%             \frac{\varepsilon}{2}\,
%                     \log\Big(
%                         \big(
%                                 I_d + \frac{4^2}{\varepsilon^2}\,(\lambda\,I_d)(\Sigma(y_{[-M-1:-1]},x_{[-M:0]}|\mathcal{T}))
%                         \big)^{1/2}
%                     \Big)
%             \Big)
%         }_{\text{(II)}}
% \end{align}
% where the equality~\eqref{eq:simplification_OT__Centering} holds by \citep[Propositions 2]{MallastoGerolinAugustoMinh_IG_2022_Closed_FormEOT} and the equality~\eqref{eq:simplification_OTCentered} holds by \cite[Theorem 2]{MallastoGerolinAugustoMinh_IG_2022_Closed_FormEOT}.
% \hfill\\
% \AK{@YX Please bound (I) and (II) using previous lemma.}
% \end{proof}

% \newpage
% \end{comment}



% \subsection{Proofs of Supporting Results}
% \label{s:}



% \begin{proposition}[{Details on the loss function from Example~\ref{eq:smooth_loss}}]
% \label{prop:ExpFlattenedSSE_ExampleDetails}
% Let $\lambda>0$, $D\in \mathbb{N}_+$, and define $\ell:\mathbb{R}^{2D}\ni (y,\hat{y})\eqdef \|y-\hat{y}\|^2 \, e^{-\lambda \, \|y-\hat{y}\|^2}\in [0,\infty)$.  Then, for each $s\in \mathbb{N}$, we have
% \[
%     \|\ell\|_{C^s}\le \AK{XXX}
% .
% \]
% \end{proposition}
% \begin{proof}[{Proof of Proposition~\ref{prop:ExpFlattenedSSE_ExampleDetails}}]

% We derive the norm $\| \ell \|_{C^s}$ explicitly. 
% Denote $z=y-\hat{y} \in \mathbb{R}^d$ with $z_i = y_i - \hat{y}_i$, $i=1$, ..., $d$. 
% Define $l(z):=l(y,\hat{y})$. By induction we can show  
% \begin{align} 
%   \frac{\partial^k l(z)}{\partial z_{\alpha_1} \cdots \partial z_{\alpha_k}} 
%    =  \big( c_k   
%    + (-\lambda)^k 2^k  \| z\|^2 
%     \big) e^{-\lambda \| z \|^2}  z_{\alpha_1} \cdots z_{\alpha_k} ,  
%     \label{ell-partial-k}
% \end{align} 
% where the coefficients $c_k$ are recursively determined by 
% \begin{align} 
% & c_1 = 2, \quad c_k = 2(-\lambda) c_{k-1} + 2 [2(-\lambda)]^{k-1} , \, k\geq 2 \notag \\ 
%  & c_k = 2 [2(-\lambda)]^{k-1} + 2[2(-\lambda)] \frac{1 - [2(-\lambda)]^{k-1}}{1-2(-\lambda)} , \, k\geq 2  \notag \\ 
% % & \quad = 2(-2\lambda)^{k-1} \frac{1-3(-\lambda)}{1-2(-\lambda)} + \frac{2(-2\lambda)}{1-(-2\lambda)} \notag \\ 
%  & \quad = (-2\lambda)^{k-1} \frac{2(1+3\lambda)}{1 + 2\lambda} + \frac{ -4\lambda }{1 + 2\lambda} . \notag 
% \end{align}  

% Under the constraint $\|z\|=r\geq 0$, we have $\max_{z\in \mathbb{R}^d} |z_{\alpha_1} \cdots z_{\alpha_k}|=r^k k^{-k/2}$.  
% Since 
% \begin{align} 
%  & \Big| \big( c_k   
%    + (-\lambda)^k 2^k  \| z\|^2 
%     \big) e^{-\lambda \| z \|^2}  z_{\alpha_1} \cdots z_{\alpha_k} \Big|    \notag \\ 
% \leq & 
%  \big( | c_k |   
%    + |(-\lambda)^k| 2^k  \| z\|^2 
%     \big) e^{-\lambda \| z \|^2}  |z_{\alpha_1} \cdots z_{\alpha_k}| \notag  \\ 
% \leq & 
%  \big( | c_k |   
%    + |(-\lambda)^k| 2^k  \| z\|^2 
%     \big) e^{-\lambda \| z \|^2}  \| z\|^k k^{-k/2} , \notag 
% \end{align} 
% it follows that for each $k=1$, ..., $s-1$ and each $\alpha\in \{1, ..., d\}^k$ fixed, 
% \begin{align} 
%  \Big\| \frac{\partial^k l(z)}{\partial z_{\alpha_1} \cdots \partial z_{\alpha_k}} \Big\|_\infty  
%    = & \Big\| \big( c_k   
%    + (-\lambda)^k 2^k  \| z\|^2 
%     \big) e^{-\lambda \| z \|^2}  z_{\alpha_1} \cdots z_{\alpha_k} \Big\|_\infty   \notag \\ 
%  \leq &   \max_{r\geq 0} \big[ \big( | c_k |   
%    + |(-\lambda)^k| 2^k  r^2 
%     \big) e^{-\lambda r^2} r^k k^{-k/2} \big]   , \notag 
% \end{align}  
% By the first order condition, the maximum is attained at $r=k^{1/2} (2\lambda)^{-1/2}$. We substitute 
% $r=k^{1/2} (2\lambda)^{-1/2}$ into the right side of the above inequality to obtain 
% \begin{align} 
%  \Big\| \frac{\partial^k l(z)}{\partial z_{\alpha_1} \cdots \partial z_{\alpha_k}} \Big\|_\infty  
%  \leq &   \max_{r\geq 0} \big[ \big( | c_k |   
%    + |(-\lambda)^k| 2^k  r^2 
%     \big) e^{-\lambda r^2} r^k k^{-k/2} \big]    \notag  \\ 
%     = &  \big( |c_k| + (2\lambda)^{k-1} k  \big) e^{- k/2}  (2\lambda)^{-k/2} \notag \\ 
%     \leq & \Big[ (2\lambda)^{k-1} \frac{2(1+3\lambda)}{1 + 2\lambda} + \frac{ 4\lambda }{1 + 2\lambda} 
%     + (2\lambda)^{k-1} k  \Big] e^{- k/2}  (2\lambda)^{-k/2} \notag \\ 
%     = & \Big[  \frac{2(1+3\lambda)}{1 + 2\lambda}  
%     +  k  \Big] e^{- k/2}  (2\lambda)^{(k-2)/2} 
%     + \frac{ 4\lambda }{1 + 2\lambda} e^{- k/2}  (2\lambda)^{-k/2} . \notag   
% \end{align}  
% The maxium of the right side of the last equality is attained at $k=$. 


% By the Rademacher-Stephanov theorem \citep[Theorems 3.1.6 and 3.1.9]{Federer_GeometricMeasureTheoryBook_1969} and \eqref{ell-partial-k}, we have that
% \begin{align} 
%  \operatorname{Lip} \Big( \frac{\partial^{s-1} l(z)}{\partial z_{\alpha_1} \cdots \partial z_{\alpha_{s-1}}} \Big)  
%    =& \max_{z\in \mathbb{R}^{2D}}  \Big| \nabla_z \Big( \frac{\partial^{s-1} l(z)}{\partial z_{\alpha_1} \cdots \partial z_{\alpha_{s-1}}} 
%     \Big) \Big|    \notag 
% \end{align} 

% \begin{align} 
% \nabla_z \Big[ \frac{\partial^{s-1} l(z)}{\partial z_{\alpha_1} \cdots \partial z_{\alpha_{s-1}}} \Big] 
% = & (-2\lambda)^{s-1} 2z e^{-\lambda\|z\|^2} z_1\cdots z_{s-1}  
% \\
%  &+ (c_{s-1} + (-2\lambda)^{s-1} \|z\|^2 ) (-2\lambda) z e^{-\lambda\|z\|^2} z_1 \cdots z_{s-1} \notag \\ 
%  \notag
%  & + (c_{s-1} + (-2\lambda)^{s-1} \|z\|^2 ) e^{-\lambda\|z\|^2} \big( \sum_{j=1}^{s-1} e_{\alpha_j} \prod_{l=1\neq j}^{s-1} z_{\alpha_l} \big) 
% \notag 
% \end{align} 


    
% \end{proof}




% \bibliographystyle{plain}
% \bibliography{refs/main,
%                 refs/qfin-datasets, 
%                 refs/qfin-pm,
%                 refs/kalman-filters}                



% \end{document}




==> Bookkeeping/Historical_Versions/2024_07_30__PreNeurIPS.tex <==
% \documentclass{article}


% % if you need to pass options to natbib, use, e.g.:
% %     \PassOptionsToPackage{numbers, compress}{natbib}
% % before loading neurips_2024


% % ready for submission
% \usepackage{neurips_2024}


% % to compile a preprint version, e.g., for submission to arXiv, add add the
% % [preprint] option:
% % \usepackage[preprint]{neurips_2024}
% \usepackage{geometry}
%  \geometry{
%  a4paper,
%  total={170mm,257mm},
%  left=17.5mm,
%  right=17.5mm,
%  top=20mm,
%  }


% % to compile a camera-ready version, add the [final] option, e.g.:
% %     \usepackage[final]{neurips_2024}


% % to avoid loading the natbib package, add option nonatbib:
% %    \usepackage[nonatbib]{neurips_2024}


% \usepackage[utf8]{inputenc} % allow utf-8 input
% \usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% % \usepackage{hyperref}       % hyperlinks
% \usepackage{url}            % simple URL typesetting
% \usepackage{booktabs}       % professional-quality tables
% \usepackage{amsfonts}       % blackboard math symbols
% \usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{microtype}      % microtypography
% % \usepackage[table]{xcolor}         % colors
% %     \definecolor{darkcerulean}{rgb}{0.03, 0.27, 0.49}
% %     \definecolor{smokyblack}{rgb}{0.06, 0.05, 0.03}
% %     \definecolor{warmblack}{rgb}{0.0, 0.26, 0.26}
% %     \definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
% %     \usepackage[colorlinks=true,
% %                 linkcolor=cobalt,
% %                 urlcolor=darkcerulean,
% %                 citecolor=warmblack]{hyperref}


% % \documentclass[aap]{imsart}
% % Theorems with 
% % \theoremstyle{plain}
% % \documentclass[twoside,11pt]{article}

% % \usepackage{blindtext}

% % Any additional packages needed should be included after jmlr2e.
% % Note that jmlr2e.sty includes epsfig, amssymb, natbib and graphicx,
% % and defines many common macros, such as 'proof' and 'example'.
% %
% % It also sets the bibliographystyle to plainnat; for more information on
% % natbib citation styles, see the natbib documentation, a copy of which
% % is archived at http://www.jmlr.org/format/natbib.pdf

% % Available options for package jmlr2e are:
% %
% %   - abbrvbib : use abbrvnat for the bibliography style
% %   - nohyperref : do not load the hyperref package
% %   - preprint : remove JMLR specific information from the template,
% %         useful for example for posting to preprint servers.
% %
% % Example of using the package with custom options:
% %
% % \usepackage[abbrvbib, preprint]{jmlr2e}
% % \usepackage[abbrvbib, preprint]{jmlr2e}

% % \documentclass[aap]{imsart}

% %% Packages
% % \RequirePackage{amsmath,amsfonts,amssymb}
% % \usepackage{amsthm}
% % \RequirePackage[numbers,sort&compress]{natbib}
% %\RequirePackage[authoryear]{natbib}%% uncomment this for author-year citations
% % \RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
% % \RequirePackage{graphicx}

% % \startlocaldefs

% %% 
% %% Copyright 2007-2020 Elsevier Ltd
% %% 
% %% This file is part of the 'Elsarticle Bundle'.
% % \documentclass[preprint,12pt,authoryear]{elsarticle}
% % \usepackage{amssymb}
% % \journal{Stochastic Processes and Their Applications}

% % % SCIMODS_Wrapped_2022
% % \documentclass[11pt]{article}


% \usepackage[utf8]{inputenc}
% % \usepackage[10pt]{extsizes} % <- Override Spring Size


% \input{math_commands}
% \usepackage{lipsum}
% % Springer
% % \raggedbottom
% % \newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
% % \setlength\heavyrulewidth{0.3ex}
% % \usepackage{lscape}


% % \ShortHeadings{Reality Only Happens Once}{Horvath, Kratsios, Limmer, Saqur, and Yang}

% \input{Bookkeeping/Commenting}

% %\author{%
% %  David S.~Hippocampus\thanks{Use footnote for providing further information
% %    about author (webpage, alternative address)---\emph{not} for acknowledging
% %    funding agencies.} \\
% %  Department of Computer Science\\
% %  Cranberry-Lemon University\\
% %  Pittsburgh, PA 15213 \\
% %  \texttt{hippo@cs.cranberry-lemon.edu} \\
%   % examples of more authors
%   % \And
%   % Coauthor \\
%   % Affiliation \\
%   % Address \\
%   % \texttt{email} \\
%   % \AND
%   % Coauthor \\
%   % Affiliation \\
%   % Address \\
%   % \texttt{email} \\
%   % \And
%   % Coauthor \\
%   % Affiliation \\
%   % Address \\
%   % \texttt{email} \\
%   % \And
%   % Coauthor \\
%   % Affiliation \\
%   % Address \\
%   % \texttt{email} \\
% %}

% \usepackage{float}
% \raggedbottom
% % \newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
% \setlength\heavyrulewidth{0.3ex}
% \usepackage{lscape}


% \renewcommand{\ge}{	\geq }
% \renewcommand{\le}{	\leq }
% \renewcommand{\geq}{\geqslant}
% \renewcommand{\leq}{\leqslant}
% % Cool Eq Colours
% \usetagform{blue}

% \usepackage{wrapfig}

% \begin{document}
% % AAP
% % \begin{frontmatter}
% \title{Reality Only Happens Once: \\ 
% Single-Path %Pathwise
% Generalization Bounds for Transformers}


% % \title{Reality Only Happens Once: \\  
% % Generalization Bounds for Transformers in One-shot Trajectory Learning } 

% \author{
% Yannick Limmer  \\
% Department of Mathematics \\
% Oxford-Man Institute \\
% University of Oxford\\
% \texttt{limmery@maths.ox.ac.uk} \\
% \And 
% Anastasis Kratsios  \\
% Department of Mathematics \\
% McMaster University \\
% Vector Institute \\
% \texttt{kratsioa@mcmaster.ca} \\
% \And    
% Xuwei Yang \\
% Department of Mathematics  \\
% McMaster University \\
% \texttt{yangx212@mcmaster.ca} \\
% \And
% Raeid Saqur \\
% Department of Computer Science \\
% University of Toronto \\
% Vector Institute \\
% \texttt{raeidsaqur@cs.toronto.edu} \\
% \And
% Blanka Horvath  \\
% Department of Mathematics \\
% Oxford-Man Institute \\
% University of Oxford\\
% \texttt{horvath@maths.ox.ac.uk} \\
% } 

% \maketitle


% \begin{abstract}
% One of the inherent challenges in deploying transformers on time series is that \emph{reality only happens once}; namely, one typically only has access to a single trajectory of the data-generating process comprised of non-i.i.d.\ observations.  We derive non-asymptotic statistical guarantees in this setting through bounds on the \textit{generalization} of a transformer network at a future-time $t$, given that it has been trained using $N\le t$ observations from a single perturbed trajectory of a Markov process.  Under the assumption that the Markov process satisfies a log-Sobolev inequality, we obtain a generalization bound which effectively converges at the rate of $\mathcal{O}(1/\sqrt{N})$.  Our bound depends explicitly on the activation function ($\operatorname{Swish}$, $\operatorname{GeLU}$, or $\tanh$ are considered), the number of self-attention heads, depth, width, and norm-bounds defining the transformer architecture.  Our bound consists of three components: (I) The first quantifies the gap between the stationary distribution of the data-generating Markov process and its distribution at time $t$, this term converges exponentially to $0$.  (II) The next term encodes the complexity of the transformer model and, given enough time, eventually converges to $0$ at the rate $\mathcal{O}(\log(N)^r/\sqrt{N})$ for any $r>0$. (III) The third term guarantees that the bound holds with probability at least $1$-$\delta$, and converges at a rate of $\mathcal{O}(\sqrt{\log(1/\delta)}/\sqrt{N})$.  
% \end{abstract}

% %%%%%%%%%%%%%%%%%%%%% Section 1 %%%%%%%%%%%%%%%%%%%%%

% \section{Introduction}
% \label{s:Intro}
% Transformers~\cite{vaswani2017attention} have become the main architectural building block in deep learning-based state-of-the-art foundation models~\cite{bommasani2021opportunities, zhao2023survey, wei2022emergent}.
% Transformers are primarily deployed on sequential learning tasks which have complex temporal relationships, and thus, transformers are trained on non-i.i.d.\ data. 
% The i.i.d.\ assumption is typically made (e.g.~\cite{neyshabur2015norm,bartlett2017spectrally,zhang2024trained}) to derive theoretical statistical guarantees, but in practice it is rarely satisfied; e.g.~in natural language processing (NLP)~\citep{zhou2021informer}, physics~\cite{PualBaschnagelStochasticPhys_book_2013}, medical research~\cite{beck1983markov}, reinforcement learning \cite{SuttonBardo_RLBook_2018}, optimal control~\cite{Nizar_ControlBook_2013}, and in finance~\cite{FollmerSchiedStochFinanceBoko_2011}. 
% This creates a mismatch between available statistical guarantees in deep learning (which often rely on the i.i.d.\ assumption) and how transformers are used in practice.

% Thus, this paper fills this gap by guaranteeing that transformers trained on a single time-series trajectory can generalize at future moments in time.  We, therefore, consider the learning problem where the user is supplied with $N$ paired samples $(X_1,Y_1),\dots,(X_N,Y_N)$, where each input $Y_n=f^{\star}(X_n)$ for a smooth (unknown) \textit{target function} $f^{\star}:\mathbb{R}^{d\times M}\to \mathbb{R}^D$ is to be learned, depending on a history length $M$, and where the inputs are generated by a time-homogeneous Markov process $\smash{X_{\cdot}\eqdef (X_n)_{n=1}^{\infty}}$.  Note that the assumption $Y_n=f^{\star}(X_n)$ results in only a mild loss of generality since if $X_{\cdot}$ is a discretized solution to a stochastic differential equation then $Y_n \approx \text{signal} + \text{additive noise}$ due to stochastic calculus considerations (see Appendix~\ref{a:stoch_example}).

% The performance of any transformer model  $\mathcal{T}:\mathbb{R}^{d\times M}\to \mathbb{R}^D$ is quantified via a smooth loss function $\ell:\mathbb{R}^D\times \mathbb{R}^D\to \mathbb{R}$.  When $M=1$, the generalization of such a $\mathcal{T}$ is measured by the gap between its \textit{empirical risk} $\mathcal{R}^{(N)}$, computed from the single-path training data, and its \textit{(true) $t$-future risk} $\mathcal{R}_t$ at a (possibly infinite) future time $N\le t\le \infty$ ($t\in \mathbb{N}_+$) 
% % (defined in Section~\ref{s:Prelim}). 
% % Our main result is illustrated in Figure~\ref{fig:phase_diagram__theoremsummary}.
% % \begin{figure}[H]
% %     \centering
% %     \input{figs/bm.tex}
% %     % \includegraphics[height=2in]{figs/genbounds.pdf}
% %     \caption{Phase diagram: Generalization bounds for transformers trained on a single path.}
% %     \label{fig:phase_diagram__theoremsummary}
% % \end{figure}
% % 
% % We consider an \textit{realizable} PAC setting problem, determined by a smooth $1$-Lipschitz \textit{target function} $f^{\star}:\mathbb{R}^d\to \mathbb{R}^D$ which we would like to learn using a sequence of random observations $\big((X_t,Y_t)\big)_{t\in \mathbb{N}}$ as our training data.  That is, for each $t\in\mathbb{N}_+$
% % \begin{align*}
% %     Y_t \eqdef f^{\star}(X_t) 
% %     %+ \varepsilon_t.
% % \end{align*}
% defined by
% % We aim to learn $f$ from a \textit{single path}.  The ability of a model to reliably recover the function $f:\mathbb{R}^d\to\mathbb{R}^D$ at time $t$, given the input $X_t$, is quantified by the \textit{$t$-future risk}
% \begin{align*}
%     \mathcal{R}_t(f)
%     \eqdef 
%     \mathbb{E}\big[
%         % \|f(X_t)-f^{\star}(X_t)\|
%         \ell(\mathcal{T}(X_t),f^{\star}(X_t))
%     \big]
% \end{align*}
% where $\mathcal{R}_{t}$ (resp.\ $\mathcal{R}_{\infty}$) is computed with respect to the distribution of $X_t$ (resp.\ \textit{stationary distribution} of $X_{\cdot}$).
% The time-$t$ excess-risk $\mathcal{R}_t$, which is generally unobservable, is estimated by a single-path estimator known as the empirical risk computed using all the noisy samples observed thus far
% \begin{align*}
%     \mathcal{R}^{(N)}(f)
%     \eqdef 
%     \frac1{N}\,\sum_{n=1}^N\,
%             % \|f(X_n)-Y_n\|
%             \ell(\mathcal{T}(X_n),f^{\star}(X_n))
%     .
% \end{align*}
% Our objective is to obtain a statistical learning guarantee bounding the gap between the empirical risk and the $t$-future risk of transformer models trained on a single path.


% Our main result is a bound on the \textit{future-generalization}, at any given time $t\ge N$, of a transformer trained from $N$ samples collected from an unknown transformation ($f^{\star}$) of any suitable unknown Markov process ($X_{\cdot}$).  
% Let $\transformerclass_{L,H,C,W}^{D,d,0}$ be the class of transformers  with $L$ transformer blocks, $H$ attention heads, weights constraint $C$, and maximum width $W$; then for respective input and output dimensions $d$ and $D$, and history length $1$ (including the current state), 
% the first takeaway of our main result (Theorem~\ref{thrm:main}) is that with probability of at least $1-\delta$
% \begin{equation}
% \label{eq:FutureG}
% \tag{FutureGen}
% % \resizebox{1\linewidth}{!}{$
%         \sup_{\mathcal{T} \in \transformer_{L,W,H}^{D,d,0}}
%         \,
%             \big|
%                 \mathcal{R}_t(\mathcal{T})-\mathcal{R}^{(N)}(\mathcal{T})
%             \big|
%     \in 
%     \mathcal{O}
%         \biggl(
%             \frac{\log(1/\delta) + \log(N)^{1/s}}{
%             \sqrt{N}
%             }
%         \biggr)
% % $}
% \end{equation}  
% where $s>0$ can be made arbitrarily large and $\mathcal{O}$ hides a dimensional constant depending on $s$.  

% \vspace{-1em}
% \subsection*{Contributions}
% \vspace{-1em}
% Our \textit{first main} contribution is the first generalization bound~\eqref{eq:FutureG} for transformers in the case of non i.i.d.\ training data at a \textit{future point in time}.  This provides the first set of statistical guarantees for transformers compatible with many time-series tasks.  More broadly speaking, our generalization is the first result which estimates the \textit{future-generalization} (in~\eqref{eq:FutureG}) of a learning model given that its performance has only been measured using present/past historical training data.

% Our \textit{secondary contribution} is a full analysis of the constants under the big $\mathcal{O}$ in our future-generalization bound via a complete estimation of the higher order sensitivities/derivatives of the transformer network.  The computation of these constants in Theorem~\ref{thm:TransformerBlockSobolevBound} (and their order estimates in Theorem~\ref{thm:TransformerBlockSobolevBoundLevel}) are explicitly expressed in terms of the number of attention heads, depth and width of the transformed model, and weight and bias restriction, as well as on the activation functions used.  
% Our analysis applies to transformers using any smooth activation function, we perform an in-depth analysis for the $\operatorname{Swish}$~ \cite{ramachandran2017searching}, $\operatorname{GeLU}$~\cite{hendrycks2016gaussian}, and the $\tanh$ activation functions.  This allows us to analyze the impact of each of these choices on the future generalization of transformers.    

% \vspace{-1em}
% \subsection{Related Work}
% \label{s:PrelatedWork}
% \vspace{-1em}
% The mathematical foundations of transformer networks have recently come into focus in the deep learning theory community.  Most of the available statistical guarantees for transformers either concern: in-context learning for linear transformers \cite{zhang2024trained,garg2022can}, transformers \cite{von2023transformers,akyrek2023what} trained with gradient descent, or instance-dependant bounds \cite{trauger2023sequence} for general transformers.  
% % Unfortunately, these results assume that the transformers are trained on i.i.d.\ data. Thus, these results do not apply to the aforementioned time series prediction problems where data is not i.i.d.\ but is generated by a Markov process.  
% These results, however, do not apply in time series analysis contexts where each training sample is not independent of the others but is rather generated by some recursive stochastic process, e.g.\ a Markov process.

% Analytic counterparts to the statistical guarantees for transformers have also emerged.  These include universal approximation theorems for transformer networks \cite{yun2019transformers,yun2020n,fang2023attention} and contained universal approximation results for networks leveraging generalized attention mechanisms \cite{kratsios2022universal}, and the identification of function classes which can be efficiently approximated by transformers special classes \cite{likhosherstov2021expressive,frieder2024mathematical}.  From the computability standpoint, transformers are Turing complete  \cite{bhattamishra2020computational}. 

% Generalization bounds for multilayer perceptions (MLPs) have been actively studied for years.  For classification problems, these generalization bounds often rely on bounding the VC-dimension of classes of MLPs, depending on their depth, width, norm bounds on their parameters and activation functions \cite{bartlett1998almost,MR3960917}, or similar quantities.  In regression problems, one instead controls the Rademacher complexity of similar classes of MLPs \cite{bartlett2017spectrally,neyshabur2018the,pmlr-v97-yin19b}, due to the results such as \cite{koltchinskii2001rademacher,bartlett2002rademacher}, or turns to instance-dependant bounds which control the path-norm of the MLP \cite{neyshabur2015norm, golowich2020size,galanti2024norm} and local variants of these quantities; e.g.~\cite{Bartlett_LocalRadComplex_AnnStat_2005} or~\cite{hou2023instance}.  
% % These path norms are effectively the upper bounds of the Lipschitz constant of the instantiated model.  
% Our generalization bounds also partially borrow ideas from both of these directions, but instead, we use high-order sensitivities (partial derivatives) of our transformer networks to obtain tighter bounds for large enough $N$.  
% This does not yield a faster rate, since the $\mathcal{O}(1/\sqrt{N})$ rate is generally optimal, by the central limit theorem,
% % and cannot generally be removed from~\Cref{hprob}, 
% but it allows us to better control the constants in the generalization bound and thus yields more precise bounds.  Thus, a key part of our \textit{technical contributions} is the computation of these higher-order derivatives ($C^s$-norms) both of the transformer and the MLP models using smooth activation functions.  

% These statistical learning results assume that the data samples are i.i.d.  However, time-series data is rarely i.i.d, they are often generated by Markov processor at least embeddable into a Markovian setting~\cite{cuchiero2019markovian,MR4181950}.  Though there are generalization bounds for non-i.i.d.\ relying on martingale arguments e.g.~\cite{pmlr-v32-kontorovicha14} and concentration of measure phenomena for martingale sums e.g.~\cite{MartingaleSumsbook2015,boucheron2013concentration} those results primarily focus on Lipschitz functions; thus, they do not consider higher-order derivatives. Our results add to this literature since we rely on the concentration of measure phenomena for Markov processes with respect to smooth counterparts of the $1$-Wasserstein distance (a tool used in many martingale arguments, e.g.~\cite{kontorovich2017concentration}, for Lipschitz classes).


% Our main result operates under the assumption that the stationary distribution of the Markov chain and its kernels all satisfy a log-Sobolev inequality (LSI).  Since their introduction, LSIs have been heavily studied \cite{GrossLogSobolev,LedouxNourdinPEccati_SteinGAFA_OTIneq_2015,Zimmerman_JFALogSobolev,InglisPapageourgio_JFAGibbsLogSobolev_PTRF_2019,ChenChewiNilesWeed_MixtureDimFreLogSob_JFA_2021} and have found numerous applications in differential privacy \cite{minami2016differential,ye2022differentially}, optimization \cite{LeCunetal_JStatMech_EntropSGD_2019}, random matrix theory \cite{Winger_AnnMath_1955_I,Winger_AnnMath_1955_II}, optimal transport \cite{DoleraMaini_AHPCStat_LipContinuityProbOT}, since they typically imply~\cite{Gozlan_LSI_II_AHPC_DFRatesSnowflake,Gozlan_LSI_IC_VPDE__DFConcentration} and effectively characterizes \cite{Gozlan_LSI_III_AnnProb_2009} dimension-free rate for concentration of measure.

% We require that the data-generating Markov process has an exponentially contracting Markov kernel \cite{Kloeckner_2020CounterCurse_ESAIM}.  For Markov chains, i.e.\ finite-state space Markov processes, this means that that the generator ($Q$-matrix) of the Markov chain has a \textit{spectral gap}.  These spectral gaps are actively studied in the Markov chain literature \cite{mufa1996estimation,kontoyiannis2012geometric,atchade2021approximate,MR3383563,kloeckner2019effective} since these have a finite mixing time, meaning that they distribution of such Markov chains approaches their stationary limit after a large finite time has elapsed; i.e.\ they have well-behaved (approximate) mixing times~\cite{montenegro2006mathematical,hsu2015mixing,wolfer2019estimating,BZ_Mixing}.

% Our generalization bounds relied on concentration of measure arguments for the ``smooth'' integral probability metrics (IPMs) studied in~\cite{Kloeckner_2020CounterCurse_ESAIM,Riekert_ConcentrationOfMeasure2022}, by refining the arguments of~\cite{hou2023instance,benitez2023out,kratsios2024tighter} to the non-i.i.d.\  and smooth setting.  
% In the i.i.d.\ case, our computation of the maximum $C^s$-norm $(R\ge 0)$ of the class $\smash{\transformerclass_{L,W,H}^{D,d,0}}$ (Theorem~\ref{thm:TransformerBlockSobolevBound}) can be used to relate the rate at which measure concentrates (from i.i.d.\ data) for these IPMs can be bounded-above via classical quantities such as the Rademacher complexity of the class of $C^s$-functions on $\mathbb{R}^d$ with $C^s$ norm at-most $R$; see e.g.~\citep[Theorem 3.3]{EJA_2012_IPMs_EmpiricalControl}.  

% \paragraph{Further Applications of our Secondary Results}
% The upper bounds, which we compute for the $C^s$ norms of the transformers models, can be used in conjunction with classical VC-dimension \cite{vaart2023empirical}, Rademacher complexity~\cite{bartlett2002rademacher}, or optimal transport~\cite{hou2023instance} type arguments to obtain generalization bounds in the simpler setting of i.i.d.\ data where there is \textit{no notion of (future) time}, not considered here.  
% This can be done using classical tools, e.g.\ entropy estimates in~\citep[Theorem 2.7.4]{vaart2023empirical} on compact domains due to the Sobolev embedding theorem, applied to the larger class of $C^s$ on $\mathbb{R}^{d\times M}$ whose $C^s$-norms are all most equal to the one we have computed for $\smash{\transformerclass_{L,H,C, W}^{D,d,M}}$ in \Cref{thm:TransformerBlockSobolevBound,thm:TransformerBlockSobolevBoundLevel}.  


% \section{Background and Preliminaries}
% \label{s:Prelim}

% This section overviews the necessary background for a self-contained formulation of our main results.  This includes the definition of transformers and probabilistic tools such as log-Sobolev inequalities.  


% % \subsection{Log-Sobolev Inequalities and Moment Conditions}
% % \label{s:Prelim__ss:LSI_MomentConditions}
% \paragraph{Log-Sobolev Inequalities and Moment Conditions}
% % \label{s:Prelim__ss:LSI_MomentConditions}
% Fix dimensions $d,D\in \mathbb{N}_+$ and let $P$ be a Markov kernel on a non-empty Borel $\mathcal{X}\subseteq \mathbb{R}^d$ with initial distribution $X_0\sim \mu_0\in \mathcal{P}(\mathbb{R}^d)$, and with associated Markov process $X_{\cdot}\eqdef (X_t)_{t\in \mathbb{N}_0}$ given by $X_t\sim \mu_t\eqdef P^t \mu_0$.  
% % We consider a sequence of independent, not necessarily identically distributed, random variables $\varepsilon_{\cdot}\eqdef (\varepsilon_t)_{t \in \mathbb{N}}$ taking values in $\mathbb{R}^d$ and independent of $X_{\cdot}$ with a uniformly bounded first moment
% % \begin{equation}
% % \label{eq:UBFM}
% %     \Delta_{\text{noise}}\eqdef \sup_{t\in \mathbb{N}_+}\, \mathbb{E}[|\varepsilon_t|] < \infty
% % .
% % \end{equation}
% The \textit{entropy functional} $\mathcal{H}_{\mu}$ associated to any Borel probability measure $\mu$ on $\mathbb{R}^d$ acts on smooth functions $g:\mathbb{R}^d\to \mathbb{R}$ by
% \begin{align*}
%     \mathbb{H}_{\mu}(g) \eqdef \mathbb{E}_{X\sim \mu}
%         \Big[
%             g(X)
%             \log\Big(
%                 \frac{g(X)}{\mathbb{E}_{Z\sim \mu}[g(Z)]}
%             \Big)
%         \Big]
% .
% \end{align*}
% The entropy functional can be used to express the log-Sobolev inequalities.  
% \begin{definition}[Log-Sobolev Inequality]
% \label{defn:LSI}
% A probability measure $\mu$ on $\mathbb{R}^d$ is said to satisfy a log-Sobolev inequality with constant $C>0$ ($\operatorname{LSI}_C$) if for every smooth function $g:\mathbb{R}^d\to\mathbb{R}$
% \begin{align*}
% \smash{
%     \mathbb{H}_{\mu}(g^2)
%     \le 
%     C \ 
%     \mathbb{E}_{X\sim \mu}[\|\nabla g(X)\|^2]
% }
% \end{align*}
% \end{definition}
% We require that the Markov process is time-homogeneous to admit a satisfactory measure.  
% Further, we require that its Markov kernel and its stationary measure all satisfy $\operatorname{LSI}_C$.
% \begin{assumption}[Satisfactions of the Log-Sobolev Inequality]
% \label{ass:MC}
% There exists a $C>0$ such that $\bar{\mu}$, $\mu_0$, and $P(x,\cdot)$ all satisfy $\operatorname{LSI}_C$, for each $x\in \mathcal{X}$.
% \end{assumption}
% Several examples of Markov processes satisfying LSI inequalities are given in~\cite{ledoux2006concentration} and Gaussian processes satisfy the Exponential Moments Assumption.
% Lastly, we require that the Markov process $X_{\cdot}$ is bounded.  This will not be required for our concentration arguments (Proposition~\ref{prop:Concentation}) but it is needed when controlling the higher order derivatives of the transformer model, which can explode when considered over an unbounded domain; i.e.\ on all of $\mathbb{R}^{Md}$.
% \begin{assumption}[Bounded Trajectories]
% \label{ass:Comp_Support}
% There is a constant $c_K>0$ such that, each $t\in \mathbb{N}_+$, $\|X_{\cdot}\| \le c_k$ holds with probability $1$.
% \end{assumption}

% % \subsection{{Multi-Index Notation and \texorpdfstring{$C^s$}{Cs}-Norms}}
% % \label{s:Prelim__ss:Notation}
% % Much of our analysis centers around the \textit{regularity} of functions, by which we mean the maximum of high-order fluctuations of a function, as quantified by its higher-order partial derivatives.  These are formalized by the $C^s$-norm, defined for any function $f:\mathbb{R}^d\to \mathbb{R}$ on a  subset of $\mathbb{R}^d$ by 
% % These are formalized using the following multi-index notation.
% %%
% % All multi-indices $\alpha \eqdef (\alpha_1, \ldots, \alpha_k) \in \N^k, k \in \N$ are denoted by Greek letters, their sums are $\vert \alpha \vert \eqdef \sum_{i=1}^k \alpha_k$, and their faculty is $\alpha!  \eqdef \prod_{i=1}^k \alpha_k!$.  
% % We order multi-indices $\alpha$ and $\beta$, denoted by $\alpha \prec \beta$, if one of the three following holds 
% % \begin{enumerate}[label=(\roman*), nosep]
% %     \item $\vert \alpha \vert < \vert \beta \vert$;
% %     \item $\vert \alpha \vert = \vert \beta \vert$, and $\alpha_1 < \beta_1$; or 
% %     \item $\vert \alpha \vert = \vert \beta \vert$, and $\alpha_i = \beta_i$ for $i \in \myset{1}{j-1}$ and $\alpha_j < \beta_j$ for $j \in \myset{2}{k}$.
% % \end{enumerate}
% % We use multi-indices to track the following operations:  Exponentiation of vectors in $x \in \R^k$, which we defined by $x^\alpha \eqdef \prod_{i=1}^k x_k^{\alpha_k}$ and derivatives of functions using the derivative operator $D^{\alpha}$, w.r.t. a multi-index $\alpha$, defined by $D^\alpha \eqdef \partial^{\vert \alpha \vert} / \partial x_1^{\alpha_1} \cdots \partial x_k^{\alpha_k}$, where, $\vert \alpha \vert > 0$ (otherwise $D^\alpha$ is the identity operator).  For any $s>0$, we define the $C^s$ norm, denoted by $\|\cdot\|_{C^s}$, of a smooth (infinitely differentiable) function $f:\mathbb{R}^d\to\mathbb{R}$ by
% % \begin{align*}
% %     \|f\|_{C^s}
% % \eqdef 
% %         \max_{k=1,\dots,s-1}\,
% %         \max_{\alpha\in \{1,\dots,d\}^k}
% %         \,
% %             \Big\|
% %                 \frac{\partial^k f}{
% %                     \partial x_{\alpha_1}\dots\partial x_{\alpha_k}
% %                 }
% %             \Big\|_{\infty}
% %     +
% %         \max_{\alpha \in \{1,\dots,d\}^{s-1}}\,
% %             \operatorname{Lip}\biggl(
% %                 \frac{\partial^{s-1}f}{\partial x_{\alpha_1}\dots\partial x_{\alpha_{s-1}}}
% %             \biggr).
% % \end{align*}
% % To streamline the analytic challenging tracking of $C^s$-norms, we will use the following \textit{order operator} $\order$ for multi-indices:
% % \begin{align*}
% %     \order: \N^k \longrightarrow \N^k, \quad \alpha_1, \ldots, \alpha_k \longmapsto \alpha_{\tau_\alpha(1)}, \ldots, \alpha_{\tau_\alpha(k)},
% % \end{align*}
% % where $\tau_\alpha: \myset{1}{k} \to \myset{1}{k}$ s.t. $\alpha_{\tau_\alpha(1)} \geq  \ldots \geq  \alpha_{\tau_\alpha(k)}$.  
% % \hfill\\
% % We write $\alpha \eqorder \beta$ if $\order(\alpha) = \order(\beta)$ for $\alpha, \beta \in \N^k$. Further, denote by $\Order^k_{n}$ the set $\{\order(\alpha) :  \alpha \in \N^k, \vert \alpha \vert = n \}$ and write $\Order^k_{\leq n} \eqdef \{\order(\alpha) :  \alpha \in \N^k, \vert \alpha \vert \leq n \}$. Further, define $N(\alpha) \eqdef \# \vert \{ \alpha' \in \N^k : \order(\alpha') = \alpha \} \vert$. 

% % The order notation, allows us to concisely tabulate the sizes of the $C^s$-norm for any $f: \mathbb{R}^k \to \R^m$, over a (non-empty) compact subset $K\subset \mathbb{R}^k$, for any multi-index $\alpha\in\Order^k_n$ an ordered multi-index as
% % \begin{align*}
% %     C^f_K(\alpha) \eqdef \max_{i \in \myset{1}{m}} \max_{\gamma \sim \alpha} \Vert D^\gamma f_i \Vert_K
% % .
% % \end{align*}

% % 

% \paragraph{The Transformer Model}

% The overall structure of transformers and their involved layers are summarized in Figure~\ref{fig:Transformer}.  
% We, thus, encourage the familiar reader to skip this section, which contains precise technical formulations of transformer classes with precise specifications on weight magnitude, depth, width, and a number of attention heads that can be rather involved.  

% \begin{figure}[!hbp]%[H]%
%      \centering
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%         \includegraphics[height=.2\textheight]{figs/Transformer/MultiHead.pdf}
%         % \vspace{15pt}
%         \caption{\textbf{Multi-Head Att. (Def.~\ref{defn:MultiHead})}}
%         % \vspace{-25pt}
%         \label{fig:MHA}
%      \end{subfigure}
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%         \includegraphics[height=.2\textheight]{figs/Transformer/TransformerBlock.pdf}
%         % \vspace{15pt}
%         \caption{\textbf{Transformer Block (Def.~\ref{defn:TransformerBlock})}}
%         % \vspace{-25pt}
%         \label{fig:TransformerBlock}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.38\textwidth}
%          \centering
%          \includegraphics[height=.2\textheight]{figs/Transformer/Transformer2.pdf}
%     % \vspace{15pt}
%     \caption{\textbf{Transformer (Def.~\ref{defn:Transformer})} }
%     % \vspace{-25pt}
%     \label{fig:Transformer}
%      \end{subfigure}
%         \caption{\textbf{Multi-Head Attention:} Consists of parallel application of the attention mechanism, described by the following steps. 1) Inputs are used three-fold, as keys, queries, and values, all are transformed by distinct linear transformations. 
%         2) Keys and queries are multiplied, scaled, and transformed by a softmax application.
%         3) This output is combined in a matrix multiplication with the values.
%         \hfill\\
%         \textbf{Transformer Block:} 
%         1) Input features are mapped to contexts via \textit{multi-head attention mechanism}.  
%         2) The output of the multi-head attention mechanism and the input features (via a skip connection) are normalized by a \textit{layer-norm}.  
%         3) The normalized contextual features are transformed non-linearly by a SLP.  
%         4) The outputs of the SLP, together with the first set of normalized context (via another skip connection), are normalized by a final \textit{layer-norm} and returned by the transformer block.
%         \hfill\\
%         \textbf{Transformers:} Iteratively feed input features through a series of transformer blocks before processing their outputs with a (fully connected affine layer).}
%         \label{fig:TLDR_Transformers}
% \end{figure}

% % \subsection{The Transformer Model}
% % \label{s:Prelim_ss:Transformer}
% % \begin{figure}[htbp]
% %     \centering
% %     \begin{subfigure}[b]{0.3\textwidth}
% %         \centering
% % \begin{tikzpicture}[
% %     node distance=.3cm and .5cm,
% %     layer/.style={rectangle, draw, rounded corners, align=center},
% %     addnorm/.style={layer, fill=yellow!20},
% %     multihead/.style={layer, fill=orange!20},
% %     feedforward/.style={layer, fill=blue!20},
% %     box/.style={draw, rounded corners, thick, inner sep=0.25cm},
% %     arrow/.style={-latex, thick}
% % ]
% % %\node (input) [draw=none, fill=none] {Input};
% % % Nodes
% % \node (mh_attention) [multihead] {Multi-Head \\ Attention};
% % \node (add_norm1) [addnorm, above=of mh_attention] {Add \& Norm};
% % \node (feed_forward) [feedforward, above=of add_norm1] {Feed \\ Forward};
% % \node (add_norm2) [addnorm, above=of feed_forward] {Add \& Norm};
% % \node (output) [draw=none, fill=none, right=of add_norm2] {Output};
% % \draw (output |- 52, 52 |- mh_attention) node (input) {Input};
% % % Box around
% % \node (encoder) [box, fit={(mh_attention) (add_norm1) (feed_forward) (add_norm2)}] {};
% % %\node [left=of encoder] (Nx) {N$\times$};
% % % Arrows
% % \draw [-latex] (mh_attention) -- (add_norm1);
% % \draw [-latex] (add_norm1) -- (feed_forward);
% % \draw [-latex] (feed_forward) -- (add_norm2);
% % % Skip connections
% % \draw [-latex, dashed] (input) |- (add_norm1.east);
% % \draw [-latex] (input) -- (mh_attention);
% % \draw [-latex] (add_norm2.east) -- (output);
% % \draw [-latex, dashed] (add_norm1.west) -- ++(-0.5,0) |- (add_norm2.west);
% % \end{tikzpicture}
% %         \caption{First subfigure}
% %     \end{subfigure}
% %     \hfill
% %     \begin{subfigure}[b]{0.6\textwidth}
% % \centering
% % \begin{tikzpicture}[
% %     node distance=.3cm and .5cm,
% %     layer/.style={rectangle, draw, rounded corners, align=center},
% %     addnorm/.style={layer, fill=yellow!20},
% %     multihead/.style={layer, fill=orange!20},
% %     feedforward/.style={layer, fill=blue!20},
% %     box/.style={draw, rounded corners, thick, inner sep=0.25cm},
% %     arrow/.style={-latex, thick}
% % ]
% % %\node (input) [draw=none, fill=none] {Input};
% % % Nodes
% % \node (keys) [multihead] {Multi-Head \\ Attention};
% % \node (queries) [addnorm, above=of mh_attention] {Add \& Norm};
% % \node (values) [feedforward, above=of add_norm1] {Feed \\ Forward};
% % \node (add_norm2) [addnorm, above=of feed_forward] {Add \& Norm};
% % \end{tikzpicture}
% %         \caption{Second subfigure}
% %     \end{subfigure}
% % \end{figure}
% %\AK{ put picture here}
% % \begin{figure}[h!]%[H]%
% % \centering
% % \end{figure}
% % \begin{wrapfigure}{l}{0.425\textwidth}
% % %  \vspace{-10pt}
% % \centering
% % \centerline{\includegraphics[width=0.1\textheight]{figs/Transformer/TransformerBlock.pdf}}
% % % \vspace{15pt}
% % \caption{\textbf{Transformer Block (Definition~\ref{defn:TransformerBlock}):} 
% % 1) Input features are mapped to contexts via \textit{multi-head attention mechanism}.  
% % 2) The output of the multi-head attention mechanism and the input features (via a skip connection) are normalized by a \textit{layer-norm}.  
% % 3) The normalized contextual features are transformed non-linearly by MLP.  
% % 4) The outputs of the MLP, together with the first set of normalized context (via another skip connection), are normalized by a final \textit{layer-norm} and returned by the transformer block.}
% % % \vspace{-25pt}
% % \label{fig:TransformerBlock}
% % \end{wrapfigure}
% % \begin{wrapfigure}{l}{0.425\textwidth}
% % %  \vspace{-10pt}
% % \centering
% % \centerline{\includegraphics[width=0.1\textheight]{figs/Transformer/TransformerBlock.pdf}}
% % % \vspace{15pt}
% % \caption{\textbf{Transformer Block (Definition~\ref{defn:TransformerBlock}):} 
% % 1) Input features are mapped to contexts via \textit{multi-head attention mechanism}.  
% % 2) The output of the multi-head attention mechanism and the input features (via a skip connection) are normalized by a \textit{layer-norm}.  
% % 3) The normalized contextual features are transformed non-linearly by MLP.  
% % 4) The outputs of the MLP, together with the first set of normalized context (via another skip connection), are normalized by a final \textit{layer-norm} and returned by the transformer block.}
% % % \vspace{-25pt}
% % \label{fig:TransformerBlock}
% % \end{wrapfigure}
%     % \begin{wrapfigure}{r}{0.5\textwidth}
%     % %  \vspace{-10pt}
%     % \centering
%     % \centerline{\includegraphics[width=1\linewidth]{figs/Transformer/Transformer.pdf}}
%     % % \vspace{15pt}
%     % \caption{\textbf{Transformer (Definition~\ref{defn:Transformer}):} Inputs are iteratively fed trough a series of transformer blocks (each as in Figure~\ref{fig:TransformerBlock}) and then processed by a (fully connected affine layer).}
%     % % \vspace{-25pt}
%     % \label{fig:Transformer}
%     % \end{wrapfigure}



% For any $F\in \mathbb{N}_+$, we will consider a weighted (parametric) variant of the \textit{layer normalization} function of \cite{ba2016layer}, which permits a variable level of regularization.  Our weighted \textit{layer normalization} is defined by $\operatorname{LayerNorm}:\mathbb{R}^F\to \mathbb{R}^F$ defined for any $u\in \mathbb{R}^F$ by 
% \begin{align*}
%     \layernorm(u;\gamma,\beta,w)\eqdef  
%     % \begin{cases}
%         \gamma\, 
%         \frac{(u-\mu_u^w)}{\sqrt{1 + (\sigma_u^w)^2}} + \beta 
%         % & \mbox{ if } u\neq 0\\
%     %     0 & \mbox{ if } u=0
%     % \end{cases}
% \end{align*}
% where $\mu_u^w\eqdef \sum_{i=1}^F\, \frac{w}{F} u_i$ and $(\sigma_u^w)^2 \eqdef \sum_{i=1}^F\, \frac{w}{F}\,\|u_i-\mu_u\|^2$, $\softplus \eqdef \ln (1 + \exp(\cdot))$, parameters $\beta\in \mathbb{R}^F$ and $\gamma \in \mathbb{R}$, and the normalization strength parameter $w\in [0,1]$ with $w=1$ being the default choice.   Here, we prohibit the layer norm from magnifying the size of its outputs when the layer-wise weighted variance $\sigma_u^w$ is small.\footnote{Note that this formulation of the layer norm avoids division by $0$ when the entries of $u$ are identical.}


% % each $F \in \N$, by
% % \begin{align*}%\label{id:Softmax}
% %     \softmax:
% %             \R^F 
% %         \to     
% %             \R^F,
% %     \quad 
% %             x 
% %         \mapsto 
% %             \left(
% %                     {\exp(x_i)}
% %                 /
% %                     {\textstyle\sum_{j = 0}^{F-1} \exp(x_j)}
% %             \right)_{i=0}^{F-1}.
% % \end{align*}


% \begin{definition}[Multi-Head Self-Attention]\label{defn:MultiHead}
% Fix $\idim \in \N$. For $x \in  \R^{(M \times \idim}$, $Q, K \in \R^{\kdim \times \idim}$, and $V \in \R^{\vdim \times \idim}$, where we have key-dimension $\kdim \in \N$ and value-dimension $\vdim \in \N$; we define
% \begin{align*}%\label{id:Attention}
%         \attention(
%             x; Q, K, V 
%         )
%     \eqdef    
%         \bigg(
%             \sum_{j=0}^M
%                 \softmax\left(
%                     \Big(
%                         \frac{\langle
%                             Qx_m, Kx_i
%                         \rangle}{\sqrt{d_k}
%                         }
%                     \Big)_{i = 0}^{M}
%                 \right)_j
%                 Vx_j
%         \bigg)_{m=1}^M
%     \in \R^{M \times \vdim}.
% \end{align*}
% For $H \in \N$, set $Q \eqdef (Q^{(h)})_{h=1}^H, K \eqdef (K^{(h)})_{h=1}^H \subseteq \R^{\kdim \times \idim}$, $V \eqdef (V^{(h)})_{h=1}^H \subseteq \R^{\vdim \times \idim}$, and $W \eqdef (W^{(h)})_{h=1}^H \subseteq \R^{\idim \times \vdim}$. For $x \in  \R^{M \times \idim}$, we define
% \begin{align*}%\label{id:MultiHead}
%         \multihead(x; Q, K, V, W) 
%     \eqdef 
%         \bigg(
%             \sum_{h = 1}^H
%                 W^{(h)} \attention(
%                     x; Q^{(h)}, K^{(h)}, V^{(h)}
%                 )_m 
%         \bigg)_{m = 1}^M \in \R^{(M) \times \idim}.
% \end{align*}
% \end{definition}

% Each transformer block takes a set of inputs and intersperses normalization (via layer norms), contextual comparisons (via multi-head attention mechanism), and non-linear transformations (via an SLP).  
% % 
% % Our transformer block extends the definition in \cite{vaswani2017attention}, allowing the intermediate feedforward neural network to pass information across all time steps instead of operating on each time step individually.
% We also allow the transformer block to extend or contract the length of the generated sequence.  

% \begin{definition}[Transformer Block]
% \label{defn:TransformerBlock}
% Fix a non-affine activation function $\sigma\in C^{\infty}(\R)$.  
% Fix a dimensional multi-index $d=(\idim, \kdim, \vdim, \ldim, \odim) \in \N^{5}$, a sequence length $M \in \N_+$, and a number of self-attention heads $H\in \mathbb{N}_+$.  
% A transformer block is a permutation equivariant map $\tblock:\mathbb{R}^{M\times \idim}\to \mathbb{R}^{M\times \odim}$ represented for each $x\in \mathbb{R}^{M\times \idim}$
% \begin{align}\label{eq:TB}
% \begin{aligned}
%         \tblock (x) 
%     & \eqdef  
%         \Big(
%         \layernorm\big(
%         B^{(1)} x'_m + B^{(2)} \big(\sigma\bullet (A\, x'_m + a)\big) ;\, \gamma_2,\beta_2,w_2
%         \big)
%         \Big)_{m=1}^M
%     \\
%         x'
%     & \eqdef 
%         \Big(
%     \layernorm\big(
%         x_m + \multihead(x; Q, K, V, W)_m;\,\gamma_1, \beta_1,w_1
%         \big)
%         \Big)_{m=1}^M
%     % \\
%     %     x_0 
%     % & \eqdef 
%     %     \reshape_{(1+M_0)\times d_0}(x)
% \end{aligned}
% \end{align}
% for $\gamma_1,\gamma_2\in \mathbb{R}$, 
% $w_1,w_2\in [0,1]$, 
% $\beta_1\in \mathbb{R}^{\idim}$, 
% $\beta_2\in \mathbb{R}^{\odim}$, 
% $A\in \mathbb{R}^{\ldim \times \idim}$, $a\in \mathbb{R}^{\ldim}$, 
% $B^{(1)} \in \mathbb{R}^{\odim \times \idim}$, $B^{(2)} \in \mathbb{R}^{\odim \times \ldim}$, and $Q, K, V, W$ as in \Cref{defn:MultiHead}.

% The class of transformer blocks with representation~\eqref{eq:TB} is denoted by $\tblockclass_{d,M,H,C}$, where $\smash{C \eqdef (C^{\gamma_1}, C^{\gamma_2}, C^{\beta_1}, C^{\beta_2}, C^a, C^A, C^{B^{(1)}}, C^{B^{(2)}}, C^{Q}, C^{K}, C^{V}, C^{W})}$. 
% % \begin{comment}
% % The restriction for $C>0$ such that
% % $
% % \vert \gamma_1 \vert, 
% % \vert \gamma_2 \vert, 
% % \vert \beta_1 \vert,
% % \vert \beta_2 \vert,
% % \vert a \vert,
% % \Vert A \Vert,
% % \Vert B^{(1)} \Vert, 
% % \Vert B^{(2)} \Vert, 
% % \Vert Q^{(h)} \Vert,
% % \Vert K^{(h)} \Vert,
% % \Vert V^{(h)} \Vert, 
% % \Vert W^{(h)} \Vert < C 
% % $ 
% % for all $h \in \myset{1}{H}$, is denoted by $\tblock^C_{d,M,H}$.
% % \end{comment}
% \end{definition}


% % \begin{figure}[h!]%[H]%
% % \centering

% % \end{figure}
% % \begin{figure}[H]
%     % \begin{wrapfigure}{r}{0.5\textwidth}
%     % %  \vspace{-10pt}
%     % \centering
%     % \centerline{\includegraphics[width=1\linewidth]{figs/Transformer/Transformer.pdf}}
%     % % \vspace{15pt}
%     % \caption{\textbf{Transformer (Definition~\ref{defn:Transformer}):} Inputs are iteratively fed trough a series of transformer blocks (each as in Figure~\ref{fig:TransformerBlock}) and then processed by a (fully connected affine layer).}
%     % % \vspace{-25pt}
%     % \label{fig:Transformer}
%     % \end{wrapfigure}
% % \end{figure}

% A transformer concatenates several transformer blocks before passing their outputs to an affine layer and ultimately outputting its prediction.

% \begin{definition}[Transformers]
% \label{defn:Transformer}
% Fix depth $L\in \mathbb{N}_+$, memory $M\in \mathbb{N}$, width $W\in \mathbb{N}^5_+$, number of heads $H\in \mathbb{N}_+$, and input-output dimensions $D,d\in\mathbb{N}_+$.  
% A transformer (network) is a map $\transformer: \mathbb{R}^{M\times D}\to \mathbb{R}^d$ with representation
% \begin{equation}
% \label{eq:Transformer_Nets}
%         \transformer(x)
%     =
%         A \big(
%             \vectorize_{1 + M, \odim^{L}}
%             \circ 
%             \tblock_L
%             \circ 
%             \dots 
%             \circ 
%             \tblock_1
%             (x)
%         \big)
%     +
%         b
% \end{equation}
% where multi-indices 
% $d^{l}=(\idim^{l},\kdim^{l},\vdim^{l},\ldim^{l},\odim^{l}) \leq W$ 
% are such that 
% $\idim^1=D$, 
% $\idim^{l+1}=\odim^l$ 
% for each $l=1, \dots,L-1$, 
% and where 
% $H \eqdef (H^l)_{l=1}^L$ are the number of self-attention heads,
% $C' \eqdef (C^l)_{l=1}^L$ the parameter bounds,
% and for $l=1,\dots,L$ 
% we have $\tblock_l \in \tblock_{d^{l},M,H^{l},C^l}$
% .
% Furthermore, $A \in \mathbb{R}^{d \times M\odim^{L}}$ and $b\in \mathbb{R}^d$.

% The set of transformer networks with representation~\eqref{eq:Transformer_Nets} and parameters bound by $C$ is denoted by $\transformerclass_{L,H,C, W}^{D,d,M}$, where $C \eqdef (*C', C^A, C^b)$. If the specification is clear, we write $\transformerclass_{L,H,C, W}^{D,d,M} \equiv \transformerclass$ for short.
% \begin{comment}
% The restriction for $C > 0$ $\tblock_l \in \tblock^C_{d^{l},M^{l},H^{l}}$ for all $l \in \myset{0}{L-1}$, together with $\vert b \vert, \Vert A \Vert < \infty$ is denoted by $\transformer_{L,W,H}^{D,d,M; C}$.
% \end{comment}
% \end{definition} 




% \paragraph{Notation}
% % \subsection{Notation}
% % \label{s:Notation_Light}
% \begin{comment}
% Much of our analysis centers around the \textit{regularity} of functions, by which we mean the maximum of high-order fluctuations of a function, as quantified by its higher-order partial derivatives.  These are formalized by the $C^s$-norm, defined for any function $f:\mathbb{R}^d\to \mathbb{R}^D$ on a  subset of $\Omega\subseteq \mathbb{R}^d$ by
% \begin{align*}
%     \|f\|_{C^s}
% \eqdef 
%         \max_{k=1,\dots,s-1}\,
%         \max_{\alpha\in \{1,\dots,d\}^k}
%         \sup_{x\in \Omega}\,
%         \,
%             \Big\|
%                 \frac{\partial^k f}{
%                     \partial x_{\alpha_1}\dots\partial x_{\alpha_k}
%                 }(x)
%             \Big\|
%     +
%         \max_{\alpha \in \{1,\dots,d\}^{s-1}}\,
%             \operatorname{Lip}\biggl(
%                 \frac{\partial^{s-1}f}{\partial x_{\alpha_1}\dots\partial x_{\alpha_{s-1}}}
%             \big|\Omega
%             \biggr),
% \end{align*}
% where $\operatorname{Lip}(g|\Omega)$ denotes the \textit{local} Lipschitz constant of a function $f$ on $\Omega$ (i.e.\ effectively maximal norm its gradient on $\Omega)$.  
% \end{comment}
% We make use of \textit{reshape operators} (standard in most deep learning software) which, for any $F_1,F_2\in \mathbb{N}_+$, are given by $\reshape_{F_1\times F_2}$ map any vector $u\in \mathbb{R}^{F_1F_2}$ to the $F_1\times F_2$ matrix
% \begin{align*}
%     \reshape_{F_1\times F_2}(x)_{i,j}\eqdef x_{(i-1)F_2 +j}
%     .
% \end{align*}
% We denote the inverse of the map $\reshape_{F_1\times F_2}$ by $\vectorize_{F_1,F_2}:\mathbb{R}^{F_1\times F_2}\to\mathbb{R}^{F_1F_2}$.  
% We also recall the definition of the \textit{softmax} function, defined by $\operatorname{softmax}(x)\eqdef 
%             (
%                     {\exp(x_i)}
%                 /
%                     {\textstyle\sum_{j = 0}^{F-1} \exp(x_j)}
%             )_{i=0}^{F-1}$ for each $F\in \mathbb{N}_+$ and each $x\in \R^F$.
% %%%%
% The maximum size of a norm in any vector in any $K\subseteq \mathbb{R}^k$ is denoted by $\Vert K \Vert \eqdef \sup_{x \in K} \Vert x \Vert$, the $\ell^{\infty}$-matrix norm of any $n\times m$ matrix $A \in \R^{n\times m}$ is denoted by $C^A \eqdef \max_{i \in \myset{1}{n}, j \in \myset{1}{m}} \vert A_{i,j}\vert$.
% Fix $d,D,s\in \mathbb{N}_+$ and a smooth function $f:\mathbb{R}^d\to \mathbb{R}^D$ then its $C^s$-norm on a (regular closed) subset $K\subseteq \mathbb{R}^D$ is defined to be 
% \begin{align*}
% % \resizebox{1\linewidth}{!}{$%% BEGIN RESIZE BOX$}
%     \|f\|_{s:K}
% \eqdef 
%         \underset{
%             \underset{\alpha\in \{1,\dots,d\}^k}{k=1,\dots,s-1}
%         }{\max}
%         \,
%             \underset{u\in K}{\sup}\,
%             \Big\|
%                 \frac{\partial^k f}{
%                     \partial x_{\alpha_1}\dots\partial x_{\alpha_k}
%                 }(u)
%             \Big\|
%     +
%         \underset{\alpha \in \{1,\dots,d\}^{s-1}}{\max}\,
%             \operatorname{Lip}\Big(
%                 \frac{\partial^{s-1}f}{\partial x_{\alpha_1}\dots\partial x_{\alpha_{s-1}}}
%             |
%             K
%             \Big),
% % $}
% \end{align*}
% where $\operatorname{Lip}(g|K)$ denotes the Lipschitz constant of a function $g:\mathbb{R}^d\to \mathbb{R}^D$ and $\alpha$ is a multi-index.  All additional notation, not required for our main-text results, is relegated to Appendix~\ref{a:Notation}.







% \vspace{-0.5em}
% \section{Main Result}
% \label{s:Main_Result}

% We consider smooth loss and target functions functions that are concentrated on a compact region, along with their derivatives. The growth rate of the $C^s$ norm of the loss function and its derivatives quantifies the degree of concentration.  
% One easily verifies that any function in the Schwartz class satisfies this former of the following conditions.
% % similar conditions are considered in the random feature model literature; see e.g.~\cite{XXX}, or polynomials.
% % \begin{definition}[Polynomial Growth of Derivatives]
% % \label{def:sGrowthRate}
% % Let $d,D\in \mathbb{R}$.  A smooth function $g:\mathbb{R}^d\to \mathbb{R}^D$ belongs to the class $C^{\infty}_{poly:C,r}(\mathbb{R}^d,\mathbb{R}^D)$ if are $C,r\ge 0$ such that: $\|g\|_{C^s} \le C\, s^{r}$ for each $s\in \mathbb{N}_+$.
% % \end{definition}
% \begin{definition}[Polynomial Growth of Derivatives]
% \label{def:sGrowthRate}
% Let $d,D\in \mathbb{R}$.  A smooth function $g:\mathbb{R}^d\to \mathbb{R}^D$ is in   the class $C^{\infty}_{poly:C,r}([0,1]^d,\mathbb{R}^D)$ if are $C,r\ge 0$ such that: $\|g\|_{C^s([0,1]^d)} \le C\, s^{r}$ for each $s\in \mathbb{N}_+$.
% \end{definition}
% In Appendix~\ref{s:Functions_of_ControlledGrowth} we show that, in one dimension, any real analytic function whose power series expansion at $0$, has coefficients growing at an $\mathcal{O}((s+1)^r)$ rate belongs to $g\in C^{\infty}_{poly:C,r}([0,1],\mathbb{R})$.  One can easily extend this argument to multiple dimensions to obtain further examples.  


% We consider an \textit{realizable} PAC learning problem, determined by a smooth $1$-Lipschitz \textit{target function} $f^{\star}:\mathbb{R}^d\to \mathbb{R}^D$ which we would like to learn using a sequence of random observations $\big((X_t,Y_t)\big)_{t\in \mathbb{N}}$ as our training data.  That is, for each $t\in\mathbb{N}_+$
% \begin{align*}
%     Y_t \eqdef f^{\star}(X_t) 
%     %+ \varepsilon_t.
% \end{align*}
% We aim to learn $f$ from a \textit{single path}.  The ability of a model to reliably recover the function $f:\mathbb{R}^d\to\mathbb{R}^D$ at time $t$, given the input $X_t$, is quantified by the \textit{$t$-future risk}
% \begin{align*}
%     \mathcal{R}_t(f)
%     \eqdef 
%     \mathbb{E}\big[
%         % \|f(X_t)-f^{\star}(X_t)\|
%         \ell(f(X_t),f^{\star}(X_t))
%     \big]
% .
% \end{align*}
% The time-$t$ excess-risk $\mathcal{R}_t$, which is generally unobservable, is estimated by a single-path estimator known as the empirical risk computed using all the noisy samples to observed thus far
% \begin{align*}
%     \mathcal{R}^{(N)}(f)
%     \eqdef 
%     \frac1{N}\,\sum_{n=1}^N\,
%             % \|f(X_n)-Y_n\|
%             \ell(f(X_t),f^{\star}(X_t))
%     .
% \end{align*}
% Our objective is to obtain a statistical learning guarantee on the quality of our estimate of the target function given by the \textit{time $t \,(\in \mathbb{N}_+$) generalization gap}
% $%\begin{align*}
%     \big|\mathcal{R}_t(f)-\mathcal{R}^{(N)}(f)\big|
%     .
% $  

% We now summarize our setting and all parameters defining it, e.g.\ dimension, number of attention heads in the transformer, growth rate of the derivatives of the target and loss functions, etc.

% \begin{setting}
% \label{setting}
% Let $D,d,
% % M,
% L,H,*C^{\prime},C^A,C^b\in \mathbb{N}_+$, $C\eqdef (*C^{\prime},C^A,C^b)$, $r_f,r_{\ell},C_f,C_{\ell} \ge 0$, and consider the hypothesis class $\transformerclass_{L,H,C}^{D,d,
% 1%M
% }$.  Fix a target function $f^{\star}\in C^{\infty}_{poly:C_f,r_f}(\mathbb{R}^d,\mathbb{R}^D)$ and a loss function, $\ell\in C^{\infty}_{poly:C_{\ell},r_{\ell}}(\mathbb{R}^{2D},\mathbb{R})$ and suppose that Assumptions~\ref{ass:MC} and~\ref{ass:Comp_Support} hold.
% \end{setting}
 
% Having formalized our setting, we may now state our main result, which is a version of~\eqref{eq:FutureG}.  This version provides insights on the future-generalization of transformers via: 1) explicit constants and 2) explicit \textit{phase transition times} above which the convergence rate in~\eqref{eq:FutureG} accelerates by a polylogarithmic factor.  We express these times of convergence rate acceleration are expressed using the following \textit{convergence rate function}
% \begin{equation}
% \tag{rate}
% \label{eq:rate_function__definition}
%         \operatorname{rate}_s(N)
%     \eqdef 
%         \begin{cases}
%            \frac{
%                \log(
%                     c\, N
%                 )^{d-2s+s/d}
%            }{
%                c_2\,  N^{s/d}
%            } 
%             & \mbox{ if } d>2s \quad {\color{gray}{\text{ (\textit{initial phases})}}}\\
%            %%%%
%            \frac{
%                \log(
%                     c\, N
%                 )
%            }{
%                 c\, N^{1/2}
%            } 
%             & \mbox{ if } d=2s \quad  {\color{gray}{\text{ (\textit{critical phase})}}}\\
%             \frac{
%                \log(
%                     c\, N
%                 )^{d/( 2s + 1 )}
%            }{
%                 c\, N^{1/2}
%            } 
%             & \mbox{ if } 
%             % 1=
%             d<2s  \quad {\color{gray}{\text{ (\textit{eventual phases})}}}\\       %%%%
%         \end{cases}
% \end{equation}
% where $c\eqdef 1 - \kappa$, $c_2\eqdef c^{s/d}$, and $0< \kappa< 1$ are constants depending only on the data-generating Markov process. 

% \begin{theorem}[Pathwise Generalization Bounds for Transformers]
% \label{thrm:main}
% In Setting~\ref{setting}, there is a $\kappa\in(0,1)$, depending only on $X_{\cdot}$, and a $t_0\in \mathbb{N}_0$ such that: for each $t_0\le N \le t \le \infty$ and $\delta \in (0,1]$ the following holds with probability at-least $1-\delta$
% \begin{align*}
% \resizebox{1\linewidth}{!}{$
%         \underset{\mathcal{T}\in 
%             \transformerclass_{L,H,C}^{D,d,0}
%         }{\sup}
%         \,
%             \big|
%                 \mathcal{R}_{\max\{t,N\}}(\mathcal{T})-\mathcal{R}^{(N)}(\mathcal{T})
%             \big|
%     \lesssim
%         \overset{\infty}{\underset{{s=0}}{\sum}}
%         \,
%             I_{N\in [\tau_{s},\tau_{s+1})}
%             \,
%             % C^{\transformerclass}_{K}(s)
%             C_{\ell,\transformer,K,s}
%         \biggl(
%             %% Time-Shift Term
%                 % I_{t<\infty}\,
%                 \underbrace{
%                     \kappa^t
%                 }_{\term{time}}
%                 \,
%             %%% Mean Term
%                 +\,
%                 \underbrace{
%                     %%% 
%                     % Rate
%                     \operatorname{rate}_s(N)
%                 }_{\term{complexity}}
%             +
%                 %%% Concentration Term
%                 \underbrace{
%                     \frac{
%                         \sqrt{2\ln(1/\delta)}
%                     }{
%                         N^{1/2}
%                     }
%                 }_{\term{hprob}}
%     \biggr)
% $}
% \end{align*}
% where $\operatorname{rate}_s(N)$ is defined in~\eqref{eq:rate_function__definition}, and the constant $C_{\ell,\transformer,s,K}$ is Table~\ref{tab:constants} and the \textit{transition times} $(\tau_s)_{s=0}^{\infty}$ are given iteratively by $\tau_0\eqdef 0$ and for each $s\in \mathbb{N}_+$
% \begin{equation*}
% % \label{eq:phasetransitions}
% \resizebox{1\hsize}{!}{$
%     \tau_s
% \eqdef 
%     \inf\,
%     \biggl\{ 
%         t\ge \tau_{s-1}
%     :\,
%             % C^{\transformerclass}_{K}(s)
%             C_{\ell,\transformer,K,s}
%             ( \kappa^t + \operatorname{rate}_s(N)+
%             \frac{\sqrt{\log(1/\delta)}}{\sqrt{N}}
%             ) 
%         \le 
%             % C^{\transformerclass}_{K}(s-1)
%             C_{\ell,\transformer,K,s-1}
%             ( \kappa^t + \operatorname{rate}_{s-1}(N)+
%             \frac{\sqrt{\log(1/\delta)}}{\sqrt{N}}
%             )
%     \biggr\}
% .
% $}
% \end{equation*}
% Furthermore, $c\eqdef 1-\kappa$, $c_2\eqdef c^{s/d}$, $\kappa^{\infty}\eqdef \lim_{t\to \infty}\, \kappa^t= 0$, and $\lesssim$ hides an absolute constant.
% \end{theorem}




% \subsection{Discussion}

% Theorem~\ref{thrm:main} implies the order estimate in~\eqref{eq:FutureG}.  This is because $C_{\ell,\mathcal{T},K,s}$ is constant in $N$ and $\operatorname{rate}_s(N)<\operatorname{rate}_{s-1}(N)$; thus, for every $s>0$ the right-hand side our bound is eventually bounded by any $C_{\ell,\transformer,K,s}
%         (
%             %% Time-Shift Term
%                 % I_{t<\infty}\,
%                     \kappa^t
%                 \,
%             +
%                 %%% Concentration Term
%                         \sqrt{2\ln(1/\delta)}/N^{1/2}
%                 %%% Mean Term
%                 +\,
%                     %%% 
%                     % Rate
%                     \operatorname{rate}_s(N)
%     )$ for $N$ large enough. 
% However, unlike the order estimate~\eqref{eq:FutureG}, Theorem~\ref{thrm:main} provides an explicit description of the actual size of the future-generalization gap in terms of three factors which we now interpret.


% % \subsection{Breakdown of The Future Time Generalization Bound}
% \paragraph{Non-Stationarity Term:} \Cref{time} quantifies the rate at which the data-generating Markov process $X_{\cdot}$ becomes stationary.  This term only depends on the time $t$ and a constant $0<\kappa<1$ determined only by $X_{\cdot}$.  We use the notational convention $\kappa^{\infty}\eqdef \lim\limits_{t\to \infty}\,\kappa^t = 0$ to describe the limiting case.

% \vspace{-1em}
% \paragraph{Model Complexity Term (Phase Transitions):} 
% \begin{wrapfigure}{r}{0.35\textwidth}
%   \begin{center}
%     \includegraphics[width=1\linewidth]{figs/TransitionValues.pdf}
%   \end{center}
%   \caption{\textbf{Transition times:} (y-axis) when the future-generalization bound accelerates by a polylogarithmic factor (in $N$) for a single transformer block in terms of the input dimension $d$ (x axis).}
%   % , i.e. for every $s, d$ the smallest $N$, such that $C_{s-1}/N^{(s-1)/d} > C_s/N^{s/d}$
%   % }
% \end{wrapfigure}
% \Cref{complexity} captures the complexity of the transformer network in terms of the number of self-attention heads, depth, width, and the activation function used to define the class $\transformer_{L,W,H}^{D,d,0}$.  
% Each constant $C_1\le \dots \le C_s\le \dots$ collects the higher-order sensitivities ($s^{th}$ order partial derivatives; where $s\in \mathbb{N}_+$) of the transformer model.  Each $0=\tau_0\le \tau_1\le\dots \le \tau_s\le $ indicates the times at which there is a phase-transition in the convergence rate of the generalization bound accelerates.  Once $t\ge \tau_s$, then the convergence rate of~\Cref{complexity} accelerates, roughly speaking, by a reciprocal log-factor of $1/\log(N)$.  
% Observe that the rate function is asymptotically equal to the rate function from the central limit theorem, as $s$ tends to infinity; that is, $\lim\limits_{s\to \infty}\, \operatorname{rate}_s(N) = 1/(c\sqrt{N})$.  
% %%%%
% The rate~\eqref{eq:rate_function__definition} is the (optimal) rate at which the empirical measure generated by observations from a Markov process converges to its stationary distribution in $1$-Wasserstein distance~\cite{Kloeckner_2020CounterCurse_ESAIM,Riekert_ConcentrationOfMeasure2022}.  The polylogarithmic factor is removable if the data is i.i.d; in which the rate cannot be improved further~\cite{graf2007foundations,dereich2013constructive}.

% \paragraph{Probabilistic Validity Term:} \Cref{hprob} captures the cost of the bound being valid with probability at least $1-\delta$.  
% The convergence rate of this term cannot be improved due to the central limit theorem. It is responsible for the overall convergence rate of our generalization bound being ``stuck'' at the optimal rate of $\mathcal{O}(1/\sqrt{N})$ from the central limit theorem; as the other two terms converge exponentially to $0$.


% \paragraph{The Constant $C_{\ell,\transformer,K,s}$:} The constant $C_{\ell,\transformer,K,s}$, in Theorem~\ref{thrm:main__technicalversion}, encodes the maximal size of the first $s$ partial derivatives of any transformer in the class $\transformerclass$.  
% Thus, it encodes the complexity of the class $\transformerclass$ (e.g.\ int terms of number of attention heads, depth, width, etc...), the size of the compact set $K$, and the smoothness of the loss function and target functions. 

% We note that, any uniform generalization bound for smooth functions thus necessarily contains constants of the same order \textit{hidden within the big} $\mathcal{O}$.  See e.g. the entropy bound in~\citep[Theorem 2.71]{vaart2023empirical} which yields VC-dimension bounds via standard Dudley integral estimates in the i.i.d.\ case.  

% Critically, when the function class is defined by function composition, i.e.\ as in deep learning, then these maximal partial derivatives tend to grow factorially in $s$.  This is a feature of the derivatives of composite functions in high dimensions as characterized by the multi-variate chain rule (i.e.\ the Fa\'{a} di Bruno formula~\cite{faa1855sullo,ConstantineSavits96}).  The combinatorics of these partial derivatives is encoded by the coefficients in the well-studied bell-polynomials~\cite{bell1934exponential,mihoubi2008bell,wang2009general} whose growth rate has been recently understood in~\cite{KO2022} and contains factors of the order of $\mathcal{O}(
% \big( \frac{ 2 s}{e\ln s} ( 1 + o(1) ) \big)^s
% )$.  

% Remark that, in the feedforward case, i.e.\ when no layernorms or multihead attention are used, then the $s=1$ case is bounded above by the well-studied path-norms; see e.g.~\cite{bartlett2017spectrally,neyshabur2015norm}, which are simply the product of the weight matrices of in the network and serve as a simple upper-bound for the largest Lipschitz constant (i.e.\ $C^1$ norm) of the class $\transformerclass$.   These constants are included as very specific cases of our constant bounds; whose general expression is complicated and is relegated to the appendix in Theorems~\ref{thm:TransformerBlockSobolevBound} and~\ref{thm:DerivativeBoundByLevel}.  
% In the case of a single transformer block, the $C_{\ell,\transformer,K,s}$ is of the order of
%     \begin{align*}
%     % \label{eq:order_estimate_ModelComplexityConstant}
%     \resizebox{0.95\linewidth}{!}{$%% BEGIN RESIZE BOX$}
%         \mathcal{O}\Big(
%             \underbrace{
%                 c_{\ell,f^{\star}}
%                 \vphantom{\biggl(\biggr)^{s^4}}
%             }_{\text{Loss \& Target}}
%             \,
%             \underbrace{
%                 C^{\layernorm}_{K\tagA}({\cleq s})^s
%                 C^{\layernorm}_{K\tagC}({\cleq s})^{s^3}
%                 \vphantom{\biggl(\biggr)^{s^4}}
%             }_{\text{Layernorms}}
%             \underbrace{
%                 C^{\neuraln}_{K\tagB}({\cleq s})^{s^s}
%                 \vphantom{\biggl(\biggr)^{s^4}}
%             }_{\text{Perceptron}}
%             \,
%                 \underbrace{
%                     \biggl(
%                         1 + C^{\multihead}_K(\cleq s)
%                     \biggr)^{s^4}
%                     \vphantom{\biggl(\biggr)^{s^4}}
%                  }_{\text{Multihead Attention}}
%             \underbrace{
%                 % \odim^{s^2}\idim^{2 s^3}
%                 D^{s^2}\,d^{2s^3}
%                 \vphantom{\biggl(\biggr)^{s^4}}
%             }_{\text{dimensions}}
%             \,
%             \underbrace{
%                  C_s
%                  ^{s^s + s^3 + s^4}
%                  \vphantom{\biggl(\biggr)^{s^4}}
%             }_{\text{Generic: $s$-th order Derivative}}
%         \Big)
%     $}
%     \end{align*}
%     where the ``generic higher-order derivative constant'' is $C_s \eqdef\frac{ 2 s}{e\ln s} ( 1 + o(1) )$.  Order estimates on each of these terms are in Table~\ref{tab:constants}, precise analytical estimates are derived in Appendix~\ref{sec:RegularityTransfomerBuildingBlocks}, and numerical estimates are given in Appendix~\ref{s:dettables} (see also \Cref{fig:boundillustration}).  
%     % \del{The latter especially concretely shows the impact of the choice of activation function; e.g.\ transformers activated with soft plus or Swish have notably tighter bounds than those with $\tanh$.}
%      If no layer norms, SLP, or multi head attention mechanisms are included in the class, then their respective terms in our order estimate should be taken to be $1$.
% \begin{table}[ht!]%[H]
%     \centering
% 	\ra{1.3}
%     \caption{Bounds on the terms in defining the constant $C_{\ell,\transformer,K,s}$, in Theorem~\ref{thrm:main__technicalversion}, for a single attention block. }
% \begin{tabular}{@{}cl@{}}
% \cmidrule[0.3ex](){1-2}
% Term & Bound $(\mathcal{O})$
% \\    
% \midrule
% $c_{\ell,f^{\star}}$ & $
%             %%% Precise 
%             % s^{r_{\ell} + 2s^2} 
%             % \Big(\frac{ C_f \, 2D  }{e\ln s } \Big)^s 
%             C_f^s
%             \,
%             s^{r_{\ell} + 2s^2} 
%             C_s^s %(I grew it from  2D -> s but it looks cleaner and is easier to explain tbh)
%             $
% \\
% $\layernorm$
%  & 
%  $   
%     s^{(1+s)/2}
%     C_s^s
%     % \big(
%         %     \frac{
%         %         s^{5/2}
%         %     }{
%         %         e^{3/4}\ln(s)
%         %     }
%         % \,
%         % (
%         %     1 + o(1)
%         % )
%     % \big)^s
%  $
% \\ 
%  $\neuraln$ & {\footnotesize $
%                 \|B^{(1)}\|%_{\infty}
%             +
%                 \|B^{(2)}\|%_{\infty}
%                 \|A\|^s%_{\infty}^s
%                 \|\sigma\|_{s:
%                         \big[\pm \|a\|_{\infty}\pm\sqrt{\idim}\big]
%                     }
%                 \operatorname{Width}(\neuraln)
%                 \,
%                 \tilde{C}_s^s
%         $
%         }
% \\
%  $\multihead$  & 
%  % { \footnotesize $s! 
%  %        d_2 
%  %        C^{W}
%  %        d_0
%  %    (M + 1)
%  %    C^V
%  %    s!
%  %        (2 d_0 d_1 \Vert K \Vert C^{Q}C^{K})^{s}
%  %    \left(
%  %        \Vert K \Vert
%  %    +
%  %        s d_0M
%  %    \right)
%  %        % \Big[ \frac{ 2 sM}{e\ln s} ( 1 + o(1) ) \Big]^{s}
%  %        C_s^s
%  %    $}
% %\\
% % $\multihead$  & { \footnotesize $n! 
% %        d_2 
% %        C^{W}
% %        d_0
% %    (M + 1)
% %    C^V
% %    C^{\smax}_{\dotp[K]}(\cleq n)
% %        C^{\dotp}_K({\cleq n})^{n}
% %    \left(
% %        \Vert K \Vert
% %    +
% %        n d_0M
% %    \right)
% %        \Big[ \frac{ 2 nM}{e\ln n} ( 1 + o(1) ) \Big]^{n}
% %    $}
% %\\
% %$\smax$ & n!
% %\\
% %$\dotp$ & {\footnotesize $2 d_0 d_1 (1 \vee \Vert K \Vert ) C^{Q}C^{K}$}
% $
%     % M^2
%     \|W\|
%     \|V\|
%         (c_{d} \|Q\|\|K\|)^{s}
%     \,\,
%         \Big(
%             s^2
%              \big(\frac{s}{e}\big)^{2s}
%             C_s^s
%         \Big)
% $
% \\
% \bottomrule
% \end{tabular}
% \caption*{Here $C_s\eqdef \frac{ 2 s}{e\ln s} ( 1 + o(1) )$, $\tilde{C}_s\eqdef s^{1/2}\big(\frac{n}{e}\big)^sC_s^s$, $c_d\eqdef 2\max
% \{\idim, \kdim, \vdim, \ldim, \odim\}$, $\operatorname{Width}(\neuraln)$ is the width of the neural network $\neuraln$, where $\|\cdot\|$ denotes the componentwise max matrix/vector norm.}
% % }% END Resize box
% \label{tab:constants}
% \end{table}


% Figure~\ref{fig:boundillustration} illustrates the effect of various building blocks in the construction of a transformer (e.g.\ activation choice, multihead attention (MHA), layernorms) through their effect on the constants in our generalization bounds.  Consequentially, we show the effect on the phase-transition times $(\tau_t)_{t=0}^{\infty}$, defined in Theorem~\ref{thrm:main}, dictating when the bound accelerates by a polylogarithmic factor in $N$.

% \begin{figure*}[t!]%[b!]
%     \centering
%     \begin{subfigure}[t]{0.33\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figs/ActivationBounds.pdf}
%         %\caption{Lorem ipsum}
%     \end{subfigure}%
%     \hfill 
%     \begin{subfigure}[t]{0.33\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figs/BuildingBlocks.pdf}
%         %\caption{Lorem ipsum}
%     \end{subfigure}%
%     \hfill 
%     \begin{subfigure}[t]{0.33\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figs/TBlockComp.pdf}
%         %\caption{Lorem ipsum}
%     \end{subfigure}%
%     % \hfill 
%     % \begin{subfigure}[t]{0.33\textwidth}
%     %     \centering
%     %     \includegraphics[width=\textwidth]{figs/TransitionValues.pdf}
%     %     %\caption{Lorem ipsum}
%     % \end{subfigure}
%     \caption{{Effects of Transformer Components of~\ref{eq:FutureG}}: (left to right.) The first figure shows the $C^s$ bound of various activation functions according to results in \Cref{sec:Activation}. The second illustrates $C^s$ bounds for Multi-Head Attention (\Cref{defn:MultiHead}), single-layer perceptrons, and the layer norm. 
%     The third shows the $C^s$-bound of a transformer block (\Cref{defn:TransformerBlock}), distinguishing if the bound was computed level-specific (\Cref{cor:DerivativeBoundByLevel}) or type specific (\Cref{thm:DerivativeBoundByType}).
%     The parameters used for the above plots are the base cases of \Cref{tab:Activations,tab:NeuralNet,tab:LayerNorm,tab:TBlock,tab:MultiHead}.
%     }
%     \label{fig:boundillustration}
% \end{figure*}

% % \begin{table}[H]%[ht!]%
% %     \centering
% % 	\ra{1.3}
% %     \caption{Non-asymptotic bounds on $\operatorname{rate}_s(N)$, which encodes the \textit{cost} of accelerating the convergence rate of term~\eqref{complexity} by leveraging the information on the higher-order $(s)$ derivatives of the transformer into the generalization bound in Theorem~\ref{thrm:main}.
% %     }
% %         % \resizebox{\columnwidth}{!}{%
% %     		\begin{tabular}{@{}ll@{}}
% %     			\cmidrule[0.3ex](){1-2}
% %     			\textbf{Dimension ($d$) vs.\ Derivative ($s$)} & $\operatorname{rate}_s(N)$ 
% %     			\\    
% %     			\midrule
% %     		(Fast) $s>d/2$
% %     		    & 
% %     		      $\frac{
% %                        \log\big(
% %                             c\, N
% %                         \big)^{d/(2s + 1)}
% %                     }{
% %                         c\, N^{1/2}
% %                     }
% %                 $
% %     		\\
% %             (Critical) $s=d/2$
% %     			& 
% %                 $\frac{
% %                        \log\big(
% %                             c\, N
% %                         \big)
% %                    }{
% %                         c\, N^{1/2}
% %                    } $
% %     		\\
% %             (Slow) $s<d/2$ & 
% %             $
% %                     \frac{
% %                        \log\big(
% %                             c\, N
% %                         \big)^{d-2s+(s/d)}
% %                    }{
% %                        c_2\,  N^{s/d}
% %                    } 
% %                 $ \\
% %     			\bottomrule
% %     		\end{tabular}
% %     		% }% END Resize box
% %         \label{tab:rates}
% % \end{table}



% % Our main result is formulated in the case where the transformer networks generate predictions using the previous time-series input and not the past $1+M$ steps, i.e.\ $M=0$.  One can, of course, increase the state space of the Markov process from $d$ to $Md$ dimensions by including the past $1+d$ steps of the input time series to obtain the general case. 



% \subsection{Explanation of Proof}
% \label{s:Discssion__ss:Overview_Proof}

% The first step in deriving our generalization bounds is to quantify the regularity of the transformer model as a function of its depth, number of attention heads, and norm of its weight matrices.  
% By \textit{regularity}, we mean the number and size of the continuous partial derivatives admitted by the transformer. To quantify the size of the partial derivatives of the transformer we first remark that it is \textit{smooth}; that is, it admits continuous partial derivatives of all orders (see Theorem~\ref{prop:TransformerIsSmooth}).

% We will uniformly bound the generalization capabilities of the class of transformers $\mathcal{T}\in \transformerclass_{L,W,H}^{D,d,0}$ by instead uniformly bounding the generalization of any $C^s$ functions on $\mathbb{R}^d$ with $C^s$-norm at most equal to the largest $C^s$-norm in the class $\transformerclass_{L,W,H}^{D,d,0}$.  That is, we control the right-hand side of
% \begin{equation}
% \label{eq:risk_bound__decomposition}
% %\smash{
%         {
%        \textstyle 
%        \sup_{\mathcal{T}\in \transformerclass_{L,W,H}^{D,d,M}}\,
%         \,
%         \big|
%             \mathcal{R}_t(\mathcal{T})-\mathcal{R}^{(N)}(\mathcal{T})
%         \big|
%     \le 
%         % \inf_{s\in \N_+}
%         % \,
%             % \underbrace{
%         \sup_{\hat{f}\in \mathcal{C}^s_R(\mathbb{R}^d)}
%         \,
%         \big|
%             \mathcal{R}_t(\hat{f})-\mathcal{R}^{(N)}(\hat{f})
%         \big|
%             % }_{\mbox{Term to Bound}}
%             }
% %}
% \end{equation}
% where {$R\eqdef \sup_{\mathcal{T} \in \transformerclass_{L,W,H}^{D,d,M}} \,
% \|
%     \ell(\mathcal{T},f^{\star})
% \|_{C^s}
% $} describes the higher-order fluctuations of the ``difference'' between the target function $f^{\star}$ and any transformer in $\smash{\transformerclass_{L,H,W,C}^{D,d,0}}$, as quantified by the loss function $\ell$.  
% % 
% Our first step is thus to bound $R$ by upper-bounding maximal size of the $s^{th}$ partial derivatives of all transformers in $\smash{\transformerclass_{L,W,H}^{D,d,M}}$.  Explicit bounds are computed in Theorem~\ref{thm:TransformerBlockSobolevBound}, and their order estimates (as a function of $s$) are given in Theorem~\ref{thm:TransformerBlockSobolevBoundLevel}.  
% Combing these estimates with the maximal $s^{th}$ partial derivatives of the loss and target function, via a Fa\'{a} di Bruno-type formula (in Theorem~\ref{lem:mdFDBestimate} or Lemma~\ref{thm:DerivativeBoundByLevel}), which is a multivariant higher-order chain rule, yields our estimate for $R$ in~\eqref{eq:risk_bound__decomposition}.

% % \begin{theorem}[$C^s$-Norm Bound of Transformers]
% % \label{prop:transformerSobolevBound}
% %     % Fix $n \in \N_+$. 
% %     Fix $n,L,H,C,D,d,M \in \N_+$. 
% %     % In the notation of \Cref{defn:Transformer} and the multivariate notation established in \Cref{not:Multivariate,not:Order,not:DerivativeBounds} let 
% %     For any $\transformer \in \transformerclass_{L,H,C}^{D,d,M}$, 
% %     any compact $K_0 \subset \R^{M \times D}$, and any $\alpha \in \N^{M \times D}$, $\vert \alpha \vert \eqdef n$ we have
% %     \begin{align}\label{id:TransformerSobolevBound1}
% %         C^{\transformer}_{K_{0}}(\alpha)
% %         &\leq
% %         \odim^LM\alpha!
% %         \cdot
% %         C^A 
% %         \cdot
% %         C^L(\alpha),
% %     \end{align}
% %     where $C^{1}(\alpha) \eqdef C^{\tblock_1}_{K_{0}}(\alpha)$ and for $l \in \myset{2}{L}$, 
% %     \begin{align}\label{id:TransformerSobolevBound2}
% %         C^{l}(\alpha) \eqdef 
% %         &\leq
% %         \alpha! \sum_{\beta \in \Order^{\Tilde{d}_l}_{\leq n}}  N(\beta)C^{\tblock_l}_{K_{l-1}}(\beta)
% %         \sum_{\eta, \zeta \in \calP'(\order(\alpha),\beta)} 
% %         \prod_{j=1}^{n} \frac{
% %             C^l(\order(\zeta^{(j)}))^{\vert \eta^{(j)} \vert}
% %         }{
% %             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
% %         }
% %     \end{align}
% %     where $K_l \eqdef \tblock_l[K_{l-1}]$,  $\Tilde{d}_{l} \eqdef (1+M_{l})\idim^{l}$, and a bound for $C^{\tblock_l}_{K_{l-1}}(\beta)$ is given by \Cref{thm:TransformerBlockSobolevBound}, only depending on the transformer block class $\tblockclass_{d^l, M^l, H^l, C^l}$.
% % \end{theorem}
% % \paragraph{Step 2 - Generalization Bounds for $(s,R)$-Smooth Functions}
% % For any $s,R>0$, we use $\mathcal{C}^s_R(\mathbb{R}^d)$ to denote the closed ball of a given radius $R>0$ about the zero function in $C^s(\mathbb{R}^d)$.  
% Now that we have bounded $R$, appearing in the supremum term in~\eqref{eq:risk_bound__decomposition}, it remains to translate this into a generalization bound.  We can do this by relating it to the so-called \textit{smooth Wasserstein distance} $d_s$
% % , which is a type of integral probability metric, 
% between the distribution of the Markov chain at time $\mu_t$ and its empirical distribution $\smash{\mu^{(N)}\eqdef 1/{N}\sum_{n=1}^N\, \delta_{X_n}}$ obtained by collecting samples up to time $N$.  The \textit{smooth Wasserstein distance} $d_s$, studied by \cite{Kloeckner_2020CounterCurse_ESAIM,Riekert_ConcentrationOfMeasure2022,hou2022instance}, is the integral probability metric (IPM)-type distance quantifying the distance between any two Borel probability measures $\mu,\nu$ on $\R^d$ as the maximal distance which they can produced when tested on any function in $C^s_1(\R^d)$; that is
% \begin{align*}
% % \smash{
%     d_s(\mu,\nu) 
%     \eqdef 
%         \sup_{g\in \mathcal{C}^s_1(\mathbb{R}^d)}\, 
%         % \mu[g]-\nu[g]
%         \mathbb{E}_{X\sim \mu}[g(X)]
%         -
%         \mathbb{E}_{Y\sim \nu}[g(Y)]
% .
% % }
% \end{align*}
% % \begin{remark}
% % When $s=1$, $d_s$ is simply the $1$-Wasserstein distance used in adversarial learning \citep{arjovsky2017wasserstein}.  This can be seen from the Kantorovich-Rubinstein duality, see \citep[Theorem 5.10 and Equation (5.11)]{VillaniBook_2009}, as well as the characterization of $1$-Lipschitz functions as Lebesgue almost-everywhere once continuously differentiable functions by the Rademacher-Stephanov Theorem, see \citep[Theorems 3.1.6-3.1.9]{Federer_GeometricMeasureTheoryBook_1969}.  
% % \end{remark}
% The right-hand side (RHS) of~\eqref{eq:risk_bound__decomposition} can be expressed as $R$ times the $d_s$ distance between the (true) distribution $\mu_t$ of the process $X_{\cdot}$ at time $t$ and the (empirical) distribution $\mu^{(N)}$ collected from samples
% \begin{equation}
% \label{eq:risk_bound__decomposition2}
% % \smash{
%         % \sup_{\hat{f}\in \mathcal{C}^s_R(\mathbb{R}^d)}
%         % \,
%         % \big|
%         %     \mathcal{R}_t(\hat{f})-\mathcal{R}^{(N)}(\hat{f})
%         % \big|
%         \mbox{RHS}\, 
%         \eqref{eq:risk_bound__decomposition}
%     % =
%         % \sup_{\hat{f}\in \mathcal{C}^s_R(\mathbb{R}^d)}
%         % \,
%         %         \mathbb{E}_{X\sim \mu_t}[\ell(\hat{f}(X_t),f^{\star}(X))]
%         %         -
%         %         \mathbb{E}_{Y\sim \mu^{(N)}}[\ell(\hat{f}(X_t),f^{\star}(X))]
%     \le 
%         % \Biggl(
%         \sup_{\hat{f}\in C^s_R(\mathbb{R}^d)}\,\|\ell(\hat{f},f^{\star})\|_{C^s}
%         % \Biggr)
%         \,
%         d_s(\mu_t,\mu^{(N)})
% .
% % }
% \end{equation}
% The $d_s$ distance between the process $X_{\cdot}$ at time $t$, i.e.~$\mu_t$, and the running empirical distribution $\mu^{(N)}$ can be accomplished in two steps.  First, we \textit{fast-forward time} and bound the $d_s$-distance between $\mu^{(N)}$ and the \textit{stationary distribution} $\mu_{\infty}$ of the data-generating Markov chain $X_{\cdot}$ (at time $t=\infty$).  We then \textit{rewind time} and bound the $d_s$-distance between the stationary distribution $\mu_{\infty}$ and the distribution $\mu_t$ of the Markov process up to time $t$; by setting up the i.i.d.\ concentration of measure results of~\cite{kloeckner2019effective,Riekert_ConcentrationOfMeasure2022}.  This last step is possible since our assumptions on $X_{\cdot}$ essentially guarantee that it has a finite (approximate) mixing time.


% \vspace{-1em}
% \section{Conclusion}\label{s:Conclusion}
% We provided a theoretical foundation for the \textit{future-generalization} of transformer trained on a single perturbed realization of a time-series trajectory (Theorem~\ref{thrm:main}).  Our results thus help provide insight on the reliability of LLMs outside the i.i.d.\ framework and their principled use in time-series analysis.  

% We obtain explicit estimates on the constants in these generalization bounds which relied on \textit{explicitly} bounding all the higher-order derivatives of transformers; in terms of their number of attention heads, activation functions, depth, width, and weights constraints (Theorems~\ref{thm:TransformerBlockSobolevBound} and~\ref{thm:TransformerBlockSobolevBoundLevel}).  These bounds can equally be used in conjunction with classical tools, e.g.\ Rademacher or VC-type bounds in the i.i.d.\ setting, or other applications where one needs to understand the higher-order sensitivities of transformers to their inputs.  


% % \begin{comment}
% \vspace{-1em}
% \section{Limitations and Future Work}
% \label{s:Conclusion__ss:FutureWork}
% Several dynamical systems and financial markets have long-term memory and thus are non-Markovian.  In future work, it would be interesting to extend our results to cover such settings as well.  
% % It would be interesting to relax Assumption~\ref{ass:Comp_Support} to only hold with high probability.  Doing so would then automatically include any Gaussian process and even non-Markovian stochastic differential equations, see~\citep[Proposition 4.2]{Acciaio2022_GHT}, where the drift and diffusion can depend on its entire path.

% % \section*{Broader Impact}
% % \label{s:BroaderImpact}
% % Though we focused on using our main result applied to \textit{future} times $t\ge N$ used for forecasting/predicting, it can equally be applied to validate time-series models on historical time-series data, i.e.\ when $t<N$.   The latter has the potential to be a viable means to validating/\textit{backtesting} deep learning-based time series models used by large-scale financial institutions, e.g.\ and serve the basis for future regulation by international financial regulators \cite{king2011basel} on deep learning models; of where current regulation is lacking.  In this way, our results are not only purely theoretical but can be used to positively guide educated decisions on which deep learning models can cause institutional instability/financial crises when deployed by large financial actors, e.g.\ backs or large investment funds. 

% % \end{comment}

% % \clearpage \newpage
% % \if@neuripsfinal
% %     \paragraph{Acknowledgements} 
%     % AK acknowledges financial support from an NSERC Discovery Grant No.\ RGPIN-2023-04482 and their McMaster Startup Funds. RS is supported by Canada NSERC CGS-D Doctoral Grant. 
%     % RS and AK acknowledge that resources used in preparing this research were provided, in part, by the Province of Ontario, the Government of Canada through CIFAR, and companies sponsoring the Vector Institute \href{https://vectorinstitute.ai/partnerships/current-partners/}{https://vectorinstitute.ai/partnerships/current-partners/}.
% % \fi




% \bibliographystyle{plain}
% \bibliography{refs/main,
%                 refs/qfin-datasets, 
%                 refs/qfin-pm,
%                 refs/kalman-filters,
%                 refs/rebutal}           




% \newpage
% \appendix
% %\addcontentsline{toc}{section}{Appendix} % Add the appendix text to the document TOC
% %\part{Appendix} % Start the appendix part
% %\parttoc

% \DoToC



% \section{Notation}
% \label{a:Notation}

% \begin{notation}[Multi-index Notation]\label{not:Multivariate}
% We will fix the following multivariate notation.
% \begin{itemize}[nosep]
%     \item Multi-indices $\alpha \eqdef (\alpha_1, \ldots, \alpha_k) \in \N^k, k \in \N$ are denoted by Greek letters.
%     \item The sum of entries is given by $\vert \alpha \vert \eqdef \sum_{i=1}^k \alpha_k$.
%     \item Its faculty is defined by $\alpha!  \eqdef \prod_{i=1}^k \alpha_k!$,
%     \item We denote the derivative w.r.t. $\alpha$ by $D^\alpha \eqdef \partial^{\vert \alpha \vert} / \partial x_1^{\alpha_1} \cdots \partial x_k^{\alpha_k}$ if $\vert \alpha \vert > 0$ else $D^\alpha$ is the identity operator.
%     \item For a vector $x \in \R^k$, we write $x^\alpha \eqdef \prod_{i=1}^k x_k^{\alpha_k}$.
%     \item We define the relation $\alpha \prec \beta$ for $\beta \in \N^k$ if one of the three following holds 
%     \begin{enumerate}[label=(\roman*), nosep]
%         \item $\vert \alpha \vert < \vert \beta \vert$;
%         \item $\vert \alpha \vert = \vert \beta \vert$, and $\alpha_1 < \beta_1$; or 
%         \item $\vert \alpha \vert = \vert \beta \vert$, and $\alpha_i = \beta_i$ for $i \in \myset{1}{j-1}$ and $\alpha_j < \beta_j$ for $j \in \myset{2}{k}$.
%     \end{enumerate}
%     \item Unit vectors $e_i \in \{0,1\}^k$ are defined by $(e_i)_j = 0$ for $i \neq j$ and  $(e_i)_i = 1$.
% \end{itemize}
% \end{notation}
% For any $s>0$, the norm $\|\cdot\|_{C^s}$ of a smooth function $f:\R^d\to \R$ is defined by
% \begin{align*}
%     \|f\|_{C^s}
% \eqdef 
%         \max_{k=1,\dots,s-1}\,
%         \max_{\alpha\in \{1,\dots,d\}^d}
%         \,
%             \Big\|
%                 \frac{\partial^k f}{
%                     \partial x_{\alpha_1}\dots\partial x_{\alpha_k}
%                 }
%             \Big\|_{\infty}
%     +
%         \max_{\alpha \in \{1,\dots,d\}^{s-1}}\,
%             \operatorname{Lip}\big(
%                 \frac{\partial^{s-1}f}{\partial x_{\alpha_1}\dots\partial x_{\alpha_{s-1}}}
%             \big)
% \end{align*}
% We use the following notation to streamline the analytic challenges the tacking of $C^s$-norms.
% \begin{notation}[Order operator for multi-indeces]\label{not:Order}
% Define the order operator $\order$ for multi-indeces by
% \begin{align*}
%     \order: \N^k \longrightarrow \N^k, \quad \alpha_1, \ldots, \alpha_k \longmapsto \alpha_{\tau_\alpha(1)}, \ldots, \alpha_{\tau_\alpha(k)},
% \end{align*}
% where $\tau_\alpha: \myset{1}{k} \to \myset{1}{k}$ s.t. $\alpha_{\tau_\alpha(1)} \geq  \ldots \geq  \alpha_{\tau_\alpha(k)}$.  We write $\alpha \eqorder \beta$ if $\order(\alpha) = \order(\beta)$ for $\alpha, \beta \in \N^k$. Further, denote by $\Order^k_{n}$ the set $\{\order(\alpha) :  \alpha \in \N^k, \vert \alpha \vert = n \}$ and write $\Order^k_{\leq n} \eqdef \{\order(\alpha) :  \alpha \in \N^k, \vert \alpha \vert \leq n \}$. Eventually, define $N(\alpha) \eqdef \# \vert \{ \alpha' \in \N^k : \order(\alpha') = \alpha \} \vert$. 
% \end{notation}

% We will use the following notation to tabulate the sizes of a $C^s$-norm.
% \begin{notation}[Derivatives]\label{not:DerivativeBounds} Let $k \in \N$, $K \in \R^k$ be a set, $f: K \to \R^m$ a function and $\alpha\in\Order^k_n$ an ordered multi-index. Then,
% \begin{itemize}[nosep]
%     \item the uniform bound of $\alpha$-like derivatives on $K$ is given by 
%     \begin{align*}
%         C^f_K(\alpha) \eqdef \max_{i \in \myset{1}{m}} \max_{\gamma \sim \alpha} \Vert D^\gamma f_i \Vert_K,
%     \end{align*}
%     \item we define the bound at / up to derivative level $n$ by
%     \begin{align*}
%         C^f_K(n) \eqdef \max_{\alpha \in \Order^k_{n}} C^f_K(\alpha), \quad\quad 
%         C^f_K(\cleq n) \eqdef \max_{\alpha \in \Order^k_{\cleq n}} C^f_K(\alpha),
%     \end{align*}
%     \item we write $\Vert K \Vert \eqdef \sup_{x \in K} \Vert x \Vert$, and 
%     \item for a matrix $A \in \R^{n\times m}$ we write $C^A \eqdef \max_{i \in \myset{1}{n}, j \in \myset{1}{m}} \vert A_{i,j}\vert$.
% \end{itemize}
% \end{notation}
% When segmenting, truncating, or manipulating time series we will using the following notation.
% \begin{notation}[Time Series Notation]
% The following notation is when indexing paths of any time series.
% \begin{itemize}[nosep]
%     \item \emph{Realized Path up to time $t$} is denoted by $x_{\le t}\eqdef (x_s)_{s\in \mathbb{Z},\,s\le t}$.
%     \item \emph{Segment of a Path} Given a sequence $x\in \mathbb{R}^{\mathbb{Z}}$ and integers $s\le t$, we denote $x_{[s:t]}\eqdef (x_i)_{i=s}^t$.
%     % \item \emph{Temporal Re-centering Operator}. Set $\tau_t:\,{\mathbb{R}^{d}}^{\mathbb{Z}}\to {\mathbb{R}^{d}}^{\mathbb{N}}$, for all $x_{\cdot}\in {\mathbb{R}^{d}}^{\mathbb{Z}}$ and $s\in \mathbb{Z}$ with $\tau_t(x_{\cdot})_s\eqdef x_{s-t}$.
%     % \item \emph{Extension Operator}. Define $E_M:{\mathbb{R}^{d}}^{\mathbb{M}}\to{\mathbb{R}^{d}}^{\mathbb{Z}}$, for all $x_{\cdot}\in {\mathbb{R}^{d}}^{M}$ and $s\in \mathbb{N}$ via $E_M(x_{\cdot})_s\eqdef x_{s}I_{M\le s\le 0}$.
%     % \item \emph{Restriction Operator}. Fix $R_M:{\mathbb{R}^{d}}^{\mathbb{Z}}\to {\mathbb{R}^{d}}^{\mathbb{M}}$, for all $x_{\cdot}\in {\mathbb{R}^{d}}^{\mathbb{Z}}$ and $s\in \mathbb{N}$ by $R_M(x_{\cdot})\eqdef (x_s)_{-M<s\le 0}$.
% \end{itemize}
% \end{notation}
% Lastly, we recorded some additional notations that were required throughout our manuscript.
% \begin{notation}[Miscellaneous]
% The following notation is when indexing paths of any time series.
% \begin{itemize}[nosep]
%     \item \emph{$N$-Simplex}. For $N \in \N$ we write $\Delta_N\eqdef \{u\in [0,1]^N:\,\sum_{i=1}^N\,u_i=1\}$.
%     \item \emph{Infinite powers}: For $c\in (0,1)$, we define $c^{\infty}\eqdef \lim\limits_{t\to \infty}\, c^t = 0$.
% \end{itemize}
% \end{notation}

% \section{Elucidation of Constants in Theorem~\ref{thrm:main}}
% \label{s:dettables}
% The aim of this section is to elucidate the magnitude of the constants appearing in Theorem~\ref{thrm:main}.  We aim of to make each of these concrete by numerically estimating them, which we report in a series of tables.  Importantly, we see how subtle choices of the activation function used to define the transformer model can have dramatic consequences on the size of these constants, which could otherwise be hidden in big $\mathcal{O}$ notation.\footnote{The source code to compute derivative bounds is available at \url{https://anonymous.4open.science/r/transfomer-bounds-B476}.} 

% Interestingly, in \Cref{tab:Activations,tab:NeuralNet}, we see that the $\operatorname{softplus}$ activation function produces significantly tighter bounds than the $\tanh$ activation function through much smaller constants, and the $\operatorname{GeLU}$ and $\operatorname{SWISH}$ activation functions are a relatively comparable second-place.

% The bounds depicted in \Cref{tab:NeuralNet} exhibits a notable trait of independence from both input dimension and the compactum they are defined on.  Notably, the selection of latent dimensionality demonstrates a relatively minor influence in contrast to the pronounced impact of parameter bounds. This suggests that while adjusting the latent dimension may have some effect, the primary driver of the derivative bound lies within the constraints imposed on the parameters. Despite the seemingly conservative nature of the chosen parameter-bounds, it is important to acknowledge their alignment with the parameter ranges observed in trained transformer-models. 

% Note that the latter can be observed as well for Multi-Head attention (\Cref{tab:MultiHead}), however, we see that here the input dimension (composed of $\idim$ and $M$) is of greater importance with respect to the derivative bound. 

% \begin{table}[H]%[bp]%[ht!]%
%     \centering
% 	\ra{1.3}
%     \caption{$C^s$-bounds of activation functions based on numerical maximization of analytic derivatives in \Cref{sec:Activation}.}
%         % \resizebox{\columnwidth}{!}{%
%         \small
% \begin{tabular}{rrrrr}
% \toprule
% Bound & $\operatorname{softplus}$ & $\operatorname{GeLU}$ & $\tanh$ & $\operatorname{Swish}$
% \\    
% \midrule 
% $C^{1}$ & \texttt{\footnotesize  0.25} & \texttt{\footnotesize    1.12} & \texttt{\footnotesize        4.00} & \texttt{\footnotesize 1.10}  \\
% $C^{2}$ & \texttt{\footnotesize  0.10} & \texttt{\footnotesize    0.48} & \texttt{\footnotesize        8.00} & \texttt{\footnotesize 0.50}  \\
% $C^{3}$ & \texttt{\footnotesize  0.12} & \texttt{\footnotesize    0.75} & \texttt{\footnotesize       16.00} & \texttt{\footnotesize 0.31}  \\
% $C^{4}$ & \texttt{\footnotesize  0.13} & \texttt{\footnotesize    1.66} & \texttt{\footnotesize       32.00} & \texttt{\footnotesize 0.50}  \\
% $C^{5}$ & \texttt{\footnotesize  0.25} & \texttt{\footnotesize    4.34} & \texttt{\footnotesize      156.65} & \texttt{\footnotesize 0.66}  \\
% $C^{6}$ & \texttt{\footnotesize  0.41} & \texttt{\footnotesize   12.95} & \texttt{\footnotesize     1651.32} & \texttt{\footnotesize 1.50}  \\
% $C^{7}$ & \texttt{\footnotesize  1.06} & \texttt{\footnotesize   42.77} & \texttt{\footnotesize    20405.43} & \texttt{\footnotesize 2.91}  \\
% $C^{8}$ & \texttt{\footnotesize  2.39} & \texttt{\footnotesize  153.76} & \texttt{\footnotesize   292561.95} & \texttt{\footnotesize 8.50}  \\
% $C^{9}$ & \texttt{\footnotesize  7.75} & \texttt{\footnotesize  594.17} & \texttt{\footnotesize  4769038.09} & \texttt{\footnotesize21.76}  \\
% $C^{10}$& \texttt{\footnotesize 22.25} & \texttt{\footnotesize 2445.69} & \texttt{\footnotesize 87148321.71} & \texttt{\footnotesize77.50}  \\
% \bottomrule
% \end{tabular} 
% % }% END Resize box
% \label{tab:Activations}
% \end{table}

% The bound of the layer-norm (see \Cref{tab:LayerNorm}) seems to be particularly effected by the domain it is defined on, which can be problematic if it appears in later layers. An immediate solution is the usage of its parameter $\gamma$, a more drastic approach would be applications in combination with an upstream sigmoid activation.

% Eventually, as also shown in \Cref{fig:boundillustration}, we included in \Cref{tab:MultiHead,tab:TBlock} a comparison of using type-specific bounds (see \Cref{thm:DerivativeBoundByType}) or level-specific bounds (\Cref{thm:DerivativeBoundByLevel}) in the computation of the constants. This effect seems to become more evident with higher number of function compositions.


% %\afterpage{\clearpage  }

% % \begin{table}[p]
% % \small
% % \centering
% % \caption{Derivative type-specific bounds of Neural Networks based on their activation function, according to \Cref{lem:FeedForward}. We used $\idim = 10$, $\ldim = 64$, $C^{A}, C^{B^{(1)}}, C^{B^{(2)}} = 1$.}
% % \begin{tabular}{lcccc}
% % \toprule
% % Derivative Type & softplus & tanh & GeLU & SWISH \\
% % \midrule
% % (1, 0, ...) & \texttt{\footnotesize17.00} & \texttt{\footnotesize129.00} & \texttt{\footnotesize73.25} & \texttt{\footnotesize71.39} \\
% % (1, 1, 0, ...) & \texttt{\footnotesize22.16} & \texttt{\footnotesize384.00} & \texttt{\footnotesize103.22} & \texttt{\footnotesize102.39} \\
% % (2, 0, ...) & \texttt{\footnotesize50.47} & \texttt{\footnotesize1.02E+03} & \texttt{\footnotesize237.41} & \texttt{\footnotesize236.78} \\
% % (1, 1, 1, 0, ...) & \texttt{\footnotesize30.16} & \texttt{\footnotesize896.00} & \texttt{\footnotesize151.46} & \texttt{\footnotesize122.11} \\
% % (2, 1, 0, ...) & \texttt{\footnotesize76.31} & \texttt{\footnotesize2.82E+03} & \texttt{\footnotesize399.40} & \texttt{\footnotesize283.67} \\
% % (3, 0, ...) & \texttt{\footnotesize236.94} & \texttt{\footnotesize8.96E+03} & \texttt{\footnotesize1.25E+03} & \texttt{\footnotesize870.75} \\
% % (1, 1, 1, 1, 0, ...) & \texttt{\footnotesize38.33} & \texttt{\footnotesize1.92E+03} & \texttt{\footnotesize257.73} & \texttt{\footnotesize154.11} \\
% % (2, 1, 1, 0, ...) & \texttt{\footnotesize125.68} & \texttt{\footnotesize9.98E+03} & \texttt{\footnotesize1.15E+03} & \texttt{\footnotesize500.23} \\
% % (2, 2, 0, ...) & \texttt{\footnotesize267.71} & \texttt{\footnotesize2.20E+04} & \texttt{\footnotesize2.52E+03} & \texttt{\footnotesize1.06E+03} \\
% % (3, 1, 0, ...) & \texttt{\footnotesize393.39} & \texttt{\footnotesize3.20E+04} & \texttt{\footnotesize3.67E+03} & \texttt{\footnotesize1.56E+03} \\
% % (4, 0, ...) & \texttt{\footnotesize1.34E+03} & \texttt{\footnotesize9.83E+04} & \texttt{\footnotesize1.16E+04} & \texttt{\footnotesize5.33E+03} \\
% % (1, 1, 1, 1, 1, 0, ...) & \texttt{\footnotesize54.32} & \texttt{\footnotesize3.97E+03} & \texttt{\footnotesize535.68} & \texttt{\footnotesize196.23} \\
% % (2, 1, 1, 1, 0, ...) & \texttt{\footnotesize492.57} & \texttt{\footnotesize5.71E+04} & \texttt{\footnotesize7.74E+03} & \texttt{\footnotesize1.40E+03} \\
% % (2, 2, 1, 0, ...) & \texttt{\footnotesize1.08E+03} & \texttt{\footnotesize1.26E+05} & \texttt{\footnotesize1.72E+04} & \texttt{\footnotesize3.06E+03} \\
% % (3, 1, 1, 0, ...) & \texttt{\footnotesize1.57E+03} & \texttt{\footnotesize1.84E+05} & \texttt{\footnotesize2.49E+04} & \texttt{\footnotesize4.46E+03} \\
% % (3, 2, 0, ...) & \texttt{\footnotesize2.60E+03} & \texttt{\footnotesize2.97E+05} & \texttt{\footnotesize4.03E+04} & \texttt{\footnotesize7.49E+03} \\
% % (4, 1, 0, ...) & \texttt{\footnotesize4.31E+03} & \texttt{\footnotesize4.80E+05} & \texttt{\footnotesize6.51E+04} & \texttt{\footnotesize1.26E+04} \\
% % (5, 0, ...) & \texttt{\footnotesize1.33E+04} & \texttt{\footnotesize1.34E+06} & \texttt{\footnotesize1.81E+05} & \texttt{\footnotesize4.13E+04} \\
% % (1, 1, 1, 1, 1, 1, 0, ...) & \texttt{\footnotesize80.46} & \texttt{\footnotesize1.40E+04} & \texttt{\footnotesize1.36E+03} & \texttt{\footnotesize292.23} \\
% % (2, 1, 1, 1, 1, 0, ...) & \texttt{\footnotesize3.30E+03} & \texttt{\footnotesize1.23E+06} & \texttt{\footnotesize1.02E+05} & \texttt{\footnotesize1.21E+04} \\
% % (2, 2, 1, 1, 0, ...) & \texttt{\footnotesize7.22E+03} & \texttt{\footnotesize2.70E+06} & \texttt{\footnotesize2.24E+05} & \texttt{\footnotesize2.65E+04} \\
% % (2, 2, 2, 0, ...) & \texttt{\footnotesize1.21E+04} & \texttt{\footnotesize4.50E+06} & \texttt{\footnotesize3.74E+05} & \texttt{\footnotesize4.44E+04} \\
% % (3, 1, 1, 1, 0, ...) & \texttt{\footnotesize1.05E+04} & \texttt{\footnotesize3.93E+06} & \texttt{\footnotesize3.26E+05} & \texttt{\footnotesize3.86E+04} \\
% % (3, 2, 1, 0, ...) & \texttt{\footnotesize1.62E+04} & \texttt{\footnotesize6.00E+06} & \texttt{\footnotesize4.99E+05} & \texttt{\footnotesize5.94E+04} \\
% % (3, 3, 0, ...) & \texttt{\footnotesize2.96E+04} & \texttt{\footnotesize1.07E+07} & \texttt{\footnotesize8.96E+05} & \texttt{\footnotesize1.09E+05} \\
% % (4, 1, 1, 0, ...) & \texttt{\footnotesize2.53E+04} & \texttt{\footnotesize9.30E+06} & \texttt{\footnotesize7.74E+05} & \texttt{\footnotesize9.28E+04} \\
% % (4, 2, 0, ...) & \texttt{\footnotesize3.53E+04} & \texttt{\footnotesize1.27E+07} & \texttt{\footnotesize1.06E+06} & \texttt{\footnotesize1.29E+05} \\
% % (5, 1, 0, ...) & \texttt{\footnotesize5.91E+04} & \texttt{\footnotesize2.06E+07} & \texttt{\footnotesize1.73E+06} & \texttt{\footnotesize2.17E+05} \\
% % (6, 0, ...) & \texttt{\footnotesize1.61E+05} & \texttt{\footnotesize4.98E+07} & \texttt{\footnotesize4.27E+06} & \texttt{\footnotesize5.91E+05} \\
% % \bottomrule
% % \end{tabular}
% % \label{tab:NeuralNet}
% % \end{table}

% \begin{table}[H]%[p]
% \centering
% \small
% \caption{Derivative Bounds of the Perceptron Layer by derivative level according to \Cref{lem:FeedForward}.}
% \label{tab:NeuralNet}
% \begin{tabular}{ccc|ccccc}
% \toprule
% \multicolumn{3}{c|}{Parameters} & \multicolumn{5}{c}{Derivative Level} \\
%  $\sigma$ & $\ldim$ & $C^{\{A, B^{(1)}, B^{(2)}\}}$ & 1 & 2 & 3 & 4 & 5 \\
% \midrule
% softmax & 64 & 1.0 & \texttt{\footnotesize 	17.00} & \texttt{\footnotesize 	50.47} & \texttt{\footnotesize 	236.94} & \texttt{\footnotesize 	1.34E+03} & \texttt{\footnotesize 	1.33E+04} \\ \hline
% tanh & &  & \texttt{\footnotesize 	129.00} & \texttt{\footnotesize 	1.02E+03} & \texttt{\footnotesize 	8.96E+03} & \texttt{\footnotesize 	9.83E+04} & \texttt{\footnotesize 	1.34E+06} \\
% GeLU & &  & \texttt{\footnotesize 	73.25} & \texttt{\footnotesize 	237.41} & \texttt{\footnotesize 	1.25E+03} & \texttt{\footnotesize 	1.16E+04} & \texttt{\footnotesize 	1.81E+05} \\
% SWISH& &  & \texttt{\footnotesize 	71.39} & \texttt{\footnotesize 	236.78} & \texttt{\footnotesize 	870.75} & \texttt{\footnotesize 	5.33E+03} & \texttt{\footnotesize 	4.13E+04} \\ \hline
%  &16 &      & \texttt{\footnotesize 	5.00} & \texttt{\footnotesize 	12.62} & \texttt{\footnotesize 	59.23} & \texttt{\footnotesize 	334.15} & \texttt{\footnotesize 	3.31E+03} \\
%  &32 &      & \texttt{\footnotesize 	9.00} & \texttt{\footnotesize 	25.24} & \texttt{\footnotesize 	118.47} & \texttt{\footnotesize 	668.30} & \texttt{\footnotesize 	6.63E+03} \\
%  &128 &     & \texttt{\footnotesize 	33.00} & \texttt{\footnotesize 	100.95} & \texttt{\footnotesize 	473.87} & \texttt{\footnotesize 	2.67E+03} & \texttt{\footnotesize 	2.65E+04} \\
%  &256 &     & \texttt{\footnotesize 	65.00} & \texttt{\footnotesize 	201.90} & \texttt{\footnotesize 	947.75} & \texttt{\footnotesize 	5.35E+03} & \texttt{\footnotesize 	5.30E+04} \\ \hline
%  & & 0.01   & \texttt{\footnotesize 	17.00} & \texttt{\footnotesize 	44.32} & \texttt{\footnotesize 	180.94} & \texttt{\footnotesize 	919.87} & \texttt{\footnotesize 	6.52E+03} \\
%  & & 0.1    & \texttt{\footnotesize 	17.00} & \texttt{\footnotesize 	44.38} & \texttt{\footnotesize 	181.00} & \texttt{\footnotesize 	919.92} & \texttt{\footnotesize 	6.52E+03} \\
%  & & 10.0     & \texttt{\footnotesize 	17.00} & \texttt{\footnotesize 	660.15} & \texttt{\footnotesize 	5.62E+04} & \texttt{\footnotesize 	4.17E+06} & \texttt{\footnotesize 	6.73E+08} \\
%  & & 100.0    & \texttt{\footnotesize 	17.00} & \texttt{\footnotesize 	6.16E+04} & \texttt{\footnotesize 	5.60E+07} & \texttt{\footnotesize 	4.17E+10} & \texttt{\footnotesize 	6.73E+13} \\
% \bottomrule
% \end{tabular}
% \end{table}

% % \begin{table}[p]
% % \centering
% % \small
% % \caption{Derivative type-specific bounds of the $\layernorm$ according to \Cref{lem:LayerNorm}, parameters bound by $1$.}
% % \setlength{\tabcolsep}{0.5em}
% % \begin{tabular}{@{}lccccccc@{}}
% % \toprule
% % $k$ (input dim)         & 10  & 5 & 20 &  &  & & \\
% % $\Vert K \Vert$ & 10  &  &  & 0.1 & 1.0 & 100.0 & 1000.0 \\
% % \midrule
% % (1, 0, ...) & \texttt{\footnotesize321.71} & \texttt{\footnotesize321.71} & \texttt{\footnotesize321.71} & \texttt{\footnotesize1.73} & \texttt{\footnotesize18.67} & \texttt{\footnotesize1.67E+04} & \texttt{\footnotesize1.52E+06} \\
% % (1, 1, 0, ...) & \texttt{\footnotesize7.75E+03} & \texttt{\footnotesize7.75E+03} & \texttt{\footnotesize7.75E+03} & \texttt{\footnotesize36.52} & \texttt{\footnotesize63.51} & \texttt{\footnotesize7.50E+06} & \texttt{\footnotesize7.50E+09} \\
% % (2, 0, ...) & \texttt{\footnotesize5.87E+03} & \texttt{\footnotesize5.87E+03} & \texttt{\footnotesize5.87E+03} & \texttt{\footnotesize36.44} & \texttt{\footnotesize60.89} & \texttt{\footnotesize5.63E+06} & \texttt{\footnotesize5.63E+09} \\
% % (1, 1, 1, 0, ...) & \texttt{\footnotesize7.91E+05} & \texttt{\footnotesize7.91E+05} & \texttt{\footnotesize7.91E+05} & \texttt{\footnotesize58.08} & \texttt{\footnotesize185.68} & \texttt{\footnotesize7.88E+09} & \texttt{\footnotesize7.88E+13} \\
% % (2, 1, 0, ...) & \texttt{\footnotesize5.28E+05} & \texttt{\footnotesize5.28E+05} & \texttt{\footnotesize5.28E+05} & \texttt{\footnotesize57.25} & \texttt{\footnotesize151.18} & \texttt{\footnotesize5.25E+09} & \texttt{\footnotesize5.25E+13} \\
% % (3, 0, ...) & \texttt{\footnotesize2.86E+05} & \texttt{\footnotesize2.86E+05} & \texttt{\footnotesize2.86E+05} & \texttt{\footnotesize55.67} & \texttt{\footnotesize118.12} & \texttt{\footnotesize2.84E+09} & \texttt{\footnotesize2.84E+13} \\
% % (1, 1, 1, 1, 0, ...) & \texttt{\footnotesize1.42E+08} & \texttt{\footnotesize1.42E+08} & \texttt{\footnotesize1.42E+08} & \texttt{\footnotesize77.64} & \texttt{\footnotesize2.04E+03} & \texttt{\footnotesize1.42E+13} & \texttt{\footnotesize1.42E+18} \\
% % (2, 1, 1, 0, ...) & \texttt{\footnotesize8.89E+07} & \texttt{\footnotesize8.89E+07} & \texttt{\footnotesize8.89E+07} & \texttt{\footnotesize75.26} & \texttt{\footnotesize1.36E+03} & \texttt{\footnotesize8.86E+12} & \texttt{\footnotesize8.86E+17} \\
% % (2, 2, 0, ...) & \texttt{\footnotesize5.64E+07} & \texttt{\footnotesize5.64E+07} & \texttt{\footnotesize5.64E+07} & \texttt{\footnotesize73.66} & \texttt{\footnotesize932.89} & \texttt{\footnotesize5.61E+12} & \texttt{\footnotesize5.61E+17} \\
% % (3, 1, 0, ...) & \texttt{\footnotesize4.35E+07} & \texttt{\footnotesize4.35E+07} & \texttt{\footnotesize4.35E+07} & \texttt{\footnotesize72.87} & \texttt{\footnotesize760.23} & \texttt{\footnotesize4.33E+12} & \texttt{\footnotesize4.33E+17} \\
% % (4, 0, ...) & \texttt{\footnotesize1.86E+07} & \texttt{\footnotesize1.86E+07} & \texttt{\footnotesize1.86E+07} & \texttt{\footnotesize71.42} & \texttt{\footnotesize402.92} & \texttt{\footnotesize1.85E+12} & \texttt{\footnotesize1.85E+17} \\
% % (1, 1, 1, 1, 1, 0, \,) & \texttt{\footnotesize1.06E+08} & \texttt{\footnotesize1.06E+08} & \texttt{\footnotesize1.06E+08} & \texttt{\footnotesize212.95} & \texttt{\footnotesize1.20E+04} & \texttt{\footnotesize1.06E+12} & \texttt{\footnotesize1.06E+16} \\
% % (2, 1, 1, 1, 0, ...) & \texttt{\footnotesize3.97E+09} & \texttt{\footnotesize3.97E+09} & \texttt{\footnotesize3.97E+09} & \texttt{\footnotesize174.75} & \texttt{\footnotesize1.23E+04} & \texttt{\footnotesize3.90E+15} & \texttt{\footnotesize3.90E+21} \\
% % (2, 2, 1, 0, ...) & \texttt{\footnotesize4.44E+09} & \texttt{\footnotesize4.44E+09} & \texttt{\footnotesize4.44E+09} & \texttt{\footnotesize145.51} & \texttt{\footnotesize1.02E+04} & \texttt{\footnotesize4.39E+15} & \texttt{\footnotesize4.39E+21} \\
% % (3, 1, 1, 0, ...) & \texttt{\footnotesize4.27E+09} & \texttt{\footnotesize4.27E+09} & \texttt{\footnotesize4.27E+09} & \texttt{\footnotesize133.13} & \texttt{\footnotesize9.06E+03} & \texttt{\footnotesize4.22E+15} & \texttt{\footnotesize4.22E+21} \\
% % (3, 2, 0, ...) & \texttt{\footnotesize3.33E+09} & \texttt{\footnotesize3.33E+09} & \texttt{\footnotesize3.33E+09} & \texttt{\footnotesize120.30} & \texttt{\footnotesize6.65E+03} & \texttt{\footnotesize3.30E+15} & \texttt{\footnotesize3.30E+21} \\
% % (4, 1, 0, ...) & \texttt{\footnotesize2.57E+09} & \texttt{\footnotesize2.57E+09} & \texttt{\footnotesize2.57E+09} & \texttt{\footnotesize105.79} & \texttt{\footnotesize4.99E+03} & \texttt{\footnotesize2.54E+15} & \texttt{\footnotesize2.54E+21} \\
% % (5, 0, ...) & \texttt{\footnotesize1.15E+09} & \texttt{\footnotesize1.15E+09} & \texttt{\footnotesize1.15E+09} & \texttt{\footnotesize95.24} & \texttt{\footnotesize2.29E+03} & \texttt{\footnotesize1.14E+15} & \texttt{\footnotesize1.14E+21} \\
% % \bottomrule
% % \end{tabular}
% % \label{tab:LayerNorm}
% % \end{table}

% \begin{table}[htbp]
% \small
% \centering
% \caption{Layer Norm}
% \label{tab:LayerNorm}
% \begin{tabular}{ccc|ccccc}
% \toprule
% \multicolumn{3}{c|}{Parameters} & \multicolumn{5}{c}{Derivative Level} \\
%  $k$ & $\Vert K \Vert$ & $\gamma$ & 1 & 2 & 3 & 4 & 5 \\
% \midrule
% 5 & 10.0 & 0.1  & \texttt{\footnotesize 	18.67} & \texttt{\footnotesize 	28.56} & \texttt{\footnotesize 	104.49} & \texttt{\footnotesize 	1.49E+03} & \texttt{\footnotesize 	4.93E+03} \\ \hline
% 3 &      &      & \texttt{\footnotesize 	18.67} & \texttt{\footnotesize 	28.56} & \texttt{\footnotesize 	104.49} & \texttt{\footnotesize 	945.21} & \texttt{\footnotesize 	4.93E+03} \\ 
% 10 &      &      & \texttt{\footnotesize 	18.67} & \texttt{\footnotesize 	28.56} & \texttt{\footnotesize 	104.49} & \texttt{\footnotesize 	1.49E+03} & \texttt{\footnotesize 	4.93E+03} \\ 
%    20 &      &      & \texttt{\footnotesize 	18.67} & \texttt{\footnotesize 	28.56} & \texttt{\footnotesize 	104.49} & \texttt{\footnotesize 	1.49E+03} & \texttt{\footnotesize 	4.93E+03} \\ \hline
%    & 0.1&      & \texttt{\footnotesize 	0.17} & \texttt{\footnotesize 	3.61} & \texttt{\footnotesize 	5.37} & \texttt{\footnotesize 	7.05} & \texttt{\footnotesize 	8.87} \\
%    & 1.0&      & \texttt{\footnotesize 	1.73} & \texttt{\footnotesize 	5.20} & \texttt{\footnotesize 	6.95} & \texttt{\footnotesize 	8.71} & \texttt{\footnotesize 	10.64} \\
%    &100.0 &      & \texttt{\footnotesize 	321.71} & \texttt{\footnotesize 	7.68E+03} & \texttt{\footnotesize 	7.88E+05} & \texttt{\footnotesize 	1.42E+08} & \texttt{\footnotesize 	4.39E+09} \\
%    &1000.0 &      & \texttt{\footnotesize 	321.71} & \texttt{\footnotesize 	7.68E+03} & \texttt{\footnotesize 	7.88E+05} & \texttt{\footnotesize 	1.42E+08} & \texttt{\footnotesize 	4.39E+09} \\\hline
%       &       & 0.01    & \texttt{\footnotesize 	1.73} & \texttt{\footnotesize 	2.07} & \texttt{\footnotesize 	2.24} & \texttt{\footnotesize 	2.42} & \texttt{\footnotesize 	2.59} \\
%    &       &  1.0    & \texttt{\footnotesize 	321.71} & \texttt{\footnotesize 	7.75E+03} & \texttt{\footnotesize 	7.91E+05} & \texttt{\footnotesize 	1.42E+08} & \texttt{\footnotesize 	4.44E+09} \\
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{table}[p]
% \footnotesize
% \centering
% \setlength{\tabcolsep}{0.5em}
% \caption{Derivative Bounds of Transformer Block by derivative level according to \Cref{thm:TransformerBlockSobolevBoundLevel}.}
% \label{tab:TBlock}
% \begin{tabular}{cccc|ccccc}
% \toprule
% \multicolumn{4}{c|}{Parameters} & \multicolumn{5}{c}{Derivative Level} \\
%  $\idim$ & {\tiny $C^{\{K, Q, V, W \}}$} & {\tiny $C^{\{A, B^{(1,2)}\}}$} & $\gamma$ & 1 & 2 & 3 & 4 & 5 \\
% \midrule
% 5&0.01&0.001& 0.01& \texttt{\footnotesize 	21.15} & \texttt{\footnotesize 	1.13E+04} & \texttt{\footnotesize 	4.81E+06} & \texttt{\footnotesize 	2.59E+09} & \texttt{\footnotesize 	2.22E+11} \\ \hline
% \multicolumn{4}{c|}{ --- using derivative level --- } & \texttt{\footnotesize 212.70} & \texttt{\footnotesize1.53E+06} & \texttt{\footnotesize7.47E+09} & \texttt{\footnotesize4.55E+13} & \texttt{\footnotesize3.75E+16} \\ \hline
% 10&&& & \texttt{\footnotesize 	111.32} & \texttt{\footnotesize 	4.51E+05} & \texttt{\footnotesize 	1.71E+09} & \texttt{\footnotesize 	1.45E+13} & \texttt{\footnotesize 	8.70E+16} \\
% 20&&& & \texttt{\footnotesize 	1.29E+03} & \texttt{\footnotesize 	1.25E+08} & \texttt{\footnotesize 	3.47E+13} & \texttt{\footnotesize 	1.85E+19} & \texttt{\footnotesize 	2.20E+24} \\\hline

% &0.001&& & \texttt{\footnotesize 	21.15} & \texttt{\footnotesize 	1.13E+04} & \texttt{\footnotesize 	4.81E+06} & \texttt{\footnotesize 	2.59E+09} & \texttt{\footnotesize 	2.22E+11} \\
% &0.1&& & \texttt{\footnotesize 	21.16} & \texttt{\footnotesize 	1.13E+04} & \texttt{\footnotesize 	4.83E+06} & \texttt{\footnotesize 	2.61E+09} & \texttt{\footnotesize 	2.32E+11} \\
% &1.0&& & \texttt{\footnotesize 	22.30} & \texttt{\footnotesize 	4.64E+04} & \texttt{\footnotesize 	6.96E+08} & \texttt{\footnotesize 	1.70E+13} & \texttt{\footnotesize 	1.95E+17} \\\hline

% &&0.0001& & \texttt{\footnotesize 	5.05} & \texttt{\footnotesize 	126.27} & \texttt{\footnotesize 	1.12E+04} & \texttt{\footnotesize 	4.94E+06} & \texttt{\footnotesize 	6.87E+08} \\
% &&0.01& & \texttt{\footnotesize 	182.17} & \texttt{\footnotesize 	1.12E+06} & \texttt{\footnotesize 	4.66E+09} & \texttt{\footnotesize 	2.43E+13} & \texttt{\footnotesize 	1.71E+16} \\
% &&0.1& & \texttt{\footnotesize 	1.79E+03} & \texttt{\footnotesize 	1.12E+08} & \texttt{\footnotesize 	4.65E+12} & \texttt{\footnotesize 	2.42E+17} & \texttt{\footnotesize 	1.70E+21} \\\hline

% &&&0.0001 & \texttt{\footnotesize 	0.21} & \texttt{\footnotesize 	108.21} & \texttt{\footnotesize 	4.44E+04} & \texttt{\footnotesize 	2.27E+07} & \texttt{\footnotesize 	1.58E+09} \\
% &&&0.001 & \texttt{\footnotesize 	2.09} & \texttt{\footnotesize 	1.09E+03} & \texttt{\footnotesize 	4.46E+05} & \texttt{\footnotesize 	2.29E+08} & \texttt{\footnotesize 	1.60E+10} \\
% &&&0.1 & \texttt{\footnotesize 	240.09} & \texttt{\footnotesize 	2.45E+05} & \texttt{\footnotesize 	7.31E+08} & \texttt{\footnotesize 	4.96E+12} & \texttt{\footnotesize 	8.79E+15} \\ 
% \bottomrule
% \end{tabular}
% \end{table}


% \begin{sidewaystable}[p]
% \centering
% \caption{Derivative Bounds of Multi-Head Attention by derivative level according to \Cref{cor:MultiHead}.}
% \small
% \begin{tabular}{cccccccc|ccccc}
% \toprule
% \multicolumn{8}{c|}{Parameters} & \multicolumn{5}{c}{Derivative Level} \\
%  $\idim$ & $M$ & $\kdim$ & $C^K$ & $C^Q$ & $C^V$ & $C^W$ & $\Vert K \Vert$
%  & 1 & 2 & 3 & 4 & 5 \\
% \midrule
% 5& 1 & 3 & 0.1 & 0.1 & 0.1 & 0.1 & 1.0  & \texttt{\footnotesize 	7.67} & \texttt{\footnotesize 	46.08} & \texttt{\footnotesize 	184.82} & \texttt{\footnotesize 	931.81} & \texttt{\footnotesize 	5.73E+03} \\ \hline
% \multicolumn{8}{c|}{ --- using derivative level ---}  & \texttt{\footnotesize 	7.67} & \texttt{\footnotesize 	46.15} & \texttt{\footnotesize 	 186.90} & \texttt{\footnotesize 1.01E+03} & \texttt{\footnotesize 	7.84E+03} \\ \hline
% 10 & & &     &     &     &     &       & \texttt{\footnotesize 	7.82E+03} & \texttt{\footnotesize 	4.87E+04} & \texttt{\footnotesize 	8.14E+05} & \texttt{\footnotesize 	2.95E+08} & \texttt{\footnotesize 	2.38E+11} \\
% 20&  &   &     &     &     &     &      & \texttt{\footnotesize 	1.57E+04} & \texttt{\footnotesize 	1.09E+05} & \texttt{\footnotesize 	1.03E+07} & \texttt{\footnotesize 	9.25E+09} & \texttt{\footnotesize 	1.50E+13} \\ \hline 
%  & 5 &   &     &     &     &     &      & \texttt{\footnotesize 	3.90E+03} & \texttt{\footnotesize 	2.37E+04} & \texttt{\footnotesize 	1.34E+05} & \texttt{\footnotesize 	9.96E+06} & \texttt{\footnotesize 	3.83E+09} \\
%  &20 &   &     &     &     &     &      & \texttt{\footnotesize 	4.71E+06} & \texttt{\footnotesize 	2.85E+07} & \texttt{\footnotesize 	7.11E+08} & \texttt{\footnotesize 	2.66E+12} & \texttt{\footnotesize 	1.40E+16} \\\hline
%  &   & 3 &     &     &     &     &      & \texttt{\footnotesize 	7.67} & \texttt{\footnotesize 	45.99} & \texttt{\footnotesize 	183.98} & \texttt{\footnotesize 	920.53} & \texttt{\footnotesize 	5.53E+03} \\
%  &   &10 &     &     &     &     &      & \texttt{\footnotesize 	7.70} & \texttt{\footnotesize 	46.41} & \texttt{\footnotesize 	190.35} & \texttt{\footnotesize 	1.07E+03} & \texttt{\footnotesize 	1.03E+04} \\
%  &   &20 &     &     &     &     &      & \texttt{\footnotesize 	7.75} & \texttt{\footnotesize 	47.52} & \texttt{\footnotesize 	226.02} & \texttt{\footnotesize 	2.87E+03} & \texttt{\footnotesize 	1.23E+05} \\\hline
%  &   &   & 0.01&     &     &     &      & \texttt{\footnotesize 	7.90} & \texttt{\footnotesize 	54.45} & \texttt{\footnotesize 	740.55} & \texttt{\footnotesize 	6.51E+04} & \texttt{\footnotesize 	9.33E+06} \\
%  &   &   & 1.0 &     &     &     &      & \texttt{\footnotesize 	7.65} & \texttt{\footnotesize 	45.91} & \texttt{\footnotesize 	183.61} & \texttt{\footnotesize 	918.01} & \texttt{\footnotesize 	5.51E+03} \\
%  &   &   &     & 0.01&     &     &      & \texttt{\footnotesize 	7.65} & \texttt{\footnotesize 	45.91} & \texttt{\footnotesize 	183.61} & \texttt{\footnotesize 	918.01} & \texttt{\footnotesize 	5.51E+03} \\
%  &   &   &     & 1.0 &     &     &      & \texttt{\footnotesize 	7.90} & \texttt{\footnotesize 	54.45} & \texttt{\footnotesize 	740.55} & \texttt{\footnotesize 	6.51E+04} & \texttt{\footnotesize 	9.33E+06} \\
%  &   &   &     &     & 0.01&     &      & \texttt{\footnotesize 	0.77} & \texttt{\footnotesize 	4.61} & \texttt{\footnotesize 	18.48} & \texttt{\footnotesize 	93.18} & \texttt{\footnotesize 	573.32} \\
%  &   &   &     &     & 1.0 &     &      & \texttt{\footnotesize 	76.75} & \texttt{\footnotesize 	460.80} & \texttt{\footnotesize 	1.85E+03} & \texttt{\footnotesize 	9.32E+03} & \texttt{\footnotesize 	5.73E+04} \\
%  &   &   &     &     &     & 0.01&      & \texttt{\footnotesize 	0.77} & \texttt{\footnotesize 	4.61} & \texttt{\footnotesize 	18.48} & \texttt{\footnotesize 	93.18} & \texttt{\footnotesize 	573.32} \\
%  &   &   &     &     &     & 1.0 &      & \texttt{\footnotesize 	76.75} & \texttt{\footnotesize 	460.80} & \texttt{\footnotesize 	1.85E+03} & \texttt{\footnotesize 	9.32E+03} & \texttt{\footnotesize 	5.73E+04} \\
%  &   &   &0.001&0.001&0.001&0.001&      & \texttt{\footnotesize 	1.02E+03} & \texttt{\footnotesize 	8.06E+04} & \texttt{\footnotesize 	4.95E+07} & \texttt{\footnotesize 	5.70E+10} & \texttt{\footnotesize 	8.04E+13} \\
%  &   &   &0.01 &0.01 &0.01 & 0.01&      & \texttt{\footnotesize 	0.08} & \texttt{\footnotesize 	0.46} & \texttt{\footnotesize 	1.84} & \texttt{\footnotesize 	9.18} & \texttt{\footnotesize 	55.08} \\
%  &   &   &1.0  &1.0  &1.0  & 1.0 &      & \texttt{\footnotesize 	0.00} & \texttt{\footnotesize 	0.00} & \texttt{\footnotesize 	0.02} & \texttt{\footnotesize 	0.09} & \texttt{\footnotesize 	0.55} \\\hline
%  &   &   &     &     &     &     &0.1   & \texttt{\footnotesize 	0.77} & \texttt{\footnotesize 	32.14} & \texttt{\footnotesize 	142.34} & \texttt{\footnotesize 	752.79} & \texttt{\footnotesize 	4.68E+03} \\
%  &   &   &     &     &     &     &10.0  & \texttt{\footnotesize 	79.00} & \texttt{\footnotesize 	259.65} & \texttt{\footnotesize 	5.54E+03} & \texttt{\footnotesize 	5.73E+05} & \texttt{\footnotesize 	8.04E+07} \\
%  &   &   &     &     &     &     &100.0 & \texttt{\footnotesize 	1.02E+03} & \texttt{\footnotesize 	7.66E+04} & \texttt{\footnotesize 	4.88E+07} & \texttt{\footnotesize 	5.63E+10} & \texttt{\footnotesize 	7.90E+13} \\
% \bottomrule
% \end{tabular}
% \label{tab:MultiHead}
% \end{sidewaystable}


% \clearpage

% \section{Supporting Technical Results on the \texorpdfstring{$C^s$}{Cs}-Norms of Smooth Functions}
% \label{s:Technical_Results}

% This section contains many of the technical tools on which we build our analysis.  Most results concern smooth functions, especially their derivatives and those of compositions thereof.  However, the first set of results concerns the integral probability metric $d_s$.

% \subsection{Integral Probability Metrics and Restriction to Compact Sets}
% \label{ss:IMPs}

% Fix $d\in \mathbb{N}_+$ and a non-empty compact subset $K\subseteq \mathbb{R}^d$.  
% Observe that any Borel probability measure $\mu$ on $K$ can be canonically extended to a compactly supported Borel probability measure $\mu^+$ on all of $\mathbb{R}^d$ via
% \begin{align*}
%     \mu^+(B)\eqdef \mu(B\cap K),
% \end{align*}
% for any Borel subset $B$ of $\mathbb{R}^d$; noting only that $B\cap K$ is Borel.  


% Let $\mathcal{P}(K)$ denote the set of Borel probability measures on $K$.
% Suppose that $K$ is a regular compact set, i.e.\ the closure of its interior is itself.  As usual, see~\cite{evans2022partial}, for any $s\in \mathbb{N}_+$, we denote the set of functions from the interior of $K$ to $\mathbb{R}$ with $s$ continuous partial derivatives thereon and with a continuous extension to $K$ by $C^s(K)$.  This space, is a Banach space when equipped with the (semi-)norm
% \begin{align*}
% \resizebox{1\linewidth}{!}{$%% BEGIN RESIZE BOX$}
%     \|f\|_{s:K}
% \eqdef 
%         \max_{k=1,\dots,s-1}\,
%         \max_{\alpha\in \{1,\dots,d\}^k}
%         \,
%             \sup_{u\in K}\,
%             \Big\|
%                 \frac{\partial^k f}{
%                     \partial x_{\alpha_1}\dots\partial x_{\alpha_k}
%                 }(u)
%             \Big\|
%     +
%         \max_{\alpha \in \{1,\dots,d\}^{s-1}}\,
%             \operatorname{Lip}\biggl(
%                 \frac{\partial^{s-1}f}{\partial x_{\alpha_1}\dots\partial x_{\alpha_{s-1}}}
%             \biggr)
% .
% $}
% \end{align*}
% We may define an associated integral probability metric $d_{s:K}$ on $\mathcal{P}(K)$ via
% \begin{align*}
%     d_{s:K}(\mu,\nu) 
%     \eqdef 
%     \sup_{f\in C^s(K)}\,
%         \|
%                 \mathbb{E}_{X\sim \mu}[f(X)]
%             -
%                 \mathbb{E}_{X\sim \mu}[f(X)]
%         \|
% \end{align*}
% for any $\mu,\nu\in \mathcal{P}(K)$.  The main purpose of this technical subsection is simply to reassure ourselves, and the reader, that quantities $d_{s:K}(\mu,\nu)$ and $d_s(\mu^+,\nu^+)$ are equal for any $\mu,\nu \in \mathcal{P}(K)$.  Therefore, we may use them interchangeably.

% \begin{lemma}[Consistency of Smooth IMP Extension - Beyond Regular Compact Sets]
% \label{lem:res_ext}
% Fix $d,s\in \mathbb{N}_+$ and let $K$ be a non-empty regular compact subset of $\mathbb{R}^d$.  For any $\mu,\nu\in \mathcal{P}(K)$ the following holds
% \begin{align*}
%     d_{s:K}(\mu,\nu)=d_s(\mu^+,\nu^+)
% .
% \end{align*}
% \end{lemma}
% \begin{proof}%[{Proof of Lemma~\ref{lem:res_ext}}]
% Let $\operatorname{int}(K)$ denote the interior of $K$,
% By the Whitney extension theorem, as formulated in \citep[Theorem A]{fefferman2005sharp}, for any $f\in C^s(K)$ there exists a $C^s$-extension $F:\mathbb{R}^d\to \mathbb{R}$ of $f|_{\operatorname{int}(K)}$ to all of $\mathbb{R}^d$; i.e.\ $F|_{\operatorname{int}(K)} =f $ and $\in C^s(\mathbb{R}^d)$.  
% Since any continuous function is uniformly continuous on a compact set, $\operatorname{int}(K)$ is dense in $K$, and since uniformly continuous functions are uniquely determined by their values on compact sets, then $f$ coincides with $F$ on all of $K$ (not only on $\operatorname{int}(K)$).

% For any $\mu\in \mathcal{P}(K)$, by definition of $\mu^+$ we have that
% \begin{align*}
%         \mathbb{E}_{X\sim \mu^+}[F(X)] 
%     = 
%         \mathbb{E}_{X\sim \mu^+}[F(X)I_{X\in K}]
%     =
%         \mathbb{E}_{X\sim \mu^+}[f(X)I_{X\in K}]
%     =
%         \mathbb{E}_{X\sim \mu}[f(X)]
% .
% \end{align*}
% Therefore, for any $\mu,\nu \in \mathcal{P}(K)$ we conclude that and each $f\in C^s(K)$ there exists some $F\in C^s(\mathbb{R}^d)$ such that
% \begin{align*}
%         \mathbb{E}_{Y\sim \mu}[f(Y)] 
%             - 
%         \mathbb{E}_{Y\sim \nu}[f(Y)]
%     =
%         \mathbb{E}_{X\sim \mu^+}[F(X)] 
%             - 
%         \mathbb{E}_{X\sim \nu^+}[F(X)] 
% .
% \end{align*}
% Consequentially, $d_{s:K}(\mu,\nu)\leq d_s(\mu^+,\nu^+)$.  Conversely, since the restriction of any $g\in C^s(\mathbb{R}^d)$ to $K$ belongs to $C^s(K)$ then the reverse inequality holds; namely, $d_{s:K}(\mu,\nu)\geq d_s(\mu^+,\nu^+)$.  
% % This concludes our proof.
% \end{proof}

% By Lemma~\ref{lem:res_ext} we henceforth may interpret any such $\mu$ as its extension $\mu^+$, without loss of generality.
% % , whenver convenient to do so.


% \subsection{{Examples  of Functions in The Classes \texorpdfstring{$C^s_{poly:C,r}([0,1]^d,\mathbb{R})$ and $C^s_{exp:C,r}([0,1]^d,\mathbb{R})$}{Cs-Poly and Cs-Exp}}}
% \label{s:Functions_of_ControlledGrowth}

% In several learning theory papers, especially in the kernel ridge regression literature e.g.~\cite{simon2023eigenlearning,barzilai2023generalization,tsigler2023benign,simon2023eigenlearning,cheng2024characterizing,cheng2024characterizingV2}, one often quantifies the \textit{learnability} of a target function in terms of some sort of decay/growth rates of its coefficients in an appropriate expansion; e.g.\ the decay of its coefficients in an eigenbasis associated to a kernel.  These decay/growth rates are often equivalent to the smoothness of a function%
% \footnote{See e.g.~\citep[page 120-121]{atkinson2012spherical} for an example between the decay rate of the Laplacian eigenspectrum characterize the smoothness of the functions in the RKHS of radially symmetric kernels.}.  
% Therefore, in a like spirit, we unpack the meaning of the smoothness condition in Assumption~\ref{def:sGrowthRate} which impacts the learning rates in Theorem~\ref{thrm:main} by giving examples of functions in the classes $C^s_{poly:C,r}([0,1]^d,\mathbb{R})$ and $C^s_{exp:C,r}([0,1]^d,\mathbb{R})$.

% For brevity and transparency in our illustration, we consider the one-dimensional case.  In particular, this shows that the class is far from being void.
% \begin{proposition}[{Functions with Polynomially/Exponentially Growing $C^s$-Norms on $[0,1]$}]
% \label{prop:Examples_Functions_inPoly}
% Fix $d\in \mathbb{N}_+$ and let $K$ be a non-empty regular compact subset of $\mathbb{R}^d$.  If $f:\mathbb{R}\to \mathbb{R}$ is real-analytic with power-series expansion at $0$ given by 
% \begin{align*}
%         f(x) 
%     = 
%         \sum_{i=0}^{\infty}\, 
%             \frac{\beta_i\, x^i}{i!}
% .
% \end{align*}
% If there are $C,r>0$ such that
% \begin{enumerate}
%     \item[(i)] \textbf{Polynomial Growth:} $|\beta_i|\le Ce^{i\,r} \,\,(\forall i \in \mathbb{N})$ 
%     then $f\in C^{\infty}_{poly:C,r}([0,1],\mathbb{R})$,
%     \item[(ii)] \textbf{Exponential Growth:} $|\beta_i|\le C(1+i)^r \,\,(\forall i \in \mathbb{N})$ 
%     then $f\in C^{\infty}_{poly:C,r}([0,1],\mathbb{R})$,
% \end{enumerate}
% \end{proposition}
% \begin{proof}
% Since $f$ is real-analytic we may consider its Maclaurin-Taylor series expansion which coincides with $\sum_{i=0}^{\infty}\, \frac{\beta_i\, x^i}{i!}$; meaning that for each $i\in \mathbb{N}$ we have $\beta_i=\partial^i \, f(0)$.
% Therefore, standard analytic estimates and manipulations of the Maclaurin-Taylor series, see e.g.~\citep[page 173]{rudin1964principles}, yield
% \begin{equation}
% \label{eq:MLT_Estimates}
% \begin{aligned}
%     \max_{0\le x \le 1}
%     \,
%         \Big|
%             \sum_{i=0}^{\infty}\, 
%                 \frac{\beta_i\, x^i}{i!}
%             -
%             f(x)
%         \Big|
%     \le &
%         \frac{1}{(s+1)!}\,
%         \sup_{0 \le x \le 1}
%             \,
%             \Big|
%                 \big(
%                     \sum_{i=0}^{\infty}\, 
%                     \frac{\beta_i\, x^i}{i!}
%                 \big)^{s+1}
%                 -
%                 \partial f^{s+1}(x)
%             \Big|
% \\
%     \le &
%         \frac{1}{(s+1)!}\,
%          \beta_s(s+1)!
% .
% \end{aligned}
% \end{equation}
% If (i) holds, then the right-hand side of~\eqref{eq:MLT_Estimates} is bounded above by $C\, (s+1)^r$ and $f\in C^{\infty}_{poly:C,r}([0,1],\mathbb{R})$.  If, instead, (ii) holds then the right-hand side of~\eqref{eq:MLT_Estimates} is bounded above by $C\, e^{s\,r}$ and $f\in C^{\infty}_{exp:C,r}([0,1],\mathbb{R})$.
% \end{proof}






















% \section{Proof of \texorpdfstring{Theorem~\ref{thrm:main}}{The Main Result}}
% \label{s:Proof_of_MainResult}

% Section~\ref{s:Discssion__ss:Overview_Proof}, the proof will be largely broken down into two steps.  First, we derive our concentration of measure result for the empirical mean compared to the true mean general of an arbitrary $C^s$ function applied to a random input, where the $C^s$-norm of the $C^s$ function is at most $R\ge 0$ (in Subsection~\ref{s:Proofs__ss:ConcentrationProof}).  

% Next, (in Subsection~\ref{s:Proofs__ss:ConcentrationProof}), we use the Fa\`{a} di Bruno-type results in Section~\ref{s:Compositions_and__FaadiBruno} to bound the maximal $C^s$ norm over the relevant class of transformer networks.  We do this by first individually bounding each of the $C^s$-norms of its constituent pieces, namely the multi-head attention layers, the SLP blocks with smooth activation functions, and then ultimately, we bound the $C^s$-norms of the composition of transformer blocks using the earlier Fa\`{a} di Bruno-type results.  

% \begin{figure}[H]%[hp]%
%      \centering
%         \centerline{\includegraphics[width=.5\linewidth]{figs/TransformerGeneralization.pdf}}
%         \caption{Workflow of the proof technique used to derive Theorem~\ref{thrm:main}.}
%         \label{fig:worklow}
% \end{figure}

% Our main result (Theorem~\ref{thrm:main}) is then then obtained upon merging these two sets of estimates.  The workflow which we use can be applied to derive generalization bounds for other machine learning, and is summarized in Figure~\ref{fig:worklow}.








% \subsection{Step 0 - Bounds on the \texorpdfstring{$C^s$}{Cs} Regularity of Multivariate Composite Functions}
% \label{s:Compositions_and__FaadiBruno}

% In this section, we will derive a bound for the Sobolev norm of multivariate composite functions.

% \subsubsection{Multivariate Fa\`a di Bruno formula revisited}
% We begin by establishing notation and stating the multivariate Fa\`a di Bruno formula from \cite{ConstantineSavits96}.

% \begin{theorem}[Multivariate Fa\`a di Bruno Formula, \cite{ConstantineSavits96}]\label{thm:FaaDiBruno}
%     Let $n, m, k \in \N$, $\alpha \in \N^k$ with $\vert \alpha \vert = n$, and define 
%     \begin{align*}
%         h(x_1, \ldots, x_k) \eqdef f^{(1)}(g^{(1)}(x_1, \ldots, x_k), \ldots, g^{(m)}(x_1, \ldots, x_k)).
%     \end{align*}
%     Then, using the multivariate notation from \Cref{not:Multivariate},
%     \begin{align*}
%         D^\alpha h(x) 
%         =
%         \sum_{1 \leq |\beta| \leq n} (D^\beta f)(g(x))
%         \sum_{\eta, \zeta \in \calP(\alpha,\beta)} \alpha! 
%         \prod_{j=1}^{n} \frac{
%             [D^{\zeta^{(j)}} g(x)]^{\eta^{(j)}}
%         }{
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         }.
%     \end{align*}
%     where 
%     \begin{multline*}
%         \calP(\alpha, \beta) = \Big\{ \eta \eqdef (\eta^{(1)}, \ldots, \eta^{(n)}) \in (\N^m)^n, \zeta\eqdef (\zeta^{(1)}, \ldots, \zeta^{(n)}) \in (\N^k)^n : \\
%          \exists j \leq m: \eta^{(i)} = 0, \zeta^{(i)} = 0 \text{ for } i < j, |\eta^{(i)}| > 0 \text{ for } i \geq j, \\
%          \textstyle 0 \prec \zeta^{(j)} \prec \ldots \prec \zeta^{(n)}, \sum_{i=1}^{n} \eta^{(i)} = \beta \text{ and } \sum_{i=1}^{n} |\eta^{(i)}|\zeta^{(i)} = \alpha \Big\} .
%     \end{multline*}
% \end{theorem}
% \begin{proof}
%     See \cite{ConstantineSavits96}.
% \end{proof}

% \begin{comment}
% \subsection{Bounds in Derivative-Depth}
% The goal of this section is to bound the derivative of composite functions by grouping over the multi-indices sum, i.e. all derivatives $D^\alpha$ with $\vert \alpha \vert = n$ are bounded uniformly.

% \begin{theorem}\label{thm:GeneralDerivativeBound}
%     In the notation of \Cref{thm:FaaDiBruno}, we have for a compact set $K \subseteq \R^k$
%     \begin{align*}
%         C^h_K(n)
%         &\leq
%         n!
%         \sum_{n' = 1}^n  \binom{n' + m - 1}{m - 1}  C^f_{g[K]}(n') 
%         \sum_{\eta, \zeta \in \calP^{d, k}_{n, n'}}
%         \prod_{j=1}^{n} 
%         \frac{1}{\eta^{(j)}!}
%         \left(\frac{
%             C^g_K(\vert \zeta^{(j)}\vert)
%         }{
%             \zeta^{(j)}!
%         }\right)^{|\eta^{(j)}|}.
%     \end{align*}
%     where 
%     \begin{itemize}[nosep]
%         \item $C^h_K(n) \eqdef \max_{\vert \alpha \vert = n}\Vert D^\alpha h\Vert_K$,
%         \item $C^f_{g[K]}(n') \eqdef \max_{\vert \alpha \vert = n'}\Vert D^\alpha f\Vert_{g[K]}$, 
%         \item $C^g_K(n') \eqdef \max_{\vert \alpha \vert = n'}\Vert D^\alpha g\Vert_K$,
%     \end{itemize}
%     and 
%     \begin{align*}
%     \calP^{d, k}_{n, n'} \eqdef \Big\{ &\eta \eqdef (\eta^{(1)}, \ldots, \eta^{(n)}) \in (\N^m)^n, \zeta\eqdef (\zeta^{(1)}, \ldots, \zeta^{(n)}) \in (\N^k)^n : \\
%     & \exists j \leq m: \eta^{(i)} = 0, \zeta^{(i)} = 0 \text{ for } i < j, |\eta^{(i)}| > 0 \text{ for } i \geq j, \\
%     & \textstyle 0 \prec \zeta^{(j)} \prec \ldots \prec \zeta^{(n)}, \big\vert \sum_{i=1}^{n} \eta^{(i)} \vert = n' \text{ and }  \vert \sum_{i=1}^{n} |\eta^{(i)}|\zeta^{(i)} \big\vert = n \Big\} .
% \end{align*}
% \end{theorem}

% \begin{proof}
% We have    
% \begin{align*}
%     \Vert D^\alpha h \Vert_K
%     &\leq
%     \sum_{1 \leq |\beta| \leq n} \Vert D^\beta f\Vert_{g[K]}
%     \sum_{\eta, \zeta \in \calP(\alpha,\beta)} \alpha! 
%     \prod_{j=1}^{n} \frac{
%         \prod_{i=1}^{m}
%         \Vert (D^{\zeta^{(j)}} g)_i \Vert_K^{\eta^{(j)}_i}
%     }{
%         \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%     } \\
%     &\leq
%     \sum_{1 \leq |\beta| \leq n} \Vert D^\beta f\Vert_{g[K]}
%     \sum_{\eta, \zeta \in \calP(\alpha,\beta)} \alpha! 
%     \prod_{j=1}^{n} 
%     \frac{1}{\eta^{(j)}!}
%     \left(\frac{
%         C^g_K(\vert \zeta^{(j)}\vert)
%     }{
%         \zeta^{(j)}!
%     }\right)^{|\eta^{(j)}|}.
% \end{align*}
% Defining 
% \begin{align*}
%     \calP_n(\beta) \eqdef \Big\{ &\eta \eqdef (\eta^{(1)}, \ldots, \eta^{(n)}) \in (\N^m)^n, \zeta\eqdef (\zeta^{(1)}, \ldots, \zeta^{(n)}) \in (\N^k)^n : \\
%     & \exists j \leq m: \eta^{(i)} = 0, \zeta^{(i)} = 0 \text{ for } i < j, |\eta^{(i)}| > 0 \text{ for } i \geq j, \\
%     & \textstyle 0 \prec \zeta^{(1)} \prec \ldots \prec \zeta^{(n)}, \sum_{i=1}^{n} \eta^{(i)} = \beta \text{ and }  \big\vert \sum_{i=1}^{n} |\eta^{(i)}|\zeta^{(i)} \big\vert = n \Big\} .
% \end{align*}
% results in 
% \begin{align*}
%     C^h_K(n)
%     &\leq
%     n!
%     \sum_{1 \leq |\beta| \leq n} \Vert D^\beta f\Vert_{g[K]}
%     \sum_{\eta, \zeta \in \calP_n(\beta)}
%     \prod_{j=1}^{n} 
%     \frac{1}{\eta^{(j)}!}
%     \left(\frac{
%         C^g_K(\vert \zeta^{(j)}\vert)
%     }{
%         \zeta^{(j)}!
%     }\right)^{|\eta^{(j)}|} \\
%     &\leq
%     n!
%     \sum_{1 \leq |\beta| \leq n}  C^f_{g[K]}(\vert \beta \vert)   
%     \sum_{\eta, \zeta \in \calP^{d, k}_{n, |\beta|}}
%     \prod_{j=1}^{n} 
%     \frac{1}{\eta^{(j)}!}
%     \left(\frac{
%         C^g_K(\vert \zeta^{(j)}\vert)
%     }{
%         \zeta^{(j)}!
%     }\right)^{|\eta^{(j)}|} \\
%     & =
%     n!
%     \sum_{n' = 1}^n  \binom{n' + m - 1}{m - 1}  C^f_{g[K]}(n') 
%     \sum_{\eta, \zeta \in \calP^{d, k}_{n, n'}}
%     \prod_{j=1}^{n} 
%     \frac{1}{\eta^{(j)}!}
%     \left(\frac{
%         C^g_K(\vert \zeta^{(j)}\vert)
%     }{
%         \zeta^{(j)}!
%     }\right)^{|\eta^{(j)}|}.
% \end{align*}
% \end{proof}

% \end{comment}
% \begin{comment}
% \begin{corollary}\label{cor:GeneralDerivativeBound2}
%     In the notation of \Cref{thm:GeneralDerivativeBound}, it holds that 
%     \begin{align*}
%         C^h_K(n)
%         \leq
%         \sum_{n' = 1}^n  
%         B(n, n')
%         C^f_{g[K]}(n') 
%         \prod_{l=1}^n \big(1 + C^g_K(l)\big)^{n'} ,
%     \end{align*}
% \end{corollary}
% \begin{proof}
%     Since  $\sum_{i=1}^{s} \vert \eta^{(i)} \vert = n'$, we have
%     \begin{align*}
%         C^h_K(n)
%         &\leq
%         n!
%         \sum_{n' = 1}^n  \binom{n' + m - 1}{m - 1}  C^f_{g[K]}(n') 
%         \sum_{\eta, \zeta \in \calP^{d, k}_{n, n'}}
%         \prod_{j=1}^{n} 
%         \frac{1}{\eta^{(j)}!}
%         \left(\frac{
%             C^g_K(\vert \zeta^{(j)}\vert)
%         }{
%             \zeta^{(j)}!
%         }\right)^{|\eta^{(j)}|} 
%     \\
%         &\leq
%         n!
%         \sum_{n' = 1}^n  \binom{n' + m - 1}{m - 1}  C^f_{g[K]}(n') 
%         \sum_{\eta, \zeta \in \calP^{d, k}_{n, n'}}
%         \prod_{j=1}^{n} 
%         \frac{\big(1 + C^g_K(\vert \zeta^{(j)}\vert)\big)^{|\eta^{(j)}|} }{\eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}}
%     \\
%         &\leq
%         n!
%         \sum_{n' = 1}^n  \binom{n' + m - 1}{m - 1}  C^f_{g[K]}(n') 
%         \sum_{\eta, \zeta \in \calP^{d, k}_{n, n'}}
%         \prod_{j=1}^{n} 
%         \frac{
%         \big(1 + C^g_K(j)\big)^{n'} 
%         }{
%         \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         }
%     \\
%         &=
%         \sum_{n' = 1}^n  \binom{n' + m - 1}{m - 1}  C^f_{g[K]}(n') 
%         \prod_{l=1}^n \big(1 + C^g_K(l)\big)^{n'} 
%         \sum_{\eta, \zeta \in \calP^{d, k}_{n, n'}}
%         \prod_{j=1}^{n} 
%         \frac{
%         n!
%         }{
%         \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         }
%     \end{align*}.
% \end{proof}
% \end{comment}
% \begin{comment}
% \begin{corollary}
%     In the notation of \Cref{cor:GeneralDerivativeBound2}, if there exists an $\Tilde{n} \leq n$ such that $C_K^g(\Tilde{n}) = 0$ it holds that 
%     \begin{align*}
%         C^h_K(n)
%         \leq
%         \sum_{n' = 1}^n  
%         B'(n, n')
%         C^f_{g[K]}(n') 
%         \prod_{l=1}^{\Tilde{n} - 1} \big(1 + C^g_K(l)\big)^{n'}.
%     \end{align*}
%     where 
%     \begin{align*}
%         B'(n, n')
%         \eqdef 
%         \binom{n' + m - 1}{m - 1}
%         \sum_{\eta, \zeta \in \calP^{d, k}_{n, n'}}
%         \prod_{j=1}^{n} 
%         \frac{
%         n! \mathbbm{1}_{\{\zeta^{(j)}<\Tilde{n}\}}
%         }{
%         \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         }.
%     \end{align*}
% \end{corollary}
% \begin{proof}
%     Analogue to \Cref{cor:GeneralDerivativeBound2}.
% \end{proof}
% \end{comment}
% \begin{comment}

% \begin{corollary}[Max derivative]
%     In the notation of \Cref{cor:GeneralDerivativeBound2}, 
%     \begin{align*}
%         C^h_K(n)
%         &\leq
%         \sum_{n' = 1}^n C^f_{g[K]}(n') 
%         (C^g_K)^{n'}
%         B(n, n')
%     \end{align*}
%     where $C^g_K \eqdef \max_{k \in \myset{1}{n}} C^g_K(k)$ and 
%     \begin{align*}
%         B(n, n')
%         \eqdef 
%         \binom{n' + m - 1}{m - 1}
%         \sum_{\eta, \zeta \in \calP^{d, k}_{n, n'}}
%         \prod_{j=1}^{n} 
%         \frac{
%         n!
%         }{
%         \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         }.
%     \end{align*}
% \end{corollary}
% \begin{proof}
%     Follows directly from $\sum_{i=1}^{n}\eta^{(i)} = n'$.
% \end{proof}

% \yannick{I believe this is tighter than \Cref{cor:GeneralDerivativeBound2} and more useful.}

% \end{comment}


% \subsubsection{Universal Bounds}
% \label{ss:UnivBounds}

% \begin{theorem}\label{thm:DerivativeBoundByLevel}
% In the notation of \Cref{thm:FaaDiBruno}, we have for a compact set $K \subseteq \R^k$ and an multi-index $\alpha \in \N^k$, $\vert \alpha \vert = n$,
% \begin{align*}
%         C^h_K(\alpha)
%     \leq
%         \max_{n' \in \myset{1}{n}}
%         C^g_{g[K]}({n'})
%         C^f_K({\cleq n})^{n'}
%         \sum_{1 \leq |\beta| \leq n} 
%         \sum_{\eta, \zeta \in \calP(\alpha,\beta)} \alpha! 
%         \prod_{j=1}^{n} \frac{
%             1
%         }{
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         } 
% \end{align*}
% where $C^h_K(\cdot)$, $C^f_{g[K]}(\cdot)$, $C^g_K(\cdot)$ are defined as in \Cref{not:DerivativeBounds}. 
% \end{theorem}
% \begin{proof}
%     Using \Cref{thm:FaaDiBruno},
%     \begin{align*}
%         C^h_K(\alpha)
%     &\leq
%     \sum_{1 \leq |\beta| \leq n} \Vert D^\beta f\Vert_{g[K]}
%     \sum_{\eta, \zeta \in \calP(\alpha,\beta)} \alpha! 
%     \prod_{j=1}^{n} \frac{
%         \prod_{i=1}^{m}
%         \Vert (D^{\zeta^{(j)}} g)_i \Vert_K^{\eta^{(j)}_i}
%     }{
%         \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%     } 
%     \\
%     &\leq
%     \sum_{1 \leq |\beta| \leq n} 
%     C^g_{g[K]}({|\beta|})
%     \sum_{\eta, \zeta \in \calP(\alpha,\beta)} \alpha! 
%     \prod_{j=1}^{n} \frac{
%         \prod_{i=1}^{m}
%         C^f_K({\cleq n})^{\eta^{(j)}_i}
%     }{
%         \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%     } 
%     \\
%     &\leq
%     \sum_{1 \leq |\beta| \leq n} 
%     C^g_{g[K]}({|\beta|})
%     C^f_K({\cleq n})^{|\beta|}
%     \sum_{\eta, \zeta \in \calP(\alpha,\beta)} \alpha! 
%     \prod_{j=1}^{n} \frac{
%         1
%     }{
%         \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%     } 
%     \\
%     &\leq
%     \max_{n' \in \myset{1}{n}}
%     C^g_{g[K]}({n'})
%     C^f_K({\cleq n})^{n'}
%     \sum_{1 \leq |\beta| \leq n} 
%     \sum_{\eta, \zeta \in \calP(\alpha,\beta)} \alpha! 
%     \prod_{j=1}^{n} \frac{
%         1
%     }{
%         \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%     }.
%     \end{align*}
% \end{proof}

% Next, we refine the strategy used in~\cite{hou2023instance} to convert our uniform risk-bound to a concentration of measure problem. Once done, the remainder of the proof will be to obtain bounds on the rate at which this measure concentrates.

% % \yannick{$k \to n$ $\checkmark$}

% % \yannick{$d \to k$ $\checkmark$}

% % \yannick{$D \to m$ $\checkmark$}

% % \yannick{$m \to \gamma$ $\checkmark$}

% \begin{lemma} 
% \label{lem:mdFDBestimate}
% For $\alpha\in\{1, \cdots, k\}^n$, it satisfies that 
% \begin{align}
%         \sum_{1 \leq |\beta| \leq n} 
%         \sum_{\eta, \zeta \in \calP(\alpha,\beta)} \alpha! 
%         \prod_{j=1}^{n} \frac{1}
%         {
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         } 
%    =  \Big[ \frac{ 2m |\alpha|}{e\ln |\alpha|} ( 1 + o(1) ) \Big]^{|\alpha|}   
%    \notag 
%   %  = 
%  %   \sum \frac{|\alpha|! \, 
%   %( 2 m )^{\sum_{j=1}^{|\alpha|} m_j} }
%   %{m_1! (1!)^{m_1} \cdots m_{|\alpha|}! %(|\alpha|!)^{m_{|\alpha|}}}, \notag 
% \end{align} 
% where $\calP(\alpha, \beta)$ is as defined in Theorem~\ref{thm:FaaDiBruno}. 
% \end{lemma} 
% \begin{proof} 
% Consider functions  
% \begin{align} 
%  & g^{(i)}(x) = g^{(i)}(x_1, \cdots, x_d) \eqdef \exp\big( \sum_{j=1}^d x_j \big) : \, \mathbb{R}^d \to \mathbb{R}, \quad 
%  i = 1, ..., 2m , \notag  \\ 
%  &  f( g^{(1)}, \cdots , g^{(2m)} ) \eqdef \exp\big( \sum_{i=1}^{2m} g^{(i)} \big) : \,  
% \mathbb{R}^{2m} \to \mathbb{R} , \notag 
% \end{align} 
% Since 
% \begin{align} 
%  \frac{\partial }{\partial g^{(i)}} f(g^{(1)}, \cdots , g^{(2m)}) = f(g^{(1)}, \cdots , g^{(2m)}) , \notag 
% \end{align} 
% it follows that 
% \begin{align} 
% &  (D^\beta f)(g^{(1)}(x), \cdots, g^{(2m)}(x)) = f (g^{(1)}(x), \cdots, g^{(2m)}(x)) , \quad 
% \forall \, \beta \in \{1, \cdots, 2m \}^n . \notag  
% \end{align} 


% Since 
%  \begin{align} 
% & \frac{\partial }{\partial x^j }  f(g^{(1)}(x_1, \cdots, x_k), \cdots , g^{(2m)}(x_1, \cdots, x_k))   \notag \\ 
%  =& \sum_{i=1}^{2m} \frac{\partial }{\partial g^{(i)}}   f(g^{(1)}(x_1, \cdots, x_k), \cdots , g^{(2m)}(x_1, \cdots, x_k)) 
%  \frac{\partial g^{(i)}(x_1, \cdots, x_k)}{\partial x_j}    \notag \\ 
%   =& \sum_{i=1}^{2m}    f(g^{(1)}(x_1, \cdots, x_k), \cdots , g^{(2m)}(x_1, \cdots, x_k)) 
%   g^{(i)}(x_1, \cdots, x_k) \notag   \\ 
% = & \sum_{i=1}^{2m} \frac{\partial }{\partial g^{(i)}}   f(g^{(1)}(x), \cdots , g^{(2m)}(x)) 
%  \frac{\partial g^{(i)}(x)}{\partial x_j}    \notag \\ 
%   =&  f(g^{(1)}(x), \cdots , g^{(2m)}(x))  
%   \sum_{i=1}^{2m} g^{(i)}(x)  \notag 
% \end{align} 
% and 
% \begin{align} 
%  &  \frac{\partial g^{(i)}(x_1, \cdots, x_k)}{\partial x_j} = g^{(i)}(x_1, \cdots, x_k) ,  \notag 
% \end{align} 
% we can show by the Fa\`{a} di Bruno formula that 
% \allowdisplaybreaks
% \begin{align} 
%  & D^\alpha f(g^{(1)}(x), \cdots, g^{(2m)}(x)) \notag \\ 
%     &= D^\alpha  \exp\big( \sum_{i=1}^{2m} g^{(i)}(x) \big) \notag \\
%     &=  \sum \frac{|\alpha|!}{\gamma_1! (1!)^{\gamma_1} \cdots \gamma_{|\alpha|}! (|\alpha|!)^{\gamma_{|\alpha|}}} \big( D^{\gamma_1+\cdots + \gamma_{|\alpha|}}  \exp \big) \big( \sum_{i=1}^{2m} g^{(i)}(x) \big)
%   \prod_{j=1}^{|\alpha|} \Big[ m^j (  \sum_{i=1}^{2m} g^{(i)}(x) ) \Big]^{\gamma_j} ,  
%   \notag 
% \end{align} 
% where the summation on the right side of the last equality is over all $|\alpha|$-tuples $(\gamma_1, \cdots, \gamma_{|\alpha|})\geq 0$ such that $1\cdot \gamma_1 + 2\cdot \gamma_2 + \cdots + |\alpha|\cdot \gamma_{|\alpha|}=|\alpha|$.   




% By the multivariate Fa\`a di Bruno formula. For each $n=1$, ..., $s-1$ fixed, and for each $\alpha\in \{1, \cdots, k\}^n$, we have 
% \begin{align} 
% & D^\alpha f(g^{(1)}(x), \cdots, g^{(2m)}(x)) \notag \\ 
% = &
%         \sum_{1 \leq |\beta| \leq n} (D^\beta f)(g^{(1)}(x), \cdots, g^{(2m)}(x))
%         \sum_{\eta, \zeta \in \calP(\alpha,\beta)} \alpha! 
%         \prod_{j=1}^{n} \frac{
%             [D^{\zeta^{(j)}} (g^{(1)}(x), \cdots, g^{(2m)}(x))]^{\eta^{(j)}}
%         }{
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         } .  \notag 
% \end{align} 
% Taking $x = (x_1,\cdots, x_k) = 0$, we have 
% \begin{align} 
%  D^\alpha f(g^{(1)}(0), \cdots, g^{(2m)}(0)) 
%   &=  \sum \frac{|\alpha|!}{\gamma_1! (1!)^{\gamma_1} \cdots \gamma_{|\alpha|}! (|\alpha|!)^{\gamma_{|\alpha|}}} 
%   \exp(2m)
%   \prod_{j=1}^{|\alpha|} ( 2 m )^{\gamma_j} 
%   \notag \\ 
%      (m^\beta f)(g^{(1)}(0), \cdots, g^{(2m)}(0)) &= f (g^{(1)}(0), \cdots, g^{(2m)}(0)) = \exp(2m) , \notag \\ 
%    D^{\zeta^{(j)}} (g^{(1)}(x), \cdots, g^{(2m)}(x)) &= (1, \cdots, 1) . \notag 
% \end{align} 
% Substituting the above derivatives into the Fa\`a di Bruno formula, we obtain 
% \begin{align} 
%   \sum_{1 \leq |\beta| \leq n}  
%         \sum_{\eta, \zeta \in \calP(\alpha,\beta)} \alpha! 
%         \prod_{j=1}^{k} \frac{ 1 }
%         {
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         } 
%     =&  \sum \frac{|\alpha|!}{\gamma_1! (1!)^{\gamma_1} \cdots \gamma_{|\alpha|}! (|\alpha|!)^{\gamma_{|\alpha|}}} 
%   \prod_{j=1}^{|\alpha|} ( 2 m )^{\gamma_j}    \notag \\ 
%   \leq & 
%   (2m)^{|\alpha|} 
%   \sum \frac{|\alpha|!}{\gamma_1! (1!)^{\gamma_1} \cdots \gamma_{|\alpha|}! (|\alpha|!)^{\gamma_{|\alpha|}}} 
%   \notag \\ 
%   =& 
%  (2m)^{|\alpha|}  \Big( \frac{|\alpha|}{e \ln |\alpha| } \Big)^{|\alpha|} (1+o(1))^{|\alpha|} , \notag 
% \end{align} 
% where the last equality follows from \cite[Theorem 2.1]{KO2022}, 
% \begin{align} 
% \sum \frac{|\alpha|!}{\gamma_1! (1!)^{\gamma_1} \cdots \gamma_{|\alpha|}! (|\alpha|!)^{\gamma_{|\alpha|}}} 
% = 
% \Big( \frac{|\alpha|}{e \ln |\alpha| } \Big)^{|\alpha|} (1+o(1))^{|\alpha|} 
% .
%   \notag 
% \end{align} 
% % as $|\alpha| \to \infty$. 
% \end{proof} 


% \begin{corollary}[Level Specific $C^s$-Norm Bounds for Transformer Blocks]\label{cor:DerivativeBoundByLevel}
% In the notation of \Cref{thm:DerivativeBoundByLevel}, it holds for $n \in \N, {n > 1}$ that
% \begin{align*}
%         C^h_K(\cleq n)
%     \leq
%         \max_{n' \in \myset{1}{n}}
%         C^g_{g[K]}({n'})
%         C^f_K({\cleq n})^{n'}
%         \Big[ \frac{ 2m n}{e\ln n} ( 1 + o(1) ) \Big]^{n}.
% \end{align*}
% and if $C^f_K({\cleq n}) \geq 1$, 
% \begin{align*}
%         C^h_K(\cleq n)
%     \leq
%         C^g_{g[K]}({\cleq n})
%         C^f_K({\cleq n})^{n}
%         \Big[ \frac{ 2m n}{e\ln n} ( 1 + o(1) ) \Big]^{n}.
% \end{align*}
% \end{corollary}
% \begin{proof}
%     Follows directly from \Cref{thm:DerivativeBoundByLevel} and \Cref{lem:mdFDBestimate}.
% \end{proof}









% \subsubsection{Bounds in Derivative Type}
% \label{ss:BoDerType}

% The goal of this section is to bound the derivative of composite functions by grouping with respect to $\eqorder$, defined in \Cref{not:Order}.
% \begin{theorem}\label{thm:DerivativeBoundByType}
% In the notation of \Cref{thm:FaaDiBruno}, we have for a compact set $K \subseteq \R^k$ and an ordered multi-index $\alpha \in \Order^k_{n}$
% \begin{align*}
% C^h_K(\alpha)
%     &\leq
%     \alpha! \sum_{\beta \in \Order^m_{\leq n}}  N(\beta) C^f_{g[K]}(\beta)
%     \sum_{\eta, \zeta \in \calP'(\alpha,\beta)} 
%     \prod_{j=1}^{n} \frac{
%         C^g_K(\order(\zeta^{(j)}))^{\vert \eta^{(j)} \vert}
%     }{
%         \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%     },
% \end{align*}
% where $C^h_K(\cdot)$, $C^f_{g[K]}(\cdot)$, $C^g_K(\cdot)$ are defined as in \Cref{not:DerivativeBounds}; and 
% \begin{multline*}
%     \calP'(\alpha, \beta) = \Big\{ \eta \eqdef (\eta^{(1)}, \ldots, \eta^{(n)}) \in (\N^m)^n, \zeta\eqdef (\zeta^{(1)}, \ldots, \zeta^{(n)}) \in (\N^k)^n : \\
%     \exists j \leq m: \eta^{(i)} = 0, \zeta^{(i)} = 0 \text{ for } i < j, |\eta^{(i)}| > 0 \text{ for } i \geq j, \\
%     \textstyle 0 < \zeta^{(j)} \vartriangleleft \ldots \vartriangleleft \zeta^{(n)}, \sum_{i=1}^{n} \eta^{(i)} = \beta \text{ and } \sum_{i=1}^{n} |\eta^{(i)}|\zeta^{(i)} = \alpha \Big\} ,
% \end{multline*}
% where $\alpha \vartriangleleft \beta$ for $\alpha, \beta \in \N^k$ if $\vert \alpha \vert \leq \vert \beta \vert$ and  $\alpha \neq \beta$.
% \end{theorem}
% \begin{proof}
% We have for $\alpha \in \Order^k_{n}$
% \begin{align*}
%     C^h_K(\alpha)
%     &\leq
%     \max_{\gamma \eqorder \alpha}
%     \sum_{1 \leq |\beta| \leq n} \Vert D^\beta f\Vert_{g[K]}
%     \sum_{\eta, \zeta \in \calP(\gamma,\beta)} \alpha! 
%     \prod_{j=1}^{n} \frac{
%         \prod_{i=1}^{m}
%         \Vert (D^{\zeta^{(j)}} g)_i \Vert_K^{\eta^{(j)}_i}
%     }{
%         \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%     } \\
%     &\leq
%     \sum_{1 \leq |\beta| \leq n} C^f_{g[K]}(\order (\beta))
%     \max_{\gamma \eqorder \alpha}
%     \sum_{\eta, \zeta \in \calP(\gamma,\beta)} \alpha! 
%     \prod_{j=1}^{n} \frac{
%         C^g_K(\order(\zeta^{(j)}))^{\vert \eta^{(j)} \vert}
%     }{
%         \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%     }.
% \end{align*}
% Then 
% \begin{align*}
%     \mySet{\eta, (\order(\zeta^{(1)}), ..., \order(\zeta^{(n)}))}{ (\eta, \zeta) \in \calP'(\alpha, \beta)}
% \end{align*}
% is invariant in $\alpha$ with respect to $\eqorder$ and thus
% \begin{align*}
%     C^h_K(\alpha)
%     &\leq
%     \sum_{1 \leq |\beta| \leq n} C^f_{g[K]}(\order (\beta))
%     \sum_{\eta, \zeta \in \calP'(\alpha,\beta)} \alpha! 
%     \prod_{j=1}^{n} \frac{
%         C^g_K(\order(\zeta^{(j)}))^{\vert \eta^{(j)} \vert}
%     }{
%         \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%     }.
% \end{align*}
% Further, notice that
% \begin{align*}
%     \mySet{((\vert \eta^{(1)}\vert, \eta^{(1)}!), \ldots, (\vert \eta^{(n)}\vert, \eta^{(n)}!)), \zeta}{ (\eta, \zeta) \in \calP'(\alpha, \beta)}
% \end{align*}
% is invariant in $\beta$ with respect to $\eqorder$ and the assertion follows.
% \end{proof}

% \begin{corollary}\label{cor:DerivativeBoundAffine}
%     In the notation of \Cref{thm:DerivativeBoundByType}, if $f$ is affine-linear, 
%     \begin{align*}
%         C^h_K(\alpha)
%         &\leq
%         m \alpha! C^f_{g[K]}(e_1)
%         C^g_K(\alpha),
%     \end{align*}
%     where $C^f_{g[K]}(e_1)$ is the maximum weight of the matrix representing $f$. 
% \end{corollary}
% \begin{proof}
%     \Cref{thm:DerivativeBoundByType} yields
%     \begin{align*}
%         C^h_K(\alpha)
%         &\leq
%         m \alpha! C^f_{g[K]}(e_1)
%         \sum_{\eta, \zeta \in \calP'(\alpha,\beta)} 
%         \prod_{j=1}^{n} \frac{
%             C^g_K(\order(\zeta^{(j)}))^{\vert \eta^{(j)} \vert}
%         }{
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         },
%     \end{align*}
%     and since $\calP'(\alpha, e_1) = \{(0, ..., 0, e_1), (0, ..., 0, \alpha) \}$ the result follows.
% \end{proof}

% \begin{comment}
% \subsection{Special Cases}

% \begin{corollary}[Affine linear transformations]
% In the notation of \Cref{thm:GeneralDerivativeBound}, if $f$ is affine-linear, 
%     \begin{align*}
%         C^h_K(n)
%         &\leq
%         C^f_{g[K]}(1) 
%         C^g_K(n)
%         \sum_{\vert \alpha \vert = n}
%         \frac{
%         m \cdot n! 
%         }{
%             \alpha !
%         }.
%     \end{align*}
% \end{corollary}
% \begin{proof}
%     \Cref{thm:GeneralDerivativeBound} yields
%     \begin{align*}
%         C^h_K(n)
%         &\leq
%         n!
%         \sum_{n' = 1}^n  \binom{n' + m - 1}{m - 1}  C^f_{g[K]}(n') 
%         \sum_{\eta, \zeta \in \calP^{d, k}_{n, n'}}
%         \prod_{j=1}^{n} 
%         \frac{1}{\eta^{(j)}!}
%         \left(\frac{
%             C^g_K(\vert \zeta^{(j)}\vert)
%         }{
%             \zeta^{(j)}!
%         }\right)^{|\eta^{(j)}|}.
%     \end{align*}
%     Since $C^f_{g[K]}(n') = 0$  for $n'>1$, 
%     \begin{align*}
%         C^h_K(n)
%         &\leq
%         m \cdot n! \cdot
%           C^f_{g[K]}(1) 
%         \sum_{\eta, \zeta \in \calP^{d, k}_{n, 1}}
%         \prod_{j=1}^{n} 
%         \frac{1}{\eta^{(j)}!}
%         \left(\frac{
%             C^g_K(\vert \zeta^{(j)}\vert)
%         }{
%             \zeta^{(j)}!
%         }\right)^{|\eta^{(j)}|}.
%     \end{align*}
%     The definition of $\calP^{d, k}_{n, 1}$ forces $\zeta^{(j)}, \eta^{(j)} = 0$ for $j < n$, $|\eta^{(n)}| = \eta^{(n)}! = 1$, as well as $\vert \zeta^{(n)}\vert = n$, which yields
%     \begin{align*}
%         C^h_K(n)
%         &\leq
%         m \cdot n! \cdot
%           C^f_{g[K]}(1) 
%         \sum_{\eta, \zeta \in \calP^{d, k}_{n, 1}}
%         \left(\frac{
%             C^g_K(n)
%         }{
%             \zeta^{(n)}!
%         }\right)\\
%         &\leq
%         C^f_{g[K]}(1) 
%         C^g_K(n)
%         \sum_{\vert \alpha \vert = n}
%         \frac{
%         m \cdot n! 
%         }{
%             \alpha !
%         }.
%     \end{align*}
% \end{proof}
% \end{comment}

% \begin{comment}
% \subsection{Combinatorics}

% Recall 
%     \begin{align*}
%         B(n, n')
%         \eqdef 
%         \binom{n' + m - 1}{m - 1}
%         \sum_{\eta, \zeta \in \calP^{d, k}_{n, n'}}
%         \prod_{i=1}^{n} 
%         \frac{
%         n!
%         }{
%         \eta^{(i)}!(\zeta^{(i)}!)^{|\eta^{(i)}|}
%         }.
%     \end{align*}
% where
%     \begin{align*}
%     \calP^{d, k}_{n, n'} 
%     = \Big\{ &\eta \eqdef (\eta^{(1)}, \ldots, \eta^{(n)}) \in (\N^m)^n, \zeta\eqdef (\zeta^{(1)}, \ldots, \zeta^{(n)}) \in (\N^k)^n : \\
%     & \exists j \leq m: \eta^{(i)} = 0, \zeta^{(i)} = 0 \text{ for } i < j, |\eta^{(i)}| > 0 \text{ for } i \geq j, \\
%     & \textstyle 0 \prec \zeta^{(j)} \prec \ldots \prec \zeta^{(n)},  \sum_{i=1}^{n} \vert \eta^{(i)} \vert = n' \text{ and }  \vert \sum_{i=1}^{n} |\eta^{(i)}|\zeta^{(i)} \big\vert = n \Big\} .
%     \end{align*}
% This yields
% \begin{align*}
%     B(n, n') = 
%         \binom{n' + m - 1}{m - 1}
%         \sum_{j=1}^n
%         \sum_{\eta \in E^{d, k}_{n, n', j}}
%         \sum_{\zeta \in Z^{d, k}_{n, n', j}(\eta) }
%         \prod_{i=1}^{n} 
%         \frac{
%         n!
%         }{
%         \eta^{(i)}!(\zeta^{(i)}!)^{|\eta^{(i)}|}
%             },
% \end{align*}
% where 
% \begin{align*}
%     E^{d, k}_{n, n', j} 
%     = \Big\{ &\eta \eqdef (\eta^{(1)}, \ldots, \eta^{(n)}) \in (\N^m)^n: \\
%     & \eta^{(i)} = 0 \text{ for } i < j, |\eta^{(i)}| > 0 \text{ for } i \geq j, 
%     \textstyle  \sum_{i=1}^{n} \vert \eta^{(i)} \vert = n' \Big\} ,
%     \\
%     Z^{d, k}_{n, n', j}(\eta) 
%     = \Big\{ &\eta \eqdef (
%     \zeta\eqdef (\zeta^{(1)}, \ldots, \zeta^{(n)}) \in (\N^k)^n : \\
%     & \zeta^{(i)} = 0 \text{ for } i < j, 
%     \textstyle 0 \prec \zeta^{(j)} \prec \ldots \prec \zeta^{(n)}, \text{ and }  \sum_{i=1}^{n} |\eta^{(i)}|\vert \zeta^{(i)} \vert = n \Big\} .
% \end{align*}
% With writing $\eta! \eqdef \prod_{i=1}^n \eta^{(i)}!$, we arrive at 
% \begin{align*}
%      B(n, n') &= 
%         \binom{n' + m - 1}{m - 1}
%         \sum_{j=1}^n
%         \sum_{\eta \in E^{d, k}_{n, n', j}}
%         \frac{1}{\eta!}
%         \sum_{\zeta \in Z^{d, k}_{n, n', j}(\eta) }
%         \prod_{i=1}^{n} 
%         \frac{
%         n!
%         }{
%         (\zeta^{(i)}!)^{|\eta^{(i)}|}
%         }. \\
%         &= 
%         \binom{n' + m - 1}{m - 1}
%         \sum_{j=1}^n
%         \sum_{\substack{\gamma \in \N^n , \vert \gamma \vert = n'}}
%         D(\gamma)
%         \sum_{\zeta \in Z^{d, k}_{n, n', j}(\gamma) }
%         \prod_{i=1}^{n} 
%         \frac{
%         n!
%         }{
%         (\zeta^{(i)}!)^{\gamma_i}
%         },
% \end{align*}
% where 
% \begin{align*}
%     D(\gamma) \eqdef  \sum_{{\eta \in E^{d, k}_{n, n', j} , \vert \eta^{(i)}\vert = \gamma_i }}
%         \frac{1}{\eta!}.
% \end{align*}
    
% \end{comment}






% \subsection{Step 1 - Concentration of Measure\texorpdfstring{ - Bounding the Right-Hand Side of~\eqref{eq:risk_bound__decomposition}}{}}
% \label{s:Proofs__ss:ConcentrationProof}

% We are now ready to derive our main concentration of measure results used to derive our risk-bound.  This corresponds to bounding term~\ref{eq:risk_bound__decomposition} by controlling the integral probability term $d_s(\mu_t,\mu^{(N)}$ in~\eqref{eq:risk_bound__decomposition2}, with high probability, where the randomness is due to the randomness of the empirical measure $\mu^{(N)}$.

% Instead of the compact support Assumption~\ref{ass:Comp_Support}, our concentration of measure rate, with the same convergence rate, holds under the following weaker condition.
% \begin{assumption}[Exponential Moments]
% \label{ass:Exp_Moment}
% There exist $\lambda,\tilde{C}>0$ and $\gamma\in (0,1)$ such that: for each $x\in \mathcal{X}$ we have $\mathbb{E}_{X\sim P(x,\cdot)}[e^{\lambda|X|}]\le \gamma\, e^{\lambda|x|}+\tilde{C}$.
% \end{assumption}
% Before formulating our concentration result, we remark that Assumption~\ref{ass:Comp_Support} implies~\ref{ass:Exp_Moment}, but not conversely.

% \begin{proposition}[Excess Risk-Bound]
% \label{prop:Concentation}
% Under Assumptions~\ref{ass:MC} and~\ref{ass:Exp_Moment}, let $f^{\star}:\mathbb{R}^d\to \mathbb{R}^D$, $\ell:\mathbb{R}^{2D}\to \mathbb{R}$, and $R,r>0$ be a such that the composite map $\mathbb{R}^d\ni x\mapsto \ell(f^{\star}(x),f(x))$ belongs to $\mathcal{C}_{R}^s(\mathbb{R}^d)$ for all $f\in C^2_r(\mathbb{R}^d)$.
% % \hfill\\
% Then, there exists some $\kappa\in(0,1)$ depending only on the Markov chain $X_{\cdot}$ and some $t_0\in \mathbb{N}_0$ such that for each $t_0\le N < t \le \infty$, each ``rate-to-constant-tradeoff parameter'' $s\in \mathbb{N}_+$, and every ``confidence level'' $\delta \in (0,1]$ the following
% \begin{align*}
%         \sup_{g\in \mathcal{C}^s_R(\mathbb{R}^d)}
%         \,
%         \frac{
%             \big|
%                 \mathcal{R}_{\max\{t,N\}}(g)-\mathcal{R}^{(N)}(g)
%             \big|
%         }{R}
%     \lesssim
%             %% Time-Shift Term
%                 % I_{t<\infty}\,
%                 \kappa^t\,
%             +
%                 %%% Concentration Term
%                 \frac{
%                     \sqrt{2\ln(1/\delta)}
%                 }{
%                     N^{1/2}
%                 }
%                 %%% Mean Term
%                 +\,
%                 %%% NEW: Generate Rate
%                 \begin{cases}
%                    \frac{
%                        \log\big(
%                             c\, N
%                         \big)^{d/(2s + 1)}
%                    }{
%                         c\, N^{1/2}
%                    } 
%                     & \mbox{ if } 
%                     % 1=
%                     d<2s\\
%                    %%%%
%                    \frac{
%                        \log\big(
%                             c\, N
%                         \big)
%                    }{
%                         c\, N^{1/2}
%                    } 
%                     & \mbox{ if } d=2s\\
%                 %%%%
%                    \frac{
%                        \log\big(
%                             c\, N
%                         \big)^{d-2s+(s/d)}
%                    }{
%                        c_2\,  N^{s/d}
%                    } 
%                     & \mbox{ if } d=2s\\
%                 \end{cases}
% \end{align*}
% holds with probability at least $1-\delta$; where $0<\kappa <1$, and we use the notation $\kappa^{\infty}\eqdef 0$.
% \end{proposition}


% \begin{proof}[{Proof of Proposition~\ref{prop:Concentation}}]
% % \hfill\\
% % \noindent\textbf{Computing the $C^s$-norms of $\ell(f,\hat{f})$}
% % \AK{Need Xuwei's Lemma here}
% By hypothesis, $\tilde{f}\in C^s_r(\mathbb{R}^d)$ the induced map
% \begin{equation}
% \label{eq:composite_to_concentrate}
% \begin{aligned}
% f:  \mathbb{R}^{d}& \to \mathbb{R} \\
% x & \mapsto f(x)\eqdef \ell\big(f^{\star}(x),\tilde{f}(x)\big)
% \end{aligned}
% \end{equation}
% belongs to $C_R^s(\mathbb{R}^d)$.

% % \hfill\\
% \paragraph{Conversion to a Concentration of Measure Problem.}
% Denote the empirical (random) measure associated with the samples $\{(X_n,Y_n)\}_{n=1}^N$ by $\mu^{(N)}\eqdef \frac1{N}\sum_{n=1}^N\, \delta_{(X_n,Y_n)}$.
% Note that the generalization bound is $0$ for any constant function; therefore, we consider the bound over $C_R^s(\mathbb{R}^d)\setminus \operatorname{Lip}_0$ where $\operatorname{Lip}_0$ denotes the set of constant functions from $\mathbb{R}^d$ to $\mathbb{R}$.  Note the bijection between $C_R^s(\mathbb{R}^d)\setminus \operatorname{Lip}_0$ and $C_1^s(\mathbb{R}^d)\setminus \operatorname{Lip}_0$ given by $f\mapsto \frac1{\max\{1,\|f\|_{C^s(\mathbb{R}^d)}\}} f$.  Therefore, we compute
% \allowdisplaybreaks
% \begin{align}
% \nonumber
%         \big|
%             \mathcal{R}_{
%             t%\max\{t,N\}
%             }(f)-\mathcal{R}^{(N)}(g)
%         \big|
%     \le &
%         \sup_{g\in \mathcal{C}^s_R(\mathbb{R}^d)}
%         \,
%         \big|
%             \mathcal{R}_{
%             t%\max\{t,N\}
%             }(f)-\mathcal{R}^{(N)}(g)
%         \big|
% \\
% \nonumber
%     \le &
%         R\,
%         \sup_{g\in \mathcal{C}^s_1(\mathbb{R}^d)}
%         \,
%         \big|
%             \mathcal{R}_{
%             t%\max\{t,N\}
%             }(g)-\mathcal{R}^{(N)}(g)
%         \big|
%     \\
% \nonumber
%     \le &
%         R\, d_{C^s}(\mu_{\max\{t,N\}},\mu^{(N)})
%     \\
%     \label{eq:TB_Bounded}
%     \le &
%         R\, \big(
%             \underbrace{
%                 d_{C^s}(\mu_{
%                 t%\max\{t,N\}
%                 },\bar{\mu})
%             }_{\term{term_II}}
%     % \\
%     % &
%         +
%             \underbrace{
%                 d_{C^s}(\bar{\mu},\mu^{(N)})
%             }_{\term{term_I}}
%     \big)
% .
% \end{align}
% Next, we bound terms $\text{(I)}$ and $\text{(II)}$.  

% \paragraph{Bounding Term~\eqref{term_II}.}
% Under the log-Sobolev Assumption~\ref{ass:MC},~\cite[Theorem 1.3]{BobkovGotze_1999_JFA} can be applied to $\bar{\mu}$ and $P(x,\cdot)$ for each $x\in \mathcal{X}$, implying that the transport inequalities hold: for each $\nu\in\mathcal{P}(\mathcal{X})$ and each $\tilde{\mu}\in \{\bar{\mu},\mu_0\}\cup \{P(x,\cdot)\}_{x\in \mathcal{X}}$
% \begin{equation}
% \label{eq:term_II__transport_inequalities}
%     \mathcal{W}_1(\tilde{\mu},\nu)^2
% \le 
%     2C^2\, \operatorname{KL}(\nu|\tilde{\mu})
% \end{equation}
% where we recall the definition of the Kullback–Leibler divergence $\operatorname{KL}(\nu|\mu)\eqdef \mathbb{E}_{X\sim \nu}[\log(\frac{d\nu}{d\mu}(X))]$.  Thus,~\eqref{eq:term_II__transport_inequalities} implies that the following exponential contractility property of the Markov kernel: there exists some $\kappa \in (0,1)$ such that for each $x,\tilde{x}\in \mathcal{X}$ and every $t\in \mathbb{N}_+$
% \begin{equation}
% \label{eq:exp_contract}
%     \mathcal{W}_1\big(P^t(x,\cdot),P^t(\tilde{x},\cdot)\big)
%     \le 
%     \kappa^t\, \|x-\tilde{x}\|
%     .
% \end{equation}
% Furthermore,~\eqref{eq:exp_contract} implies that 
% the conditions for~\citep[Theorem 1.5]{Riekert_ConcentrationOfMeasure2022} are met; whence, for every $\varepsilon\ge 0$ and each $N\in \mathbb{N}$ the following holds with probability at-least $
% 1-\exp\big(\frac{-N\,\varepsilon^2(1-\kappa)^2}{2C^2}\big)
% $
% \begin{equation}
% \label{eq:term_II__concentration}
%         \eqref{term_II}
%     =
%         d_s(\bar{\mu},\mu^{(N)})
%     \le 
%         \mathbb{E}\big[d_s(\bar{\mu},\mu^{(N)})\big]
%         +
%         \varepsilon
% ,
% \end{equation}
% for some $C>0$.
% Upon setting $\varepsilon \eqdef 
% \frac{C\sqrt{2\ln(1/\delta)}}{\sqrt{N\,(1-\kappa^2)}}$,~\eqref{eq:term_II__concentration} implies that: for every $N\in \mathbb{N}$ and each $\delta \in (0,1]$ the following holds with probability at-least $1-\delta$
% \begin{equation}
% \label{eq:term_II__concentration___mod}
%         \eqref{term_II}
%     =
%         d_s(\bar{\mu},\mu^{(N)})
%     \le 
%         \underbrace{
%             \mathbb{E}\big[d_s(\bar{\mu},\mu^{(N)})\big]
%         }_{\term{term_III}}
%         +
%         \frac{C\sqrt{2\ln(1/\delta)}}{\sqrt{N\,(1-\kappa^2)}}
% .
% \end{equation}
% It remains to bound the expectation term~\eqref{term_III} in~\eqref{eq:term_II__concentration___mod} to bound term~\eqref{term_II}.

% Under the exponential moment assumption~\ref{ass:Exp_Moment}, we have that
% \begin{equation}
% \label{eq:exp_moment_repackaged}
% \mathbb{E}_{X\sim P(x,\cdot)}[e^{\beta|X|}-1]\le \gamma\, (e^{\beta|x|}-1) + (C-1+\gamma)
% .
% \end{equation}
% Therefore \citep[Proposition 1.3]{Riekert_ConcentrationOfMeasure2022}, implies that $\sup_{t\in \mathbb{N}_0}\, \mathbb{E}[e^{\beta|X_t|}-1]<\infty$.  Whence, \citep[Assumption 2]{Riekert_ConcentrationOfMeasure2022} holds with Young function $\Phi(x)=\frac1{\max\{1,\sup_{t\in \mathbb{N}_+\}}\mathbb{E}[e^{\beta|X_t}-1]}\,(e^{\beta|X_t|}-1)$; namely, $\sup_{t\in \mathbb{N}_0}\, \mathbb{E}[\Phi(|X_t|)]\le 1$.  Consequentially,~\citep[Theorem 1.1]{Riekert_ConcentrationOfMeasure2022} applies from which we conclude that there is some $t_0\in \mathbb{N}_+$ such that for all $N\ge t_0$
% \begin{equation}
% \label{eq:Bound_on_Expectation}
%     \eqref{term_III}
%     =
%     \mathbb{E}\big[d_s(\bar{\mu},\mu^{(N)})\big]
%     \lesssim
%     \,
%     \log\big(
%         (1-\kappa)\, N
%     \big)^{s}
%     \,
%     %%% NEW: Generate Rate
%         \begin{cases}
%            \frac{
%                \log\big(
%                     (1-\kappa)\, N
%                 \big)^{d/(2s) + 1}
%            }{
%                 (1-\kappa)^{1/2}\, N^{1/2}
%            } 
%             & \mbox{ if } 1=d<2s\\
%            %%%%
%            \frac{
%                \log\big(
%                     (1-\kappa)\, N
%                 \big)
%            }{
%                 (1-\kappa)^{1/2}\,N^{1/2}
%            } 
%             & \mbox{ if } d=2s\\
%         %%%%
%            \frac{
%                \log\big(
%                     (1-\kappa)\, N
%                 \big)^{d-2s+s/d}
%            }{
%                 (1-\kappa)^{s/d}\, N^{s/d}
%            } 
%             & \mbox{ if } d=2s\\
%         \end{cases}
% .
% \end{equation}


% Combining the order estimate of~\eqref{term_III} in~\eqref{eq:Bound_on_Expectation} with the estimate in~\eqref{eq:term_II__concentration___mod} implies that: for every $N\ge t_0$ and each $\delta \in (0,1]$ we have
% \begin{equation}
% \label{eq:term_II__concentration___done}
%         \eqref{term_II}
%     =
%         d_s(\bar{\mu},\mu^{(N)})
%     \lesssim
%         \,
%         %%% Concentration Term
%         \frac{
%             \sqrt{2\ln(1/\delta)}
%         }{
%             N^{1/2}
%         }
%         %%% Mean Term
%         +\,
%         %%% NEW: Generate Rate
%             \begin{cases}
%                \frac{
%                    \log\big(
%                         c\, N
%                     \big)^{d/(2s) + 1}
%                }{
%                     c\, N^{1/2}
%                } 
%                 & \mbox{ if } 1=d<2s\\
%                %%%%
%                \frac{
%                    \log\big(
%                         c\, N
%                     \big)
%                }{
%                     c\, N^{1/2}
%                } 
%                 & \mbox{ if } d=2s\\
%             %%%%
%                \frac{
%                    \log\big(
%                         c\, N
%                     \big)^{d-2s+s/d}
%                }{
%                    c_2\,  N^{s/d}
%                } 
%                 & \mbox{ if } d=2s\\
%             \end{cases}
% \end{equation}
% where $c\eqdef (1-\kappa), c_2\eqdef c^{s/d}\in (0,1)$, and $\lesssim$ suppresses the absolute constant $\max\{1,C\}>0$.

% \paragraph{Bounding Term~\eqref{term_I}.}
% Next, we bound~\eqref{term_I} by computing
% \allowdisplaybreaks
% \begin{align}
% \nonumber
%     \eqref{term_I} = 
%         d_{C^s}(\mu_{
%         t%\max\{t,N\}
%         },\bar{\mu})
%     \eqdef &
%         \sup_{g\in \mathcal{C}^s_1(\mathbb{R}^d)}\, \mu_{
%         t%\max\{t,N\}
%         }[g]-\bar{\mu}[g]
% \\
%     \le & 
%     \label{eq:inclusion_CsLip}
%         \sup_{g\in \operatorname{Lip}_1(\mathbb{R}^d)}\, \mu_{
%         t%\max\{t,N\}
%         }[g]-\bar{\mu}[g]
% \\
%     = & 
%     \label{eq:KRDuality}
%         \mathcal{W}_1(\mu_{
%         t%\max\{t,N\}
%         },\bar{\mu})
% \\
%     = & 
%     % \label{eq:stationarity}
%         \mathcal{W}_1(P^t\mu_0,\bar{\mu})
% \\
%     = & 
%     \label{eq:stationarity}
%         \mathcal{W}_1(P^t\mu_0,P^t\bar{\mu})
% \\
%     \le & 
%     \label{eq:exp_contract2}
%         \kappa^t\, 
%         \mathcal{W}_1(\mu_0,\bar{\mu})
%     \eqdef 
%         \kappa^t\,C
% \end{align}
% where~\eqref{eq:inclusion_CsLip} held by definition of the MMD $d_{C^s}$ and by the inclusion of $\mathcal{C}_1^s(\mathbb{R}^d)\subset \operatorname{Lip}_1(\mathbb{R}^d)$,~\eqref{eq:KRDuality} held by Kantorovich duality (see \citep[Theorem 5.10]{VillaniBook_2009}),~\eqref{eq:stationarity} held since $\bar{\mu}$ is the stationary probability measure for the Markov chain $X_{\cdot}$, it is invariant to the action of the Markov kernel, and~\eqref{eq:exp_contract2} followed from \citep[Corollary 21]{olivera2019density} since we deduced the exponential contractility property~\eqref{eq:exp_contract} of the Markov kernel.  Note that $C\eqdef \mathcal{W}_1(\mu_0,\bar{\mu})$ is a constant depending only on the initial and stationary distributions of the Markov chain.

% \paragraph{Conclusion.}
% Incorporating the estimates for~\eqref{term_I} and~\eqref{term_II} into the right-hand side of~\eqref{eq:TB_Bounded} implies that: for every $t,N\ge t_0$, $s\in \mathbb{N}_+$, and each $\delta\in (0,1]$ the following holds
% \begin{align*}
% \resizebox{1\linewidth}{!}{$%% BEGIN RESIZE BOX$}
% \begin{aligned}
%         \sup_{g\in \mathcal{C}^s_R(\mathbb{R}^d)}
%         \,
%         \frac{
%             \big|
%                 \mathcal{R}_{\max\{t,N\}}(g)-\mathcal{R}^{(N)}(g)
%             \big|
%         }{R}
%     \lesssim &
%             %% Time-Shift Term
%                 I_{t<\infty}\,\kappa^t\,
%             +
%                 %%% Concentration Term
%                 \frac{
%                     \sqrt{2\ln(1/\delta)}
%                 }{
%                     N^{1/2}
%                 }
%         %%% Mean Term
%                 +\,
%                 %%% NEW: Generate Rate
%                 \begin{cases}
%                    \frac{
%                        \log\big(
%                             c\, N
%                         \big)^{d/(2s + 1)}
%                    }{
%                         c\, N^{1/2}
%                    } 
%                     & \mbox{ if } 1=d<2s\\
%                    %%%%
%                    \frac{
%                        \log\big(
%                             c\, N
%                         \big)
%                    }{
%                         c\, N^{1/2}
%                    } 
%                     & \mbox{ if } d=2s\\
%                 %%%%
%                    \frac{
%                        \log\big(
%                             c\, N
%                         \big)^{d-2s+(s/d)}
%                    }{
%                        c_2\,  N^{s/d}
%                    } 
%                     & \mbox{ if } d=2s\\
%                 \end{cases}
% \end{aligned}
% $}
% \end{align*}
% with probability at-least $1-\delta$; where $c\eqdef (1-\kappa)$ and $\kappa\in (0,1)$; where $I_{t<\infty}k^{\infty}\eqdef 0$ if $t=\infty$.
% \end{proof}


% \subsection{Step 2 (A) - Bounding the \texorpdfstring{$C^s$}{Cs} Regularity of Transformer Building Blocks}
% \label{sec:RegularityTransfomerBuildingBlocks}

% We begin by the following simple remark, that if the activation function used to defined the transformer is smooth, then so must the entire transformer model.
% \begin{proposition}[Transformers with Smooth Activation Functions are Smooth]
% \label{prop:TransformerIsSmooth}
%     Fix $D, d, M, L, H, C$, as in \Cref{defn:Transformer}, then every transformer $\transformer \in \transformerclass_{L,H,C}^{D,d,M}$ is smooth.
% \end{proposition}

% \begin{proof}[{Theorem~\ref{prop:TransformerIsSmooth}}]
%     The smoothness of $\attention$ follows directly from the smoothness of $\softmax$, which immediately implies smoothness of $\multihead$ since the operators used for its definition are smooth. Furthermore, the $\layernorm$ is smooth due to its smooth and lower-bounded denominator and the activation function $\sigma$ is smooth by definition, therefore we conclude that $\tblock \in \tblock_{d',M',H'}$ is smooth for every $d', M', H' \in \N$ and we obtain smoothness of $\transformer \in \transformer_{L,W,H}^{D,d,M}$ as a consequence.
% \end{proof}


% \subsubsection{The Softmax Function}
% \begin{lemma}[Representation of higher-order $\softmax$ derivatives]\label{lem:SoftmaxDerivativeRepresentation}
% For $F \in \N$ and
% \begin{align*}%\label{id:Softmax}
%     \smax:
%             \R^F 
%         \to     
%             \R^F,
%     \quad 
%             x 
%         \mapsto 
%             \left(
%                     {\exp(x_i)}
%                 /
%                     {\textstyle\sum_{j = 0}^{F-1} \exp(x_j)}
%             \right)_{i=1}^{F}.
% \end{align*}
% there exists for any multi-index $\alpha \in \N^F$ and $m \in \myset{1}{F}$ indicators $(a_{i, j}^k)_{i, j \in I(\alpha)}^{k \in \myset{1}{\vert \alpha \vert!}} \subseteq \{0, 1\}$ such that 
% \begin{align}
%     \smax^{(\alpha)} (x_m) = \sum_{k = 1}^{\vert \alpha \vert!} \smax(x_{m}) \prod_{i,j \in I(\alpha)} (a^k_{i,j}  - \smax(x_{j})), \label{id:SoftmaxDerivativeShape}
% \end{align}
% where $I(\alpha)\eqdef \{(i, j): i = 1, \ldots, F, j = 1, \ldots, \alpha_i\}$.
% \end{lemma}
% \begin{proof}
%     For $\vert \alpha \vert = 0$, we have $n \in \myset{1}{F}$ s.t. $\alpha_n = 1$, therfore 
%     \begin{align*}
%         \smax^{(\alpha)} (x_m) = \frac{\partial \smax}{\partial x_{n}} (x_{m}) = \smax(x_{m})\left( \delta_{m n} - \smax(x_{n})\right),
%     \end{align*}
%     which is of the form \eqref{id:SoftmaxDerivativeShape}. Now, let $\alpha \in \N^F$ arbitrary, therefore, by defining $\alpha' \in \N^F$ by $\alpha'_i \eqdef \alpha_i$ for $i \neq n$ and $\alpha'_n \eqdef \alpha_n - 1$ (w.l.o.g. $\alpha_n > 0$). We have 
%     \begin{align*}
%         \smax^{(\alpha)} (x_m) 
%         & = \frac{\partial \smax^{(\alpha')}}{\partial x_{n}} (x_{m}) \\
%         & = \frac{\partial}{\partial x_{n}} \sum_{k = 1}^{\vert \alpha' \vert!} \smax(x_{m}) \prod_{i,j \in I(\alpha')}(a^{\prime k}_{i,j}  - \smax(x_{j})).
%     \end{align*}
%     Since for any $k$
%     \begin{align*}
%         & \frac{\partial}{\partial x_{n}} \smax(x_{m}) \prod_{i,j \in I(\alpha')}(a^{\prime k}_{i,j}  - \smax(x_{j})) \\
%         & = \smax(x_{m})\left( \delta_{m n} - \smax(x_{n})\right)  \prod_{i,j \in I(\alpha')} (a^{\prime k}_{i,j}  - \smax(x_{j})) \\ 
%         & \quad +  \smax(x_{m}) \sum_{i',j' \in I(\alpha')}  
%          - \smax(x_{j'})\left(\delta_{j',n} - \smax(x_{n})\right) 
%         \prod_{\substack{i,j \in I(\alpha) \\ (i,j) \neq (i',j')}}(a^{\prime k}_{i,j}  - \smax(x_{j})),
%     \end{align*}
%     we can define $(a_{i, j}^k)_{i, j \in I(\alpha)}^{k \in \myset{1}{\vert \alpha' \vert + 1}} \subseteq \{0, 1\}$ such that
%     \begin{align*}
%         \frac{\partial}{\partial x_{n}} \smax(x_{m}) \prod_{i,j \in I(\alpha')}(a^{\prime k}_{i,j}  - \smax(x_{j}))
%         = \sum_{k=1}^{\vert \alpha \vert}\smax(x_{m}) \prod_{i,j \in I(\alpha)} (a^{k}_{i,j}  - \smax(x_{j})). 
%     \end{align*}
%     Since $\vert \alpha \vert ! = \vert \alpha \vert \cdot \vert \alpha' \vert !$, this concludes the proof.
% \end{proof} 

% \begin{comment} 
% \begin{proof} 
% \begin{align} 
%   \softmax^{(\alpha)}(x_0, x_1, ..., x_{F-1})  = 
%   \Big( \Big( \frac{e^{x_0}}{\sum_{j=0}^{F-1} e^{x_j} } \Big)^{(\alpha)} , \, 
%     \Big( \frac{e^{x_1}}{\sum_{j=0}^{F-1} e^{x_j} } \Big)^{(\alpha)} , \, \cdots, \, 
%      \Big( \frac{e^{x_{F-1}}}{\sum_{j=0}^{F-1} e^{x_j} } \Big)^{(\alpha)} \Big) \notag 
% \end{align} 

% The $i$-th component of the softmax function can be represented as 
% \begin{align} 
% &  \frac{e^{x_i}}{\sum_{j=0}^{F-1} e^{x_j} } = f_i( g(x_0, x_1, ..., x_{F-1})    ) 
%   \notag \\ 
%   & g(x_0, x_1, ..., x_{F-1}) = \big( g_0, g_1, ..., g_{F-1} \big)
%   = \big( e^{x_0}, e^{x_1}, \, ..., \, e^{x_{F-1}} \big) \notag \\ 
%   & f_i (g_0, g_1, ..., g_{F-1}) = \frac{g_i}{ \sum_{j=0}^{F-1} g_j } . \notag 
% \end{align} 
% For simplicity of notation, we denote $x=(x_0, x_1, ..., x_{F-1}) \in \mathbb{R}^F$. 
% By Theorem~\ref{thm:FaaDiBruno}, we have 
% \begin{align} 
%  D^\alpha f_i(g(x)) 
%  = \sum_{1 \leq |\beta| \leq n} (D^\beta f_i)(g(x)) 
%  \sum_{\eta, \zeta \in \calP(\alpha,\beta)} \alpha! 
%         \prod_{j=1}^{n} \frac{
%             [D^{\zeta^{(j)}} g(x)]^{\eta^{(j)}}
%         }{
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         }. 
%         \notag 
% \end{align} 

% \begin{align} 
%  D^{\zeta^{(j)}} g(x) = \big( D^{\zeta^{(j)}} g_0(x), D^{\zeta^{(j)}} g_1(x), \, ..., \, 
%   D^{\zeta^{(j)}} g_{F-1}(x) \big)  \notag 
% \end{align} 

% We can show by induction that for $i\neq j_1$, ..., $j_n$
% \begin{align} 
%  \frac{\partial^{\alpha_1+\cdots + \alpha_n} f_i}{\partial g_{j_1}^{\alpha_1} \cdots \partial g_{j_n}^{\alpha_n}} 
%   = (-1)^{\alpha_1+\cdots + \alpha_n} (\alpha_1+\cdots + \alpha_n)! \frac{g_i}{ ( \sum_{j=0}^{F-1} g_j )^{\alpha_1+\cdots + \alpha_n+1} }   \notag 
% \end{align} 
% \end{proof} 
% \end{comment} 

% \begin{lemma}[Bound of higher-order $\softmax$ derivatives]
%     With \Cref{not:DerivativeBounds}, it holds for any set $K \in \R^k, k\in \N$ and any $\alpha \in \Order^k_{< \infty}$ that
%     \begin{align*}
%         C^{\smax}(\alpha) \leq \vert \alpha \vert!.
%     \end{align*}
% \end{lemma}
% \begin{proof}
%     This is a direct consequence of the representation in \Cref{lem:SoftmaxDerivativeRepresentation} together with $\Vert \smax \Vert = 1$.
% \end{proof}


% \subsubsection{The Multi-Head Self-Attention Mechanism}

% \begin{lemma}[Bound of Dot product]\label{lem:Dotp}
%     In the notation of \Cref{defn:MultiHead} and for $m \in \myset{1}{M}$
%     \begin{align*}
%         \dotp_m(\,\cdot\,; Q, K): 
%                 \R^{M\idim} 
%             \longrightarrow 
%                 \R^{M}
%             , \quad
%                 x
%             \longmapsto
%                 \langle
%                     Qx_m, Kx_j
%                 \rangle_{j = 0}^{M} 
%     \end{align*}
%     we have using \Cref{not:DerivativeBounds}
%     \begin{enumerate}
%     \item $ C^{\dotp_m}_K(e_1) \leq  2 \idim \kdim \Vert K \Vert C^{Q}C^{K}$, where $C^Q \eqdef \max_{i, i' \in \myset{1}{\kdim}\times \myset{1}{\idim}} \vert Q_{i, i'}\vert$, $C^K$ analogously, and $\Vert K \Vert \eqdef \max_{x \in K} \Vert x \Vert$. Additionally,
%     \item  $ C^{\dotp_m}_K( \alpha ) \leq  2 \kdim  C^{Q}C^{K}$, for $\vert \alpha \vert = 2$, and 
%     \item $C^{\dotp_m}_K(\alpha) = 0$ for $\vert \alpha \vert > 2$.
%     \end{enumerate}
%     Since all bounds are not dependent on $m$ we write $C^{\dotp}$ short for $C^{\dotp_m}$.
% \end{lemma}
% \begin{proof}%
%     \begin{enumerate}[wide]%
%     \item  Let $l = (l_1, l_2) \in \myset{1}{M} \times \myset{1}{\idim}$. 
%     Assume $l_1 = m$. If $j \neq m$, then
%         \begin{align*}
%                 D^{e_l}\dotp_m(x; Q, K)_j 
%             =   
%                 D^{e_l}
%                 \sum_{i=1}^{\kdim}
%                  (Kx_j)_i
%                 \sum_{i'=1}^{\idim}
%                     Q_{i, i'}(x_m)_{i'}
%             =   
%                 \sum_{i=1}^{\kdim}
%                 \bigg(\sum_{i'=1}^{\idim}
%                     K_{i, i'}(x_j)_{i'}
%                     \bigg)
%                 Q_{i, l_2},
%         \end{align*}
%     implying
%     \begin{align}\label{id:DotPSimple}
%             \Vert D^{e_l}\dotp_m(x; Q, K) \Vert 
%         \leq 
%             \Vert K \Vert
%             \sum_{i=1}^{\kdim}
%             Q_{i, l_2}
%             \sum_{i'=1}^{\idim}
%                 K_{i, i'}
%         \leq 
%             \idim \kdim
%             \Vert K \Vert
%             C^{Q}C^{K}
%         .
%     \end{align}
%     If $j = m$, 
%         \begin{align*}
%                 D^{e_l}\dotp_m(x; Q, K)_j 
%             &=   
%                 D^{e_l}
%                 \sum_{i=1}^{\kdim}
%                 \bigg(\sum_{i'=1}^{\idim}
%                     K_{i, i'}(x_m)_{i'}
%                     \bigg)
%                 \bigg(\sum_{i'=1}^{\idim}
%                     Q_{i, i'}(x_m)_{i'}
%                     \bigg) \\ 
%             &=   
%                 \sum_{i=1}^{\kdim}
%                     \bigg(
%                     K_{i, l_2}
%                 \sum_{i'=1}^{\idim}
%                     Q_{i, i'}(x_m)_{i'}
%                 +
%                     Q_{i, l_2}
%                 \sum_{i'=1}^{\idim}
%                     K_{i, i'}(x_m)_{i'}
%                     \bigg)
%         \end{align*}
%    therefore implying     
%     \begin{align*}
%             \Vert D^{e_l}\dotp_m(x; Q, K) \Vert 
%         \leq 
%             2 \idim \kdim
%             \Vert K \Vert
%             C^{Q}C^{K}
%         .
%     \end{align*}
%     If $l_1 \neq m$ then for $j \neq l_1$, $D^{e_l}\dotp_m(x; Q, K)_j = 0$, for $j = l_1$
%     \begin{align*}
%                 D^{e_l}\dotp_m(x; Q, K)_j 
%             =   
%                 D^{e_l}
%                 \sum_{i=1}^{\kdim}
%                 (Qx_m)_i
%                 \sum_{i'=1}^{\idim}
%                 K_{i, i'}(x_j)_{i'}
%             =   
%                 \sum_{i=1}^{\kdim}
%                 \bigg(\sum_{i'=1}^{\idim}
%                     Q_{i, i'}(x_m)_{i'}
%                     \bigg)
%                 K_{i, l_2},
%         \end{align*}
%         and we obtain \eqref{id:DotPSimple} analogously.
%     \item If $l_1 = m$ and $j \neq m$
%     \begin{align*}
%         D^{e_l}\bigg(
%             (x_m)_{l_2}
%                 \sum_{i=1}^{\kdim}
%                 \bigg(\sum_{i'=1}^{\idim}
%                     k_{i, i'}(x_j)_{i'}
%                     \bigg)
%                 q_{i, l_2}
%             \bigg) = 0,
%     \end{align*}
%     implying $\Vert D^{2e_l}\dotp_m(x; Q, K) \Vert \leq 0$, what analogously holds for $l_1 \neq m$. However, for $l_1 = m$ and  $j = m$
%     \begin{align*}
%         D^{e_l}\bigg(
%                 \sum_{i=1}^{\kdim}
%                     K_{i, l_2}
%                 \sum_{i'=1}^{\idim}
%                     Q_{i, i'}(x_m)_{i'}
%                 +
%                     Q_{i, l_2}
%                 \sum_{i'=1}^{\idim}
%                     K_{i, i'}(x_m)_{i'} \bigg)
%          = 
%                 \sum_{i=1}^{\kdim}
%                     K_{i, l_2}
%                     Q_{i, l_2}
%                 +
%                     Q_{i, l_2}
%                     K_{i, l_2}
%     \end{align*}
%     we have
%     \begin{align*}
%             \Vert D^{2e_l}\dotp_m(x; Q, K) \Vert 
%         \leq 
%             2 
%             \kdim 
%             C^{Q}C^{K}
%         .
%     \end{align*}
%     \item  Let $l' = (l'_1, l'_2) \in \myset{1}{M} \times \myset{1}{\idim}$. Assume $l_1 = m$, $j \neq m$. If $l'_1 \neq j$, $D^{e_l + e_{l'}}\dotp_m(x; Q, K)_j = 0$. For $l'_1 = j$ follows $D^{e_l + e_{l'}}\dotp_m(x; Q, K)_j =  \sum_{i = 1}^{\kdim} K_{i, l'_2}Q_{i, l_2}$. If $l_1 = m$, $j \neq m$, we have  $D^{e_l + e_{l'}}\dotp_m(x; Q, K)_j = 0$ in the case that $l'_1 \neq m$, and for $l'_1 \neq m$ we obtain
%     \begin{align*}
%         D^{e_l + e_{l'}}\dotp_m(x; Q, K)_j = 
%                 \sum_{i=1}^{\kdim}
%                     K_{i, l_2}
%                     Q_{i, l'_2}
%                 +
%                     Q_{i, l_2}
%                     K_{i, l'_2}.
%     \end{align*}
%     This means, we can use the bound 
%     \begin{align*}
%             \Vert D^{e_l + e_{l'}}\dotp_m(x; Q, K) \Vert 
%         \leq 
%             2 
%             \kdim 
%             C^{Q}C^{K}
%         .
%     \end{align*}
% \end{enumerate}
% \end{proof}
% \begin{lemma}[Bound of Self-Attention for Derivative Type]\label{lem:Attention}
%     Using the notation of  \Cref{not:DerivativeBounds}, \Cref{defn:MultiHead} and \Cref{lem:Dotp}, it holds that
%    \begin{align*}%\label{id:Attention}
%     C_K^{
%         \attention
%     }(\alpha)
%     \leq    
%     \idim
%     M
%     C^V
%     \left(
%         \Vert K \Vert
%         C_K^{
%             \smax \circ \dotp
%         }(\alpha)
%     +
%         \sum_{l=1}^{M\idim}
%         \alpha_l
%         C_K^{
%             \smax \circ \dotp
%         }(\alpha - e_l)
%     \right)
% \end{align*} 
% where 
% \begin{align}
% C^{\smax \circ \dotp}_K(\alpha)
%     &\leq
%     \alpha! \sum_{\beta \in \Order^{M}_{\leq n}}  N(\beta) C^{\smax}_{\dotp[K]}(\beta)
%     \sum_{\eta, \zeta \in \calP'(\alpha,\beta)} 
%     \prod_{j=1}^{n} \frac{
%         C^{\dotp}_K(\order(\zeta^{(j)}))^{\vert \eta^{(j)} \vert}
%     }{
%         \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%     }. \label{id:SmaxDpCompositeBound}
% \end{align}
% \end{lemma}
% \begin{proof}
%     Fix $\alpha \in \N^k$, and note that
%     \begin{align*}
%         \Vert
%             D^{\alpha}
%             \attention(
%                 x; Q, K, V 
%             ) 
%         \Vert
%         \leq
%         \max_{m\in \myset{1}{M}}
%         \max_{i\in \myset{0}{\vdim}}
%         \Vert
%             D^{\alpha}
%             \attention(
%                 x; Q, K, V 
%             )_{m,i}
%         \Vert
%     \end{align*}
%     and
%     \begin{align*}
%          \Vert
%         D^{\alpha}
%         \attention(&
%             x; Q, K, V 
%         )_{m,i}
%         \Vert \\
%         &\leq
%         \sum_{j=1}^M
%         \sum_{i'=0}^{\idim}
%         \Vert
%             D^{\alpha}
%             \smax \circ \dotp(x; Q, K)_j
%             V_{i, i'}(x_j)_{i'}
%         \Vert \\
%         &\leq
%         \idim M
%         \max_{j\in \myset{1}{M}}
%         \max_{i'\in \myset{0}{\idim}}
%         \Vert
%             D^{\alpha}
%             \smax \circ \dotp(x; Q, K)_j
%             V_{i, i'}(x_j)_{i'}
%         \Vert.
%     \end{align*}
%     Due to the extended Leibnitz rule \cite{Hardy06}, we have
%     \begin{multline*}
%         \Vert
%             D^{\alpha}
%             \smax \circ \dotp(x; Q, K)_j
%             V_{i, i'}(x_j)_{i'}
%         \Vert
%         \\ \leq
%         \Vert
%             D^{\alpha}
%             \smax \circ \dotp(x; Q, K)_j
%             V_{i, i'}(x_j)_{i'}
%         \Vert
%         +
%         \sum_{l=1}^{M\idim}
%         V_{i, i'}
%         \alpha_l
%         \Vert
%             D^{\alpha - e_l}
%             \smax \circ \dotp(x; Q, K)_j
%         \Vert.
%     \end{multline*}
%     % \yannick{This does not make sense if $\alpha_l = 0$}
%     \Cref{id:SmaxDpCompositeBound} follows directly from \Cref{thm:DerivativeBoundByType}.
% \end{proof}

% \begin{corollary}[Bound of Self-Attention for Derivative Level]\label{cor:Attention}
%     Using the setting of \Cref{lem:Attention}, for $n \in \N$,
%    \begin{align}%\label{id:Attention}
%     C_K^{
%         \attention
%     }(n)
%     \leq    
%     \idim
%     M
%     C^V
%     C_K^{
%         \smax \circ \dotp
%     }(\cleq n)
%     \left(
%         \Vert K \Vert
%     +
%         n \idim M
%     \right)
%     \label{id:AttenstionBoundByLevel}
% \end{align} 
% where 
% \begin{align}
% C^{\smax \circ \dotp}_K(\cleq n)
%     &\leq
%         C^{\smax}_{\dotp[K]}(\cleq n)
%         C^{\dotp}_K({\cleq n})^{n}
%         \Big[ \frac{ 2 nM}{e\ln n} ( 1 + o(1) ) \Big]^{n}.
%     \label{id:SmaxDpCompositeBoundII}
% \end{align}
% \end{corollary}
% \begin{proof}
%     \Cref{id:AttenstionBoundByLevel} follows directly from \Cref{lem:Attention}; and \eqref{id:SmaxDpCompositeBoundII} is a consequence of \Cref{cor:DerivativeBoundByLevel}.
% \end{proof}


% \begin{corollary}[Bound of Multi-head Self-Attention]\label{cor:MultiHead}
%     In the notation of \Cref{defn:MultiHead}, \Cref{thm:DerivativeBoundByType} and \Cref{lem:Dotp} it holds that 
%     \begin{align*}
%         C^{\multihead}_K(\alpha)
%         &\leq
%         \alpha! 
%         \vdim 
%         C^{W}
%         C^{\attention}_K(\alpha)
%     \end{align*}
%     where 
%     \begin{align*}
%         C^{\attention}_K \eqdef  \max_{h \in \myset{1}{H}}C^{\attention(\, \cdot\,; Q^{(h)}, K^{(h)}, V^{(h)})}_K , \quad C^{W} \eqdef \max_{h \in \myset{1}{H}} W^{(h)}.
%     \end{align*}
% In particular, we have the following order estimate
% \begin{align*}
%         C^{\multihead}_K(\le n)
%     \in
%         \mathcal{O}\biggl(
%             M^2
%             \Vert K \Vert
%             \|W\|
%             \|V\|
%                 (c_{\idim,\kdim}\Vert K \Vert \|Q\|\|K\|)^{n}
%             \,\,
%                 n^2
%                  \Big(\frac{n}{e}\Big)^{2n}
%                 C_n^n
%         \biggr)
%     .
% \end{align*}
% \end{corollary}
% \begin{proof}
%     From \Cref{cor:DerivativeBoundAffine} and \Cref{lem:Attention} we directly obtain
%    \begin{equation}
%     \label{eq:precise_bound_MHG}
% \begin{aligned}
%         C^{\multihead}_K(\alpha)
%     \leq & 
%          n! 
%             \vdim 
%             C^{W}
%             \idim
%         M
%         C^V
%         n!
%             (2 \idim \kdim \Vert K \Vert C^{Q}C^{K})^{n}
% \\
%     & \times 
%         \left(
%             \Vert K \Vert
%         +
%             n \idim M
%         \right)
%             \Big[ \frac{ 2 nM}{e\ln n} ( 1 + o(1) ) \Big]^{n}
%     .
% \end{aligned}
% \end{equation}
%    Applying Stirling's approximation, we have that 
%    \begin{equation}
%     \label{eq:orderbound}
%         C^{\multihead}_K(\alpha)
%     \in
%         \mathcal{O}\biggl(
%             M^2
%             \Vert K \Vert
%             \|W\|
%             \|V\|
%                 (c_{\idim,\kdim}\Vert K \Vert \|Q\|\|K\|)^{n}
%             \,\,
%                 n^2
%                  \Big(\frac{n}{e}\Big)^{2n}
%                 C_n^n
%         \biggr)
% ,
%    \end{equation}
% where $C_n\eqdef \frac{ 2 n M}{e\ln n} ( 1 + o(1) )$ and $c_{\idim,\kdim}\eqdef 2 \idim \kdim$.
% \end{proof}





% \subsubsection{The Activation Functions}\label{sec:Activation}
% \begin{lemma}[Derivatives of $\softplus$]\label{lem:Softplus}
%     For 
%     \begin{align*}
%         \softplus: \R \to \R, \quad x \mapsto \ln (1 + \exp(\cdot))
%     \end{align*}
%     it holds 
%     \begin{align*}
%         \softplus^{(1)}(x) = \sigmoid(x) \eqdef 1 / (1 + \exp(-x))
%     \end{align*}
%     and for $n \in \N$
%     \begin{align*}
%         \softplus^{(n + 1)}(x) = \sigmoid^{(n)}(x) = \sum_{k=0}^n(-1)^{n+k}k!S_{n,k}\sigmoid(x)(1-\sigmoid(x))^k,
%     \end{align*}
%     where $S_{n,k}$ are the Stirling numbers of the second kind, $S_{n,k} \eqdef \frac{1}{k!} \sum_{j=0}^{k} (-1)^{k-j} \binom{k}{j} j^n$.
% \end{lemma}
% \begin{proof}
% We start with Fa\`a di Bruno's formula,
% \begin{align*}
%     \frac{d^n}{dt^n}\sigmoid(x)=\frac{d^n}{dx^n}\frac{1}{f(x)}=\sum_{k=0}^n(-1)^kk!f^{-(k+1)}(x)B_{n,k}(f(x)),
% \end{align*}
% where \(f(x) \eqdef 1 + \exp(-x)\) and \(B_{n,k}(f(x))\) denotes the Bell polynomials evaluated on $f(x)$. Next, we know the \(k\)-th derivative of \(f(x)\) is given by
% \begin{align*}
%    \frac{d^k}{dt^k}f(x)=(1-k)_k+ke^{-x}.
% \end{align*}
% Now, using the definition of the Bell polynomials \(B_{n,k}(f(t))\), we have
% \begin{align*}
%     B_{n,k}(f(x))=(-1)^nS_{n,k}e^{-kx},
% \end{align*}
% where \(S_{n,k}\) represents the Stirling numbers of the second kind. Substituting the expression for \(B_{n,k}(f(x))\) into the derivative of \(\sigmoid(x)\), we obtain
% \begin{align*}
%     \frac{d^n}{dx^n}\sigmoid(x)=\sum_{k=0}^n(-1)^{n+k}k!S_{n,k}\sigmoid(x)(1-\sigmoid(x))^k.
% \end{align*}
% \end{proof}

% \begin{corollary}\label{cor:Softplus}
% In the setting of \Cref{lem:Softplus}, for $n \in \N$,
%     \begin{align*}
%         C^{\softplus}(n) \leq         \sum_{k=0}^n 
%         \frac{k^k k!S_{n,k}}{(k+1)^{k+1}}.
%     \end{align*}
% \end{corollary}
% \begin{proof}
%     For $k \in \N$ and $x \in [0,1]$, we have
%     \begin{align*}
%         f^k(x) \eqdef x(1-x)^k, \quad 
%         (f^k)'(x) = (1-(k+1)x)(1-x)^{k-1};
%     \end{align*}
%     which amounts to $(f^k)'(x) = 0$ at $1/(k+1)$, i.e. 
%     \begin{align*}
%         \max_{x \in [0,1]}f(x) = \frac{1}{k+1}\left(
%             \frac{k}{k+1}
%         \right)^k
%         = 
%             \frac{k^k}{(k+1)^{k+1}}
%     .
%     \end{align*}
% \end{proof}

% \begin{lemma}[Derivatives of $\operatorname{GELU}$]
% %https://arxiv.org/abs/2305.12073 
% \label{lem:GELU}
% For 
%     \begin{align*}
%         \operatorname{GELU}: \R \to \R, \quad x \mapsto x \Phi(x) , 
%     \end{align*}
% it holds 
% \begin{align}
%        & \operatorname{GELU}'(x) = \Phi(x) + x\phi(x), \notag \\ 
%         & \operatorname{GELU}^{(n)}(x) = n \varphi^{(n-2)}(x) + x \phi^{(n-1)}(x), \quad n\geq 2 ,  
%         \label{GELUn}
%     \end{align}
% with $\phi(x)=\frac{1}{\sqrt{2\pi}}e^{-x^2/2}$, $\Phi(x)=\int_{-\infty}^x \phi(u) du$. 
% The $n$-th derivative of $\phi(x)$ is given by 
% \begin{align*}
%  \frac{d^n}{d x^n} \phi(x) = \frac{1}{\sqrt{2\pi}} e^{-x^2/2} \Big[ \sum_{k=0}^{\lfloor n / 2 \rfloor} \binom{n}{2k} 2^{k} 
%   \frac{\Gamma(\frac{2k+1}{2})}{\Gamma(\frac{1}{2})} x^{n-2k} \Big] . \notag  
% \end{align*}
%  \begin{comment} 
% \yannick{is that not easier if we put $$
%  \frac{d^n}{d x^n} \phi(x) = \frac{1}{\sqrt{2\pi}} e^{-x^2/2} \Big[ \sum_{k=0}^{\lfloor n / 2 \rfloor} \binom{n}{2k} 2^{k} 
%   \frac{\Gamma(\frac{2k+1}{2})}{\Gamma(\frac{1}{2})} x^{n-2k} \Big] , \notag  
%  $$}
% \begin{align} 
%  \frac{d^n}{d x^n} \phi(x) = \frac{1}{\sqrt{2\pi}} e^{-x^2/2} \Big[ \sum_{k=0}^n \binom{n}{k} B_{(2n+k)\frac{1-(-1)^k}{2}} 2^{k/2} 
%   \frac{\Gamma(\frac{k+1}{2})}{\Gamma(\frac{1}{2})} x^{n-k} \Big] , \notag  
% \end{align} 
% with  
% \begin{align} 
%  B_{(2n+k)\frac{1-(-1)^k}{2}} 
%  = 
%  \begin{cases} 
%  1 , \quad & \mbox{$k$ even},  \\ 
%  0, \quad & \mbox{$k$ odd} . 
%  \end{cases} \notag 
% \end{align} 
% \end{comment}
% \end{lemma}

% \begin{proof} 
% By induction we can show that \eqref{GELUn} holds. 
% And the representation of the $n$-th derivative of $\phi(x)$ follows from~\cite{Oliveira2012RepresentationOT}. 
% \end{proof} 

% \begin{corollary}\label{cor:GELU}
%     For $n \geq 2$, it holds in the setting of \Cref{lem:GELU}
%     \begin{align*}
%         C^{\operatorname{GELU}}(n) \leq \frac{1}{\sqrt{2\pi}\Gamma(\frac{1}{2})} \left( n a_{n-2} b_{n-2} + a_{n-1} c_{n-1}
%         \right),
%     \end{align*}   
%     where 
%     \begin{align*}
%         a_n \eqdef \sum_{k=0}^{\lfloor n / 2 \rfloor} \binom{n}{2k} 2^{k} 
%         \Gamma\left(\frac{2k+1}{2}\right), \quad 
%         b_n \eqdef \max_{x \in \R} e^{-\frac{x^2}{2}} \sum_{k=0}^{\lfloor n / 2 \rfloor} x^{n-k} , \quad 
%         c_n \eqdef \max_{x \in \R} e^{-\frac{x^2}{2}} x \sum_{k=0}^{\lfloor n / 2 \rfloor} x^{n-k}.
%     \end{align*}
% \end{corollary}


% \begin{lemma}[Derivatives of $\tanh$]\label{lem:tanh}
% %https://math.stackexchange.com/questions/2625632/nth-derivative-of-tanh 

% For $\tanh: \mathbb{R} \mapsto \mathbb{R}$, the $n$-th derivatives have the representation  
% \begin{align} 
% & \frac{d^n}{d x^n} \tanh{x} = C_n(\tanh{x}) ,\notag \\ 
% & C_n(z) = (-2)^n (z+1) \sum_{k=0}^n \frac{k!}{2^k} \binom{n}{k} (z-1)^k , \quad n\geq 1 . \notag 
% \end{align} 
% \end{lemma}

% \begin{proof} 
% See~\cite{Boyadzhiev2007}. 
% \end{proof} 
% \begin{corollary}\label{cor:tanh}
%     In the setting of \Cref{lem:tanh}, for $n \in \N$, $C^{\tanh}(n) = \max_{z \in [-1, 1]} C_n(z)$.
% \end{corollary}




% \begin{lemma}[Derivatives of $\operatorname{SWISH}$]
% For 
%     \begin{align*}
%         \operatorname{SWISH}: \R \to \R, \quad x \mapsto \frac{x}{1+e^{-x}} 
%     \end{align*}
%     it holds for $n\geq 1$ 
%     \begin{align} 
%     \frac{d^n}{d x^n} \operatorname{SWISH}(x) 
%     = n \sum_{k=1}^{n} (-1)^{k-1} (k-1)! S_{n, k} \sigmoid^k(x) 
%     + x \sum_{k=1}^{n+1} (-1)^{k-1} (k-1)! S_{n+1, k} \sigmoid^k(x) , \notag  
%     \end{align} 
% where $S_{n,k}$ are Stirling numbers of the second kind, i.e., 
% \begin{align} 
%  S_{n,k} = \frac{1}{k!} \sum_{j=0}^k (-1)^j \binom{k}{j} (k-j)^n . \notag
% \end{align} 
% \end{lemma}

% \begin{proof} 
% By induction, we can show that 
% \begin{align} 
% \frac{d^n}{d x^n} \operatorname{SWISH}(x) = n \sigmoid^{(n-1)}(x) + x \sigmoid^{(n)}(x) , \quad n \geq 1 . \notag 
% \end{align}  
% By~\cite[Theorem 2]{MINAI1993845}, the derivatives of the sigmod function can be represented as  
% \begin{align}
% \sigmoid^{(n)}(x) = \sum_{k=1}^{n+1} (-1)^{k-1} (k-1)! S_{n+1, k} \sigmoid^k(x) , \ n\geq 1 . \notag 
% \end{align} 
% Combining the above two equations, we obtain the general form of the $n$-th derivative of the SWISH function.  
% \end{proof} 


% \subsubsection{The Layer Norm}
% \begin{lemma}[Bound of the Layer Norm for Derivative Type]\label{lem:LayerNorm}
%     Fix $k \in \N$, $\beta\in \mathbb{R}^k$, $\gamma \in \mathbb{R}$, and $w\in [0,1]$. For the layer norm, given by 
%     \begin{gather*}
%         \layernorm: \R^k \rightarrow \R^k,\quad  x \mapsto  
%         \gamma\, 
%         f(x)
%         g\circ\Sigma(x) + \beta; 
%     \\
%         f: \R^k \rightarrow \R^k,\quad  x \mapsto  x-M(x);
%     \qquad
%         g: \R \rightarrow \R, \quad  u \mapsto  \frac{1}{\sqrt{1 + u}};
%     \\
%         M: \R^k \rightarrow \R, \quad  x \mapsto  \frac{w}{k} \sum_{i=1}^k\,  x_i;
%     \qquad
%         \Sigma: \R^k \rightarrow \R, \quad  x \mapsto  \frac{w}{k}\, \sum_{i=1}^k\,  (x_i-M(x))^2;
%     \end{gather*}
%     holds for a compact symmetric set $K$ (using \Cref{not:DerivativeBounds})
%     \begin{multline*}
%         C^{\layernorm}_K(\alpha) \leq  
%         \alpha! \gamma
%         \sum_{m = 1}^{n=1} \frac{(2m+1)!! }{2^{2m}}
%         \bigg(
%     %&
%         \sum_{\substack{\alpha' \leq \alpha\\ \vert \alpha' \vert = n-1}} 
%             \sum_{\eta, \zeta \in \calP'(\alpha', m)} 
%             \prod_{j=1}^{n} \frac{
%                 C^\Sigma_K(\order(\zeta^{(j)}))^{\vert \eta^{(j)} \vert}
%             }{
%                 \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%             }
%     \\ %&
%     +
%             \sum_{\eta, \zeta \in \calP'(\alpha, m)} 
%             \prod_{j=1}^{n} \frac{
%                 C^\Sigma_K(\order(\zeta^{(j)}))^{\vert \eta^{(j)} \vert}
%             }{
%                 \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%             }
%         \bigg),
%     \end{multline*}
%     where $C^\Sigma_K(\alpha) = 2w \Vert K \Vert$ for $\vert \alpha \vert = 1$, $C^\Sigma_K(\alpha) = 2w$ for $\vert \alpha \vert = 2$, and $C^\Sigma_K(\alpha) = 0$ otherwise.
% \end{lemma}
% \begin{proof}
% Note that 
% \begin{align*} %https://math.stackexchange.com/questions/2011926/proving-nth-derivative-of-sqrtx-by-induction
%     g^{(n)}(x) = (-1)^n \frac{(2n+1)!}{n!2^{2n}} (1+x)^{-\frac{1}{2}-n},
% \end{align*}
% implying $C^g_K(n) \leq (2n+1)!! 2^{-2n}$, $!!$ denoting the double factorial. We have further $C^{f}_K(\alpha) \leq \mathbbm{1}_{\vert \alpha \vert = 1}$ and a direct computation yields
% \begin{align*}
%     C^\Sigma_K(\alpha) \leq \begin{cases}
%         2w\Vert K \Vert 
%         &
%         \text{ for } \vert \alpha \vert = 1
%         \\
%         2w
%         &
%         \text{ for } \vert \alpha \vert = 2
%         \\
%         0
%         &
%         \text{ else. } 
%     \end{cases}
% \end{align*}
% By \Cref{thm:DerivativeBoundByType}, 
% \begin{align*}
%     C^{g\circ \Sigma}_K(\alpha)
%     &\leq
%     \alpha! \sum_{m = 1}^n C^g_{\Sigma[K]}(m)
%     \sum_{\eta, \zeta \in \calP'(\alpha, m)} 
%     \prod_{j=1}^{n} \frac{
%         C^\Sigma_K(\order(\zeta^{(j)}))^{\vert \eta^{(j)} \vert}
%     }{
%         \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%     }.
% \end{align*}
% According to the general multivariate Leibnitz rule, it holds that 
% \begin{align*}
% D^{\alpha}(f \cdot (g \circ \Sigma)) 
% = \sum_{\beta \leq \alpha}  \frac{\alpha!}{\beta!(\alpha - \beta)!} D^{\beta}f \cdot D^{\alpha - \beta}(g\circ \Sigma) %\prod_{i=1}^k{\alpha_i \choose \beta_i}.
% \end{align*}
% which implies
% \begin{align*}
%         C^{\layernorm}_K (\alpha)
%     \leq  
%         C^{g\circ \Sigma}_K(\alpha) \Vert K \Vert
%         +
%         \sum_{\beta \leq \alpha, \vert \beta \vert = 1}  \frac{\alpha!}{(\alpha - \beta)!} 
%             C^{g\circ \Sigma}_K(\alpha - \beta). %\prod_{i=1}^k{\alpha_i \choose \beta_i}
% \end{align*}
% \end{proof}

% \begin{corollary}[Bound of the Layer Norm for Derivative Level]\label{cor:LayerNorm}
%     In the setting of \Cref{lem:LayerNorm}, it holds that
%     \begin{align*}
%         C^{\layernorm}_K(\cleq n) \leq 2w \Vert K \Vert(2n+1)!! 2^{-2n} (\Vert K \Vert + kn) 
%         \Big[ \frac{ 2 n}{e\ln n} ( 1 + o(1) ) \Big]^{n}.
%     \end{align*}
% Furthermore, we have the asymptotic estimate 
% \begin{align*}
%         C^{g\circ \Sigma}_K(\cleq n)
%     \in 
%         \mathcal{O}\Big(
%             w \|K\|
%             \,
%             n^{1/2}
%             \big(
%                     \frac{
%                         n^{5/2}
%                     }{
%                         e^{3/4}\ln(n)
%                     }
%                 \,
%                 (
%                     1 + o(1)
%                 )
%             \big)^n
%         \Big)
% .
% \end{align*}
% \end{corollary}
% \begin{proof}
%     Analogue to the proof of \Cref{lem:LayerNorm},
% \begin{align*}
%         C^{\layernorm}_K (\cleq n)
%     \leq  
%         \Vert K \Vert C^{g\circ \Sigma}_K(\cleq n) 
%         +
%         k  n 
%             C^{g\circ \Sigma}_K(\cleq n-1) %\prod_{i=1}^k{\alpha_i \choose \beta_i},
%     \leq  
%         (\Vert K \Vert + kn) C^{g\circ \Sigma}_K(\cleq n), 
% \end{align*}
% where we can use \Cref{cor:DerivativeBoundByLevel} to bound
% \begin{align}
% \nonumber
%     C^{g\circ \Sigma}_K(\cleq n)
%     &\leq
%     C^g_{\Sigma[K]}(\cleq n)
%         C^\Sigma_K({\cleq n})^{n}
%         \Big[ \frac{ 2 n}{e\ln n} ( 1 + o(1) ) \Big]^{n}
%     \\
% \label{eq:reducemeplease}
%     &\leq 2w \Vert K \Vert(2n+1)!! 2^{-2n}
%         \Big[ \frac{ 2 n}{e\ln n} ( 1 + o(1) ) \Big]^{n}.
% \end{align}
% Since $2n+1$ is odd, for each $n\in \mathbb{N}_+$, then sterling approximation \textit{for double factorial} yields the asymptotic
% \begin{equation}
% \label{eq:stirling_redux}
%         (2n+1)!! 
%     \in 
%         \mathcal{O}\Big(
%             \sqrt{2 n}\left(\frac{n}{e}\right)^{n/2}
%         \Big)
% .
% \end{equation}
% Merging~\eqref{eq:stirling_redux} with the right-hand side of~\eqref{eq:reducemeplease} yields
% \begin{align*}
%         C^{g\circ \Sigma}_K(\cleq n)
%     \in 
%         \mathcal{O}\Big(
%             w \|K\|
%             \,
%             n^{1/2}
%             \big(
%                     \frac{
%                         n^{5/2}
%                     }{
%                         e^{3/4}\ln(n)
%                     }
%                 \,
%                 (
%                     1 + o(1)
%                 )
%             \big)^n
%         \Big)
% .
% \end{align*}
% \end{proof}


% \subsubsection{The Multilayer Perceptron (Feedforward Neural Network) with Skip Connection}
% \begin{definition}[Single-Layer Feedforward Neural Network with Skip Connection]\label{defn:ff}
% Fix a non-affine activation function $\sigma\in C^{\infty}(\R)$ and dimensions $\idim, \ldim, \odim \in \N$.
% A feedforward neural network is a map $\neuraln:\mathbb{R}^{\idim}\to \mathbb{R}^{\odim}$ represented for each $x\in \mathbb{R}^{\idim}$ by
% \begin{align}\label{eq:FF}
%         \neuraln (x) 
%     & \eqdef  
%         B^{(1)} x + B^{(2)} \big(\sigma\bullet (A\, x + a)\big)
% \end{align}
% for
% $A\in \mathbb{R}^{\ldim \times \idim}$, $a\in \mathbb{R}^{\ldim}$, 
% $B^{(1)} \in \mathbb{R}^{\odim \times \idim}$, and $B^{(2)} \in \mathbb{R}^{\odim \times \ldim}$.
% \end{definition}
% \begin{lemma}[Bound of Neural Networks for Derivative Type]\label{lem:FeedForward}
%     In the notation of \Cref{not:DerivativeBounds}, \Cref{lem:Dotp}, and \Cref{defn:ff}, it holds that
%     \begin{align*}
%         C^{\neuraln}_K(\alpha)
%         &\leq
%             C^{B^{(1)}}\mathbbm{1}_{\vert \alpha \vert = 1}
%         +
%             \ldim (\alpha!)^2 C^{B^{(2)}}
%             \sum_{m=1}^n  C^\sigma_{{h}[K]}(m)
%         \cdot
%         (C^{A})^m
%         \sum_{\eta, \zeta \in \calP'(\alpha,m)} 
%         \prod_{j=1}^{n} \frac{
%             \mathbbm{1}_{\vert \zeta^{(j)} \vert \leq 1}
%         }{
%             \eta^{(j)}!
%         },
%     \end{align*}
%     where $h[K]$ is defined as the image of $h(x) \eqdef Ax + a$ on $K$. 
% \end{lemma}
% \begin{proof}
%     Write $\neuraln(x) =  B^{(1)} x + B^{(2)}((g_i(x))_{i=1}^{\ldim})$, where for $i \in \myset{1}{\ldim}$
%     \begin{align*}
%         g_i(x) \eqdef \sigma((Ax + a)_i).
%     \end{align*}
%     If we define $h_i(x) \eqdef h(x)_i$, we follow with \Cref{thm:DerivativeBoundByType}
%     \begin{align*}
%     C^{g_i}_K(\alpha)
%         &\leq
%         \alpha! \sum_{m=1}^n  C^\sigma_{{h}[K]}(m)
%         \cdot
%         (C^{A})^m
%         \sum_{\eta, \zeta \in \calP'(\alpha,m)} 
%         \prod_{j=1}^{n} \frac{
%             \mathbbm{1}_{\vert \zeta^{(j)} \vert \leq 1}
%         }{
%             \eta^{(j)}!
%         }
%         \eqdef
%     C^{g}_K(\alpha)
%         ,
%     \end{align*}
%     and due to the component wise application of the activation function it holds that \begin{align*}
%         \Vert D^\alpha \max_{i \in \myset{1}{\ldim}} g_i(x) \Vert_K = \max_{i \in \myset{1}{\ldim}} C^{g_i}_K(\alpha) \leq C^{g}_K(\alpha).
%     \end{align*}
%     Using \Cref{cor:DerivativeBoundAffine}, we obtain
%     \begin{align*}
%         C^{\neuraln}_K(\alpha)
%         &\leq
%             C^{B^{(1)}}\mathbbm{1}_{\vert \alpha \vert = 1}
%         +
%             \ldim \alpha! C^{B^{(2)}}
%             C^g_K(\alpha).
%     \end{align*}
% \end{proof}

% \begin{corollary}[Bound of Neural Networks for Derivative Level]\label{cor:FeedForward}
%     In the setting of \Cref{lem:FeedForward},
%     \begin{align*}
%         C^{\neuraln}_K(\cleq n)
%         &\leq
%             C^{B^{(1)}}
%         +
%             \ldim n! C^{B^{(2)}}
%         C^\sigma_{{h}[K]}({\cleq n})
%         (C^{A})^{n}
%         \Big[ \frac{ 2 n}{e\ln n} ( 1 + o(1) ) \Big]^{n}.
%     \end{align*}
% If, moreover, $K=[-M_1,M_2]^{\idim}$ then 
% \begin{align*}
%         C^{\neuraln}_K(\cleq n)
%     \in 
%         \mathcal{O}
%         \Big(
%                 \|B^{(1)}\|_{\infty}
%             +
%                 \|B^{(2)}\|_{\infty}
%                 \|A\|_{\infty}^n
%                 \|\sigma\|_{n:
%                         \operatorname{Ball}(a,\sqrt{\idim |M_1+M_2|})
%                     }
%                 \operatorname{Width}(\neuraln)
%                 \,
%                 n^{1/2}\big(\frac{n}{e}\big)^n
%                 C_n^n
%         \Big)
% \end{align*}
% \end{corollary}
% \begin{proof}
% Arguing analogously to the proof of~\Cref{lem:FeedForward}, barring the usage of \Cref{cor:DerivativeBoundByLevel}, we 
% obtain the estimate
% \begin{align}
% \label{eq:pre_order_estimate}
%     C^{\neuraln}_K(\cleq n)
%     &\leq
%         C^{B^{(1)}}
%     +
%         \ldim n! C^{B^{(2)}}
%     C^\sigma_{{h}[K]}({\cleq n})
%     (C^{A})^{n}
%     \Big[ \frac{ 2 n}{e\ln n} ( 1 + o(1) ) \Big]^{n}
% .
% \end{align}
% Let $C_n\eqdef\frac{ 2 n}{e\ln n} ( 1 + o(1) ) $
% Using Stirling's approximation and the definition of the component-wise $\|\cdot\|_{\infty}$ norm of a matrix,~\eqref{eq:pre_order_estimate} becomes
% \begin{align}
%     C^{\neuraln}_K(\cleq n)
%     &
%     \in \mathcal{O}
%     \Big(
%             \|B^{(1)}\|_{\infty}
%         +
%             \|B^{(2)}\|_{\infty}
%             \|A\|_{\infty}^n
%             C^\sigma_{{h}[K]}({\cleq n})
%             \ldim 
%             \,
%             n^{1/2}\big(\frac{n}{e}\big)^n
%             C_n^n
%     \Big)
% .
% \end{align}
% If, there is some $M_1,M_2\le 0$, such that $K=[0,\beta]^d$ then using the estimate between the $\|\cdot\|_2$ and $\|\cdot\|_{\infty}$ norms on $\mathbb{R}^{\idim}$ and the linearity of $A$ we estimate 
% \begin{align*}
%     C^\sigma_{{h}[K]}({\cleq n}) 
% \le 
%     C^\sigma_{
%         \operatorname{Ball}(a,\sqrt{\idim |M_1+M_2|})
%     }({\cleq n}) 
% \le 
%     \|\sigma\|_{n:
%         \operatorname{Ball}(a,\sqrt{\idim |M_1+M_2|})
%     }
% .
% \end{align*}
% Upon $\operatorname{Width}(\neuraln)\eqdef \max\{\idim,\odim,\ldim\}$, the estimate~\eqref{eq:pre_order_estimate} implies that $C^{\neuraln}_K(\cleq n)$ is of the order of
% \begin{align}
% \label{eq:pre_order_estimate__Kisabox}
%     % C^{\neuraln}_K(\cleq n)
%     % &
%     % \in 
%     \mathcal{O}
%     \Big(
%     &
%             \|B^{(1)}\|_{\infty}
%         +
%             \|B^{(2)}\|_{\infty}
%             \|A\|_{\infty}^n
%             \|\sigma\|_{n:
%                     % \operatorname{Ball}(a,\sqrt{\idim |M_1+M_2|})
%                     [-\|a\|_{\infty}-\sqrt{\idim |M_1+M_2|},
%                     \|a\|_{\infty}+\sqrt{\idim |M_1+M_2|}]
%                 }
%     \\
%     \nonumber
%     & \times 
%             \operatorname{Width}(\neuraln)
%             \,
%             n^{1/2}\big(\frac{n}{e}\big)^n
%             C_n^n
%     \Big)
% .
% \end{align}
% \end{proof}







% \subsection{Step 2 (B) - Transformers}
% \label{s:Proofs__TransformerCsNorms}
% We may now merge the computations in Subsection~\ref{sec:RegularityTransfomerBuildingBlocks}, with the Fa`{a} di Bruno-type from Section~\ref{s:Compositions_and__FaadiBruno} to uniformly bound the $C^s$-norms of the relevant class transformer networks.  Our results are derived in two verions: the first is of ``derivative type'' (which is much smaller and more precise but consequentially more complicated) and the second is in ``derivative level'' form (cruder but simpler but also looser).   

% \begin{theorem}[By Derivative Type]\label{thm:TransformerBlockSobolevBound} 
%     Let $K$ be a compact set, $\tblock$ a transformer block as in \Cref{defn:TransformerBlock}, and $\alpha \in \Order^{M\idim}_n, n \in \N$. Then,
%     \begin{align*}
%         C^{\tblock}_K(\alpha) &\leq
%         \alpha! \sum_{\beta \in \Order^{\odim}_{\leq n}}  N(\beta) C^{\layernorm}_{K\tagA}(\beta)
%         \sum_{\eta, \zeta \in \calP'(\alpha,\beta)} 
%         \prod_{j=1}^{n} \frac{
%             C\tagA_K(\order(\zeta^{(j)}))^{\vert \eta^{(j)} \vert}
%         }{
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         }, 
%     \end{align*}
%     where for all $\gamma \in \Order^{M\idim}_{\leq n}$:
%     \begin{align*}
%         C\tagA_K(\gamma) & \eqdef 
%         \gamma! \sum_{\beta \in \Order^{\idim}_{\leq n}}  N(\beta) C^{\neuraln}_{K\tagB}(\beta)
%         \sum_{\eta, \zeta \in \calP'(\gamma,\beta)} 
%         \prod_{j=1}^{n} \frac{
%             C\tagB_K(\order(\zeta^{(j)}))^{\vert \eta^{(j)} \vert}
%         }{
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         },
%     \\
%         C\tagB_K(\gamma) & \eqdef
%         \gamma! \sum_{\beta \in \Order^{\idim}_{\leq n}}  N(\beta) C^{\layernorm}_{K\tagC}(\beta)
%         \sum_{\eta, \zeta \in \calP'(\gamma,\beta)} 
%         \prod_{j=1}^{n} \frac{
%             C\tagC_K(\order(\zeta^{(j)}))^{\vert \eta^{(j)} \vert}
%         }{
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         },
%     \\
%         C\tagC_K(\gamma) & \eqdef \mathbbm{1}_{\vert \gamma \vert = 1} + C^{\multihead}_K(\gamma).
%     \end{align*}
%     In the above, $K\tagC = \bigcup_{m = 0}^M\multihead_m[K]$, $K\tagB = \layernorm[K\tagC]$, and $K\tagA = \neuraln[K\tagB]$.
    
%     For respective multi-indices, a bound for $C^{\layernorm}_{K\tagA}, C^{\layernorm}_{K\tagC}$ is given by \Cref{lem:LayerNorm}, $C^{\neuraln}_{K\tagB}$ is bounded in \Cref{lem:FeedForward}, and a bound for $C^{\multihead}_{K}$ is given in \Cref{cor:MultiHead}.
% \end{theorem}
% \begin{proof}
%     This is a direct consequence of \Cref{thm:DerivativeBoundByType}.
% \end{proof}

% \begin{theorem}[By Derivative Level]\label{thm:TransformerBlockSobolevBoundLevel} 
%     Let $K$ be a compact set, $\tblock$ a transformer block as in \Cref{defn:TransformerBlock}, and $n \in \N$. Then,
%     \begin{multline*}
%         C^{\tblock}_K(\cleq n) \leq
%         C^{\layernorm}_{K\tagA}({\cleq n})
%         \left(
%             \odim
%             C^{\neuraln}_{K\tagB}({\cleq n})
%         \right)^n
%         \left(
%             \idim^2
%             C^{\layernorm}_{K\tagC}({\cleq n})
%         \right)^{n^2}
%         \\
%         \cdot
%         \left(
%              1 + C^{\multihead}_K(\cleq n)
%          \right)^{n^3}
%         \Big[ \frac{ 2 n}{e\ln n} ( 1 + o(1) ) \Big]^{n + n^2 + n^3}
%     \end{multline*}
%     where, $K\tagC = \bigcup_{m = 0}^M\multihead_m[K]$, $K\tagB = \layernorm[K\tagC]$, and $K\tagA = \neuraln[K\tagB]$.
    
%     A bound for $C^{\layernorm}_{K\tagA}, C^{\layernorm}_{K\tagC}$ is given by \Cref{cor:LayerNorm}, $C^{\neuraln}_{K\tagB}$ is bounded in \Cref{cor:FeedForward}, and a bound for $C^{\multihead}_{K}$ is given in \Cref{cor:MultiHead}.
% \end{theorem}
% \begin{proof}
%     \Cref{cor:DerivativeBoundByLevel} yields
%     \begin{align*}
%         C^{\tblock}_K(\cleq n) &\leq
%         C^{\layernorm}_{K\tagA}({\cleq n})
%         C\tagA_K({\cleq n})^{n}
%         \Big[ \frac{ 2\odim n}{e\ln n} ( 1 + o(1) ) \Big]^{n}.
%     \end{align*}
%     where 
%     \begin{align*}
%         C\tagA_K(\cleq n) & \eqdef 
%         C^{\neuraln}_{K\tagB}({\cleq n})
%         C\tagB_K({\cleq n})^{n}
%         \Big[ \frac{ 2\idim n}{e\ln n} ( 1 + o(1) ) \Big]^{n},
%     \\
%         C\tagB_K(\cleq n) & \eqdef
%         C^{\layernorm}_{K\tagC}({\cleq n})
%         C\tagC_K({\cleq n})^{n}
%         \Big[ \frac{ 2\idim n}{e\ln n} ( 1 + o(1) ) \Big]^{n},
%     \\
%         C\tagC_K(\cleq n) & \eqdef 1 + C^{\multihead}_K(\cleq n),
%     \end{align*}
%     which concludes the proof.
% \end{proof}


% \begin{theorem}[$C^s$-Norm Bound of Transformers]
% \label{prop:transformerSobolevBound}
%     % Fix $n \in \N_+$. 
%     Fix $n,L,H,C,D,d,M \in \N_+$. 
%     % In the notation of \Cref{defn:Transformer} and the multivariate notation established in \Cref{not:Multivariate,not:Order,not:DerivativeBounds} let 
%     For any $\transformer \in \transformerclass_{L,H,C}^{D,d,M}$, 
%     any compact $K_0 \subset \R^{M \times D}$, and any $\alpha \in \N^{M \times D}$, $\vert \alpha \vert \eqdef n$ we have
%     \begin{align}\label{id:TransformerSobolevBound1}
%         C^{\transformer}_{K_{0}}(\alpha)
%         &\leq
%         \odim^LM\alpha!
%         \cdot
%         C^A 
%         \cdot
%         C^L(\alpha),
%     \end{align}
%     where $C^{1}(\alpha) \eqdef C^{\tblock_1}_{K_{0}}(\alpha)$ and for $l \in \myset{2}{L}$, 
%     \begin{align}\label{id:TransformerSobolevBound2}
%         C^{l}(\alpha) \eqdef 
%         &\leq
%         \alpha! \sum_{\beta \in \Order^{\Tilde{d}_l}_{\leq n}}  N(\beta)C^{\tblock_l}_{K_{l-1}}(\beta)
%         \sum_{\eta, \zeta \in \calP'(\order(\alpha),\beta)} 
%         \prod_{j=1}^{n} \frac{
%             C^l(\order(\zeta^{(j)}))^{\vert \eta^{(j)} \vert}
%         }{
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         }
%     \end{align}
%     where $K_l \eqdef \tblock_l[K_{l-1}]$,  $\Tilde{d}_{l} \eqdef M_{l}\idim^{l}$, and a bound for $C^{\tblock_l}_{K_{l-1}}(\beta)$ is given by \Cref{thm:TransformerBlockSobolevBound}, only depending on the transformer block class $\tblockclass_{d^l, M^l, H^l, C^l}$.
% \end{theorem}
% \begin{proof}[Proof of {Theorem~\ref{prop:transformerSobolevBound}}]
%     The bounds \eqref{id:TransformerSobolevBound1} are a direct consequence of \Cref{thm:DerivativeBoundByType} and \eqref{id:TransformerSobolevBound2} follows directly from \Cref{cor:DerivativeBoundAffine}.
% \end{proof}


% \subsection{Step 2 (C) - Merging the \texorpdfstring{$C^s$-Norm Bounds}{Regularity Estimates} for Transformers with the Loss Function}
% \label{s:Proofs__MergingCsNorms}

% In this section, we consider the following generalization of the class in Definition~\ref{def:sGrowthRate}.
% \begin{definition}[Smoothness Growth Rate]
% \label{def:sGrowthRate_v2}
% Let $d,D\in \mathbb{R}$.  A smooth function $g:\mathbb{R}^d\to \mathbb{R}^D$ is said to belong to the class $C^{\infty}_{poly:C,r}(\mathbb{R}^d,\mathbb{R}^D)$ (resp.\ $C^{\infty}_{exp:C,r}(\mathbb{R}^d,\mathbb{R}^D)$) if there exist $C,r\ge 0$ such that: for each $s\in \mathbb{N}_+$ 
% \begin{enumerate}
%     % \item[(i)] \textbf{Logarithmic Decay:} $\|\ell\|_{C^s} \le C_{\ell}\, \log(1+s)^{-r_{\ell}}$
%     \item[(i)] \textbf{Polynomial Growth -  $C^{\infty}_{poly:C,r}(\mathbb{R}^d,\mathbb{R}^D)$:} $\|g\|_{C^s} \le C\, s^{r}$,
%     \item[(ii)] \textbf{Exponential Growth -  $C^{\infty}_{exp:C,r}(\mathbb{R}^d,\mathbb{R}^D)$:} $\|g\|_{C^s} \le C\, e^{s\,r}$,
% \end{enumerate}
% \end{definition}


% The next lemma will help us relate the $C^s$-regularity of a model, a target function, and a loss function to their composition and product.  
% We use it to relate the $C^s$-regularity of a transformed model $\mathcal{T}:\mathbb{R}^d\to \mathbb{R}^D$, the target function $f^{\star}:\mathbb{R}^d\to \mathbb{R}^D$, and the loss function $\ell:\mathbb{R}^{2D}\to \mathbb{R}$ to their composition
% \begin{equation}
% \begin{aligned}
% \ell_{\mathcal{T}}:  \mathbb{R}^{d}& \to \mathbb{R} \\
% x & \mapsto \ell\big(\mathcal{T}(x),f^{\star}(x)\big)
% .
% \end{aligned}
% \end{equation}
% One we computed have the $C^s$-regularity of $\ell_{\mathcal{T}}$, we can apply a concentration of measure-type argument based on an optimal transport-type duality, as in~\cite{amit2022integral,hou2023instance,benitez2023out,kratsios2024tighter}, to obtain our generalization bounds.  A key technical point where our analysis largely deviates from the mentioned derivations, is that we are not relying on any i.i.d.\ assumptions.



% More generally, the next lemma allows us to bound the size of $\|\ell(\hat{f},f^{\star})\|_{C^s}$ using bounds on $C^s$ norms of $\transformerclass$ computed in Theorem~\ref{prop:transformerSobolevBound}, the target function $f^{\star}$, and on the loss function $\ell$.  Naturally, to use this result, we must assume a given level of regularity of the target function, as in Definition~\ref{def:sGrowthRate}.
% \begin{lemma}[$C^s$-Norm of loss of between two functions]
% \label{lem:control_loss__SSE}
% Let $d,D,s\in \mathbb{N}_+$, $f_1,f_2:\mathbb{R}^d\to \mathbb{R}^D$ be of class $C^{s}$ and $\ell:\mathbb{R}^{2D}\to\mathbb{R}$ be smooth.  If there are constants $C_1,C_2, \widetilde{C}_1,\dots,\widetilde{C}_s\geq 0$ such that:
% $\|f_i\|_{C^s} \le C_i$ for $i=1,2$ and for $j=1,\dots,s$ we have
% $\|\ell\|_{C^j} \le \widetilde{C}_j$ then for all $s>0$ large it satisfies 
% \begin{align} 
%  \label{eq:called_bound} 
%   \big\| \ell( f_1, f_2 ) \big\|_{C^s}  
%  = 
%  \begin{cases} 
%   \mathcal{O} \big[ \big( \frac{ 2D s }{e\ln s } (1+o(1)) \big)^s  \big] , \, & \mbox{if $\max_{1\leq k } \widetilde{C}_k  (C_1 C_2 )^k$ is bounded} , \\ 
%   \\ 
%   \mathcal{O} \big[  \widetilde{C}_{s}   
%    \big( C_1 C_2 \frac{ 2D s }{e\ln s } (1+o(1)) \big)^s  \big] , \, & \mbox{if $\max_{1\leq k } \widetilde{C}_k  (C_1 C_2 )^k$ is unbounded} .   
%  \end{cases} 
% \end{align} 
% Particularly, if $\ell \in C^{\infty}_{poly:C,r}(\mathbb{R}^{2D},\mathbb{R})$,  
%                     i.e., $\|\ell\|_{C^j}\le C\, j^{r}$ , then 
%                     \begin{align} 
%                     \big\| \ell( f_1, f_2 ) \big\|_{C^s} = 
% \mathcal{O} \big[  C s^r \big( C_1 C_2 \frac{ 2D s }{e\ln s } (1+o(1)) \big)^s  \big] ;  
% \label{eq:called_bound__polynomial_case}
%                     \end{align}
% if $\ell \in C^{\infty}_{exp:C,r}(\mathbb{R}^{2D},\mathbb{R})$, i.e., 
%             $\|\ell\|_{C^j} \le C\,e^{j\,r}$, then 
%             \begin{align} 
%             \big\| \ell( f_1, f_2 ) \big\|_{C^s} = 
% \mathcal{O} \big[  C e^{s r} \big( C_1 C_2 \frac{ 2D s }{e\ln s } (1+o(1)) \big)^s  \big] . 
% \label{eq:called_bound__exponential_case}
%             \end{align} 

% \begin{comment} 
% \begin{subequations} 
%     \begin{align}[left={\big\| \ell( f_1, f_2 ) \big\|_{C^s} =\empheqlbrace}]  
%            & \mathcal{O} \big[  C s^r \big( C_1 C_2 \frac{ 2D s }{e\ln s } (1+o(1)) \big)^s  \big], 
%             \, 
%             \text{ if $\ell \in C^{\infty}_{poly:C,r}(\mathbb{R}^{2D},\mathbb{R})$,  
%                     i.e., $\|\ell\|_{C^j}\le C\, j^{r}$ , } 
%             \label{eq:called_bound__polynomial_case}
%        \\
%           & \mathcal{O} \big[  C e^{s r} \big( C_1 C_2 \frac{ 2D s }{e\ln s } (1+o(1)) \big)^s  \big], 
%            \, 
%            \text{ if $\ell \in C^{\infty}_{exp:C,r}(\mathbb{R}^{2D},\mathbb{R})$, i.e., 
%             $\|\ell\|_{C^j} \le C\,e^{j\,r}$. }
%             \label{eq:called_bound__exponential_case}
%     \end{align}
% \end{subequations}
% \end{comment} 
% \end{lemma}
% Lemma~\ref{lem:control_loss__SSE} allows us to obtain a bound on the term $\sup_{\hat{f}\in C^s_R(\mathbb{R}^d)}\,\|\ell(\hat{f},f^{\star})\|_{C^s}$ in~\eqref{eq:risk_bound__decomposition2}, using Theorem~\ref{prop:transformerSobolevBound} and our assumptions on $\ell$ and on $f^{\star}$.  

% \begin{proof} [{Proof of Lemma~\ref{lem:control_loss__SSE}}]
% We first derive the general bound; which we then specialize to the case where the growth rate of $\ell$ is known. 
% We first observe that
% \begin{align} 
% %\label{eq:definition_Cs__norm}
%  \big\| \ell( f_1, f_2 ) \big\|_{C^s} 
%   = 
%   &
%     \underbrace{
%         \max_{k=1, \cdots, s-1} \max_{\alpha \in \{1, \cdots, d\}^k} \| D^\alpha \ell(f_1(x), f_2(x)) \|_\infty 
%     }_{\term{t:A}}
% \notag 
%   \\
%   + 
%   &
%   \underbrace{
%     \max_{\alpha \in \{1, \cdots, d\}^{s-1} } \operatorname{Lip}\big(  D^\alpha \ell(f_1(x), f_2(x))  \big) 
%     }_{\term{t:B}}
% .
%  \notag 
% \end{align} 
% \paragraph{{General Case - Term~\Cref{t:A}}:}
% By \Cref{cor:DerivativeBoundByLevel}, we have
% % By Theorem~\ref{thm:FaaDiBruno}, we can represent the derivatives of $\ell(f_1(x), f_2(x))$ through the multivariate Fa\`a di Bruno formula. For each $k=1$, ..., $s-1$ fixed, and for each $\alpha\in \{1, \cdots, d\}^k$, we have 
% % \begin{align} 
% %  D^\alpha \ell(f_1(x), f_2(x)) 
% %         =
% %         \sum_{1 \leq |\beta| \leq k} (D^\beta \ell)(f_1(x), f_2(x))
% %         \sum_{\eta, \zeta \in \calP(\alpha,\beta)} \alpha! 
% %         \prod_{j=1}^{k} \frac{
% %             [D^{\zeta^{(j)}} (f_1(x), f_2(x))]^{\eta^{(j)}}
% %         }{
% %             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
% %         } .  \notag 
% % \end{align} 
% %It follows from the triangle inequality and the positive homogeneity of the $\|\cdot \|_\infty$ norm that  
% \allowdisplaybreaks 
% \begin{align} 
% % &
% \Big\| (D^\alpha \ell)(f_1(x), f_2(x)) \Big\|_\infty 
% % \\  
% % \leq  & \sum_{1 \leq |\beta| \leq k}  \big\| (D^\beta \ell)(f_1(x), f_2(x)) \big\|_\infty 
% %         \sum_{\eta, \zeta \in \calP(\alpha,\beta)} \alpha! 
% %         \prod_{j=1}^{k} \frac{
% %            \big\|  [D^{\zeta^{(j)}} (f_1(x), f_2(x))]^{\eta^{(j)}} \big\|_\infty 
% %         }{
% %             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
% %         } 
% % \notag \\ 
% % \leq & 
% % \sum_{1 \leq |\beta| \leq k}  \widetilde{C}_{|\beta|}  
% %         \sum_{\eta, \zeta \in \calP(\alpha,\beta)} a! 
% %         \prod_{j=1}^{k} \frac{
% %           (C_1 C_2 )^{|\eta^{(j)}|}  
% %         }{
% %             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
% %         } \notag \\ 
% %          \leq & 
% % \sum_{1 \leq |\beta| \leq k}  \widetilde{C}_{|\beta|}  
% %         \sum_{\eta, \zeta \in \calP(\alpha,\beta)} \alpha !
% %         \frac{
% %           (C_1 C_2 )^{ \sum_{j=1}^k |\eta^{(j)}|}  
% %         }{ \prod_{j=1}^k
% %            \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
% %         } 
% %         \notag \\ 
% %  = & 
% % \sum_{1 \leq |\beta| \leq k}  \widetilde{C}_{|\beta|}  (C_1 C_2 )^{  |\beta|}  
% %         \sum_{\eta, \zeta \in \calP(\alpha,\beta)} \alpha !
% %         \prod_{j=1}^k
% %         \frac{
% %           1
% %         }{
% %            \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
% %         }   
% %         \notag \\ 
% %         \leq & 
% %         \big[ \max_{1\leq k \leq s-1} \widetilde{C}_{k}  (C_1 C_2 )^{  k } \big]   
% %         \sum_{1 \leq |\beta| \leq k}    
% %         \sum_{\eta, \zeta \in \calP(\alpha,\beta)} \alpha !
% %         \prod_{j=1}^k
% %         \frac{
% %           1
% %         }{
% %            \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
% %         }   
% %         \notag \\ 
%  \leq & 
%  \big[ \max_{1\leq k \leq s-1} \widetilde{C}_{k}  (C_1 C_2 )^{ k } \big]  \cdot 
%    \mathcal{O} \Big[ \Big( \frac{ 2D k }{e\ln k } ( 1+o(1) ) \Big)^{k} \Big]   , 
% \label{eq:bound_t:A}
% \end{align} 
% %where the last equality is due to Lemma~\ref{lem:mdFDBestimate}. 

% From~\eqref{eq:bound_t:A} we have for all large $s>0$ that   
% \begin{align} 
% \begin{aligned}
% &
%  \max_{k=1, \cdots, s-1} \max_{\alpha \in \{1, \cdots, d\}^k} \| D^\alpha \ell(f_1(x), f_2(x)) \|_\infty 
%  \\
%  & = 
%  \begin{cases} 
%   \mathcal{O} \big[ \big( \frac{ 2D s }{e\ln s } (1+o(1)) \big)^s  \big] , \, & \mbox{if $\max_{1\leq k } \widetilde{C}_k  (C_1 C_2 )^k$ is bounded} , \\ 
%   \\ 
%   \mathcal{O}\Big[
%     \widetilde{C}_s   
%    \Big( C_1 C_2 \frac{ 2D s }{e\ln s } (1+o(1)) \Big)^s \Big]   , \, & \mbox{if $\max_{1\leq k } \widetilde{C}_k  (C_1 C_2 )^k$ is unbounded} .   
%  \end{cases} 
% \end{aligned}
% \notag 
% \end{align} 



% \paragraph{{General Case - Term~\Cref{t:B}}:}
% For each $\alpha\in \{1, \cdots, d\}^{s-1}$, by the multivariate Fa\`a di Bruno formula, we have    
% \begin{align}
%         D^\alpha \ell(f_1(x), f_2(x)) 
%         =
%         \sum_{1 \leq |\beta| \leq s-1} (D^\beta \ell)(f_1(x), f_2(x)) 
%         \sum_{\eta, \zeta \in \calP(\alpha,\beta)} \alpha! 
%         \prod_{j=1}^{s-1} \frac{
%             [D^{\zeta^{(j)}}(f_1(x), f_2(x))]^{\eta^{(j)}}
%         }{
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         }. 
%         \notag 
%     \end{align} 
% The Lipschitz constants of the derivatives satisfy 
% \allowdisplaybreaks
% \begin{align}
%     &  \operatorname{Lip} \big(  D^\alpha \ell(f_1(x), f_2(x)) \big)  \notag \\ 
%     = & 
%         \sum_{1 \leq |\beta| \leq s-1} \operatorname{Lip} \big( (D^\beta \ell)(f_1(x), f_2(x)) \big)   
%         \sum_{\eta, \zeta \in \calP(\alpha,\beta)} \alpha! 
%         \prod_{j=1}^{s-1} \frac{
%            \operatorname{Lip}\big( [D^{\zeta^{(j)}}(f_1(x), f_2(x))]^{\eta^{(j)}} \big) 
%         }{
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         } 
%         \notag \\ 
%     \leq  & 
%         \sum_{1 \leq |\beta| \leq s-1} \widetilde{C}_{|\beta|+1}   
%         \sum_{\eta, \zeta \in \calP(\alpha,\beta)} \alpha ! 
%         \prod_{j=1}^{s-1} \frac{
%            (C_1 C_2)^{|\eta(j)|}  
%         }{
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         } \notag \\ 
%    = & 
%         \sum_{1 \leq |\beta| \leq s-1} \widetilde{C}_{|\beta|+1}   (C_1 C_2)^{|\beta |}
%         \sum_{\eta, \zeta \in \calP(\alpha,\beta)} \alpha ! 
%         \prod_{j=1}^{s-1} \frac{ 1 }{
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         } \notag \\ 
%     \leq & 
%     \big[ \max_{1\leq k \leq s-1} \widetilde{C}_{k+1}   (C_1 C_2)^{k} \big]  
%     \sum_{1 \leq |\beta| \leq s-1} 
%         \sum_{\eta, \zeta \in \calP(\alpha,\beta)} \alpha ! 
%         \prod_{j=1}^{s-1} \frac{ 1 }{
%             \eta^{(j)}!(\zeta^{(j)}!)^{|\eta^{(j)}|}
%         }  \notag  \\ 
%     = & 
%  \big[ \max_{1\leq k \leq s-1} \widetilde{C}_{k+1}  (C_1 C_2 )^{ k } \big]  \cdot 
%   \mathcal{O} \Big[ \Big( \frac{ 2D s }{e\ln s} (1+o(1)) \Big)^s  \Big] , 
% \label{eq:bound_t:B}
%     \end{align} 
% where the last equality is due to Lemma~\ref{lem:mdFDBestimate}. 

% From~\eqref{eq:bound_t:B} we have for all $s>0$ large that 
% \begin{align} 
% \begin{aligned}
%   &\max_{\alpha \in \{1, \cdots, d\}^{s-1} } \operatorname{Lip}\big(  D^\alpha \ell(f_1(x), f_2(x))  \big) 
% \\
%  & = 
%  \begin{cases} 
%   \mathcal{O} \big[ \big( \frac{ 2D s }{e\ln s } (1+o(1)) \big)^s  \big] , \, & \mbox{if $\max_{1\leq k } \widetilde{C}_k  (C_1 C_2 )^k$ is bounded} , \\ 
%   \\ 
%   \mathcal{O} \big[  \widetilde{C}_{s}   
%    \big( C_1 C_2 \frac{ 2D s }{e\ln s } (1+o(1)) \big)^s  \big] , \, & \mbox{if $\max_{1\leq k } \widetilde{C}_k  (C_1 C_2 )^k$ is unbounded} .   
%  \end{cases} 
% \end{aligned}
% \notag 
% \end{align} 



% %    \begin{align} 
% %   \operatorname{Lip} \big( [D^{\zeta^{(j)}}(f_1(x), f_2(x))]^{\eta^{(j)}} \big)  
% % = & \operatorname{Lip} \big( [D^{\zeta^{(j)}}f_1(x), \,  D^{\zeta^{(j)}} f_2(x)]^{\eta^{(j)}} \big)  
% %    \notag \\ 
% %    = & (C_1 C_2)^{|\eta(j)|} \notag 
% %    \end{align} 

% %By the Rademacher-Stephanov theorem \citep[Theorems 3.1.6 and 3.1.9]{Federer_GeometricMeasureTheoryBook_1969}, 
% %\begin{align} 
% % \operatorname{Lip} \big( D^\alpha \ell(f_1(x), f_2(x)) \big)  
% % = & \max_{x\in \mathbb{R}^d} \Big| \nabla_x \Big(  D^\alpha \ell(f_1(x), f_2(x)) \Big) \Big| \notag \\ 
% % = & \max_{x\in \mathbb{R}^d} \Big| \big( D_{x_1}  D^\alpha \ell(f_1(x), f_2(x)) , \cdots, D_{x_d}  D^\alpha 
% % \ell(f_1(x), f_2(x)) \big) \Big|  
% % \notag 
% %\end{align} 

% \paragraph{Completing the General Case:}
% Combining our estimates for terms~\Cref{t:A} and~\Cref{t:B} respectively obtained in~\eqref{eq:bound_t:A} and~\eqref{eq:bound_t:B},
% we obtain an upper-bound for $\| \ell( f_1, f_2 ) \|_{C^s}$ via 
% \begin{align} 
%   \big\| \ell( f_1, f_2 ) \big\|_{C^s}  
%  = 
%  \begin{cases} 
%   \mathcal{O} \big[ \big( \frac{ 2D s }{e\ln s } (1+o(1)) \big)^s  \big] , \, & \mbox{if $\max_{1\leq k } \widetilde{C}_k  (C_1 C_2 )^k$ is bounded} , \\ 
%   \\ 
%   \mathcal{O} \big[  \widetilde{C}_{s}   
%    \big( C_1 C_2 \frac{ 2D s }{e\ln s } (1+o(1)) \big)^s  \big] , \, & \mbox{if $\max_{1\leq k } \widetilde{C}_k  (C_1 C_2 )^k$ is unbounded} .   
%  \end{cases} \notag 
%  %\label{eq:called_bound} 
% \end{align} 






% \paragraph{Special Cases of Interest:}
% In particular, if $\ell$ belongs either to $C^{\infty}_{poly:C,r}(\mathbb{R}^d,\mathbb{R}^D)$ or to $C^{\infty}_{exp:C,r}(\mathbb{R}^d,\mathbb{R}^D)$, , as in Definition~\eqref{def:sGrowthRate}, then: there exists constants $C_{\ell},r_{\ell}>0$ s.t.\ for each $j=1,\dots,s$ we have
% \begin{enumerate}
%     \item[(i)] \textbf{Polynomial Growth -  $C^{\infty}_{poly:C,r}(\mathbb{R}^{2D},\mathbb{R})$ Case:} 
%     \begin{align*}
%             \|\ell\|_{C^j}
%         \le
%             C\, j^{r}
%         \eqdef 
%             \tilde{C}_j
%     ,
%     \end{align*}
%     \item[(ii)] \textbf{Exponential Growth -  $C^{\infty}_{exp:C,r}(\mathbb{R}^{2D},\mathbb{R})$ Case:} 
%     \begin{align*}
%             \|\ell\|_{C^j} 
%         \le 
%             C\,e^{j\,r}
%         \eqdef 
%             \tilde{C}_j
%     .
%     \end{align*}
% \end{enumerate}
% %%
% %%
% Consequentially, in cases (i) and (ii), the bound in~\eqref{eq:called_bound} respectively becomes
% \begin{enumerate}
%     \item[(i)] \textbf{Polynomial Growth -  $C^{\infty}_{poly:C,r}(\mathbb{R}^{2D},\mathbb{R})$ Case:} 
% \begin{align}
%  \big\| \ell( f_1, f_2 ) \big\|_{C^s} 
%   \le & 
%     \mathcal{O} \big[  C s^r   
%    \big( C_1 C_2 \frac{ 2D s }{e\ln s } (1+o(1)) \big)^s  \big] , 
% \notag 
% %\label{eq:called_bound__polynomial_case}
% \end{align}
%     \item[(ii)] \textbf{Exponential Growth -  $C^{\infty}_{exp:C,r}(\mathbb{R}^{2D},\mathbb{R})$ Case:} 
% \begin{align}
%  \big\| \ell( f_1, f_2 ) \big\|_{C^s} 
%   \le & 
%     \mathcal{O} \big[  C e^{s r}   
%    \big( C_1 C_2 \frac{ 2D s }{e\ln s } (1+o(1)) \big)^s  \big] . 
% \notag 
% %\label{eq:called_bound__exponential_case}
% \end{align}
% \end{enumerate}

% \end{proof} 


% \begin{comment}
% \newpage
% \section{Old: Bounding Higher Derivative Norms in Transformer Models}
% \subsection{Results based on the chain rule}

% Recall the chain rule
% \begin{align*}
% \frac{df_n \circ f_{n-1} \circ ... \circ f_1}{dx} = \frac{df_n}{df_{n-1}} \cdot \frac{df_{n-1}}{df_{n-2}} \cdot \ldots \cdot \frac{df_2}{df_1} \cdot \frac{df_1}{dx}.
% \end{align*}
% Here, the functions \( f_1, f_2, \ldots, f_n \) represent the compositions of transformations in the transformer class, and \( x \) is the input variable. Each \( {df_i}/{df_{i-1}} \) denotes the derivative of the \( i \)th transformation with respect to the \( (i-1) \)th transformation. This equation enables us to compute the derivative of the composite transformation with respect to the input variable.

% If we are interested in higher order derivatives, we can make use of Faa di Bruno's formula, which for \( f \circ g(x) \) and \( n \in \mathbb{N} \) is given by
% \begin{align*}
% \frac{d^n}{dx^n} f(g(x)) = \sum \frac{n!}{\prod_{k=1}^{n} m_k! (k!)^{m_k}} \cdot f^{(m_1 + m_2 + \cdots + m_n)}(g(x)) \cdot \prod_{k=1}^{n} g^{(k)}(x)^{m^k},
% \end{align*}
% where the sum is taken over all \(n\)-tuples of non-negative integers \((m_1, m_2, \ldots, m_n)\) satisfying the constraint \(1\cdot m_1 + 2\cdot m_2 + \cdots + n\cdot m_n = n\). Let's simplify notation by 
% \begin{align*}
%     \mathcal{M}^n &\eqdef \mySet{m := (m_1, m_2, \ldots, m_n) \in \N^n}{1\cdot m_1 + 2\cdot m_2 + \cdots + n\cdot m_n = n}, \\
%     \vert m \vert &\eqdef \sum_{k=1}^n m_k, \quad \forall m \in \mathcal{M}^n, \\
%     \alpha(m) &\eqdef \frac{n!}{\prod_{k=1}^{n} m_k! (k!)^{m_k}}, \quad \forall m \in \mathcal{M}^n,
% \end{align*}
% and we arrive at 
% \begin{align*}
%     \frac{d^n}{dx^n} f(g(x)) = \sum_{m \in \mathcal{M}^n} \alpha(m) \cdot f^{(\vert m \vert)}(g(x)) \cdot \prod_{k=1}^{n} g^{(k)}(x)^{m^k}.
% \end{align*}
% Since for all $m \in \mathcal{M}^n$
% \begin{align*}
%     \Big\Vert \prod_{k=1}^{n} g^{(k)}(x)^{m^k} \Big \Vert_\infty 
%     =
%     \prod_{k=1}^{n} \big\Vert g^{(k)}(x)^{m^k} \big\Vert_\infty 
%     \leq 
%     \prod_{k=1}^{n} \left( 1 + \Vert g^{(k)}(x)\Vert_\infty^{n}  \right),
% \end{align*}
% we have 
% \begin{align*}
%     \Big\Vert \frac{d^n}{dx^n} f(g(x)) \Big\Vert_\infty 
%     & \leq 
%     M(n)
%     \prod_{k=1}^{n} \left( 1 + \Vert g^{(k)}(x)\Vert_\infty^{n}  \right)
%     \sum_{k = 1}^N \Vert f^{(k)}(g(x)) \Vert_\infty, \\
%     & \leq 
%     M(n)
%     \prod_{k=1}^{n} \left( 1 + \Vert g^{(k)}(x)\Vert_\infty^{n}  \right)
%     \sum_{k = 1}^N \Vert f^{(k)}(x) \Vert_\infty,
% \end{align*}
% where $M(n) := \max_{k=1}^n \sum_{m \in \mathcal{M}, \vert m \vert = k} \alpha(m)$.



% \subsection{Explicit derivatives}

% \begin{lemma}[Derivatives of $\softmax$]
% For 
% \begin{align*}%\label{id:Softmax}
%     \softmax:
%             \R^F 
%         \to     
%             \R^F,
%     \quad 
%             x 
%         \mapsto 
%             \left(
%                     {\exp(x_i)}
%                 /
%                     {\textstyle\sum_{j = 0}^{F-1} \exp(x_j)}
%             \right)_{i=0}^{F-1}.
% \end{align*}
% it holds for a multi-index $m := (m_1, \ldots, m_k) \in \myset{0}{F-1}^k, k \in \N$ that 
% \begin{align*}
%     \softmax^{(m)} (x) = \sum \softmax(x_{m_0}) \prod_{i=1}^k (...  - \softmax(x_{m_i}))
% \end{align*}
% \end{lemma}
% \begin{proof}
%     For $m_0, m_1 \in \myset{0}{F-1}$ we have
%     \begin{align*}
%         \frac{\partial \softmax}{\partial x_{m_1}} (x_{m_0}) = \softmax(x_{m_0})\left( \delta_{m_0m_1} - \softmax(x_{m_1})\right)
%     \end{align*}
%     For $m_2 \in \myset{0}{F-1}$ we have
%     \begin{align*}
%         \frac{\partial \softmax}{\partial x_{m_1}x_{m_2}} (x_{m_0}) &=
%         \softmax(x_{m_0})
%         \left( \delta_{m_0m_2} - \softmax(x_{m_2})\right)
%         \left( \delta_{m_0m_1} - \softmax(x_{m_1})\right) \\
%         &-
%         \softmax(x_{m_0})
%         \softmax(x_{m_1})
%         \left( \delta_{m_1m_2} - \softmax(x_{m_2})\right)
%     \end{align*}
%     For $m_3 \in \myset{0}{F-1}$ we have
%     \begin{align*}
%         &\frac{\partial \softmax}{\partial x_{m_1}x_{m_2}x_{m_3}} (x_{m_0}) \\
%         =
%         &+
%         \softmax(x_{m_0})
%         \left( \delta_{m_0m_1} - \softmax(x_{m_1})\right) 
%         \left( \delta_{m_0m_2} - \softmax(x_{m_2})\right)
%         \left( \delta_{m_0m_3} - \softmax(x_{m_3})\right) \\
%         &-
%         \softmax(x_{m_0})
%         \left( \delta_{m_0m_1} - \softmax(x_{m_1})\right) 
%         \softmax(x_{m_2})
%         \left( \delta_{m_2m_3} - \softmax(x_{m_3})\right) \\
%         &-
%         \softmax(x_{m_0})
%         \softmax(x_{m_1})
%         \left( \delta_{m_0m_2} - \softmax(x_{m_2})\right)
%         \left( \delta_{m_1m_3} - \softmax(x_{m_3})\right) \\
%         &-
%         \softmax(x_{m_0})
%         \softmax(x_{m_1})
%         \left( \delta_{m_1m_2} - \softmax(x_{m_2})\right) 
%         \left( \delta_{m_0m_3} - \softmax(x_{m_3})\right) \\
%         &-
%         \softmax(x_{m_0})
%         \softmax(x_{m_1})
%         \left( \delta_{m_1m_2} - \softmax(x_{m_2})\right) 
%         \left( \delta_{m_1m_3} - \softmax(x_{m_3})\right) \\
%         &+
%         \softmax(x_{m_0})
%         \softmax(x_{m_1})
%         \softmax(x_{m_2})
%         \left( \delta_{m_2m_3} - \softmax(x_{m_3})\right) \\
%         %
%         %
%         %
%     \end{align*}
% \end{proof}
% \begin{lemma}[Derivatives of $\softplus$]
%     For 
%     \begin{align*}
%         \softplus: \R \to \R, \quad x \mapsto \ln (1 + \exp(\cdot))
%     \end{align*}
%     it holds 
%     \begin{align*}
%         \softplus^{(1)}(x) = \sigmoid(x) \eqdef 1 / (1 + \exp(-x))
%     \end{align*}
%     and for $n \in \N$
%     \begin{align*}
%         \softplus^{(n + 1)}(x) = \sigmoid^{(n)}(x) = \sum_{k=0}^n(-1)^{n+k}k!S_{n,k}\sigmoid(x)(1-\sigmoid(x))^k,
%     \end{align*}
%     where $S_{n,k}$ are the Stirling numbers of the second kind, $S_{n,k} \eqdef \frac{1}{k!} \sum_{j=0}^{k} (-1)^{k-j} \binom{k}{j} j^n$.
% \end{lemma}
% \begin{proof}
% We start with Fa\`a di Bruno's formula,
% \begin{align*}
%     \frac{d^n}{dt^n}\sigmoid(x)=\frac{d^n}{dx^n}\frac{1}{f(x)}=\sum_{k=0}^n(-1)^kk!f^{-(k+1)}(x)B_{n,k}(f(x)),
% \end{align*}
% where \(f(x) \eqdef 1 + \exp(-x)\) and \(B_{n,k}(f(x))\) denotes the Bell polynomials evaluated on $f(x)$. Next, we know the \(k\)-th derivative of \(f(x)\) is given by
% \begin{align*}
%    \frac{d^k}{dt^k}f(x)=(1-k)_k+ke^{-x}.
% \end{align*}
% Now, using the definition of the Bell polynomials \(B_{n,k}(f(t))\), we have
% \begin{align*}
%     B_{n,k}(f(x))=(-1)^nS_{n,k}e^{-kx},
% \end{align*}
% where \(S_{n,k}\) represents the Stirling numbers of the second kind. Substituting the expression for \(B_{n,k}(f(x))\) into the derivative of \(\sigmoid(x)\), we obtain
% \begin{align*}
%     \frac{d^n}{dx^n}\sigmoid(x)=\sum_{k=0}^n(-1)^{n+k}k!S_{n,k}\sigmoid(x)(1-\sigmoid(x))^k.
% \end{align*}
% \end{proof}

% \begin{lemma}[Derivatives of $\layernorm$]
% For 
% \begin{align*}
%     \layernorm(x;\gamma,\beta,w)\eqdef  
%         \gamma\, 
%         \frac{(x-\mu_x^w)}{1 + \softplus(\sigma_x^w)} + \beta 
% \end{align*}
% it holds for a multi-index $m := (m_1, \ldots, m_k) \in \myset{0}{F-1}^k, k \in \N$ that 
% \begin{align*}
%     \layernorm^{(m)}(x;\gamma,\beta,w) = ...
% \end{align*}
% \end{lemma}
% \begin{proof}
%     Define 
%     \begin{align*}
%     \begin{cases}
%         f(x) := \gamma (x - \mu_x^w) \\ 
%         g(x) := {1}/({1 + \softplus(\sigma_x^w)}),
%     \end{cases}
%     \end{align*}
%     then we see
%     \begin{align*}
%         \layernorm^{(m)}(x;\gamma,\beta,w) = f(x)g^{(m)} + \sum_{i=1}^k\frac{\partial f}{\partial x_{m_i}}(x)\frac{\partial g}{\partial x_{m_1} \cdots x_{m_{i-1}} x_{m_{i+1}}x_{m_k}}(x).
%     \end{align*}
%     Note that we can write $g = h \circ \softplus \circ \sigma^w$ for 
%     \begin{align*}
%         h(x) := \frac{1}{1+x}.
%     \end{align*}
%     \yannick{There exists a special formula for one dimensional compositions, see \cite{ConstantineSavits96}.}
% \end{proof}



% \newpage
% \end{comment}

% % \section{Shirayev-Wonham Filtering}
% % \paragraph{From \cite[Chapter 9]{LipShiryaev_I_2001}.}
% % Consider a complete probability space $(\Omega, \mathcal{F}, P)$ equipped with a nondecreasing sequence of right-continuous sub-$\sigma$-algebras $\mathcal{F}_t, 0 \leq t \leq T$. Let $\theta = (\theta_t, \mathcal{F}_t)$, $0 \leq t \leq T$, denote a real right-continuous Markov process taking values in the countable set $E = \{\alpha, \beta, \gamma, \ldots\}$. Additionally, let $W = (W_t, \mathcal{F}_t)$, $0 \leq t \leq T$, be a standard Wiener process independent of $\theta$, and let $\xi_0$ be a $\mathcal{F}_0$-measurable random variable independent of $\theta$. We assume the existence of nonanticipative functionals $A_t(\epsilon, x)$ and $B_t(x)$ that define
% % \begin{align}
% %     d\xi_t = A_t(\theta_t, \xi) dt + B_t(\xi)dW_t
% % \end{align}
% % and satisfy the following conditions.
% % \begin{gather}
% %     A^2_t(\epsilon_t, x) \leq L_1 \int_0^t (1 + x_s^2)dK(s) + L_2(1 + \epsilon^2_t + x^2_t), 
% %     \label{id:LS1}
% % \\
% %     0 < C \leq B^2_t(x) \leq L_1 \int_0^t (1 + x_s^2)dK(s) + L_2(1 + x^2_t),  
% %     \label{id:LS2}
% % \\
% %     |A_t(\epsilon_t, x) - A_t(\epsilon_t, y)|^2 + |B_t(x) - B_t(y)|^2
% %     \leq L_1 \int_0^t (x_s - y_s)^2 dK(s) + L_2(x_t - y_t)^2, 
% %     \label{id:LS3}
% % \end{gather}
% % where $C, L_1, L_2$ are certain constants, $K(s)$ is a non-decreasing right continuous function, $0 \leq K(s) \leq 1, x \in C_T, y \in C_T, \epsilon_t \in E, 0 \leq t \leq T$.

% % Along with \Cref{id:LS1,id:LS2,id:LS3} it will also be assumed that
% % \begin{align}
% %     M\xi^2_0 < \infty,
% %     \label{id:LS4}
% % \end{align}
% % and
% % \begin{align}
% %     M \int_0^T \theta^2_t dt < \infty. 
% %     \label{id:LS5}
% % \end{align}

% % Define 
% % \begin{align*}
% %     p_\beta(t) &\eqdef P(\theta_t = \beta), \\
% %     p_{\beta\alpha}(t, s) &\eqdef P(\theta_t = \beta|\theta_s = \alpha), \quad 0 \leq s < t \leq T, \quad \beta, \alpha \in E,
% % \end{align*}
% % and assume there exist a function $\lambda_{\alpha\beta}(t), 0 \leq t \leq T, \alpha, \beta \in E$, that is 
% % \begin{gather}
% %     \text{continuous over \(t\),  (uniformly over \(\alpha, \beta\))}
% %     \label{id:LS6}
% %     \\
% %     |\lambda_{\alpha\beta}(t)| \leq K 
% %     \label{id:LS7}
% %     \\
% %     |p_{\beta\alpha}(t + \Delta, t) - \delta(\beta, \alpha) - \lambda_{\alpha\beta}(t) \cdot \Delta| \leq o(\Delta),
% %     \label{id:LS8}
% % \end{gather}
% % where \(\delta(\beta, \alpha)\) is a Kronecker's symbol and the value \(o(\Delta)/\Delta \rightarrow 0 \) as \(\Delta \rightarrow 0\) (uniformly over \(\alpha, \beta\)).  

% % \begin{theorem}
% % Let the \Cref{id:LS1,id:LS2,id:LS3,id:LS4,id:LS5,id:LS6,id:LS7,id:LS8} be fulfilled. Then the a posteriori probability $\pi_\beta(t)$, $\beta \in \mathcal{E}$, satisfies a system of equations
% % \begin{align*}
% % \pi_\beta(t) = p_\beta(0) + \int_0^t \mathcal{L}^*\pi_\beta(u)du + \int_0^t \pi_\beta(u)\frac{A_u(\beta, \xi) - \bar{A}_u(\xi)}{B_u(\xi)} d\bar{W}_u,
% % \end{align*}
% % where
% % \begin{align*}
% % \mathcal{L}^*\pi_\beta(u) &= \sum_{\gamma \in \mathcal{E}} \lambda_{\gamma\beta}(u)\pi_\gamma(u), \\
% % \bar{A}_u(\xi) &= \sum_{\gamma \in \mathcal{E}} A_u(\gamma, \xi)\pi_\gamma(u),
% % \end{align*}
% % and $ \bar{W} = (\bar{W}_t, \mathcal{F}_t) $ is a Wiener process with
% % \begin{align*}
% %     \bar{W}_t = \int_0^t \frac{d\xi_u - \bar{A}_u(\xi)du}{B_u(\xi)}.
% % \end{align*}
% % \end{theorem}

% % \newpage

% \begin{comment}
% \section{Old and Future Ideas}
% \subsection{Embedding Uncertainty Into the Transformer Model}

% \AK{History instead of memory, to align with RL community.}

% \yannick{Do we need it with the new approach?}

% Fix a regularization parameter $\varepsilon>0$.  
% For $d\in \mathbb{N}_+$ any measures $\mu,\nu \in \mathcal{P}(\mathbb{R}^d)$ with density with respect to the Lebesgue measure on $\mathbb{R}^d$ and with exponential moments, we define their \textit{entropy-regularized $2$-Wasserstein distance}, denoted by $\operatorname{OT}^{\varepsilon}$, by
% \begin{align*}
%     \operatorname{OT}^{\varepsilon}(\mu,\nu)
%     \eqdef
%     \min_{\pi\in \operatorname{Cpl}(\mu,\nu)}
%     \,
%     \mathbb{E}_{(X_1,X_2)\sim \pi}\biggl[
%         \|X_1-X_2\|^2
%         -
%         \varepsilon\,
%         \mathbb{E}_{Z\sim \mu}\Big[
%             \log\Big(\frac{p_{\nu}}{p_{\mu}}(Z)\Big)
%         \Big]
%     \biggr]
% \end{align*}
% where $p_{\nu}$ and $p_{\mu}$ are the respective Radon-Nikodym derivatives of $\nu$ and $\mu$ with respect to the Lebesgue measure on $\mathbb{R}^d$.


% Fix memory hyperparameters hyperparameter $\alpha>0$ and $M\in \mathbb{N}_+$.  
% %
% Unlike classical time series models, the sequential deep learning models $\hat{f}^1,\dots,\hat{f}^k$ do not capture uncertainty.  Here, instead of postulating a single distribution/measure on the space of inputs and output as in \cite{xxx}, a family of probability measures as in robust finance \cite{xxx} or PAC learning theory \cite{xxx}, or even considering extremal worst-case results over all possible paths as in \cite{xxx}, we instead progressively infer randomness.  That is, we construct a sequence/discrete-flow of probability measures capturing the error distribution of each sequential deep learning model.
% %
% Each model $\mathcal{T}\in \mathcal{T}_{L,W,H}^{D,d:M}$ is lifted to a measure-valued model taking values in the space $\mathcal{N}_d$ of Gaussian measures on $\mathbb{R}^d$.  We can do this by leveraging the sequential structure of the learning problem.  

% Specifically, consider a map 
% \begin{equation}
% \label{eq:uncertain_transformer}
% \begin{aligned}
%     \boldsymbol{\mathcal{T}}:\mathbb{R}^{2M\,d}\times \mathbb{R}^{2M\,D} & \to \mathcal{N}_d
%     \\
%     y_{[-2M-2:-1]}\times x_{[-2M:0]} & \mapsto \mathcal{N}_d\big(\mathcal{T}(x_{[-M:0]}),\Sigma(y_{[-M-1:-1]},x_{[-M:0]}|\mathcal{T})\big)
% \end{aligned}
% \end{equation}
% where we have indexed vectors in $\mathbb{R}^{M\,d}$ by one shifted time-step in the past, to emphasize that they correspond to \textit{historically} observed targets, and where for each $j,k=1,\dots,D$, the $j,k^{th}$ entry of the \textit{uncertainty} matrix $\Sigma_{j,k}\eqdef \Sigma(y_{[-M-1:-1]},x_{[-M:0]}|\mathcal{T})_{j,k}$ is given by
% \begin{equation*}
% \begin{aligned}
%     \Sigma_{j,k}
%         % \Sigma(y_{[-M-1:-1]},x_{[-M:0]}|\mathcal{T})|\mathcal{T}))_{j,k}
%     &
%     \eqdef 
%         \frac1{
%             1
%             -
%             \sum_{s=t-M}^t\,
%                 e^{-\alpha 2\,(t-s)}
%         }
%     \,
%         \sum_{s=-M}^0
%             e^{-\alpha(t-s)}
%             \,
%             \big(
%                 (E_s)_j
%                 -(\bar{E}_s)_j
%             \big)
%             \big(
%                 (E_s)_k
%                 -(\bar{E}_s)_k
%             \big)
%     \\
%     E_s & \eqdef 
%         \|\mathcal{T}(x_{[-M-s-1:-s-1]}) - y_{-s}\|^2
% \end{aligned}
% \end{equation*}
% where, $s=-M,\dots,0$, and $j,k=1,\dots,D$.

% \begin{lemma}
% \label{lem:regularity_2}
% Fix regularization hyperparameters $\varepsilon,\lambda>0$ and a map $\boldsymbol{\mathcal{T}}$ as in~\eqref{eq:uncertain_transformer} as consider the associated \textit{loss} $\ell(\cdot|\mathcal{T}):\boldsymbol{\mathcal{T}}:\mathbb{R}^{(3+2M)\,d}\times \mathbb{R}^{2M\,D} \to \mathcal{R}$ mapping each $y_{[-2M-2:0]}\times x_{[-2M:0]} \in \mathbb{R}^{(3+2M)\,d}\times \mathbb{R}^{2M\,D}$ by
% \begin{equation}
% \begin{aligned}
%     % \ell(\cdot|\mathcal{T}):\boldsymbol{\mathcal{T}}:\mathbb{R}^{(3+2M)\,d}\times \mathbb{R}^{2M\,D} & \to \mathcal{R}
%     % \\
%     % y_{[-2M-2:-1]}\times x_{[-2M:0]} & \mapsto 
%     \operatorname{OT}^{\varepsilon}
%         \Big(
%                 \mathcal{N}_d(y_0,\lambda\,I_d)
%             \,
%             ,
%             \,
%                 \mathcal{N}_d\big(\mathcal{T}(x_{[-M:0]}),\Sigma(y_{[-M-1:-1]},x_{[-M:0]}|\mathcal{T})\big)
%         \Big).
% \end{aligned}
% \end{equation}
% \AK{@Yannick and @Xuwei we want the smoothness of this map, ie its $C^k$ norms; using the previous first lemma.
% }    
% \end{lemma}
% \begin{proof}[{Proof of Lemma~\ref{lem:regularity_2}}]
% Fix $y_{[-2M-2:0]}\times x_{[-2M:0]} \in \mathbb{R}^{(3+2M)\,d}\times \mathbb{R}^{2M\,D}$.  We compute
% \allowdisplaybreaks
% \begin{align}
% \nonumber
%     &
%         \operatorname{OT}^{\varepsilon}
%         \Big(
%                 \mathcal{N}_d(y_0,\lambda\,I_d)
%             \,
%             ,
%             \,
%                 \mathcal{N}_d\big(\mathcal{T}(x_{[-M:0]}),\Sigma(y_{[-M-1:-1]},x_{[-M:0]}|\mathcal{T})\big)
%         \Big)
%     \\
%     \label{eq:simplification_OT__Centering}
%     = & 
%         \|y_0-\mathcal{T}(x_{[-M:0]})\|^2
%     \\
%     \nonumber
%     & +
%         \operatorname{OT}^{\varepsilon}
%             \Big(
%                     \mathcal{N}_d(0,\lambda\,I_d)
%                 \,
%                 ,
%                 \,
%                     \mathcal{N}_d\big(0,\Sigma(y_{[-M-1:-1]},x_{[-M:0]}|\mathcal{T})\big)
%             \Big)
%     \\
%     \label{eq:simplification_OTCentered}
%     = & 
%         \|y_0-\mathcal{T}(x_{[-M:0]})\|^2
%     \\
%     \nonumber
%     & +
%         % I used this naming
%         % K_0 \eqdef \lambda\,I_d
%         % K_1 \eqdef \Sigma(y_{[-M-1:-1]},x_{[-M:0]}|\mathcal{T})
%     \operatorname{tr}(\lambda\,I_d) 
%     +
%     \operatorname{tr}\big(
%         \Sigma(y_{[-M-1:-1]},x_{[-M:0]}|\mathcal{T})
%     \big)
%     \\
%     \nonumber
%     &
%     - 
%     \frac{\varepsilon}{2}\,
%         \big(
%             % Constant Factor Bit
%             d\log(2) - 2d
%         \big)
%     \\
%     \nonumber
%         % Important Bit
%     &
%         -
%         \frac{\varepsilon}{2}\,
%             \operatorname{tr}\Big(
%                 \big(
%                         I_d + \frac{4^2}{\varepsilon^2}\,(\lambda\,I_d)(\Sigma(y_{[-M-1:-1]},x_{[-M:0]}|\mathcal{T}))
%                 \big)^{1/2}
%             \Big)
%     \\
%     \nonumber
%     &
%             -\frac{\varepsilon}{2}\,
%                 \log\Big(
%                     \big(
%                             I_d + \frac{4^2}{\varepsilon^2}\,(\lambda\,I_d)(\Sigma(y_{[-M-1:-1]},x_{[-M:0]}|\mathcal{T}))
%                     \big)^{1/2}
%                 \Big)
%         \Big)
% %%%%%
% %%%%%
% %%%%%
% %%%% Simple simplifications
% %%%%%
% %%%%%
% %%%%%
%     \\
%     \nonumber
%     = & 
%         \|y_0-\mathcal{T}(x_{[-M:0]})\|^2
%     \\
%     \nonumber
%     & +
%         % I used this naming
%         % K_0 \eqdef \lambda\,I_d
%         % K_1 \eqdef \Sigma(y_{[-M-1:-1]},x_{[-M:0]}|\mathcal{T})
%     d\lambda
%     +
%     \operatorname{tr}\big(
%         \Sigma(y_{[-M-1:-1]},x_{[-M:0]}|\mathcal{T})
%     \big)
%     \\
%     \nonumber
%     &
%     - 
%     \frac{\varepsilon\,d(\log(2) - 2)}{2}\,
%     \\
%     \nonumber
%         % Important Bit
%     &
%         -
%         \frac{\varepsilon}{2}\,
%             \operatorname{tr}\Big(
%                 \big(
%                         I_d + \frac{4^2}{\varepsilon^2}\,(\lambda\,I_d)(\Sigma(y_{[-M-1:-1]},x_{[-M:0]}|\mathcal{T}))
%                 \big)^{1/2}
%             \Big)
%     \\
%     \nonumber
%     &
%             -\frac{\varepsilon}{2}\,
%                 \log\Big(
%                     \big(
%                             I_d + \frac{4^2}{\varepsilon^2}\,(\lambda\,I_d)(\Sigma(y_{[-M-1:-1]},x_{[-M:0]}|\mathcal{T}))
%                     \big)^{1/2}
%                 \Big)
%         \Big)
% %%%%%
% %%%%%
% %%%%%
% %%%% Simple simplifications II (Just baby factoring)
% %%%%%
% %%%%%
% %%%%%
%     \\
%     \nonumber
%     = & 
%         \|y_0-\mathcal{T}(x_{[-M:0]})\|^2
%     +
%     d
%     \big(
%     \lambda +1 - \log(2)/2
%     \big)
%     +
%     \operatorname{tr}\big(
%         \Sigma(y_{[-M-1:-1]},x_{[-M:0]}|\mathcal{T})
%     \big)
%     \\
%     \nonumber
%         % Important Bit
%     &
%         -
%         \underbrace{
%             \frac{\varepsilon}{2}\,
%             \operatorname{tr}\Big(
%                 \big(
%                         I_d + \frac{4^2}{\varepsilon^2}\,(\lambda\,I_d)(\Sigma(y_{[-M-1:-1]},x_{[-M:0]}|\mathcal{T}))
%                 \big)^{1/2}
%             \Big)
%         }_{\text{(I)}}
%     \\
%     \nonumber
%     &
%         -
%         \underbrace{
%             \frac{\varepsilon}{2}\,
%                     \log\Big(
%                         \big(
%                                 I_d + \frac{4^2}{\varepsilon^2}\,(\lambda\,I_d)(\Sigma(y_{[-M-1:-1]},x_{[-M:0]}|\mathcal{T}))
%                         \big)^{1/2}
%                     \Big)
%             \Big)
%         }_{\text{(II)}}
% \end{align}
% where the equality~\eqref{eq:simplification_OT__Centering} holds by \citep[Propositions 2]{MallastoGerolinAugustoMinh_IG_2022_Closed_FormEOT} and the equality~\eqref{eq:simplification_OTCentered} holds by \cite[Theorem 2]{MallastoGerolinAugustoMinh_IG_2022_Closed_FormEOT}.
% \hfill\\
% \AK{@YX Please bound (I) and (II) using previous lemma.}
% \end{proof}

% \newpage
% \end{comment}




% \subsection{Step 3 - Combining Steps 1 and 2 and Completing The Proof of \texorpdfstring{Theorem~\ref{thrm:main}}{Our Main Theorem}}
% \label{s:Proof__ss:Main}

% We are now ready to complete the proof of our main result, namely Theorem~\ref{thrm:main}.  
% Before doing so, we state a more technical and general version, which we instead prove and which directly implies the simpler version found in the main body of our manuscript.

% We operate under the following more general, but more technical set of assumptions than those considered in the main body of our text (in Setting~\ref{setting}).
% \begin{setting}[Generalized Setting]
% \label{setting_gensetting}
% Let $D,d, L,H,*C^{\prime},C^A,C^b\in \mathbb{N}_+$, set $M\eqdef 0$, and $C\eqdef (*C^{\prime},C^A,C^b)$, $r_f,r_{\ell},C_f,C_{\ell} \ge 0$.
% % , and consider the hypothesis class $\transformerclass_{L,H,C}^{D,d,0}$.  
% Suppose that Assumptions~\ref{ass:MC} and~\ref{ass:Exp_Moment} hold.

% Fix a target function $f^{\star}:\mathbb{R}^d\to \mathbb{R}^D$ and a loss function $\ell:\mathbb{R}^D\times \mathbb{R}^D\to \mathbb{R}$.  Assume either that:
% \begin{enumerate}
%     \item[(i)] \textbf{Polynomial Growth:} $f^{\star}\in C^{\infty}_{poly:C_f,r_f}(\mathbb{R}^d,\mathbb{R}^D)$ and $\ell\in C^{\infty}_{poly:C_{\ell},r_{\ell}}(\mathbb{R}^{2D},\mathbb{R})$,
%     \item[(ii)] \textbf{Exponential Growth:} $f^{\star}\in C^{\infty}_{exp:C_f,r_f}(\mathbb{R}^d,\mathbb{R}^D)$ and $\ell\in C^{\infty}_{exp:C_{\ell},r_{\ell}}(\mathbb{R}^{2D},\mathbb{R})$
%     ,
%     \item[(iii)] \textbf{No Growth:} There is a constant $\bar{C}\ge 0$ such that for all $s>0$ we have $\|f^{\star}\|_{C^s},\|\ell\|_{C^s} \le \bar{C}$.
% \end{enumerate}
% \end{setting}

% \begin{example}[Example of Generalized Setting (iii)]
% \label{ex:ubderivatives}
% For every $d\in \mathbb{R}^d$, the function $f:\mathbb{R}^d\ni x\mapsto \cos\bullet x = \big(\cos(x_i)\big)_{i=1}^d$ satisfies $
% \|\frac{\partial^s}{\partial x_i^s} f\|_{\infty} \le 1
% $ for each $s\in \mathbb{N}$ and each $i=1,\dots,d$.  Thus, it is an example of a function satisfying Assumption~\ref{setting_gensetting}.
% \end{example}

% We are now ready to prove our main theorem.

% \begin{theorem}[Pathwise Generalization Bounds for Transformers]
% \label{thrm:main__technicalversion}
% In Setting~\ref{setting_gensetting}, there is a $\kappa\in(0,1)$, depending only on $X_{\cdot}$, and a $t_0\in \mathbb{N}_0$ such that: for each $t_0\le N \le t \le \infty$ and $\delta \in (0,1]$ the following holds with probability at-least $1-\delta$
% \begin{align*}
% \resizebox{1\linewidth}{!}{$
%         \sup_{\mathcal{T}\in 
%             \transformerclass_{L,H,C}^{D,d,0}
%         }
%         \,
%             \big|
%                 \mathcal{R}_{\max\{t,N\}}(\mathcal{T})-\mathcal{R}^{(N)}(\mathcal{T})
%             \big|
%     \lesssim
%         \sum_{s=1}^{\infty}\,
%             I_{N\in [\tau_{s},\tau_{s+1})}
%             \,
%             % C^{\transformerclass}_{K}(s)
%             C_{\ell,\transformer,K,s-1}
%         \biggl(
%             %% Time-Shift Term
%                 I_{t<\infty}\,
%                 \kappa^t\,
%             +
%                 %%% Concentration Term
%                 \frac{
%                     \sqrt{2\ln(1/\delta)}
%                 }{
%                     N^{1/2}
%                 }
%                 %%% Mean Term
%                 +\,
%                 %%% 
%                 % Rate
%                 \operatorname{rate}_s(N)
%     \biggr)
% $}
% \end{align*}
% where $\operatorname{rate}_s(N)$ is defined in~\eqref{eq:rate_function__definition}, and the constant $C_{\ell,\transformer,s,K}$ is Table~\ref{tab:constants} and the \textit{transition phases} $(\tau_s)_{s=0}^{\infty}$ are given iteratively by $\tau_0\eqdef 0$ and for each $s\in \mathbb{N}_+$
% \begin{align*}
% \resizebox{1\hsize}{!}{$
%     \tau_s
% \eqdef 
%     \inf\,
%     \biggl\{ 
%         t\ge \tau_{s-1}
%     :\,
%             % C^{\transformerclass}_{K}(s)
%             C_{\ell,\transformer,K,s}
%             ( \kappa^t + \operatorname{rate}_s(N)+
%             \frac{\sqrt{\log(1/\delta)}}{\sqrt{N}}
%             ) 
%         \le 
%             % C^{\transformerclass}_{K}(s-1)
%             C_{\ell,\transformer,K,s-1}
%             ( \kappa^t + \operatorname{rate}_{s-1}(N)+
%             \frac{\sqrt{\log(1/\delta)}}{\sqrt{N}}
%             )
%     \biggr\}
% .
% $}
% \end{align*}
% Furthermore, $c\eqdef 1-\kappa$, $c_2\eqdef c^{s/d}$, $\kappa^{\infty}\eqdef \lim\limits_{t\to \infty}\, \kappa^t= 0$, and $\lesssim$ hides an absolute constant.
% \end{theorem}



% \begin{proof}[{Proof of Theorem~\ref{thrm:main}}]
% Since $N$ is given, we may pick $s\in \mathbb{N}_+$ to ensure that $N\in [\tau_s,\tau_{s+1})$; where these are defined as in the statement of Theorem~\ref{thrm:main__technicalversion}.  

% Since we are in Setting~\ref{setting}, then $\ell \in C^{\infty}_{poly:C_{\ell},r_{\ell}}(\mathbb{R}^{2D},\mathbb{R})$ (resp.\ $\ell \in C^{\infty}_{exp:C_{\ell},r_{\ell}}(\mathbb{R}^{2D},\mathbb{R})$) and $f^{\star}:\mathbb{R}^d\to\mathbb{R}^D$ is smooth.  
% Therefore, Lemma~\ref{lem:control_loss__SSE} implies that there is an absolute constant $c_{\operatorname{abs}}>0$ such that for any transformer network $\transformer\in \transformerclass_{L,H,C}^{D,d,0}$, the following bound holds
% \begin{enumerate}
%     \item[(i)] \textbf{No Growth Case:} Using~\eqref{eq:called_bound} we find that
% \begin{align}
% \label{eq:FCsBound__NoGrowth}
%     \big\| \ell( \transformer, f^{\star} ) \big\|_{C^s} 
% \le & 
%     c_{\operatorname{abs}}\,
%     % \mathcal{O} 
%         \big(\frac{ 2D s }{e\ln s } (1+o(1)) \big)^s  
%         \,
%         \|\transformer\|_{C^s}^s
% \end{align}
%     \item[(ii)] \textbf{Polynomial Growth Case -  $\ell \in C^{\infty}_{poly:C_{\ell},r_{\ell}}(\mathbb{R}^{2D},\mathbb{R})$ Case:} 
% \begin{align}
% \label{eq:FCsBound__PolynomialCase}
%     \big\| \ell( \transformer, f^{\star} ) \big\|_{C^s} 
% \le & 
%     c_{\operatorname{abs}}\,
%     % \mathcal{O} 
%     % \Big(  
%             s^{r_{\ell}}   
%             \big(\frac{ 2D s }{e\ln s } (1+o(1)) \big)^s  
%             \,
%             \|f^{\star}\|_{C^s}^s
%             \,
%             \|\transformer\|_{C^s}^s
%     % \Big)
% \end{align}
%     \item[(iii)] \textbf{Exponential Growth -  $C^{\infty}_{exp:C_{\ell},r_{\ell}}(\mathbb{R}^{2D},\mathbb{R})$ Case:} 
% \begin{align}
% \label{eq:FCsBound__ExponentialCase}
%     \big\| \ell( \transformer, f^{\star} ) \big\|_{C^s} 
% \le & 
%     % \mathcal{O}
%     c_{\operatorname{abs}}
%     \,
%     % \Big(  
%             e^{s \, r_{\ell}}   
%             \big(\frac{ 2D s }{e\ln s } ( 1+o(1) ) \big)^s  
%             \,
%             \|f^{\star}\|_{C^s}^s
%             \,
%             \|\transformer\|_{C^s}^s
%     % \Big)
% .
% \end{align}
% \end{enumerate}
% Since we have assumed that $f^{\star} \in C^{\infty}_{poly:C_f,r_f}(\mathbb{R}^d,\mathbb{R}^{D})$ (resp.\ $C^{\infty}_{exp:C_f,r_f}(\mathbb{R}^d,\mathbb{R}^{D})$ or the ``no growth condition'' in Setting~\ref{setting_gensetting} (iii)) then the bounds in~\eqref{eq:FCsBound__NoGrowth},~\eqref{eq:FCsBound__PolynomialCase}, and~\eqref{eq:FCsBound__ExponentialCase}, respectively, imply that
% \begin{enumerate}
%     \item[(i)] \textbf{No Growth Case:} 
%     \begin{align}
%     \label{eq:FCsBound__NoGrowth__v2}
%         \big\| \ell( \transformer, f^{\star} ) \big\|_{C^s} 
%     \le & 
%         c_{\operatorname{abs}}\,
%         % \mathcal{O} 
%             \big(\frac{ 2D s }{e\ln s } (1+o(1)) \big)^s  
%             \,
%             % \|\transformer\|_{C^s}^s
%             C^{\transformerclass}_{K}(s)^s
%     \end{align}
%     \item[(ii)] \textbf{Polynomial Growth Case -  $\ell \in C^{\infty}_{poly:C_{\ell},r_{\ell}}(\mathbb{R}^{2D},\mathbb{R})$ Case:} 
% \begin{align}
% \label{eq:FCsBound__PolynomialCase__v2}
%     \big\| \ell( \transformer, f^{\star} ) \big\|_{C^s} 
% \le & 
%     % \mathcal{O} 
%     % \biggl(  
%     %         \Big(
%     %             s^{r_{\ell}} 
%     %             \big(\frac{ 2D s }{e\ln s } \big)^s  
%     %             \,
%     %             \big(
%     %                 C_f\, s^s
%     %             \big)^s
%     %         \Big)
%     %         \,
%     %         \|\transformer\|_{C^s}^s
%     % \biggr)
%     % =
%     % \mathcal{O} 
%     c_{\operatorname{abs}}\,
%     % \biggl(  
%             s^{r_{\ell} + 2s^2} 
%             \Big(\frac{ C_f \, 2D  }{e\ln s } (1 + o(1)) \Big)^s  
%             \,
%             % \|\transformer\|_{C^s}^s
%             C^{\transformerclass}_{K}(s)^s
%     % \biggr)
% \end{align}
%     \item[(iii)] \textbf{Exponential Growth -  $C^{\infty}_{exp:C_{\ell},r_{\ell}}(\mathbb{R}^{2D},\mathbb{R})$ Case:} 
% \begin{align}
% \label{eq:FCsBound__ExponentialCase__v2}
%     \big\| \ell( \transformer, f^{\star} ) \big\|_{C^s} 
% \le & 
%     % \mathcal{O}
%     % \biggl(  
%     %         \Big(
%     %             e^{s \, r_{\ell}}   
%     %             \big(\frac{ 2D s }{e\ln s } \big)^s  
%     %             \,
%     %             C_f^s\, e^{s^2\, r_f}
%     %         \Big)
%     %         \,
%     %         \|\transformer\|_{C^s}^s
%     % \biggr)
%     % = 
%     % \mathcal{O}
%     c_{\operatorname{abs}}\,
%     % \biggl(  
%             e^{s \, r_{\ell} + s^2 r_f} \Big(\frac{ 2D \, s }{ e \ln s} (1+o(1) )\Big)^s
%             \,
%             C_f^s  
%             \,
%             % \|\transformer\|_{C^s}^s
%             C^{\transformerclass}_{K_{0}}(s)^s
%     % \biggr)
% ,
% \end{align}
% \end{enumerate}
% where we have used the definition of the constant $C^{\transformerclass}_{K}(s)$ as a uniform upper bound of $\sup_{\transformer \in \transformerclass_{L,H,C}^{D,d,0} }$.  
% Using Theorem~\ref{thm:TransformerBlockSobolevBound} for the ``derivative type estimate'' (resp.\ref{thm:TransformerBlockSobolevBoundLevel} for the ``derivative level estimate'') concludes the implies yields a uniform upper bound (of ``derivative type'' or ``derivative level'' respectively) on $C^{\transformerclass}_{K_{0}}(s)$, i.e.\ independent of the particular transformer instance $\mathcal{T}\in \transformerclass_{L,H,C}^{D,d,0}$.  In either case, we respectively define $R>0$ to be the right-hand side of~\eqref{eq:FCsBound__PolynomialCase__v2} or~\eqref{eq:FCsBound__ExponentialCase__v2} depending on the respective assumptions made on $\ell$ and on $f^{\star}$.

% The conclusion now follows upon applying Proposition~\ref{prop:Concentation} due to the inequality in~\eqref{eq:risk_bound__decomposition}.    
% \end{proof}


% % \input{Bookkeeping/Extras/Unbounded_Case}

% \section{Example of Additive Noise Using Stochastic Calculus}
% \label{a:stoch_example}


% In this appendix, we briefly discuss why the seemingly \textit{realizable} learning setting which we have placed ourselves in, i.e.~$Y_n=f^{\star}(X_n)$, does not preclude additive noise.  Our illustration considers the class of following Markov processes.
% \begin{assumption}[Structure on $X_{\cdot}$]
% \label{ass:Markov_Structure_X}
% Let $g:\mathbb{R}^d\to [0,1]^d$ be a twice continuously differentiable function.  Let $W_{\cdot}\eqdef (W_t)_{t\ge 0}$ be $d$-dimensional Brownian motion and, for each $n\in \mathbb{N}$, define
% \begin{align*}
%     X_n \eqdef g(W_n).
% \end{align*}
% \end{assumption}
% By construction, the boundedness of the change of variables-type function $g$ in Assumption~\ref{ass:Markov_Structure_X}, implies that the process $X_{\cdot}=(X_n)_{n\in \mathbb{N}}$ is bounded (and can easily be seen to be Markovian since Brownian motion has the strong Markov property).  However, we can say more, indeed under Assumption~\ref{ass:Markov_Structure_X}, the It\^{o} Lemma (see e.g.~\citep[Theorem 14.2.4]{CohenElliotBook_2015}) implies that $X_n$ is given as the following stochastic differential equation (SDE) evaluated at integer times $n\in \mathbb{N}$
% \begin{align}
% \label{eq:SDE}
% X_n  
% &=
%     g(0) 
% + 
%     \int_0^n\,
%         \mu_s
%   \, ds
% + 
%     \int_0^n\,
%         \sigma_t^{\top} \, dW_s
% \end{align}
% where $\mu_{\cdot}=(\mu_t)_{t\ge 0}$ and $\sigma_{\cdot}=(\sigma_t)_{t\ge 0}$ are given by
% \begin{align}
% \label{eq:SDE_dynamics}
% \mu_t  \eqdef \frac{1}{2} \operatorname{tr} \big( H(g)(W_s) \big)  
% \mbox{ and }
% \sigma_t  \eqdef \nabla g(W_t)
% \end{align}
% and $H(g)$ is the Hessian of $g$ and $\operatorname{tr}$ is the trace of a matrix.
% \begin{example}
% \label{ex:simple_example}
% Set $d=1$ and $g(x)=(\sin(x)+1)/2$.  Then, for each $n\in \mathbb{N}$ we have 
% \begin{align*}
% X_n = \int_0^n -\sin(W_s)/4 ds + \int_0^t \cos(W_s)/2 \,dW_s.
% \end{align*}
% \end{example}
% In particular, the expression~\eqref{eq:SDE} shows that the input process $X_{\cdot}$ is also defined for all intermediate times between non-negative integer times; i.e.~for each $t\ge 0$ the process
% \begin{align}
% \label{eq:SDE_cnttimeext}
%     X_t
% &=
%     g(0) 
% + 
%     \int_0^t\,
%         \mu_s
%   \, ds
% + 
%     \int_0^t\,
%         \sigma_t^{\top} \, dW_s
% \end{align}
% is well-defined and coincides with $X_n$ whenever $t=n\in \mathbb{N}$.  
% We may, therefore, also consider the ``continuous-time extension'' $Y_{\cdot}\eqdef (Y_t)_{t\ge 0}$ of the target process defined for all intermediate times using~\eqref{eq:SDE_cnttimeext} by
% \begin{align*}
%         Y_t
%     \eqdef 
%         f^{\star}(X_t)
%     .
% \end{align*}
% Note that $Y_t$ coincides with the target process on non-negative integer times, as defined in our main text, by definition.  

% The convenience of these continuous-time extensions, of the discrete versions considered in our main text, is that now $Y_{\cdot}$ is the transformation of a continuous-time (It\^{o}) process of satisfying the SDE~\eqref{eq:SDE_cnttimeext} by a smooth function\footnote{Note that $f^{\star}$ was assumed to be smooth in our main result (Theorem~\ref{thrm:main}).}, namely $f^{\star}$.  Therefore, we may again apply the It\^{o} Lemma (again see e.g.~\citep[Theorem 14.2.4]{CohenElliotBook_2015}) this time to the process $X_{\cdot}$ to obtain the desired signal and noise decomposition of the target process $Y_{\cdot}$ (both in discrete and continuous time).  Doing so yields the following  decomposition
% \begin{equation}
% \label{eq:signal_noise_decomposition}
% \begin{aligned}
%     Y_t 
% = &
%     \underbrace{
%         f^{\star}(X_0)
%         +
%         \int_0^t
%         \,
%             \Big(
%                 \left (\nabla f^{\star}(X_s) \right)^{\top}
%                 \mu_t 
%                 + 
%                 \frac{1}{2} 
%                 \operatorname{tr} \big(
%                     \sigma_s^{\top} 
%                     H(f^{\star})(X_s)
%                     \sigma_s 
%                 \big)
%             \Big) 
%         \, 
%         ds
%     }_{\text{Signal (Target)}}
%     \\
%     & + 
%     \underbrace{
%     \int_0^t
%     \,
%         \left (\nabla f^{\star} \right)^{\top} \sigma_s
%     \, dW_s
%     }_{\text{Additive Noise}}
% .
% % $}
% \end{aligned}
% \end{equation}
% This shows that even if it a priori seemed that we are in the \textit{realizable PAC setting} due to the structural assumption that $Y_n=f^{\star}(X_n)$ made when defining the target process, we are actually in the standard setting where the target data $(Y_n)_{n=0}^{\infty}$ can be written as a signal plus an additive noise term.  Indeed, when $X_{\cdot}$ is simply a transformation of a Brownian motion by a bounded $C^2$-function, as in Assumption~\ref{ass:Markov_Structure_X}, then Assumption~\ref{ass:Comp_Support} held and $Y_n$ admitted the signal-noise decomposition in~\eqref{eq:signal_noise_decomposition}.


% \section{Examples}
% \label{s:Examples}

% As shown in the proof of Proposition~\ref{prop:Concentation}, Assumptions~\ref{ass:MC} and~\ref{ass:Comp_Support} are used to deduce~\eqref{eq:exp_contract}.  We only need the following relaxation of Assumption~\ref{ass:MC} to hold for the transition semi-group $(P^t)_{t\ge 0}$ of $X_{\cdot}$.
% \begin{assumption}[Exponential Contractivity]
% \label{ass:contractivity}
% There is a $\kappa\in (0,1)$ such that: for each $\mu,\nu\in \mathcal{P}(\mathbb{R}^d)$ and every $t\in \mathbb{N}_+$ one has $\mathcal{W}_1(P^t\mu,P^t\nu)\le 
% \kappa^t\, \mathcal{W}_1(\mu,\nu)$.  
% \end{assumption}
% Though this trivially holds for compactly supported i.i.d.\ data, we obtain the following broad class of simple examples.  
% \begin{example}[]
% \label{ex:Exp_Contract_SDE}
% \AK{Need to complete and verify last bit}\\
% Let $\mu:\mathbb{R}^d\to \mathbb{R}^d$ be a Lipschitz and the gradient of a strongly concave function; i.e.\ $(\mu(x)-\mu(y))^{\top}(x-y)\le -K \|x-y\|^2$ for some $K>0$ and every $x,y \in \mathbb{R}^d$. 
% Let $Z_{\cdot}\eqdef (Z_t)_{t\ge 0}$ be the (unique strong) solution to the stochastic differential equation 
% \begin{equation}
% \label{eq:evolution}
% Z_t = x + \int_0^t\, \mu(Z_s)\,ds + \int_0^t\, dW_s
% \end{equation}
% where $W_{\cdot}\eqdef (W_t)_{t\ge 0}$ is a $d$-dimensional Brownian motion.  For instance, any overdampled Langevin diffusion with strictly convex potential $U$ is of the form~\eqref{eq:evolution}, see e.g.~\cite{bolley2012convergence}, since such diffusions are precisely of the form~\eqref{eq:evolution} with $\mu=-\nabla U/2$.


% Then~\cite[Theorem 1.1]{LuoWang_ExpContractivity_2016} implies that $(Z_n)_{n=0}^{\infty}$ satisfies~\eqref{ass:contractivity} with $\kappa=e^{-K}$.  
% Let $f:\mathbb{R}^d\to [0,1]^d$ be any $1$-Lipschitz map; a consequence of the Kantorovich duality, see e.g.~\cite[Lemma 12]{hou2022instance}, implies that the push-forward map $f_{\sharp}$ is $1$-Lipschitz from the $1$-Wasserstein space on $\mathbb{R}^d$ to that over $[0,1]^d$.  Since the law each $X_n$ defining process $X_{\cdot}\eqdef (X_n)_{n=1}^{\infty}$ defined for each $n\in \mathbb{N}$ by $X_n\eqdef f(Z_n)$ takes values in the bounded set $[0,1]^d$ and its transition semi-group $(\tilde{P}_n
% =f_{\#}P_n
% )_{n=0}^{\infty}$, 
% % given for each $n\in \mathbb{N}$ by the Markov kernel presentation $\tilde{P}_n(\varphi)=
% % \int_{y\in [0,1]^d} \varphi(y) f_{\#}p_t(x,dy))_{n=0}^{\infty}$ 
% satisfies
% \[
% \mathcal{W}_1(\tilde{P}_n\mu,\tilde{P}_n\nu)\le \operatorname{Lip}(f)\,\mathcal{W}_1(P_n\mu,P_n\nu)
% \le \kappa^n\, \mathcal{W}_1(\mu,\nu).
% \]
% \end{example}
% % \begin{example}[I.I.D. Data]
% % Let $\mu$ be a compactly supported probability measure on $\mathbb{R}^d$.  Let $(X_n)_{n=0}^{\infty}$ be i.i.d.\ with law $\mu$.  Clearly, Assumption~\ref{ass:Comp_Support} holds, to see Assumption~\ref{ass:contractivity} note that $(P_n)_{n=0}^{\infty}$ where, for each $n\in \mathbb{N}_+$ $P_n$ is the identity operator, is a transition semigroup for $(X_n)_{n=0}^{\infty}$.  Therefore, for each $\mu,\nu\in $
% % \[
% % \mathcal{W}
% % \]
% % \end{example}

% %%%%%%%%%%%%%%%%%%%%% APPENDIX END   %%%%%%%%%%%%%%%%%%%%%%%%%


% %%%%%%%%%%%%%%%%%%%%% NeurIPS PAPER CHECKLIST %%%%%%%%%%%%%%%%
% \clearpage
% \input{60_neurips_paper-checklist}


% \end{document}




==> Bookkeeping/Historical_Versions/60_neurips_paper-checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
\section*{NeurIPS Paper Checklist}
\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The claims asserted in the abstract and in our instruction are substantiated both experimentally and theoretically in our main body.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer:  \answerYes{} % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We include all limitations and a discussion on plausible potential future work following our conclusion.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed not to penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All assumptions are clearly stated before our main results are stated.  All proofs are contained in the appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes we provide our code used in the numerical illustrations of our main results.  
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes we provide our code used in the numerical illustrations of our main results and all proofs of our theoretical results are included in the appendix. The code can be retrieved at: \url{https://anonymous.4open.science/r/transfomer-bounds-B476}
    % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{}%\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All details on how our experiments have been provided; even if the paper is principally theoretical. 
    % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNA{}%\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: There are no error bars to report since our numerical illustrations are non-random and simply compute our constants.
    % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our numerical computations were very small-scale computations of some constants; this required no model training and no simulation.  They can be run in seconds on any relatively recent laptop.  
    % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}
    % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper provides theoretical guarantees for pre-existing models.  
    % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{}%\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper provides theoretical guarantees for pre-existing models.  
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}%TODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper provides theoretical guarantees for pre-existing models.  
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerNA{}%TODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not use existing assets. 
    % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{}%TODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not use new assets. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We did not perform and crowdsourcing nor research with human subjects.%\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> Bookkeeping/Historical_Versions/Brainstorming/Brainstorming.tex <==
% \newpage

% \section{Questions}
% \begin{enumerate}
%     \item (When) does $\hat{M}^{k,\Delta}(X_{\cdot})_t \to M^k(\operatorname{Law}(X_t))$?
%     \item Problems:
% \begin{enumerate}
%     \item $X_{t+1}$ given $X_{[0:t]}$
%     \item $X$ is known, $Y$'s dynamics are not, predict $X|Y$
% \end{enumerate}
    
% \end{enumerate}

% \section{Brainstorming}

% \subsection{Model}
% Let $f^1,\dots,f^N:C([0:T],\mathbb{R}^d)\times [0:T] \to \mathcal{N}_D$ be DKFs (pre-trained on similar synthetic problems).  
% Consider the map \textit{(structure to be defined)} $w: C([0:T],\mathbb{R}^d)\times [0:T] \to \Delta_N$ (trainable).

% \begin{align}
%     \label{id:Model}
%     F(x,t)\mapsto 
%     \sum_{n=1}^N
%     \,
%     w(x,t)_n\,f^n(x,t)
% \end{align}


% \subsection{Objective Function}
% \[
% \min_{w}\,\,
%     \int_{\Delta}^T
%     \,
%     \underbrace{
%         \sum_{k=1}^K
%         \,
%                 \Big|
%                         M^k\Big(
%                             \sum_{n=1}^N\,w_n(Y_{[0:s]})\,f^n(Y_{[0:s]})
%                         \Big)_s
%                     -
%                         % \hat{M}^{k,\Delta}(x_{\cdot})_s
%                         M^k(\operatorname{Law}(X_s|Y_{[0:s]}))
%                         _s
%                 \Big|^2
%             ds
%     }_{\mbox{Moment Matching}}
%     % +
%     % \underbrace{
%     %     \lambda 
%     %     \,
%     %     \operatorname{KL}\Big(
%     %         \sum_{n=1}^N\,w_n(x_{\cdot}) f^n(x_{\cdot})
%     %     \Big\|
%     %         \frac1{N}\,\sum_{n=1}^N\,f^n(x_{\cdot})
%     %     \Big)
%     % }_{\mbox{Full Support Regularization}}
% \]

% \subsection{Theorems which we can write}
% \label{brs:}

% \subsubsection{Approximation Bounds}
% \begin{enumerate}
%     \item Approximation of any stochastic filter 
%     \begin{enumerate}
%         \item Stability Estimates \citep[Theorem 6]{crisan2013robust} and guarantee that $\theta$ process is a robust filter \citep[Theorem 7]{crisan2013robust},
%         \item Approximate using the same technique as the previous paper for feature map, then readout map using paper with Bea by encoding empirical measures.
%     \end{enumerate}
% \end{enumerate}

% \subsubsection{Generalization Bounds?}
% Suppose that $\mathcal{X}$ is a compact subset of $C([0:T],\mathbb{R}^d)$.


% \subsection{One step forecasting of DKF}


% We examine a scenario where a collection of processed variables, denoted as $Y^1, \dots, Y^N$, are all intricately linked to a common process, $X$. We define $f^n = X|Y^n$ for all $n \in \{1,\dots,N\}$. Further, we introduce a choice process, $Z$, \yannick{basically a cont. Markov process with discrete space} that assumes values in $\{1,\dots,N\}$ at all time points, governed by probabilities $P(Z_t = n) = w^n$ respectively.

% We propose that the evolution of a process $Y$ at time $t$ is driven by the incremental gains of $Y_t^{Z_t}$. By leveraging the law of total probability, we establish the relationship:
% \[ f := X|Y = \sum_{n=1}^{N} w^n f^n \]
% which constitutes our model.

% Consequently, for a given fixed set of probabilities $w$, we attain insights into the dynamics of $Y$ based on the behavior of $X|Y$. This understanding allows us to compare the anticipated future state with observations.

% In detail, if we have
% \begin{align*}
%     dY^n_t = G^n(t, X_t, Y^n_{[0,t]})dt + \sigma dW_t 
% \end{align*}
% then, 
% \begin{align*}
%     dY_{t} = G^{Z_t}(t, X_t, Y^{Z_t}_{[0,t]})dt + \sigma (W_{t+} - W_{t}).
% \end{align*}
% The goal is then to find the transition matrix of $Z$ s.t. $Y$ represents the data the best.


% \newpage

==> Bookkeeping/Historical_Versions/rebutal_nips.tex <==
% \documentclass[10pt]{article}
% \usepackage[utf8]{inputenc}
% \usepackage{enumitem}
% \usepackage{geometry}
% \usepackage{hyperref}
% \usepackage{tcolorbox}
% \usepackage{amssymb}

% \geometry{margin=1.5cm}
% \usepackage[normalem]{ulem}

% \newcommand{\byyan}[1]{\textcolor{cyan}{#1}}


% % \newcommand{\countcharacters}[1]{%
% %   \StrLen{hello}[\temp]%
% %    Character count: #1
% %   \temp%
% % }
% \usepackage{tokcycle}[2021-03-10]
% \usepackage{xcolor}
% \newcounter{wordcount}
% \newcounter{lettercount}
% \newcounter{wordlimit}
% \newif\ifinword
% % USER PARAMETERS
% \newif\ifrunningcount
% \newif\ifsummarycount
% \def\limitcolor{red}
% \setcounter{wordlimit}{0}
% %%
% \makeatletter
% % \tc@defx is like \def, but expands the replacement text once prior to assignment
% \newcommand\addtomacro[2]{\tc@defx#1{#1#2}}
% \newcommand\changecolor[1]{\tctestifx{.#1}{}{\addcytoks{\color{#1}{}}%
%   \tc@defx\currentcolor{#1}}}
% \makeatother
% \newcommand\dumpword{%
%   \addcytoks[1]{\accumword}%
%   \ifinword\stepcounter{wordcount}
%     \ifrunningcount\addcytoks[x]{$^{\thewordcount,\thelettercount}$}\fi
%     \ifnum\thewordcount=\value{wordlimit}\relax\changecolor{\limitcolor}\fi
%   \fi%
%   \inwordfalse
%   \def\accumword{}}
% \newcommand\addletter[1]{%
%   \tctestifcatnx A#1{\stepcounter{lettercount}\inwordtrue}{\dumpword}%
%   \addtomacro\accumword{#1}}
% \xtokcycleenvironment\countem
%   {\addletter{##1}}
%   {\dumpword\groupedcytoks{\processtoks{##1}\dumpword\expandafter}\expandafter
%     \changecolor\expandafter{\currentcolor}}
%   {\dumpword\addcytoks{##1}}
%   {\dumpword\addcytoks{##1}}
%   {\stripgroupingtrue\def\accumword{}\def\currentcolor{.}
%     \setcounter{wordcount}{0}\setcounter{lettercount}{0}}
%   {\dumpword\ifsummarycount\tcafterenv{%
%     \par(Wordcount=\thewordcount, Lettercount=\thelettercount)}\fi}


% \title{Neurips Rebuttal}
% \author{}
% \date{}
% \input{Bookkeeping/Commenting}

% \usepackage[hybrid]{markdown}

% \begin{document}

% \maketitle
% % \setcounter{wordlimit}{100}

% \section{General Response}


% \countem

% \begin{markdown}
% We want to begin by thanking all four reviewers. Their constructive feedback gave us valuable insights, motivating a very engaging discussion. While every review has individual aspects that we were able to address, there were two unified themes among most referees:  1) what examples of non-iid data-generating processes are covered by our theory, and 2) which components of the bound are entirely transformer-specific and why.

% # Examples

% There is a wide range of non-iid data-generating processes, which naturally arise in time-series analysis, signal processing, and stochastic analysis, for which our theory holds. These are any processes satisfying the following exponential ergodicity condition.

% ## Assumption: Exponential Ergodicity
% There is a κ$\in (0,1)$ such that: for each $\mu,\nu\in \mathcal{P}(\mathbb{R}^d)$ and every $t\in \mathbb{N}+$ one has 
% $$W_1(P^t\mu,P^t\nu)\le \kappa^t\, W_1(\mu,\nu).$$

% ### Constrained SDEs with Over-dampened Drift
% Consider a latent dimension ${\bar{d}}\in \mathbb{N}+$ and a Lipschitz vector field $\mu:\mathbb{R}^{\bar{d}}\to \mathbb{R}^{\bar{d}}$ which is the gradient of a strongly concave function; i.e. there is a $K>0$ such that $(\mu(x)-\mu(y))^{\top}(x-y)\le -K \|x-y\|^2$ for all $x,y\in \mathbb{R}^d$.  For any $x\in\mathbb{R}^{\bar{d}}$ let $Z^x_{\cdot}$ be the unique, strong solution (which exists by Theorem 8.2 in [1])$$Z_t^x=x+\int_0^t\mu(Z_s^x)ds + \int_0^t\, W_s $$ where $W_{\cdot}$ is a ${\bar{d}}$-dimensional Brownian motion.  We "project" this latent process down onto a constraint set using a bounded $1$-Lipschitz function $f:\mathbb{R}^{\bar{d}}\to \mathbb{R}$.  Then, the discrete-time Markov process $X_{\cdot} :=  (X_n)_{n=0}^{\infty}$ on $\mathbb{R}^d$ given by
% $$X_n^x:= f(Z_n^x)$$ satisfies our Assumptions.

% The standard example of SDEs $(Z_t^x)_{t\ge 0}$ are Langevin dynamics for a strictly convex potential $U$, i.e. $\mu=-\nabla U/2$ (see [2]).  Langevin dynamics are the backbone of several machine learning tools, such as denoising diffusion models [3] and various Bayesian optimizers [4].  

% ### Many processes are exponentially ergodic

% Our theory covers a wide range of examples, from non-iid data-generating processes rooted in machine learning to stochastic games. Indeed, our results hold even if the latent process $Z^x_{\cdot}$ is replaced:  an SDE driven by pure-jump Lévy process, Theorem 3.1 of [5], SDE of McKean-Vlasov SDEs type wherein $\mu$ depends on the distribution of $Z_t^x$ at time $t$ (these arise in mean-field games), Corollary 4.4 of [6], certain processes on compact Riemannian manifolds [7], several countable state space Markov chains, Theorem 2.4 of [9], and the iterates of locally differentiable private mechanisms (see Corollary 2.9 [10] together with Theorem 6.15 [11]).

% # 2 The Non-Asymptotic Component of Our Bound is Entirely Transformer Dependant

% In step $1$ of our proof, we derive Proposition $4$, which is a "global" non-iid version of Theorem 10 (ii) of [8]; which states that with probability at least $1-\delta$, the $t$-future generalization gap can be bounded above by 
% $$\underbrace{\sup_{\mathcal{T}} \|| \ell(\mathcal{T},f^{\star})\||}_{\text{main constant}} \big(\kappa^t + \frac{\sqrt{\ln(1/\delta)}}{\sqrt{N}} + \operatorname{rate}_s(N)\big)$$
% where $0<\kappa<1$ is the exponential ergodicity parameters from the above assumption, where the supremum is over our class of transformers with a given number of attention heads, layer norms, transformer blocks, etc, and $\||\cdot\||$ is the $C^s$-norm.

% Larger classes yield larger generalization bounds than smaller classes, but *how much bigger* is captured by 
% $$C_{\ell,\mathcal{T},f^{\star},s}:=\sup_{\mathcal{T}} \|| \ell(\mathcal{T},f^{\star})\||
% \qquad\mathbf{(1)}.$$
% The exact value of this constant depends precisely on the number of attention heads, layer norms, transformer blocks, and even the activation used in defining the transformer class.  The effect of each component of this constant, and thus our bound, is concretely detailed numerically in tables 2-6 in Appendix B.  

% Bounding **(1)** constitutes the most technical part of our result's proof, pages 28-39 in Appendix D.  The challenge in bounding **(1)** lies in the complicated interactions between the higher-order derivatives of the *attention mechanism* and the transformer blocks feeding into it (our analysis also shows that these interactions do not happen for MLPs whose higher-order derivatives are nearly trivial).  In that way, not only is the bound transformer specific, but so are the challenges in computing it.  

% [1] Da Prato, G. (2014). Introduction to stochastic analysis and Malliavin calculus. 

% [2] Bolley, F., Gentil, I., & Guillin, A. (2012). Convergence to equilibrium in Wasserstein distance for Fokker–Planck equations. Journal of Functional Analysis.

% [3] Ho, J., Jain, A., & Abbeel, P. (2020). Denoising diffusion probabilistic models. Advances in neural information processing systems.

% [4] Welling, M., & Teh, Y. W. (2011). Bayesian learning via stochastic gradient Langevin dynamics.ICML.

% [5] Luo, D., & Wang, J. (2019). Refined basic couplings and Wasserstein-type distances for SDEs with Lévy noises. Stochastic Processes and their Application.

% [6] Wang, F. Y. (2023). Exponential ergodicity for singular reflecting McKean–Vlasov SDEs. Stochastic Processes and their Applications.

% [7] Ollivier, Y. (2009). Ricci curvature of Markov chains on metric spaces. Journal of Functional Analysis.

% [8] Hou, S., Kassraie, P., Kratsios, A., Krause, A., & Rothfuss, J. (2023). Instance-dependent generalization bounds via optimal transport. The Journal of Machine Learning Research.

% [9] Eberle, A., & Majka, M. B. (2019). Quantitative contraction rates for Markov chains on general state spaces.

% [10] Kairouz, P., Oh, S., & Viswanath, P. (2014). Extremal mechanisms for local differential privacy. Advances in neural information processing systems.

% [11] Villani, C. (2009). Optimal transport: old and new. 

% % Additionally, we addressed all further individual comments and questions. We are confident that after the described changes we undertook in our draft, together with the explanations provided in the responses to individual reviewers, the average rating of 4.25 is not representative for our proposed article. For this reason, we kindly asked the reviewers to raise their respective scores and provide us with further questions or concerns if applicable. 

% \end{markdown}
% \endcountem

% \flushright Character count: \thelettercount{}


% ~

% \section{Reviewer Comments and Responses}
% \subsection{etYv}
% \begin{tcolorbox}[colback=white,colframe=black,title={Reviewer etYv, Rating 4, Confidence 1}]
% \small
% \textbf{Summary:} \\
% The paper explores the application of transformer networks to time series data, which typically consists of a single sequence of observations from a data-generating process. The authors focus on establishing non-asymptotic guarantees for the performance of transformers in predicting future events. The analysis is grounded in a scenario where the transformer is trained on a limited number of observations from a Markov process trajectory.\\

% Key contributions include the derivation of a generalization bound that improves as the number of observations increases, converging at a rate proportional to \(O(1/\sqrt{N})\). This bound is influenced by several factors related to the transformer's design, such as the type of activation function, the architecture's depth and width, and the number of attention heads.\\

% \textbf{Soundness:} 3: good \\
% \textbf{Presentation:} 3: good \\
% \textbf{Contribution:} 3: good \\

% \textbf{Strengths:} \\
% While I have not examined the proofs in detail, the authors appear to have invested significant effort into ensuring their clarity. The implications of the bounds are also well articulated.\\

% \textbf{Weaknesses:} \\
% However, I am concerned about the absence of experimental validation in the paper. For a NeurIPS submission, the lack of any experimental feels odd. Although the paper is theoretical, the introduction discusses the "mismatch between available statistical guarantees in deep learning (which often rely on the iid assumption) and how transformers are used in practice." Then the authors state that they “bridge this gap”. This statement sets an expectation, yet the paper does not provide even synthetic experiments on training with time series. Including such experiments could significantly strengthen the paper's impact for a Machine Learning conference.\\

% \textbf{Questions:} \\
% From the Neurips 2024 paper guidelines: “a paper that gives an elegant mathematical derivation of a new algorithm (Criterion \#1) may fare better if it is also demonstrated through rigorous empirical evaluation to do well (Criterion \#4), or demonstrated on a real/non-trivial application (Criterion \#3). This is because such experiments can help build a significantly stronger case for the algorithm's actual utility.”\\

% \textbf{Limitations:} \\
% Why the choice to not put any experiments?
% \end{tcolorbox}


% \begin{tcolorbox}[colback=white,colframe=blue,title={Response to Reviewer etYv}]
% \countem
% Dear reviewer etYv,
% \paragraph{Concerning "Bridging The Gap":}

% Most data-generating processes in time-series analysis, stochastic optimal control, signal processing, and economic applications simply fail to satisfy the iid This means that the vast majority of statistical learning-theoretic results, not only those tailored to transformers, do not apply to any of these contexts.  Our work thus "bridges the gap" in by being applicable to any of these scenarios.


% In our overall rebuttal, we have shown that the main result encompass a broad range of data-generating Markov processes which are standard in any of the aforementioned areas.  Specifically, our results apply to single paths of stochastic differential equations (SDE) constrained to lie in a bounded region (details above).  Moreover, one can even allow the dynamics of this process to depend on its own distribution (i.e.\ of McKean-Vlassov type) and can even be driven by non-Gaussian L\'{e}vy innovations.  


% \paragraph{Concerning Experiments:}
% Though we agree that experiments can be insightful, and we would like to highlight that *we do provide* numerical illustrations both on page $8$, explaining the role of each component in our bounds, and throughout Appendix B, which numerically computes our bounds and shows how various components of the transformer affect them: from the number of multi-head attention layers used to the choice of activation function.  

% That said, numerics are not necessary for a good-quality NeurIPS 2024 theory paper.  This can be seen by looking at the last round's Oral presentations, which represent the gold standard at NeurIPS, which all submissions strive to meet.  Some examples of oral presentations from NeurIPS 2023, which offered purely theoretical contributions to the community without numerics, are:
% \begin{itemize}
%     \item  Attias, Idan, et al. ``Optimal learners for realizable regression: Pac learning and online learning." Advances in Neural Information Processing Systems 36 (2023).
%     \item Gollakota, Aravind, et al. ``Tester-learners for halfspaces: Universal algorithms." Advances in Neural Information Processing Systems 36 (2024).
%     \item Makarychev, Konstantin, and Liren Shan. ``Random cuts are optimal for explainable k-medians." Advances in Neural Information Processing Systems 36 (2024).
%     \item Marcotte, Sibylle, Rémi Gribonval, and Gabriel Peyré. "Abide by the law and follow the flow: Conservation laws for gradient flows." Advances in neural information processing systems 36 (2024).
%     \item Park, Junhyung, et al. ``A measure-theoretic axiomatisation of causality." Advances in Neural Information Processing Systems 36 (2023): 28510-28540.
%     \textit{(Note; this one is like our submission, which does include a few numerical illustrations explaining their/our guarantees, but, like our submission, there are no experiments on real data).}
% \end{itemize}
% We also note that there are several spotlights and general NeurIPS publications each year which provide theory alone, but the list is too exhaustive to elaborate here.

% \endcountem

% \flushright Character count: \thelettercount{}

% \end{tcolorbox}
% \Yan{Apologies Yannick, I hijacked your colour.\\  
% BH: (1) I would move the statement that we \textbf{do provide} experiments further up front to a more visible location. Like this is it more like an afterthought and may go unnoticed. 
% (2) I would also add the following answer to the question "Why the choice of no experiments" the following answer: Seeing the variety of comments and questions that the reviewers asked us, confirms how delicate a challenge it is to strike a balance what to choose to showcase in the (very limited) space for each submission: This is a predominantly theoretical contribution of which we know that it will serve as a much-needed theoretical guarantee for a wide array of experiments in the future. 
% Therefore we chose to give priority to explanations of setting, assumptions and the results and let the numerical demonstrations serve as a reinforcement of the correctness and small illustration of the theory. 
% Seeing the several questions from other reviewers regarding notation as well as requests to put further parts of the proofs into the main part of the paper, reinforces that we made the right choice by letting the experiments occupy a smaller fraction of the space.}


% \subsection{TQAc}

% \begin{tcolorbox}[colback=white,colframe=black,title={Reviewer TQAc, Rating 4, Confidence 4}]
% \small
% \textbf{Summary:} \\
% This paper introduces a theoretical future-generalization of transformer, explicitly expressed in terms of the number of attention heads, depth and width of the transformed model, and so on.\\

% \textbf{Soundness:} 3: good \\
% \textbf{Presentation:} 2: fair \\
% \textbf{Contribution:} 3: good \\

% \textbf{Strengths:} \\
% The motivation is well-presented. The generalization bound is explicitly model structure-dependent, providing more insights on the transformer structure.\\

% \textbf{Weaknesses:} \\
% Symbols are dense. It’s hard to follow. \\
% More necessary theorems need to be placed in the main draft rather than in the appendix. For example, on Line 278, the theorem of \( C_{l,T,K,s} \) is necessary for understanding the impact of the model structure on generalization. \\
% FutureGen does not seem to differ from general generalization. The so-called future time merely places the training data on a temporal scale; unseen future data and generally considered unknown data in expectation are consistent. Therefore, the description that "the first result which estimates the future-generalization" needs to be rigorously stated. \\
% If you want to consider the performance of TF on time series tasks, the data setting should not only require non-iid data but also consider the dependency of data on the time dimension.\\

% \textbf{Questions:} \\
% How is the non-iid nature of the data manifested? In line 30, is \( f^\star \) the same for different \( n \)? If they are the same, does setting \( M=1 \) in the text degenerate to the iid setting?\\
% Compared to iid, what difficulties and innovations does non-iid bring to the proofs?\\
% In Theorem 1, how can we intuitively understand the impact of \( C_{l,T,K,s} \) on generalization performance? Perhaps this constant merely represents model complexity. What insights about model structure are there, and can they guide model design? Further, the attention module is the key point, does its impact explicitly appear in the results?\\
% In section 3.1, maybe Term (II) means Probabilistic Validity Term and Term (III) means Model Complexity Term (Phase Transitions). This error needs attention as it can cause confusion.\\
% Is \( T^{D,d,0}_{L,W,H} \) in section 3.1 perhaps inconsistent with the definition of \( T^{D,d,1}_{L,H,C} \) in Setting 3.1?\\

% \textbf{Limitations:} \\
% N/A
% \end{tcolorbox}

% \Yan{TODO. Go over notation and see if there is a chance to simplify things. }

% \Yan{\sout{TODO. Label II and III should be changed.}}



% \Yan{TODO. Add details about the key drivers of the bounds. }

% \Yan{TODO. Check notational consistency of \( T^{D,d,0}_{L,W,H} \) in section 3.1 with the definition of \( T^{D,d,1}_{L,H,C} \) in Setting 3.1. }

% \Yan{TODO. Theorem \texttt{[thrm:main]} needs better explanation of \( C_{l,T,K,s} \), which we currently is definied in Table \texttt{[tab:constants]}.}

% \begin{tcolorbox}[colback=white,colframe=blue,title={Response to Reviewer TQAc}]

% \countem

% ## 2. Writing
% Our aim is to communicate results on statistical properties of transformers trained on non-iid data to the widest possible audience. Including technical theorems in the main body of the paper instead of focusing on explanations (e.g., section 3.1) would limit our message to the learning theory sub-community and miss the broader machine learning community, which often uses transformers.  

% ## 3. Future Generalization vs. Generalization
% FutureGen differs substantially from classical generalization as the former is time-dependent while the latter is not.  Indeed, all the available generalization bounds for dependant random variables, which we are aware of, quantify the generalization of a model with respect to the stationary distribution of the data-generating process, which is defined *at* time $\infty$.  Those results are derived using the martingale-convergence theorem, e.g. [3], and apply to the idealized infinite time limit, not realistic finite time points.  

% Our concept of future $t$-risk is meaningful at any intermediate finite time $t$, and is defined with respect to the distribution of $X_t$
% $$
% \mathcal{R}_t(\mathcal{T}) := \mathbb{E}[\ell(\mathcal{T}(X_t),f^{\star}(X_t))]
% $$

% ## 4. Our Bound is Temporal
% The dependency of the temporal dimension of the time series is captured by κ$^t$ term in Theorem $1$.  Here, κ quantifies the distance between the distribution of the Markov process at time $t$ and its stationary distribution at time $\infty$.

% ## Q1
% The parameter $M$ is only the contextual memory of the transformer; which is independent of the data-generating process $X.$.  Rather, the non-iid nature of the data is manifested in the definition of $t$-future generalization $\mathcal{R}_t$ (below line 38) whose definition depends on the *time-dependant* random variable $X_t$.  Since the data-generating process $X_.$ is non-iid, then this distribution can change at every point in time; eg if 
% $$
% X_{t+1} := X_t + t+ \varepsilon_n \mbox{ and } \varepsilon_t\sim N(0,1)
% $$
% then the conditional mean $X_t+t$, conditioned on $X_t$, is $X_{t+1}+t$ while $X_0$ has mean $0$.  This type of time-dependence cannot occur in the simple iid setting.   Thus, future generalization depends on the temporal dimension.

% ## Q2
% The inclusion of the non-iid terms is motivated by the goal of applicability in real-life settings, which rarely adhere to the iid assumptions prevalent in classical literature. Thus, the available generalization bounds do not apply in these settings, leaving no theoretical control on the generalization gap.   

% The technical challenges in deriving non-iid generalization bounds in the proof of Proposition (7), are controlling terms (IV) and (V):

% - Term (IV), only exists in the non-iid setting. It is the gap between the distribution of $X_t$ and the stationary distribution at time $\infty$.  This is identically $0$ in the iid setting (since, there, each $X_t$ equals to its own stationary distribution).  In our non-iid setting, we control (V) by bounding the rate of ergodicity of $X_.$ (lines 801-820).  

% - Term (V) is the gap between the empirical distribution and the stationary distribution of the Markov process.  In the non-iid setting, one has access to classic tools such as Rademacher complexity or bracketing number bounds, but these all rely on the irrealistic iid assumption [1,2].  Thus, these tools cannot be used in our setting, and we can only control (V) using non-standard concentration arguments for Markov processes (lines 820-829).  

% ## Q3
% Our analysis found that the role of different components of the transformer model has surprisingly varied effects on this constant.  We find that: making transformers large using feedforward layers and layernorms is not problematic, while users should use multi-head attention strategically and sparingly.   

% - Figure 3 and Table 6 show that the inclusion of multi-head attention mechanisms in each transformer block significantly increases the magnitude of this constant, while layer norms and SLP (single layer perception) do not.  

% - Table 2 also supports practitioner wisdom by showing that the GeLU and Swish activation functions do not increase this constant much, as compared to less popular activation functions such as $\tanh$.  

% Each of these computations provides transformer-specific insights on its generalization beyond the well known fact that larger classes models generalize (see response to 71oV for more details).

% ## 1 + Q4 + Q5
% Thank you for pointing out these typos, relegating technical notation to the appendix, and ensuring that all constants, e.g. $C_{l,\mathcal{T},K,s}$, are explained in the main body. 

% [1] Van Der Vaart, A. W., Wellner, J. A., van der Vaart, A. W., Wellner, J. A. (1996). Weak convergence.

% [2] Shalev-Shwartz, S., & Ben-David, S. (2014). Understanding machine learning: From theory to algorithms.

% [3] Kontorovich, A., and Raginsky, M. (2017). Concentration of measure without independence: a unified approach via the martingale method.


% \endcountem
% \flushright Character count: \thelettercount{}

% \end{tcolorbox}
% \Yan{For the future gen vs gen result, can we point the reviewer to the section where this concept is described? Or saying something like ``we made changes in our draft to make this more clear''}

% \Yan{The comment on the temp dependence is strong :) }





% \subsection{QLiw}

% \begin{tcolorbox}[colback=white,colframe=black,title={Reviewer QLiw, Rating 6, Confidence 2}]
% \small
% \textbf{Summary:} \\
% This paper provides non-asymptotic bounds on the generalization gap of a transformer network given non-iid data from a single trajectory of a Markov process. Specifically, assuming the Markov process satisfies the Log-Sobolev Inequality (Assumption 1) and that the trajectory from the Markov process is bounded with probability 1 (Assumption 2), Theorem 1 establishes that the generalization gap is non-asymptotically bounded by three terms. The non-stationarity term quantifies the rate at which the data-generating Markov process becomes stationary, the model complexity term encodes the complexity of the transformer network, and the probabilistic validity term indicates the cost of the bound being valid with probability at least \(\delta\). All these terms converge to zero as the number of data points goes to infinity.\\

% \textbf{Soundness:} 3: good \\
% \textbf{Presentation:} 3: good \\
% \textbf{Contribution:} 2: fair \\

% \textbf{Strengths:} \\
% This is the first study to provide generalization bounds for transformers in the case of non-iid training data over a future time point. By rigorously formalizing the transformer architecture and employing higher-order derivatives of the transformer network, this work offers non-asymptotic bounds on the generalization gap. The concentration of measure arguments for integral probability metrics used in the proof enhance the novelty of the theoretical analysis.\\

% \textbf{Weaknesses:} \\
% I'm uncertain about the realism and validity of the assumptions and \(\delta\), as well as the significance of the generalization gap result over a future time point in the context of transformer optimization.\\

% \textbf{Questions:} \\
% In line 146, what does SLP stand for? The parenthesis seems unnecessary (fully connected affine layer).\\
% In line 154, typo parenthesis.\\
% In line 164, what is the definition of \(\bullet\)?\\
% In line 192, typo `functions functions'.\\
% In line 197, typo `if are'.\\
% In line 197, what is the definition of \(| \cdot |_{C^s[0,1]}\)?\\
% In line 224, label II and III should be changed.\\
% In line 297, what is \(C^s\) function?\\

% \textbf{Limitations:} \\
% Yes, authors addressed the limitations.
% \end{tcolorbox}

% \Yan{\sout{TODO. In line 146, what does SLP stand for? The parenthesis seems unnecessary (fully connected affine layer).}}

% \Yan{\sout{TODO. In line 154, typo parenthesis.}}

% \Yan{\sout{TODO. In line 164, what is the definition of \(\bullet\)?}}

% \Yan{\sout{TODO. In line 192, typo `functions functions'.}}

% \Yan{\sout{TODO. In line 197, typo `if are'.}}

% \Yan{\sout{TODO. In line 197, what is the definition of \(| \cdot |_{C^s[0,1]}\)?}}

% \Yan{\sout{TODO. In line 224, label II and III should be changed.}}

% \Yan{\sout{TODO. In line 297, what is \(C^s\) function?}}

% \begin{tcolorbox}[colback=white,colframe=blue,title={Response to Reviewer QLiw}]
% \countem


% \textbf{Realism of Assumptions $1$ and $2$}
% Thank you very much for your valuable and positive feedback.  
% All our results in fact hold upon directly assuming that the data-generating process is exponentially ergodic, i.e. that equation ($9$) in the proof of Proposition $2$, holds instead of proving it using Assumption $1$.  Doing so, implies that a long list of examples are all covered by our setting (as well as a shorter proof of that result).  

% One class of such processes are the projections of Langevin dynamics with strictly convex potential $U:\mathbb{R}^d\to \mathbb{R}$ onto any compact convex subset $C$ of $\mathbb{R}^d$.  For this let $\mu=-\nabla U/2$ and consider the solution to the stochastic differential equation
% $$
% Z_t = \int_0^t \mu(Z_s)ds + \int_0^t\, dW_s,
% $$
% where $W_{\cdot}$ is a Brownian motion.  Let $P:\mathbb{R}^d\to C$ be the (metric) projection onto $C$ and defined $X_{\cdot}:=(X_n)_{n=0}^{\infty}$ by
% $$
% X_n := x + P(Z_n)
% $$
% satisfies these conditions.  

% This example can be significantly extended to include several other processes satisfying ($9$).  In fact, the ``latent process'' $Z_{\cdot}$ may even depend on its own distribution at any given time (so-called McKean-Vlasov SDEs). For this class, our exponential ergodicity condition (9) as proven in [1] and in the case of the Brownian motion $W_{\cdot}$ being a broad range of pure-jump L\'{e}vy process, our condition (9) was as shown in [2].  Further, one does not need to rely on projections into $C$, and they can instead consider reflected SDEs, which are instantaneously reflected back into $C$ to ensure that $1$ holds. For this class, (9) was shown in [3].   Further examples of Markov processes satisfying (9) are also constructed in Theorem 2.5 of [4].  In this way, a very broad range of processes, whose trajectories satisfy our weaker assumptions, namely that (9) holds directly, and satisfying Assumption $1$; all of which are entirely outside the score of most learning theoretic results which require iid\ data. Furthermore, the projection, $P$, can be replaced by any bounded $1$-Lipschitz function, possibly mapping into a different Euclidean space.

% In our revision, we will replace Assumption $1$ by directly assuming (9), and adding some of these examples.  


% \textbf{Typos / terminology} We also thank you for pointing out those typos and missing terminology (e.g. single layer perceptron/shallow neural network (SLP) and $s$-times continuously differentiable functions ($C^s$-functions) we have corrected them and added all missing definitions in the main body of our paper.



% [1] Wang, Feng-Yu. "Exponential ergodicity for singular reflecting McKean–Vlasov SDEs." Stochastic Processes and their Applications 160 (2023): 265-293.

% [2] Luo, Dejun, and Jian Wang. "Refined basic couplings and Wasserstein-type distances for SDEs with Lévy noises." Stochastic Processes and their Applications 129.9 (2019): 3129-3173.

% [3] Wang, Feng-Yu. "Exponential ergodicity for singular reflecting McKean–Vlasov SDEs." Stochastic Processes and their Applications 160 (2023): 265-293.

% [4] Hairer, Martin, and Jonathan C. Mattingly. "Spectral gaps in Wasserstein distances and the 2D stochastic Navier–Stokes equations." (2008): 2050-2091.

% \endcountem

% \flushright Character count: \thelettercount{}

% \end{tcolorbox}

% \Yan{I think this is a very strong response and we should explicitly ask for a rating upgrade after the ``Realism'' paragraph.}

% \subsection{71oV}

% \begin{tcolorbox}[colback=white,colframe=black,title={Reviewer 71oV, Rating 3, Confidence 4}]
% \small
% \textbf{Summary:} \\
% In this submission, the authors studied the generalization error of time series data following a Markov process. The data are \(N\) observations of sample trajectories, and the goal is to predict future trajectories. The authors considered the class of Transformer networks, and they provided a uniform bound between the empirical risk and the population risk.\\

% Under several assumptions of smoothness, bounded partial derivatives, and other technical assumptions, the authors proved that the generalization bound scales with the parametric rate \(O(1/\sqrt{N})\), a nonstationarity term, and a term that reflects the model complexity.\\

% \textbf{Soundness:} 2: fair \\
% \textbf{Presentation:} 1: poor \\
% \textbf{Contribution:} 2: fair \\

% \textbf{Strengths:} \\
% Generalization bounds for non-iid data are less studied in the literature, this paper fills the gap by providing a generalization bound in this setting.\\
% The model complexity term that adapts to the smoothness parameter \(s\) is interesting. It is connected to the classic literature of nonparametric statistics.\\

% \textbf{Weaknesses:} \\
% The Transformer structure does not seem to be connected to how well the model generalizes in a substantial way. We do not gain more insights than the well-known intuition that a bigger model class induces a larger model complexity term bound in the bound. In fact, the model class does not matter much in terms of the analysis provided by the paper, as long as it is assumed that the model is sufficiently smooth.\\
% There are several key terms that are not clearly defined or less explained. Here are some examples.\\
% Where is the key constant \(C\) defined? In Theorem 1, it refers to Table 1, but it is not clearly defined there. Moreover, why does this constant depend on \(\mathcal{T}\)? In Theorem 1, on the left-hand side, the supremum is taken already over \(\mathcal{T}\).\\
% In Section 3.1, are the explanations about term (II) and (III) switched? \\
% In Definition 5, should \(Cs^r\) be \(Cr^s\)?\\
% Are there concrete examples of time series data that satisfy the assumptions? There are currently many assumptions such as boundedness of the observations, and what I feel a pretty strong assumption on the Markov process in Assumption 1. Currently, it is hard to evaluate how broadly applicable the results are.\\

% \textbf{Questions:} \\
% See above.\\

% \textbf{Limitations:} \\
% NA
% \end{tcolorbox}

% \Yan{\sout{TODO. Label II and III should be changed.}}

% \Yan{{TODO. Clarify that $C$ in Theorem \texttt{thrm:main} is dependent on the transformer class not the transfomer.}}

% \Yan{TODO. Add details about the key drivers of the bounds. }

% \begin{tcolorbox}[colback=white,colframe=blue,title={Response to Reviewer 71oV}]
% \countem
% # How the transformer structure enters into our bound

% The level of smoothness $s$ does yield the convergence rate on page $7$ (in the iid setting a generalization bound can be deduced using only the number of derivatives by Theorem $10$ of [1] or bracketing number estimates as in Corollary $2.7.4$ [2] for $C^s$-functions together with standard entropy integral estimates).  
% However, each of these estimates (including our non-iid argument) requires the computation of the key constant 
% $$
% C_{\ell,\mathcal{T},K,s}:=\max_{\mathcal{T}}\|\ell(\mathcal{T},f^{\star})\|
% $$
% where the maximum is taken over the transformer class.  The computation of this constant is necessary in order to have a truly non-asymptotic generalization bound and not simply a convergence rate. 

% It is precisely here that the structure of the class of transformers enters into the generalization bound. When $s>1$, the computation of the constant $C_{\ell,\mathcal{T},K,s}$ is highly challenging and comprises a major part of our analysis; see pages $28-37$ of our appendix.  Since these computations make up more than half of our argument, then we see that our argument depends intimately on the transformer model class.  


% # Insights gained from our analysis beyond a bigger model class induce a larger model complexity.
% Whilst we agree with the intuition that a bigger model class induces a larger model complexity term, our results are not limited to this standard insight. 

% Consider the expression of the aforementioned constant on line 278, whose behaviour is broken down in Figures $2$ and $3$, as well as several tables in Appendix $B$.  The analysis of this constant reveals the following insights on specific components of the transformer model:

% - Figure 3 - b and Table 4: The layernorm does not have any major adverse effect on the generalization bound.

%  Table 6—The multihead attention mechanism should be used sparingly since it dramatically increases this constant due to the interactions between the higher-order derivatives of the softmax functions and the transformer blocks feeding into it.
 
%  Table 3—The single perceptron layer (SLP) used in each transformer block has a negligible effect on the size of the constant in our generalization bound compared to the effect of the multi-head attention mechanism.  

% -  Figure 3 - a and Table 2: The standard Swish and Softplus activation functions have negligible effects on transformer generalization while uncommon activation functions such as tanh negatively impact transformer generalization.  

% Thus, our detailed analysis of the constant $C_{\ell,\mathcal{T},K,s}$ provides a detailed understanding of the role of each transformer component, even down to the choice of activation function, on its statistical properties.

% We would also like to highlight that the analysis of the constant $C_{\ell,\mathcal{T},K,s}$ constitutes a major part of our proofs (pages 28-39) as well as the supporting lemmata (pages 23-26) which are all solely devoted to estimating this constant as accurately as possible.  The computation of this constant, and thus its effect on the transformer class' generalization, depends explicitly on each component of the transformer model.  

% Section D.3.1-D.3.2 computes the multi-head attention mechanism contribution, D.3.3 computes the effect of each choice of activation function, D.3.4 the effect of layer norms, and D.3.5 the contribution of the MLPs in each transformer block to this constant; the results in section D.1 were then used to describe the interplay between these components of each transformer block and this key constant.


% # Breadth of Results - Processes Satisfying Our Assumptions
% In our main response, we provided a long list of data-generating Markov processes for our results holds.  We underscore that this non-exhaustive list of examples contains many SDEs, Lévy processes, and even SDEs depending on their own law (McKean-Vlasov), arising in mean-field games. All of these examples are completely outside the scope of results requiring iid data.  The bulk of results on signal processing, stochastic optimal control, and several results in dynamic game theory and economics all consider processes whose trajectories belong to these types of classes.  


% ## Typos
% We thank you for noticing these typos, such as (II) and (III) being switched; all these updates have been made.

% ## Miscellaneous
% If $g\in C^\infty_{poly: C, r}([0,1]^d, \mathbb{R}^D)$, then $g$ has polynomial growth of degree r under $C^s$-norm,  $\forall s \in \mathbb{N}_+$ (see Definition 7 (i)); which is consistent with our use in  Lemma $14$, therefore with Theorem $8$ below, and with the rest of the paper.  

% [1] Hou, S., Kassraie, P., Kratsios, A., Krause, A., and Rothfuss, J. (2023). Instance-dependent generalization bounds via optimal transport. The Journal of Machine Learning Research.

% [2] Van Der Vaart, A. W., Wellner, J. A., van der Vaart, A. W., Wellner, J. A. (1996). Weak convergence.

% \endcountem

% \flushright Character count: \thelettercount{}

% \end{tcolorbox}

% % such as (II) and (III) being switched. We also acknowledge that the presentation of the constant $C_{\ell, \mathcal{T}, K, s}$ (see line 278) in the main body is hard to follow. In our pursuit to make this paper accessible for a broader ranging audience, the purpose of Table 1 is to give bounds on the components mentioned in line 278 and relegate more technical details to the appendix. We have improved the readability and interpretibility of this table in our revised draft as well as elaborated in the appendix more on the defintion of the constant. As you will not have access to the revised version, we will give some further information here, to answer your question: For the three types of choices for $\ell$, you can find the detailed definition of the bound in (Equation 45, Line 1079), (Equation 46, Line 1080), (Equation 47, Line 1081). Note that all three depend on $C^{\mathcal{TC}}_K(s)$, the constant describing the $C^s$-bound of a transformer class on a set $K$. We provide two ways to bound this constant, one explicit (Theorem 5, Line 979ff) and one in $\mathcal{O}$-notation (Theorem 6, Line 986).


% \end{document}


==> jmlr/cmd_jmlr.tex <==
% \usepackage{amsthm}
% \smartqed  % flush right qed marks, e.g. at end of proof
\usepackage{graphicx}


%-------%
% Fonts % 
%-------%
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{booktabs}       % professional-quality tables


% General Packages
%------------------%
\usepackage{amsfonts,amssymb,bbm}
\usepackage{amsmath}
\usepackage[inline]{enumitem}
\usepackage{graphicx}
\usepackage{adjustbox}
\usepackage[UKenglish]{isodate}
\usepackage{graphicx}
\usepackage{silence}
\WarningFilter{caption}{Unknown document class (or package)}
\usepackage[format=default,font=small,labelfont=it]{caption}
\usepackage{subcaption}
\usepackage[table,x11names]{xcolor}         % colors
    \definecolor{darkcerulean}{rgb}{0.03, 0.27, 0.49}
    \definecolor{smokyblack}{rgb}{0.06, 0.05, 0.03}
    \definecolor{warmblack}{rgb}{0.0, 0.26, 0.26}
    \definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
    \definecolor{darkcobalt}{rgb}{0.1, 0.38, 0.77}
    % \usepackage[colorlinks=true,
    %             linkcolor=cobalt,
    %             urlcolor=darkcerulean,
    %             citecolor=cobalt]{hyperref}%warmblack
%%% Coloring Equation Numbers
\usepackage{mathtools}
\newtagform{blue}{\color{darkcobalt}(}{)}


\usepackage[overload]{empheq}




\usepackage{float}
\usepackage{afterpage}
\usepackage{enumitem}
\usepackage{multirow}
\usepackage{fancyvrb}
\usepackage{rotating}
    %%% Tikz
    \usepackage{tikz}
    \usepackage{tikz-cd} 
    \pgfdeclarelayer{edgelayer}
    \pgfdeclarelayer{nodelayer}
    \pgfsetlayers{edgelayer,nodelayer,main}
    %%%% Custom Node styles
    \tikzstyle{new style 0}=[fill={rgb,255: red,255; green,94; blue,247}, draw=black, shape=circle]
    \tikzstyle{pointy}=[fill=white, draw=black, shape=circle]
    %%%% Custom Edge styles
    \tikzstyle{pointy}=[->]
\usepackage{fontawesome}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{positioning, shapes.geometric, fit, backgrounds}
\usetikzlibrary{calc}



%To display labels in the PDF. Comment at the end!
% Code
\usepackage{algpseudocode}
\usepackage[linesnumbered,lined,boxed,commentsnumbered,ruled,longend]{algorithm2e}
\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
\SetCommentSty{mycommfont}

% TABLE Formatting
\raggedbottom
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
\setlength\heavyrulewidth{0.3ex}
\usepackage{lscape}



\makeatletter
\newcommand{\pushright}[1]{\ifmeasuring@#1\else\omit\hfill$\displaystyle#1$\fi\ignorespaces}
\newcommand{\pushleft}[1]{\ifmeasuring@#1\else\omit$\displaystyle#1$\hfill\fi\ignorespaces}
\makeatother


\DeclareMathOperator{\reshape}{reshape}
\DeclareMathOperator{\vectorize}{vec}
\DeclareMathOperator{\layernorm}{\mathcal{L\!N}} % Layernorm
\DeclareMathOperator{\concat}{cat}
\DeclareMathOperator{\softmax}{softmax}
\DeclareMathOperator{\smax}{smax}
\DeclareMathOperator{\softplus}{splus} %softplus
\DeclareMathOperator{\sigmoid}{sig}
\DeclareMathOperator{\attention}{Att} % ention
\DeclareMathOperator{\multihead}{\mathcal{M\!H}} %MultiHead
\DeclareMathOperator{\dotp}{dp}
% \DeclareMathOperator{\neuraln}{\mathcal{N}\!\!\!\!\mathcal{N}}
\DeclareMathOperator{\neuraln}{\operatorname{\mathcal{P\!L}}}
\DeclareMathOperator{\tblock}{\mathcal{T\!B}}
\DeclareMathOperator{\tblockclass}{\mathcal{T\!B\!C}}
\DeclareMathOperator{\transformer}{\mathcal{T}}
\DeclareMathOperator{\transformerclass}{\mathcal{T}\!\mathcal{C}}


\DeclareMathOperator{\cleq}{\mbox{\tiny$\leq$}\!}



\DeclareMathOperator{\Leb}{Leb}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\inter}{int}
\DeclareMathOperator*{\esssup}{ess\,sup}
\DeclareMathOperator{\tr}{tr}

\newcommand{\tagA}{^{(3)}}
\newcommand{\tagB}{^{(2)}}
\newcommand{\tagC}{^{(1)}}

\newcommand{\order}{\mathfrak{o}}
\newcommand{\Order}{\mathfrak{O}}
\newcommand{\n}{\mathbbm{n}}
\newcommand{\bE}{\mathbb{E}}
\newcommand{\bP}{\mathbb{P}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\1}{\mathbbm{1}}
\newcommand{\II}{I_{\varepsilon,\Gamma}}

%Modifiche comode 
\renewcommand{\phi}{\varphi}
\newcommand{\eps}{\varepsilon}
\newcommand{\al}{\alpha}
\newcommand{\om}{\omega}
\newcommand{\Om}{\Omega}
\newcommand{\lam}{\lambda}
\newcommand{\Ll}{\left}
\newcommand{\rr}{\mathbb{R}}
\newcommand*\diff{\mathop{}\!\mathrm{d}}
%\def\mathsf{1}{\mathds{1}}
\let\oldemptyset\emptyset
\let\emptyset\varnothing
\newcommand{\essinf}{\operatornamewithlimits{ess\,inf}}
\newcommand{\paren}[1]{\left( \left. #1 \right. \right)}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\BL}{BL}
\newcommand\sbullet[1][.5]{\mathbin{\vcenter{\hbox{\scalebox{#1}{$\bullet$}}}}}
\newcommand{\rhoseason}{m_{\rho}}%\rho_{\mathrm{season}}}% name of the seasonality function: m_{\rho} in [Arlot 2004]
\newcommand{\rhoseasondiscrete}[1]{m_{\rho,#1}}
\newcommand{\rhomin}{\ensuremath{\mu_{\min}}} %changed by Duccio
\newcommand{\rhomax}{\ensuremath{\mu_{\max}}} %changed by Duccio
\newcommand{\croch}[1]{\left[ \left. #1 \right. \right]}
\newcommand{\survival}{\ensuremath{\mathbb{S}}}

% Processes
\newcommand{\process}[3]{{#1}({#2})_{#3}}
\newcommand{\myset}[2]{\lbrace{#1}, \ldots, {#2}\rbrace}
\newcommand{\mySet}[2]{\left\lbrace {#1} \middle\vert {#2} \right\rbrace}


% Mathbb
\newcommand{\C}{\mathbb{C}}
\newcommand{\D}{\mathbf{D}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\N}{\mathbb{N}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\K}{\mathbb{K}}
\newcommand{\Cg}{\mathfrak{C}}
\newcommand{\bdot}{\boldsymbol{\cdot}}


% Calligrafiche
\newcommand{\Aa}{\mathcal{A}}
\newcommand{\Bb}{\mathcal{B}}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Ee}{\mathcal{E}}
\newcommand{\Ff}{\mathcal{F}}
\newcommand{\Hh}{\mathcal{H}}
\newcommand{\Ii}{\mathcal{I}}
\newcommand{\Kk}{K}
\newcommand{\Mm}{\mathcal{M}}
\newcommand{\Nn}{\mathcal{N}}
\newcommand{\Qq}{\mathcal{Q}}
\newcommand{\Ss}{\mathcal{S}}
\newcommand{\Xx}{\mathcal{X}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}

\newcommand{\eqdef}{\ensuremath{\,\raisebox{-1pt}{$\stackrel{\mbox{\upshape\tiny def.}}{=}$}}\,}
\newcommand{\eqorder}{\sim} %{\ensuremath{\,\raisebox{-1pt}{$\stackrel{\mbox{\upshape\tiny $\order$}}{\sim}$}}\,}
% \newcommand{\eqdef}{\stackrel{\mathclap{\tiny\mbox{def.}}}{=}}


%\newcommand{\sdim}{{N_\mathrm{sim}}} %Similarity score encoding dimension
%\newcommand{\pdim}{{N_\mathrm{pos}}} %Positional encoding dimension
%\newcommand{\edim}{{N}} % Encoding dimension
%\newcommand{\ddim}{{N'}} % Decoding dimension (target dimension of MLP)
%\newcommand{\rdim}{{N_\mathrm{ref}}} %Number of reference paths
%\newcommand{\tdim}{{N_\mathrm{time}}} %Number of reference time points
%\newcommand{\pldim}{{N_\mathrm{p}}} %Number of time points between linear pieces
%\newcommand{\ldim}{{d_K}} %Latent dimension, was {d_K}

\newcommand{\idim}{d_{\mathrm{in}}} % Input dimension
\newcommand{\odim}{d_{\mathrm{out}}} % Output dimension
\newcommand{\kdim}{d_{K}} % Key dimension
\newcommand{\vdim}{d_{V}} % Value dimension
\newcommand{\ldim}{d_{\mathrm{ff}}} % Feed forward latent dimension

% Cose del modello
\newcommand{\rhosummer}{\rho}% name of the length of summer
\newcommand{\rhowinter}{\rho}% name of the length of winter

% \usepackage{amsthm}
% \newtheorem{atheorem}{Theorem}
% \renewcommand{\theatheorem}{\Alph{atheorem}} % "letter-numbered" theorems
% \newtheorem{InformalTheorem}{Informal Theorem}
% \newtheorem{definition}{Definition}
% \newtheorem{proposition}{Proposition}
% \newtheorem{assumption}{Assumption}
% \newtheorem{theorem}{Theorem}
% \newtheorem{lemma}{Lemma}
% \newtheorem{corollary}{Corollary}
\newtheorem{notation}{Notation}
\newtheorem{setting}{Setting}[section]
% \newtheorem{assumptions}{Assumptions}[section]
% \theoremstyle{remark}
% \newtheorem*{remark}{Remark}
% \newtheorem{example}{Example}
% % \theoremstyle{definition}
% \newtheorem{question}{Question}


% QED Symbol 
% \usepackage{etoolbox}
% \newcommand{\addQEDstyle}[2]{\AtBeginEnvironment{#1}{\pushQED{\qed}\renewcommand{\qedsymbol}{#2}}\AtEndEnvironment{#1}{\popQED}}
% \addQEDstyle{remark}{$\triangleleft$}
% \addQEDstyle{example}{$\triangleleft$}



%%%% COMMENTING (Temporary)
\NewDocumentCommand{\luca}{mo}{
    \IfValueF{#2}{
    %%%%% NO Margin Note
                        {{\scriptsize
                            \textcolor{green}{ 
                            \textbf{L:}
                            \textit{{#1}}
                            }
                        }}
        }
    %%%% Margin Note
    \IfValueT{#2}{
                        \marginnote{{\scriptsize
                            \textcolor{green}{ 
                            \textbf{L:}
                            \textit{{#1}}
                            }
                        }}
        }
                    }
\NewDocumentCommand{\giulia}{mo}{
    \IfValueF{#2}{
    %%%%% NO Margin Note
                        {{\scriptsize
                            \textcolor{red}{ 
                            \textbf{GL:}
                            \textit{{#1}}
                            }
                        }}
        }
    %%%% Margin Note
    \IfValueT{#2}{
                        \marginnote{{\scriptsize
                            \textcolor{red}{ 
                            \textbf{GL:}
                            \textit{{#1}}
                            }
                        }}
        }
}
\NewDocumentCommand{\anastasis}{mo}{
    \IfValueF{#2}{
    %%%%% NO Margin Note
                        {{\scriptsize
                            \textcolor{violet}{ 
                            \textbf{A:}
                            \textit{{#1}}
                            }
                        }}
        }
    %%%% Margin Note
    \IfValueT{#2}{
                        \marginnote{{\scriptsize
                            \textcolor{violet}{ 
                            \textbf{A:}
                            \textit{{#1}}
                            }
                        }}
        }
                    }
                    
\NewDocumentCommand{\cody}{mo}{
    \IfValueF{#2}{
    %%%%% NO Margin Note
                        {{\scriptsize
                            \textcolor{orange}{ 
                            \textbf{A:}
                            \textit{{#1}}
                            }
                        }}
        }
    %%%% Margin Note
    \IfValueT{#2}{
                        \marginnote{{\scriptsize
                            \textcolor{orange}{ 
                            \textbf{A:}
                            \textit{{#1}}
                            }
                        }}
        }
                    }

\newcommand{\byyan}[1]{\textcolor{cyan}{#1}}
\NewDocumentCommand{\yannick}{mo}{
    \IfValueF{#2}{
    %%%%% NO Margin Note
                        {{\scriptsize
                            \textcolor{cyan}{ 
                            \textbf{Y:}
                            \textit{{#1}}
                            }
                        }}
        }
    %%%% Margin Note
    \IfValueT{#2}{
                        \marginnote{{\scriptsize
                            \textcolor{cyan}{ 
                            \textbf{Y:}
                            \textit{{#1}}
                            }
                        }}
        }
                    } 

\definecolor{darkgreen}{rgb}{0.0, 0.2, 0.13}
\NewDocumentCommand{\xuwei}{mo}{
    \IfValueF{#2}{
    %%%%% NO Margin Note
                        {{\scriptsize
                            \textcolor{darkgreen}{ 
                            \textbf{X:}
                            \textit{{#1}}
                            }
                        }}
        }
    %%%% Margin Note
    \IfValueT{#2}{
                        \marginnote{{\scriptsize
                            \textcolor{darkgreen}{ 
                            \textbf{X:}
                            \textit{{#1}}
                            }
                        }}
        }
                    }

\usepackage{appendix}
\usepackage{titletoc}
\newcommand\DoToC{%
  \startcontents
  \printcontents{}{1}{\textbf{Appendix Contents}\vskip3pt\hrule\vskip5pt}
  \vskip3pt\hrule\vskip5pt
}

% Make the "Part I" text invisible
\renewcommand \thepart{}
\renewcommand \partname{}


\usepackage{cleveref}
\newcounter{termcounter}
\renewcommand{\thetermcounter}{\Roman{termcounter}}
\crefname{term}{term}{terms}
\creflabelformat{term}{#2\textup{(#1)}#3}

\makeatletter
\def\term{\@ifnextchar[\term@optarg\term@noarg}%]
\def\term@optarg[#1]#2{%
  \textup{#1}%
  \def\@currentlabel{#1}%
  \def\cref@currentlabel{[][2147483647][]#1}%
  \cref@label[term]{#2}}
\def\term@noarg#1{%
  \refstepcounter{termcounter}%
  \textup{(\thetermcounter)}%
  \cref@label[term]{#1}}
\makeatother


%  \setcounter{termcounter}{0}

\crefname{lemma}{lemma}{lemmata}
\Crefname{lemma}{Lemma}{Lemmata}
\crefname{notation}{notation}{notations}
\Crefname{notation}{Notation}{Notations}
\crefname{assumption}{assumption}{assumptions}
\Crefname{assumption}{Assumption}{Assumptions}
\crefname{example}{Example}{Examples}
\crefname{proposition}{Proposition}{Proposition}


\usepackage{comment}
\usepackage{microtype}





==> math_commands.tex <==
% \usepackage{amsthm}
% \smartqed  % flush right qed marks, e.g. at end of proof
\usepackage{graphicx}


%-------%
% Fonts % 
%-------%
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{booktabs}       % professional-quality tables


% General Packages
%------------------%
\usepackage{amsfonts,amssymb,bbm}
\usepackage{amsmath}
\usepackage[inline]{enumitem}
\usepackage{graphicx}
\usepackage{adjustbox}
\usepackage[UKenglish]{isodate}
\usepackage{graphicx}
\usepackage{silence}
\WarningFilter{caption}{Unknown document class (or package)}
\usepackage[format=default,font=small,labelfont=it]{caption}
\usepackage{subcaption}
\RequirePackage[table,x11names]{xcolor}         % colors
    \definecolor{darkcerulean}{rgb}{0.03, 0.27, 0.49}
    \definecolor{smokyblack}{rgb}{0.06, 0.05, 0.03}
    \definecolor{warmblack}{rgb}{0.0, 0.26, 0.26}
    \definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
    \definecolor{darkcobalt}{rgb}{0.1, 0.38, 0.77}
    % \usepackage[colorlinks=true,
    %             linkcolor=cobalt,
    %             urlcolor=darkcerulean,
    %             citecolor=cobalt]{hyperref}%warmblack
%%% Coloring Equation Numbers
% \usepackage{mathtools}
% \newtagform{blue}{\color{darkcobalt}(}{)}


\usepackage[overload]{empheq}




\usepackage{float}
\usepackage{afterpage}
\usepackage{enumitem}
\usepackage{multirow}
\usepackage{fancyvrb}
\usepackage{rotating}
    %%% Tikz
    \usepackage{tikz}
    \usepackage{tikz-cd} 
    \pgfdeclarelayer{edgelayer}
    \pgfdeclarelayer{nodelayer}
    \pgfsetlayers{edgelayer,nodelayer,main}
    %%%% Custom Node styles
    \tikzstyle{new style 0}=[fill={rgb,255: red,255; green,94; blue,247}, draw=black, shape=circle]
    \tikzstyle{pointy}=[fill=white, draw=black, shape=circle]
    %%%% Custom Edge styles
    \tikzstyle{pointy}=[->]
% \usepackage{fontawesome}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{positioning, shapes.geometric, fit, backgrounds}
\usetikzlibrary{calc}



%To display labels in the PDF. Comment at the end!
% Code
\usepackage{algpseudocode}
\usepackage[linesnumbered,lined,boxed,commentsnumbered,ruled,longend]{algorithm2e}
\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
\SetCommentSty{mycommfont}

% TABLE Formatting
\raggedbottom
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
\setlength\heavyrulewidth{0.3ex}
\usepackage{lscape}



\makeatletter
\newcommand{\pushright}[1]{\ifmeasuring@#1\else\omit\hfill$\displaystyle#1$\fi\ignorespaces}
\newcommand{\pushleft}[1]{\ifmeasuring@#1\else\omit$\displaystyle#1$\hfill\fi\ignorespaces}
\makeatother


\DeclareMathOperator{\reshape}{reshape}
\DeclareMathOperator{\vectorize}{vec}
\DeclareMathOperator{\layernorm}{\mathcal{L\!N}} % Layernorm
\DeclareMathOperator{\concat}{cat}
\DeclareMathOperator{\softmax}{softmax}
\DeclareMathOperator{\smax}{smax}
\DeclareMathOperator{\softplus}{splus} %softplus
\DeclareMathOperator{\sigmoid}{sig}
\DeclareMathOperator{\attention}{Att} % ention
\DeclareMathOperator{\multihead}{\mathcal{M\!H}} %MultiHead
\DeclareMathOperator{\dotp}{dp}
% \DeclareMathOperator{\neuraln}{\mathcal{N}\!\!\!\!\mathcal{N}}
\DeclareMathOperator{\neuraln}{\operatorname{\mathcal{P\!L}}}
\DeclareMathOperator{\tblock}{\mathcal{T\!B}}
\DeclareMathOperator{\tblockclass}{\mathcal{T\!B\!C}}
\DeclareMathOperator{\transformer}{\mathcal{T}}
\DeclareMathOperator{\transformerclass}{\mathcal{T}\!\mathcal{C}}


\DeclareMathOperator{\cleq}{\mbox{\tiny$\leq$}\!}



\DeclareMathOperator{\Leb}{Leb}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\inter}{int}
\DeclareMathOperator*{\esssup}{ess\,sup}
\DeclareMathOperator{\tr}{tr}

\newcommand{\tagA}{^{(3)}}
\newcommand{\tagB}{^{(2)}}
\newcommand{\tagC}{^{(1)}}

\newcommand{\order}{\mathfrak{o}}
\newcommand{\Order}{\mathfrak{O}}
\newcommand{\n}{\mathbbm{n}}
\newcommand{\bE}{\mathbb{E}}
\newcommand{\bP}{\mathbb{P}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\1}{\mathbbm{1}}
\newcommand{\II}{I_{\varepsilon,\Gamma}}

%Modifiche comode 
\renewcommand{\phi}{\varphi}
\newcommand{\eps}{\varepsilon}
\newcommand{\al}{\alpha}
\newcommand{\om}{\omega}
\newcommand{\Om}{\Omega}
\newcommand{\lam}{\lambda}
\newcommand{\Ll}{\left}
\newcommand{\rr}{\mathbb{R}}
\newcommand*\diff{\mathop{}\!\mathrm{d}}
%\def\mathsf{1}{\mathds{1}}
\let\oldemptyset\emptyset
\let\emptyset\varnothing
\newcommand{\essinf}{\operatornamewithlimits{ess\,inf}}
\newcommand{\paren}[1]{\left( \left. #1 \right. \right)}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\BL}{BL}
\newcommand\sbullet[1][.5]{\mathbin{\vcenter{\hbox{\scalebox{#1}{$\bullet$}}}}}
\newcommand{\rhoseason}{m_{\rho}}%\rho_{\mathrm{season}}}% name of the seasonality function: m_{\rho} in [Arlot 2004]
\newcommand{\rhoseasondiscrete}[1]{m_{\rho,#1}}
\newcommand{\rhomin}{\ensuremath{\mu_{\min}}} %changed by Duccio
\newcommand{\rhomax}{\ensuremath{\mu_{\max}}} %changed by Duccio
\newcommand{\croch}[1]{\left[ \left. #1 \right. \right]}
\newcommand{\survival}{\ensuremath{\mathbb{S}}}

% Processes
\newcommand{\process}[3]{{#1}({#2})_{#3}}
\newcommand{\myset}[2]{\lbrace{#1}, \ldots, {#2}\rbrace}
\newcommand{\mySet}[2]{\left\lbrace {#1} \middle\vert {#2} \right\rbrace}


% Mathbb
\newcommand{\C}{\mathbb{C}}
\newcommand{\D}{\mathbf{D}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\N}{\mathbb{N}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\K}{\mathbb{K}}
\newcommand{\Cg}{\mathfrak{C}}
\newcommand{\bdot}{\boldsymbol{\cdot}}


% Calligrafiche
\newcommand{\Aa}{\mathcal{A}}
\newcommand{\Bb}{\mathcal{B}}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Ee}{\mathcal{E}}
\newcommand{\Ff}{\mathcal{F}}
\newcommand{\Hh}{\mathcal{H}}
\newcommand{\Ii}{\mathcal{I}}
\newcommand{\Kk}{K}
\newcommand{\Mm}{\mathcal{M}}
\newcommand{\Nn}{\mathcal{N}}
\newcommand{\Qq}{\mathcal{Q}}
\newcommand{\Ss}{\mathcal{S}}
\newcommand{\Xx}{\mathcal{X}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}

\newcommand{\eqdef}{\ensuremath{\,\raisebox{-1.2pt}{${\stackrel{\mbox{\upshape \scalebox{.42}{def.}}}{=}}$}}\,}
\newcommand{\eqorder}{\sim} %{\ensuremath{\,\raisebox{-1pt}{$\stackrel{\mbox{\upshape\tiny $\order$}}{\sim}$}}\,}
% \newcommand{\eqdef}{\stackrel{\mathclap{\tiny\mbox{def.}}}{=}}


%\newcommand{\sdim}{{N_\mathrm{sim}}} %Similarity score encoding dimension
%\newcommand{\pdim}{{N_\mathrm{pos}}} %Positional encoding dimension
%\newcommand{\edim}{{N}} % Encoding dimension
%\newcommand{\ddim}{{N'}} % Decoding dimension (target dimension of MLP)
%\newcommand{\rdim}{{N_\mathrm{ref}}} %Number of reference paths
%\newcommand{\tdim}{{N_\mathrm{time}}} %Number of reference time points
%\newcommand{\pldim}{{N_\mathrm{p}}} %Number of time points between linear pieces
%\newcommand{\ldim}{{d_K}} %Latent dimension, was {d_K}

\newcommand{\idim}{d_{\mathrm{in}}} % Input dimension
\newcommand{\odim}{d_{\mathrm{out}}} % Output dimension
\newcommand{\kdim}{d_{K}} % Key dimension
\newcommand{\vdim}{d_{V}} % Value dimension
\newcommand{\ldim}{d_{\mathrm{ff}}} % Feed forward latent dimension

% Cose del modello
\newcommand{\rhosummer}{\rho}% name of the length of summer
\newcommand{\rhowinter}{\rho}% name of the length of winter

\usepackage{amsthm}
\newtheorem{atheorem}{Theorem}
\renewcommand{\theatheorem}{\Alph{atheorem}} % "letter-numbered" theorems
\newtheorem{InformalTheorem}{Informal Theorem}
% \newtheorem{definition}{Definition}
% \newtheorem{proposition}{Proposition}
\newtheorem{assumption}{Assumption}
% \newtheorem{theorem}{Theorem}
% \newtheorem{lemma}{Lemma}
% \newtheorem{corollary}{Corollary}
\newtheorem{notation}{Notation}
\newtheorem{setting}{Setting}[section]
\newtheorem{assumptions}{Assumptions}[section]
% \theoremstyle{remark}
% \newtheorem*{remark}{Remark}
% \newtheorem{example}{Example}
% \theoremstyle{definition}
\newtheorem{question}{Question}

% QED Symbol 
\usepackage{etoolbox}
\newcommand{\addQEDstyle}[2]{\AtBeginEnvironment{#1}{\pushQED{\qed}\renewcommand{\qedsymbol}{#2}}\AtEndEnvironment{#1}{\popQED}}
\addQEDstyle{remark}{$\triangleleft$}
\addQEDstyle{example}{$\triangleleft$}



%%%% COMMENTING (Temporary)
\NewDocumentCommand{\luca}{mo}{
    \IfValueF{#2}{
    %%%%% NO Margin Note
                        {{\scriptsize
                            \textcolor{green}{ 
                            \textbf{L:}
                            \textit{{#1}}
                            }
                        }}
        }
    %%%% Margin Note
    \IfValueT{#2}{
                        \marginnote{{\scriptsize
                            \textcolor{green}{ 
                            \textbf{L:}
                            \textit{{#1}}
                            }
                        }}
        }
                    }
\NewDocumentCommand{\giulia}{mo}{
    \IfValueF{#2}{
    %%%%% NO Margin Note
                        {{\scriptsize
                            \textcolor{red}{ 
                            \textbf{GL:}
                            \textit{{#1}}
                            }
                        }}
        }
    %%%% Margin Note
    \IfValueT{#2}{
                        \marginnote{{\scriptsize
                            \textcolor{red}{ 
                            \textbf{GL:}
                            \textit{{#1}}
                            }
                        }}
        }
}
\NewDocumentCommand{\anastasis}{mo}{
    \IfValueF{#2}{
    %%%%% NO Margin Note
                        {{\scriptsize
                            \textcolor{violet}{ 
                            \textbf{A:}
                            \textit{{#1}}
                            }
                        }}
        }
    %%%% Margin Note
    \IfValueT{#2}{
                        \marginnote{{\scriptsize
                            \textcolor{violet}{ 
                            \textbf{A:}
                            \textit{{#1}}
                            }
                        }}
        }
                    }
                    
\NewDocumentCommand{\cody}{mo}{
    \IfValueF{#2}{
    %%%%% NO Margin Note
                        {{\scriptsize
                            \textcolor{orange}{ 
                            \textbf{A:}
                            \textit{{#1}}
                            }
                        }}
        }
    %%%% Margin Note
    \IfValueT{#2}{
                        \marginnote{{\scriptsize
                            \textcolor{orange}{ 
                            \textbf{A:}
                            \textit{{#1}}
                            }
                        }}
        }
                    }

\newcommand{\byyan}[1]{\textcolor{cyan}{#1}}
\NewDocumentCommand{\yannick}{mo}{
    \IfValueF{#2}{
    %%%%% NO Margin Note
                        {{\scriptsize
                            \textcolor{cyan}{ 
                            \textbf{Y:}
                            \textit{{#1}}
                            }
                        }}
        }
    %%%% Margin Note
    \IfValueT{#2}{
                        \marginnote{{\scriptsize
                            \textcolor{cyan}{ 
                            \textbf{Y:}
                            \textit{{#1}}
                            }
                        }}
        }
                    } 

\definecolor{darkgreen}{rgb}{0.0, 0.2, 0.13}
\NewDocumentCommand{\xuwei}{mo}{
    \IfValueF{#2}{
    %%%%% NO Margin Note
                        {{\scriptsize
                            \textcolor{darkgreen}{ 
                            \textbf{X:}
                            \textit{{#1}}
                            }
                        }}
        }
    %%%% Margin Note
    \IfValueT{#2}{
                        \marginnote{{\scriptsize
                            \textcolor{darkgreen}{ 
                            \textbf{X:}
                            \textit{{#1}}
                            }
                        }}
        }
                    }

\usepackage{appendix}
\usepackage{titletoc}
\newcommand\DoToC{%
  \startcontents
  \printcontents{}{1}{\textbf{Appendix Contents}\vskip3pt\hrule\vskip5pt}
  \vskip3pt\hrule\vskip5pt
}

% Make the "Part I" text invisible
\renewcommand \thepart{}
\renewcommand \partname{}


\usepackage{cleveref}
\newcounter{termcounter}
\renewcommand{\thetermcounter}{\Roman{termcounter}}
\crefname{term}{term}{terms}
\creflabelformat{term}{#2\textup{(#1)}#3}

\makeatletter
\def\term{\@ifnextchar[\term@optarg\term@noarg}%]
\def\term@optarg[#1]#2{%
  \textup{#1}%
  \def\@currentlabel{#1}%
  \def\cref@currentlabel{[][2147483647][]#1}%
  \cref@label[term]{#2}}
\def\term@noarg#1{%
  \refstepcounter{termcounter}%
  \textup{(\thetermcounter)}%
  \cref@label[term]{#1}}
\makeatother




%  \setcounter{termcounter}{0}

\crefname{lemma}{lemma}{lemmata}
\Crefname{lemma}{Lemma}{Lemmata}
\crefname{notation}{notation}{notations}
\Crefname{notation}{Notation}{Notations}
\crefname{assumption}{assumption}{assumptions}
\Crefname{assumption}{Assumption}{Assumptions}
\crefname{example}{Example}{Examples}
\crefname{proposition}{Proposition}{Proposition}
\crefname{subsubsubappendix}{appendix}{appendices}
\Crefname{subsubsubappendix}{Appendix}{Appendices}


\usepackage{comment}
\usepackage{microtype}


